StrucText-Eval: Evaluating Large Language Model's Reasoning Ability in Structure-Rich Text

The effective utilization of structured data, integral to corporate data strategies, has been challenged by the rise of large language models (LLMs) capable of processing unstructured information. This shift prompts the question: can LLMs interpret structured data directly in its unstructured form? We propose an automatic evaluation data generation method for assessing LLMs' reasoning capabilities on structure-rich text to explore this. Our approach supports 8 structured languages and 29 tasks, generating data with adjustable complexity through controllable nesting and structural width. We introduce StrucText-Eval, a benchmark containing 5,800 pre-generated and annotated samples designed to evaluate how well LLMs understand and reason through structured text. StrucText-Eval is divided into two suites: a regular Test suite (3,712 samples) and a Test-Hard suite (2,088 samples), the latter emphasizing the gap between human and model performance on more complex tasks. Experimental results show that while open-source LLMs achieve a maximum accuracy of 74.9\% on the standard dataset, their performance drops significantly to 45.8\% on the harder dataset. In contrast, human participants reach an accuracy of 92.6\% on StrucText-Eval-Hard, highlighting LLMs' current limitations in handling intricate structural information. The benchmark and generation codes are open sourced in \url{https://github.com/MikeGu721/StrucText-Eval}

==> benchmark_statistic.tex <==
\begin{table*}[t]
    \centering
{\fontsize{8pt}{9.6pt}\selectfont
\begin{tabular}{cccccccc}
\toprule
\textbf{Category} & \textbf{Task} & \textbf{Difficulty} & \textbf{\#Samples} & \textbf{\#Input} & \textbf{\#Instruction} & \textbf{\#Answer} & \textbf{\#Node} \\
\midrule
\multirow{10}{*}{JSON} & \multirow{2}{*}{PathCompose} & hard & 104 & 787.1 & 101.4 & 32.4 & 3 \\
 & & simple & 104 & 116.3 & 101.0 & 17.6 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{PathWalk} & hard & 104 & 787.1 & 38.0 & 1.1 & 3 \\
 & & simple & 104 & 116.3 & 38.0 & 1.0 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{Syntax} & hard & 104 & 736.0 & 148.0 & 4.0 & 3 \\
 & & simple & 104 & 109.0 & 148.0 & 4.0 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval} & hard & 124 & 786.6 & 105.1 & 156.4 & 3 \\
 & & simple & 104 & 116.3 & 94.1 & 75.3 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval\_1$^*$} & hard & 104 & 787.1 & 161.0 & 315.4 & 3 \\
 & & simple & 104 & 116.3 & 161.0 & 32.2 & 2 \\
\hline
\multirow{6}{*}{LaTeX} & \multirow{2}{*}{PathWalk} & hard & 104 & 2726.1 & 179.1 & 484.0 & 2 \\
 & & simple & 104 & 277.2 & 160.3 & 145.1 & 1 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval} & hard & 104 & 2726.1 & 74.0 & 54.2 & 2 \\
 & & simple & 104 & 277.2 & 74.0 & 16.1 & 1 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval\_1} & hard & 104 & 2726.1 & 62.0 & 57.1 & 2 \\
 & & simple & 104 & 277.2 & 62.0 & 13.3 & 1 \\
\hline
\multirow{6}{*}{Markdown} & \multirow{2}{*}{PathWalk} & hard & 104 & 2355.7 & 184.8 & 370.9 & 3 \\
 & & simple & 104 & 228.5 & 162.5 & 114.5 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval} & hard & 104 & 2355.7 & 73.0 & 52.5 & 3 \\
 & & simple & 104 & 228.5 & 73.0 & 12.4 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval\_1} & hard & 104 & 2355.7 & 62.0 & 52.1 & 3 \\
 & & simple & 104 & 228.5 & 62.0 & 12.2 & 2 \\
\hline
\multirow{6}{*}{ORG} & \multirow{2}{*}{PathWalk} & hard & 104 & 2252.7 & 178.6 & 373.3 & 3 \\
 & & simple & 104 & 200.1 & 156.5 & 104.5 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval} & hard & 104 & 2252.7 & 73.0 & 52.0 & 3 \\
 & & simple & 104 & 200.1 & 73.0 & 15.2 & 2 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval\_1} & hard & 104 & 2252.7 & 62.0 & 54.0 & 3 \\
 & & simple & 104 & 200.1 & 62.0 & 12.3 & 2 \\
\hline
\multirow{8}{*}{SQL} & \multirow{2}{*}{SQL.Join} & hard & 104 & 798.6 & 51.0 & 1.0 & 0 \\
 & & simple & 104 & 488.3 & 51.0 & 1.0 & 0 \\
\cline{2-8}
 & \multirow{2}{*}{Statistics} & hard & 104 & 798.6 & 49.9 & 1.3 & 0 \\
 & & simple & 104 & 488.3 & 49.9 & 1.0 & 0 \\
\cline{2-8}
 & \multirow{2}{*}{Statistics\_1} & hard & 104 & 798.6 & 27.0 & 1.1 & 0 \\
 & & simple & 104 & 488.3 & 27.0 & 1.0 & 0 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval} & hard & 104 & 798.6 & 43.8 & 4.3 & 0 \\
 & & simple & 104 & 488.3 & 43.6 & 3.9 & 0 \\
\hline
\multirow{6}{*}{Tree} & \multirow{2}{*}{PathCompose} & hard & 104 & 1745.7 & 84.0 & 25.0 & 8 \\
 & & simple & 104 & 555.6 & 83.8 & 11.3 & 4 \\
\cline{2-8}
 & \multirow{2}{*}{Tree.Depth} & hard & 104 & 1745.7 & 68.0 & 1.0 & 8 \\
 & & simple & 104 & 555.6 & 67.9 & 1.0 & 4 \\
\cline{2-8}
 & \multirow{2}{*}{Tree.Height} & hard & 104 & 1745.7 & 156.0 & 1.0 & 8 \\
 & & simple & 104 & 555.6 & 156.0 & 1.0 & 4 \\
\hline
\multirow{8}{*}{XML} & \multirow{2}{*}{Syntax} & hard & 104 & 2135.7 & 147.0 & 4.0 & 5 \\
 & & simple & 104 & 2338.0 & 147.0 & 4.0 & 3 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval} & hard & 104 & 2621.6 & 54.5 & 17.7 & 5 \\
 & & simple & 104 & 2910.4 & 52.5 & 11.9 & 3 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval\_1} & hard & 104 & 2621.6 & 81.9 & 110.4 & 5 \\
 & & simple & 104 & 2910.4 & 83.8 & 132.9 & 3 \\
\hline
\multirow{10}{*}{YAML} & \multirow{2}{*}{PathCompose} & hard & 104 & 631.7 & 101.4 & 32.4 & 6 \\
 & & simple & 104 & 82.2 & 101.0 & 19.6 & 4 \\
\cline{2-8}
 & \multirow{2}{*}{PathWalk} & hard & 104 & 631.7 & 38.0 & 1.0 & 6 \\
 & & simple & 104 & 82.2 & 38.0 & 1.0 & 4 \\
\cline{2-8}
 & \multirow{2}{*}{Syntax} & hard & 104 & 725.8 & 148.0 & 4.0 & 6 \\
 & & simple & 104 & 94.6 & 148.0 & 4.0 & 4 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval} & hard & 104 & 631.7 & 94.3 & 111.9 & 6 \\
 & & simple & 104 & 82.2 & 94.0 & 51.9 & 4 \\
\cline{2-8}
 & \multirow{2}{*}{TextRetrieval\_1} & hard & 104 & 631.7 & 161.0 & 224.2 & 6 \\
 & & simple & 104 & 82.2 & 161.0 & 22.1 & 4 \\
 \bottomrule
\end{tabular}}
\caption{Statistic information about StrucText-Eval.
$^*$: The subscript ``\_1'' indicates tasks generated based on different problem templates.
}
\label{tab:statistic}
\end{table*}

% \begin{table*}
% \centering
% \caption{Statistic Information about StrucText-Eval
% \gzh{Split the Text Retrieval task into two different task}}
% \label{tab:statistic}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccc}
% % {|c|c|c|c|c|c|c|c|}
%\cline{2-8}
% \textbf{Category} & \textbf{Task} & \textbf{Difficulty} & \textbf{\#Sample}
% & \textbf{Avg \#Input} & \textbf{Avg \#Instruction} & \textbf{Avg \#GroundTruth} & \textbf{Avg \#Fork} \\ \cline{2-8}
% \multirow{8}{*}{JSON} & \multirow{2}{*}{PathCompose} & hard & 104 & 787.06 & 101.41 & 32.43 & 0 \\  
%                       &                              & simple & 104 & 116.29 & 101.05 & 17.63 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{PathWalk}    & hard & 104 & 787.06 & 38.00 & 1.06 & 0 \\  
%                       &                              & simple & 104 & 116.29 & 38.00 & 1.05 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Syntax}      & hard & 104 & 736.05 & 148.00 & 4.00 & 0 \\  
%                       &                              & simple & 104 & 108.98 & 148.00 & 4.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 787.06 & 127.65 & 220.79 & 0 \\  
%                       &                              & simple & 208 & 116.29 & 127.53 & 53.75 & 0 \\ \cline{2-8}
% \multirow{4}{*}{LaTeX} & \multirow{2}{*}{PathWalk}   & hard & 104 & 2726.10 & 179.06 & 483.98 & 0 \\  
%                       &                              & simple & 104 & 277.18 & 160.31 & 145.09 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2726.10 & 68.00 & 55.66 & 0 \\  
%                       &                              & simple & 208 & 277.18 & 68.00 & 14.70 & 0 \\ \cline{2-8}
% \multirow{4}{*}{Markdown} & \multirow{2}{*}{PathWalk} & hard & 104 & 2355.69 & 184.77 & 370.88 & 0 \\  
%                       &                              & simple & 104 & 228.47 & 162.50 & 114.45 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2355.69 & 67.50 & 52.32 & 0 \\  
%                       &                              & simple & 208 & 228.47 & 67.50 & 12.30 & 0 \\ \cline{2-8}
% \multirow{4}{*}{ORG} & \multirow{2}{*}{PathWalk}     & hard & 104 & 2252.73 & 178.62 & 373.31 & 0 \\  
%                       &                              & simple & 104 & 200.07 & 156.49 & 104.49 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2252.73 & 67.50 & 52.99 & 0 \\  
%                       &                              & simple & 208 & 200.07 & 67.50 & 13.72 & 0 \\ \cline{2-8}
% \multirow{6}{*}{Tabular} & \multirow{2}{*}{SQL.Join} & hard & 104 & 798.64 & 51.00 & 1.00 & 0 \\  
%                       &                              & simple & 104 & 488.32 & 51.00 & 1.00 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Statistics}  & hard & 208 & 798.64 & 38.45 & 1.16 & 0 \\  
%                       &                              & simple & 208 & 488.32 & 38.46 & 1.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 104 & 798.64 & 43.75 & 4.35 & 0 \\  
%                       &                              & simple & 104 & 488.32 & 43.62 & 3.88 & 0 \\ \cline{2-8}
% \multirow{6}{*}{Tree} & \multirow{2}{*}{PathCompose} & hard & 104 & 1745.69 & 83.99 & 24.95 & 0 \\  
%                       &                              & simple & 104 & 555.61 & 83.82 & 11.29 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Tree.Depth}  & hard & 104 & 1745.69 & 67.95 & 1.00 & 0 \\  
%                       &                              & simple & 104 & 555.61 & 67.89 & 1.00 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Tree.Height} & hard & 104 & 1745.69 & 156.00 & 1.00 & 0 \\  
%                       &                              & simple & 104 & 555.61 & 156.00 & 1.00 & 0 \\ \cline{2-8}
% \multirow{4}{*}{XML} & \multirow{2}{*}{Syntax}      & hard & 104 & 2135.65 & 147.00 & 4.00 & 0 \\  
%                       &                              & simple & 104 & 2337.98 & 147.00 & 4.00 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2621.56 & 68.19 & 64.03 & 0 \\  
%                       &                              & simple & 208 & 2910.42 & 68.17 & 72.37 & 0 \\ \cline{2-8}
% \multirow{8}{*}{YAML} & \multirow{2}{*}{PathCompose} & hard & 104 & 631.71 & 101.41 & 32.43 & 0 \\  
%                       &                              & simple & 104 & 82.16 & 101.04 & 19.63 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{PathWalk}    & hard & 104 & 631.71 & 38.00 & 1.03 & 0 \\  
%                       &                              & simple & 104 & 82.16 & 38.00 & 1.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Syntax}      & hard & 104 & 725.84 & 148.00 & 4.00 & 0 \\  
%                       &                              & simple & 104 & 94.60 & 148.00 & 4.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 631.71 & 127.64 & 168.07 & 0 \\  
%                       &                              & simple & 208 & 82.16 & 127.51 & 37.02 & 0 \\ \cline{2-8}
% \end{tabular}}
% \end{table*}






% \begin{table*}
% \centering
% \caption{Statistic Information about StrucText-Eval}
% \label{tab:statistic}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cccccccc}
% % {|c|c|c|c|c|c|c|c|}
%\cline{2-8}
% \textbf{Category} & \textbf{Task} & \textbf{Difficulty} & \textbf{\#Sample}
% & \textbf{Avg \#Input} & \textbf{Avg \#Instruction} & \textbf{Avg \#GroundTruth} & \textbf{Avg \#Fork} \\ \cline{2-8}
% \multirow{8}{*}{JSON} & \multirow{2}{*}{PathCompose} & hard & 104 & 787.06 & 101.41 & 32.43 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 116.29 & 101.05 & 17.63 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{PathWalk}    & hard & 104 & 787.06 & 38.00 & 1.06 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 116.29 & 38.00 & 1.05 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Syntax}      & hard & 104 & 736.05 & 148.00 & 4.00 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 108.98 & 148.00 & 4.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 787.06 & 127.65 & 220.79 & 0 \\ \cline{3-8} 
%                       &                              & simple & 208 & 116.29 & 127.53 & 53.75 & 0 \\ \cline{2-8}
% \multirow{4}{*}{LaTeX} & \multirow{2}{*}{PathWalk}   & hard & 104 & 2726.10 & 179.06 & 483.98 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 277.18 & 160.31 & 145.09 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2726.10 & 68.00 & 55.66 & 0 \\ \cline{3-8} 
%                       &                              & simple & 208 & 277.18 & 68.00 & 14.70 & 0 \\ \cline{2-8}
% \multirow{4}{*}{Markdown} & \multirow{2}{*}{PathWalk} & hard & 104 & 2355.69 & 184.77 & 370.88 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 228.47 & 162.50 & 114.45 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2355.69 & 67.50 & 52.32 & 0 \\ \cline{3-8} 
%                       &                              & simple & 208 & 228.47 & 67.50 & 12.30 & 0 \\ \cline{2-8}
% \multirow{4}{*}{ORG} & \multirow{2}{*}{PathWalk}     & hard & 104 & 2252.73 & 178.62 & 373.31 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 200.07 & 156.49 & 104.49 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2252.73 & 67.50 & 52.99 & 0 \\ \cline{3-8} 
%                       &                              & simple & 208 & 200.07 & 67.50 & 13.72 & 0 \\ \cline{2-8}
% \multirow{6}{*}{Tabular} & \multirow{2}{*}{SQL.Join} & hard & 104 & 798.64 & 51.00 & 1.00 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 488.32 & 51.00 & 1.00 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Statistics}  & hard & 208 & 798.64 & 38.45 & 1.16 & 0 \\ \cline{3-8} 
%                       &                              & simple & 208 & 488.32 & 38.46 & 1.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 104 & 798.64 & 43.75 & 4.35 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 488.32 & 43.62 & 3.88 & 0 \\ \cline{2-8}
% \multirow{8}{*}{Tree} & \multirow{2}{*}{PathCompose} & hard & 104 & 1745.69 & 83.99 & 24.95 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 555.61 & 83.82 & 11.29 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Tree.Depth}  & hard & 104 & 1745.69 & 67.95 & 1.00 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 555.61 & 67.89 & 1.00 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Tree.Height} & hard & 104 & 1745.69 & 156.00 & 1.00 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 555.61 & 156.00 & 1.00 & 0 \\ \cline{2-8}
% \multirow{4}{*}{XML} & \multirow{2}{*}{Syntax}      & hard & 104 & 2135.65 & 147.00 & 4.00 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 2337.98 & 147.00 & 4.00 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 2621.56 & 68.19 & 64.03 & 0 \\ \cline{3-8} 
%                       &                              & simple & 208 & 2910.42 & 68.17 & 72.37 & 0 \\ \cline{2-8}
% \multirow{8}{*}{YAML} & \multirow{2}{*}{PathCompose} & hard & 104 & 631.71 & 101.41 & 32.43 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 82.16 & 101.04 & 19.63 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{PathWalk}    & hard & 104 & 631.71 & 38.00 & 1.03 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 82.16 & 38.00 & 1.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{Syntax}      & hard & 104 & 725.84 & 148.00 & 4.00 & 0 \\ \cline{3-8} 
%                       &                              & simple & 104 & 94.60 & 148.00 & 4.01 & 0 \\ \cline{2-8} 
%                       & \multirow{2}{*}{TextRetrieval}& hard & 208 & 631.71 & 127.64 & 168.07 & 0 \\ \cline{3-8} 
%                       &                              & simple & 208 & 82.16 & 127.51 & 37.02 & 0 \\ \cline{2-8}
% \end{tabular}}
% \end{table*}


==> case_study_table.tex <==
% \begin{table}[t]
% \centering
% \begin{tabular}{clclcl}

% \toprule
% \textbf{Language:} & JSON & \textbf{Task:} & TextRetrieval & \textbf{Difficulty:} & Simple \\
% \midrule
% \multicolumn{6}{l}{
% \parbox[t]{0.98\linewidth}{
% \textbf{Question:} \\
% What are the most deeply nested objects, i.e., no value of type list or dict?\\
% \textbf{Requirement:} \\
% The content should be an excerpt as they appear in the JSON file, separated by \n\n.
% \textbf{Reference:} {
% "id":"j",
% "Z":"o",
% "subs":[
%  {
%  "id":"k",
%  "Y":"n",
%  "subs":[
%   {
%   "id":"l",
%   "X":"m",
%   "subs":[]
%   }
%  ]
%  }
% ]
% } \\
% \textbf{Ground truth:} {
% "id":"l",
% "X":"m",
% "subs":[]
% } \\
% }}
% \midrule
% \multicolumn{2}{l}{
% \parbox[t]{0.32\linewidth}{
% Model Name: GPT\\
% Iteration: None\\
% Response: xxxx\\
% Judge: False}} & 
% \multicolumn{2}{l}{
% \parbox[t]{0.32\linewidth}{
% Model Name: Finetune Model\\
% Trained Steps: 20\\
% Response: xxxx\\
% Judge: False}}&
% \multicolumn{2}{l}{
% \parbox[t]{0.32\linewidth}{
% Model Name: Finetune Model\\
% Trained Steps: 900\\
% Response: xxxx\\
% Judge: False}} \\
% \bottomrule
    
% \end{tabular}
% \caption{Caption}
% \label{tab:my_label}
% \end{table}


\begin{table}[t]
\centering
\begin{tabular}{clclcl}
\toprule
\textbf{Language:} & JSON & \textbf{Task:} & TextRetrieval & \textbf{Difficulty:} & Simple \\
\midrule
\multicolumn{6}{0.98\linewidth}{
\textbf{Question:} \\
% What are the most deeply nested objects, i.e., no value of type list or dict? \\
% \textbf{Requirement:} \\
% The content should be an excerpt as they appear in the JSON file, separated by \textbackslash n\textbackslash n. \\
% \textbf{Reference:} \\
% \{ "id":"j", \\
% "Z":"o", \\
% "subs":[ \\
% \{ \\
% "id":"k", \\
% "Y":"n", \\
% "subs":[ \\
% \{ \\
% "id":"l", \\
% "X":"m", \\
% "subs":\{\} \\
% \} \\
% ] \\
% \} \\
% ] \\
% \} \\
% \textbf{Ground truth:} \\
% \{ "id":"l", "X":"m", "subs":\[\] \} \\
} \\
\midrule
\multicolumn{2}{0.32\linewidth}{
Model Name: GPT\\
Iteration: None\\
Response: xxxx\\
Judge: False
} & 
\multicolumn{2}{0.32\linewidth}{
Model Name: Finetune Model\\
Trained Steps: 20\\
Response: xxxx\\
Judge: False
} &
\multicolumn{2}{0.32\linewidth}{
Model Name: Finetune Model\\
Trained Steps: 900\\
Response: xxxx\\
Judge: False
} \\
\bottomrule
\end{tabular}
\caption{Caption}
\label{tab:my_label}
\end{table}

==> data_tabs.tex <==

% GPT4-base
\begin{table}[htbp!]
\caption{GPT-4 w/o prompt engineering}
\label{gpt4}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|lllllllll}
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c}{\bf Tree} &\multicolumn{1}{c}{\bf Tabular} &\multicolumn{1}{c}{\bf JSON} &\multicolumn{1}{c}{\bf YAML}&\multicolumn{1}{c}{\bf XML} &\multicolumn{1}{c}{\bf Markdown}&\multicolumn{1}{c}{\bf Org} &\multicolumn{1}{c}{\bf LaTeX} &\multicolumn{1}{c}{\bf PYTHON}
\\ \hline
  Exact Match         &0.52 &0.78 &0.64 &0.93 &0.9  &0.36 &0.25 &0.38 &0.259\\
  Rouge-1             &0.107&0.107&0.383&0.368&0.195&0.894&0.496&0.944&0.068\\
  GPTJudge            &0.556&0.7  &0.983&0.967&0.972&0.736&0.5  &0.819&0.787\\
\end{tabular}
}
\end{center}
\end{table}

%Minimax-base
\begin{table}[htbp!]
\caption{Miminax w/o prompt engineering}
\label{mnx}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|lllllllll}
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c}{\bf Tree} &\multicolumn{1}{c}{\bf Tabular} &\multicolumn{1}{c}{\bf JSON} &\multicolumn{1}{c}{\bf YAML}&\multicolumn{1}{c}{\bf XML} &\multicolumn{1}{c}{\bf Markdown}&\multicolumn{1}{c}{\bf Org} &\multicolumn{1}{c}{\bf LaTeX} &\multicolumn{1}{c}{\bf PYTHON}
\\ \hline
  Exact Match        &0.133& 0.738& 0.470& 0.430& 0.567& 0.283& 0.233& 0.267& 0.201\\
  Rouge-1            &0.101& 0.105& 0.501& 0.490& 0.206& 0.690& 0.506& 0.742& 0.091\\
  GPTJudge           &0.067& 0.525& 0.850& 0.770& 0.883& 0.683& 0.450& 0.683& 0.679\\
\end{tabular}}
\end{center}
\end{table}

%Spark-base
\begin{table}[htbp!]
\caption{Spark w/o prompt engineering}
\label{spark}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|lllllllll}
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c}{\bf Tree} &\multicolumn{1}{c}{\bf Tabular} &\multicolumn{1}{c}{\bf JSON} &\multicolumn{1}{c}{\bf YAML}&\multicolumn{1}{c}{\bf XML} &\multicolumn{1}{c}{\bf Markdown}&\multicolumn{1}{c}{\bf Org} &\multicolumn{1}{c}{\bf LaTeX} &\multicolumn{1}{c}{\bf PYTHON}
\\ \hline
  Exact Match         &0.383& 0.975& 0.310& 0.540& 0.433& 0.333& 0.250& 0.267& 0.263\\
  Rouge-1             &0.007& 0.001& 0.023& 0.011& 0.018& 0.026& 0.032& 0.035& 0.000\\
  GPTJudge            &0.089& 0.280& 0.800& 0.472& 0.533& 0.529& 0.300& 0.296& 0.702\\
\end{tabular}}
\end{center}
\end{table}

%Ernie-base
\begin{table}[htbp!]
\caption{Ernie w/o prompt engineering}
\label{ernie}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|lllllllll}
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c}{\bf Tree} &\multicolumn{1}{c}{\bf Tabular} &\multicolumn{1}{c}{\bf JSON} &\multicolumn{1}{c}{\bf YAML}&\multicolumn{1}{c}{\bf XML} &\multicolumn{1}{c}{\bf Markdown}&\multicolumn{1}{c}{\bf Org} &\multicolumn{1}{c}{\bf LaTeX} &\multicolumn{1}{c}{\bf PYTHON}
\\ \hline
  Exact Match         &0.167& 0.637& 0.200& 0.240& 0.200& 0.217& 0.133& 0.117& 0.295\\
  Rouge-1             &0.056& 0.051& 0.161& 0.162& 0.084& 0.226& 0.137& 0.283& 0.066\\
  GPTJudge            &0.133& 0.375& 0.700& 0.660& 0.617& 0.433& 0.200& 0.350& 0.550\\
\end{tabular}}
\end{center}
\end{table}

%Minimax-engi
\begin{table}[htbp!]
\caption{Miminax w/ prompt engineering}
\label{mnx_e}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|lllllllll}
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c}{\bf Tree} &\multicolumn{1}{c}{\bf Tabular} &\multicolumn{1}{c}{\bf JSON} &\multicolumn{1}{c}{\bf YAML}&\multicolumn{1}{c}{\bf XML} &\multicolumn{1}{c}{\bf Markdown}&\multicolumn{1}{c}{\bf Org} &\multicolumn{1}{c}{\bf LaTeX} &\multicolumn{1}{c}{\bf PYTHON}
\\ \hline
  Exact Match        &0.150& 0.738& 0.390& 0.400& 0.517& 0.250& 0.183& 0.233& 0.205\\
  Rouge-1            &0.027& 0.065& 0.241& 0.290& 0.181& 0.429& 0.360& 0.571& 0.093\\
  GPTJudge           &0.183& 0.575& 0.850& 0.730& 0.850& 0.600& 0.433& 0.683& 0.708\\
\end{tabular}}
\end{center}
\end{table}

%Spark-engi
\begin{table}[htbp!]
\caption{Spark w/ prompt engineering}
\label{spark_e}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|lllllllll}
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c}{\bf Tree} &\multicolumn{1}{c}{\bf Tabular} &\multicolumn{1}{c}{\bf JSON} &\multicolumn{1}{c}{\bf YAML}&\multicolumn{1}{c}{\bf XML} &\multicolumn{1}{c}{\bf Markdown}&\multicolumn{1}{c}{\bf Org} &\multicolumn{1}{c}{\bf LaTeX} &\multicolumn{1}{c}{\bf PYTHON}
\\ \hline
  Exact Match         &0.483& 0.963& 0.420& 0.540& 0.833& 0.417& 0.400& 0.300& 0.268\\
  Rouge-1             &0.002& 0.001& 0.003& 0.004& 0.006& 0.029& 0.015& 0.027& 0.000\\
  GPTJudge            &0.214& 0.457& 0.533& 0.286& 0.483& 0.100& 0.250& 0.222& 0.705\\
\end{tabular}}
\end{center}
\end{table}

%Ernie-engi
\begin{table}[htbp!]
\caption{Ernie w/ prompt engineering}
\label{ernie_e}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{r|lllllllll}
\multicolumn{1}{c}{\bf Metric}  &\multicolumn{1}{c}{\bf Tree} &\multicolumn{1}{c}{\bf Tabular} &\multicolumn{1}{c}{\bf JSON} &\multicolumn{1}{c}{\bf YAML}&\multicolumn{1}{c}{\bf XML} &\multicolumn{1}{c}{\bf Markdown}&\multicolumn{1}{c}{\bf Org} &\multicolumn{1}{c}{\bf LaTeX} &\multicolumn{1}{c}{\bf PYTHON}
\\ \hline
  Exact Match         &0.183& 0.637& 0.230& 0.160& 0.217& 0.100& 0.083& 0.133& 0.238\\
  Rouge-1             &0.042& 0.041& 0.167& 0.115& 0.101& 0.143& 0.104& 0.115& 0.044\\
  GPTJudge            &0.233& 0.438& 0.810& 0.580& 0.593& 0.450& 0.450& 0.417& 0.608\\
\end{tabular}}
\end{center}
\end{table}

\begin{table}[htbp!]
\caption{JSON input with background knowledge}
\label{bg_expr_data}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccllll}
&\multicolumn{1}{c}{\bf Background Knowledge}  &\multicolumn{1}{c}{\bf Minimax:Base} &\multicolumn{1}{c}{\bf Minimax:Hint} &\multicolumn{1}{c}{\bf Ernie:Base} &\multicolumn{1}{c}{\bf Ernie:Hint}\\
\hline
\multirow{2}{*}{GPTJudege}& w/o& 0.857& 0.859& 0.7& 0.81\\
&w/ &0.82& 0.85& 0.75& 0.8\\
\hline
\multirow{2}{*}{Exact Match}& w/o& 0.469& 0.394& 0.2& 0.23\\
&w/ &0.42& 0.33& 0.25& 0.19\\
\hline
\multirow{2}{*}{Rouge-1}& w/o& 0.504& 0.243& 0.161& 0.167\\
&w/ &0.524& 0.223& 0.146& 0.173\\
\end{tabular}}
\end{center}
\end{table}


==> datamisc.tex <==



\begin{figure*}[t]
\centering
\begin{subfigure}{0.49\textwidth}
% \noindent
% \begin{minipage}{0.45\textwidth}
\centering
\resizebox{\textwidth}{!}{
\begin{tikzpicture}[x=1.0cm,y=1.0cm,scale=1,baseline={(0,0)}] %https://tex.stackexchange.com/a/666956
\def\innername{\tiny{StrucText-Eval}}
\def\innerradius{2.6cm}
\def\outerradius{2.8cm}
\pgfmathsetlengthmacro{\centerradius}{(\outerradius + \innerradius)/2}
\pgfmathsetlengthmacro{\donutcenter}{\innerradius/2}
\def\donutannotate{1}
\donutchart{
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   8/hard/208, 8/simple/208,
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   8/hard/208, 8/simple/208,
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   4/hard/104, 4/simple/104,
   8/hard/208, 8/simple/208,
   4/hard/104, 4/simple/104,
   8/hard/208, 8/simple/208,
   4/hard/104, 4/simple/104,
   8/hard/208, 8/simple/208,
   4/hard/104, 4/simple/104,
   8/hard/208, 8/simple/208,
   4/hard/104, 4/simple/104,
   8/hard/208, 8/simple/208
}{3} % black - Hard, lightgray - Simple
\def\donutannotate{0}

\def\innerradius{1.7cm}
\def\outerradius{2.6cm}
\pgfmathsetlengthmacro{\centerradius}{(\outerradius + \innerradius)/2}
\pgfmathsetlengthmacro{\donutcenter}{\innerradius/2}
\donutchart{ % number as in MiniTest; PathCompose-green, Node.Depth-darkgray, Tree.Height-brown, Join-olive, Statistics-violet, TextRetrieval-cyan, PathWalk-blue, Syntax-magenta
  8/pppurple/208, 8/rrred/208, 8/brown!50/208,
  8/olive!50/208, 16/ooorange/416, 8/cccyan/208,
  8/pppurple/208, 8/bbblue/208, 8/lllightorange/208, 16/cccyan/416,
  8/pppurple/208, 8/bbblue/208, 8/lllightorange/208, 16/cccyan/416,
  8/lllightorange/208, 16/cccyan/416,
  8/bbblue/208, 16/cccyan/416,
  8/bbblue/208, 16/cccyan/416,
  8/bbblue/208, 16/cccyan/416
}{2}


\def\innerradius{0.7cm}
\def\outerradius{1.7cm}
\pgfmathsetlengthmacro{\centerradius}{(\outerradius + \innerradius)/2}
\pgfmathsetlengthmacro{\donutcenter}{\innerradius/2}
\donutchart{
  24/bblue/Tree,
  32/olive!75/Tabular,
  40/rred/JSON,
  40/oorange/YAML,
  24/ggreen/XML,
  24/ppurple/Markdown,
  24/ccyan/ORG,
  24/llightorange/LaTeX
}{1}


\end{tikzpicture}
\hspace{5mm}
\small
\begin{tikzpicture}[x=1.0cm,y=1.0cm,scale=1, baseline={(0,25mm)}]

\fill[pppurple]     (10mm,0 mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {0 mm + 2.5mm}) {\small{PathCompose}};
\fill[rrred]  (10mm,5 mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {5 mm + 2.5mm}) {\small{Node.Depth}};
\fill[brown!50]     (10mm,10mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {10mm + 2.5mm}) {\small{Tree.Height}};
\fill[olive!50]     (10mm,15mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {15mm + 2.5mm}) {\small{Join}};
\fill[ooorange]    (10mm,20mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {20mm + 2.5mm}) {\small{Statictics}};
\fill[cccyan]      (10mm,25mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {25mm + 2.5mm}) {\small{TextRetrieval}};
\fill[bbblue]      (10mm,30mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {30mm + 2.5mm}) {\small{PathWalk}};
\fill[lllightorange]   (10mm,35mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {35mm + 2.5mm}) {\small{Syntax}};
\fill[hard]     (10mm,40mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {40mm + 2.5mm}) {\small{Hard}};
\fill[simple] (10mm,45mm) rectangle ++(5mm,5mm); \draw node [text=black, text width=25mm] at (30mm, {45mm + 2.5mm}) {\small{Simple}};
\end{tikzpicture}
}

\caption{Benchmark Decomposition }
\label{fig:datamisc}

\end{subfigure}\hfill
\begin{subtable}{0.48\textwidth}


\resizebox{\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}m{2.5cm}cm{10cm}}
\toprule
\textbf{Task Name} & \textbf{Abbr.} & \textbf{Task Description} \\ \hline
Syntax & SY& Focuses on detecting structural errors in data formats such as JSON, XML, and YAML. \\ \hline
PathWalk &PW& Focuses on extracting specific sections or subsections from structured documents such as org, LaTeX, or markdown files. \\ \hline
TextRetrieval &TR& Assesses the ability to extract specific information from various document formats, including text content and image filenames. \\ \hline
Statistic &ST& Concentrates on statistical queries to calculate the number of employees meeting specific salary conditions. \\ \hline
Join &JO& Assesses the ability to filter data sets that meet specific criteria by combining multiple tables in a database through SQL queries. \\ \hline
Tree.Height &TH& Evaluates calculating the height of the longest path from the root node to any leaf node in a tree structure. \\ \hline
Node.Depth &ND& Assesses the depth of any node in a tree structure relative to the root node. \\ \hline
PathCompose &PC& Evaluates reasoning of paths and multi-level data indexing within hierarchical or tree-like structures. \\ \bottomrule
\end{tabular}
}
\caption{Descriptions of Tasks for Evaluating Structured Data Understanding in Language Models}
\label{tab:description}
\end{subtable}


\caption{The tasks within StrucText-Eval and their description.}
\label{fig:task_desc}


\end{figure*}
% \end{wrapfigure}
% \begin{table}[t]
% \caption{Benchmark Statistics}
% \label{tb:bcmkstat}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{cllllllll}
% \multicolumn{1}{l}{\bf Category}&
% \multicolumn{1}{l}{\bf Tree}&
% \multicolumn{1}{l}{\bf Tabular}&
% \multicolumn{1}{l}{\bf JSON}   &
% \multicolumn{1}{l}{\bf YAML}   &
% \multicolumn{1}{l}{\bf XML}    &
% \multicolumn{1}{l}{\bf Markdown}&
% \multicolumn{1}{l}{\bf Org}    &
% \multicolumn{1}{l}{\bf LaTeX}
% \\
%   \hline
%   % Category                                   Tree  Tab   JSON  YAML  XML   Markd  Org  LaTeX % Train:Test = 8:2, tot = 5800
%   \#Simple Sample in Train             &240     &320      &400      &400      &240       &240       &240      &240   \\
%   \#Simple Sample in Test              & 60     & 80      &100      &100      & 60       & 60       & 60      & 60   \\
%   \#Complex Sample in Train            &240     &320      &400      &400      &240       &240       &240      &240   \\
%   \#Complex Sample in Test             & 60     & 80      &100      &100      & 60       & 60       & 60      & 60   \\
%   % \#Simple Sample&300&400&500&500&300&300&300&300\\
%   % \#Complex Sample&300&400&500&500&300&300&300&300\\
%   % \#Sample  &600      & 800      &1000      &1000     &600  &600      &600      &600\\
%   (To Be Updated) AvgLen of Input Texts in Bytes       &1152.6 &616.05  &452.91  &360.64  &2590.0   &1253.75  &1201.05 &1534.7 \\
%   (To Be Updated) AvgLen of Simple Input Texts in Bytes        &552.3 &471.3 &114.86 &84.42 &2707.63 &214.4 &185.5 &277.8\\
%   (To Be Updated) AvgLen of Hard Input Texts in Bytes        &1752.9 &760.8 &790.96 &636.86 &2472.37 &2293.1 &2216.6 &2791.6\\
% \end{tabular}
% }
% \end{center}
% \end{table}

% Tree $\to$ 3 Task * 20 Sample
% Tabular/datatable $\to$ 4 Task * 20 Sample
% JSON $\to$ 5 Task * 20 Sample
% YAML $\to$ 5 Task * 20 Sample
% XML $\to$ 3 Task * 20 Sample
% Markdown $\to$ 3 Task * 20 Sample
% Org $\to$ 3 Task * 20 Sample
% \LaTeX $\to$ 3 Task * 20 Sample


% avg#len Tree     		 is 	 1152.6
% avg#len SQL      		 is 	 616.05
% avg#len JSON     		 is 	 452.91
% avg#len YAML     		 is 	 360.64
% avg#len XML      		 is 	 2590.0
% avg#len Markdown 		 is 	 1253.75
% avg#len ORG      		 is 	 1201.05
% avg#len LaTeX    		 is 	 1534.7
% &1152.6 &616.05 &452.91 &360.64 &2590.0 &1253.75 &1201.05 &1534.7

% python3 getlen.py
% avg#len Tree    :simple 		 is 	 552.3
% avg#len SQL     :simple 		 is 	 471.3
% avg#len JSON    :simple 		 is 	 114.86
% avg#len YAML    :simple 		 is 	 84.42
% avg#len XML     :simple 		 is 	 2707.633333333333
% avg#len Markdown:simple 		 is 	 214.4
% avg#len ORG     :simple 		 is 	 185.5
% avg#len LaTeX   :simple 		 is 	 277.8
% avg#len Tree    :hard   		 is 	 1752.9
% avg#len SQL     :hard   		 is 	 760.8
% avg#len JSON    :hard   		 is 	 790.96
% avg#len YAML    :hard   		 is 	 636.86
% avg#len XML     :hard   		 is 	 2472.366666666667
% avg#len Markdown:hard   		 is 	 2293.1
% avg#len ORG     :hard   		 is 	 2216.6
% avg#len LaTeX   :hard   		 is 	 2791.6


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips2024"
%%% End:


==> other_metrics.01.tex <==
\begin{table}[t]
\resizebox{\columnwidth}{!}{


% \begin{tabular}{lcccccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multicolumn{6}{c}{\textbf{Evaluation Metrics}} \\
%       & human & gpt-4o & gpt-4o-mini & rougel & bleu & EM \\
%      \hline
%      \multirow{1}{*}{GPT-4o-Turbo}    & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}-&\cellcolor{lightblue!25}51.1\\
%      \multirow{1}{*}{GPT-4o-Mini}    & \cellcolor{lightpurple!25}-& \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- &\cellcolor{lightpurple!25}39.3 \\
%      \multirow{1}{*}{Gemini1.5-Pro}    & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- &\cellcolor{lightgray!25}11.2\\
%      \multirow{1}{*}{Gemini1.5-Pro-Flash}    & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- &\cellcolor{lightgreen!25}12.9\\
%      \multirow{1}{*}{GLM-4-Plus}    & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- &\cellcolor{lightyellow!25}47.3\\
%      \multirow{1}{*}{GLM-4-Flash}    & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}-&\cellcolor{lightred!25}40.9\\
     
%      \hline
%      \hline
%      \multirow{1}{*}{QWen-2-7B}    & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- &\cellcolor{lightblue!25}29.6\\
%      \multirow{1}{*}{QWen-2-72B}    & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- &\cellcolor{lightpurple!25}42.5\\
%      \multirow{1}{*}{Llama-3.1-8B}    & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- &\cellcolor{lightgray!25}22.3\\
%      \multirow{1}{*}{Llama-3.1-70B}    & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- &\cellcolor{lightgreen!25}45.8\\
%      \multirow{1}{*}{Llama-3.1-405B}    & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}-  &\cellcolor{lightyellow!25}34.4\\
%      \multirow{1}{*}{Mistral-0.2-7B}    & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- &\cellcolor{lightred!25}7.0 \\
     
%      \bottomrule
% \end{tabular}

\begin{tabular}{lcccccc} \toprule \textbf{Model} & \textbf{Human} & \textbf{GPT-4o} & \textbf{4o-Mini} & \textbf{RougeL} & \textbf{BLEU} & \textbf{EM} \\ \midrule
GPT-4o-Turbo        & 56.13 & 55.75 & 51.00 & 51.1 & 45.94 & 40.31 \\
GPT-4o-Mini         & 36.15 & 36.02 & 40.73 & 39.3 & 46.08 & 33.93 \\
Gemini1.5-Pro       & 12.39 & 12.80 & 10.62 & 11.2 & 12.60 & 8.75 \\
Gemini1.5-Pro-Flash & 13.83 & 13.19 & 12.96 & 12.9 & 14.01 & 9.67 \\
GLM-4-Plus          & 52.90 & 52.62 & 46.02 & 47.3 & 32.75 & 38.27 \\
GLM-4-Flash         & 41.50 & 41.34 & 38.99 & 40.9 & 37.43 & 34.80 \\
\hline
\hline
QWen-2-7B           & 32.95 & 31.99 & 30.10 & 29.6 & 27.98 & 18.70 \\
QWen-2-72B          & 40.87 & 38.66 & 31.24 & 42.5 & 37.76 & 35.67 \\
Llama-3.1-8B        & 21.78 & 21.98 & 22.36 & 22.3 & 20.88 & 14.75 \\
Llama-3.1-70B       & 46.64 & 41.38 & 40.83 & 45.8 & 41.50 & 27.46 \\
Llama-3.1-405B      & 35.01 & 35.97 & 35.88 & 34.4 & 28.00 & 21.29 \\
Mistral-0.2-7B      & 7.85 & 7.33 & 7.32 & 7.0 & 5.09 & 4.47 \\ 
\bottomrule \end{tabular}

% \begin{tabular}{lcccccc} 
% \toprule 
% \textbf{Model} & \textbf{Human} & \textbf{GPT-4o} & \textbf{4o-Mini} & \textbf{RougeL} & \textbf{BLEU} & \textbf{EM} \\ \midrule GPT-4o-Turbo & 66.13 & 65.75 & 65.00 & 65.94 & 60.31 \\ GPT-4o-Mini & 56.15 & 56.02 & 55.73 & 56.08 & 53.93 \\ Gemini1.5-Pro & 32.39 & 32.80 & 33.62 & 32.60 & 38.75 \\ Gemini1.5-Pro-Flash & 33.83 & 34.19 & 34.96 & 34.01 & 39.67 \\ GLM-4-Plus & 62.90 & 62.62 & 62.02 & 62.75 & 58.27 \\ GLM-4-Flash & 57.50 & 57.34 & 56.99 & 57.43 & 54.80 \\ \hline QWen-2-7B & 47.95 & 47.99 & 48.10 & 47.98 & 48.70 \\ QWen-2-72B & 58.87 & 58.66 & 58.24 & 58.76 & 55.67 \\ Llama-3.1-8B & 41.78 & 41.98 & 42.36 & 41.88 & 44.75 \\ Llama-3.1-70B & 61.64 & 61.38 & 60.83 & 61.50 & 57.46 \\ Llama-3.1-405B & 52.01 & 51.97 & 51.88 & 52.00 & 51.29 \\ Mistral-0.2-7B & 28.85 & 29.33 & 30.32 & 29.09 & 36.47 \\ 
% \bottomrule  
% \end{tabular}
}
\caption{Performance of all LLMs and Humans on StrucText-Eval-Hard based on different metrics~(1,000 samples for each metrics).}
\label{tab:other_metrics}

\end{table}

==> overall_performance_tables.01.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{c|cccccccc}
    \hline
    & JSON & LaTeX & Markdown & ORG & Tabular & Tree & XML & YAML \\
    \hline
    erniebot\_turbo & 0.191 & 0.006 & 0.006 & 0.005 & 0.114 & 0.024 & 0.131 & 0.190 \\
    gpt4\_turbo & 0.813 & 0.592 & 0.532 & 0.461 & 0.679 & 0.431 & 0.772 & 0.789 \\
    gpt4 & 0.867 & 0.706 & 0.611 & 0.601 & 0.665 & 0.441 & 0.771 & 0.857 \\
    minimax & 0.720 & 0.508 & 0.429 & 0.363 & 0.384 & 0.316 & 0.600 & 0.635 \\
    spark & 0.325 & 0.188 & 0.139 & 0.109 & 0.038 & 0.252 & 0.511 & 0.412 \\
    \hline
\end{tabular}
\caption{Model performance on different languages.}
\label{tab:table1}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{c|cccccccc}
    \hline
    & PC & PW & SY & TR & SJ & ST & TD & TH \\
    \hline
    erniebot\_turbo & 0.020 & 0.142 & 0.232 & 0.092 & 0.016 & 0.082 & 0.045 & 0.017 \\
    gpt4\_turbo & 0.645 & 0.671 & 0.740 & 0.698 & 0.469 & 0.650 & 0.627 & 0.152 \\
    gpt4 & 0.670 & 0.752 & 0.770 & 0.774 & 0.575 & 0.587 & 0.412 & 0.387 \\
    minimax & 0.225 & 0.530 & 0.691 & 0.672 & 0.156 & 0.283 & 0.325 & 0.425 \\
    spark & 0.179 & 0.195 & 0.697 & 0.251 & 0.025 & 0.031 & 0.166 & 0.337 \\
    \hline
\end{tabular}
\caption{Model performance on different tasks.}
\label{tab:table2}
\end{table}


==> overall_performance_tables.02.tex <==
\begin{table}[t]
    \centering

    \resizebox{\textwidth}{!}{
\begin{tabular}{c|ccccccccc}
\toprule
\textbf{Model} & \textbf{Prompt} & \textbf{JSON} & \textbf{LaTeX} & \textbf{Markdown} & \textbf{ORG} & \textbf{SQL} & \textbf{Tree} & \textbf{XML} & \textbf{YAML} \\ \hline
\multirow{5}{*}{gpt4\_turbo} & Naive & 0.816 & 0.574 & 0.521 & 0.449 & 0.691 & 0.438 & 0.788 & 0.792 \\  
 & 1-shot & 0.900 & 0.708 & 0.646 & 0.646 & 0.562 & 0.562 & 0.729 & 0.838 \\  
 & 2-shot & 0.900 & 0.688 & 0.667 & 0.708 & 0.688 & 0.479 & 0.708 & 0.875 \\  
 & Rule Hint & 0.850 & 0.604 & 0.583 & 0.438 & 0.750 & 0.271 & 0.792 & 0.887 \\  
 & Hint Elicitation & 0.550 & 0.750 & 0.458 & 0.312 & 0.438 & 0.292 & 0.542 & 0.512 \\ \hline
\multirow{5}{*}{gpt4} & Naive & 1.000 & 0.750 & 0.688 & 0.500 & 0.750 & 0.396 & 0.896 & 0.900 \\  
 & 1-shot & 0.912 & 0.674 & 0.667 & 0.761 & 0.672 & 0.521 & 0.812 & 0.950 \\  
 & 2-shot & 0.950 & 0.771 & 0.717 & 0.729 & 0.812 & 0.583 & 0.854 & 0.950 \\  
 & Rule Hint & 0.963 & 0.625 & 0.596 & 0.521 & 0.578 & 0.417 & 0.854 & 0.950 \\  
 & Hint Elicitation & 0.512 & 0.708 & 0.396 & 0.500 & 0.516 & 0.292 & 0.438 & 0.537 \\ \hline
\multirow{5}{*}{minimax} & Naive & 0.825 & 0.583 & 0.438 & 0.312 & 0.391 & 0.167 & 0.604 & 0.675 \\  
 & 1-shot & 0.787 & 0.458 & 0.562 & 0.438 & 0.375 & 0.521 & 0.646 & 0.750 \\  
 & 2-shot & 0.850 & 0.521 & 0.417 & 0.438 & 0.469 & 0.438 & 0.542 & 0.787 \\  
 & Rule Hint & 0.800 & 0.438 & 0.500 & 0.438 & 0.375 & 0.167 & 0.729 & 0.650 \\  
 & Hint Elicitation & 0.338 & 0.542 & 0.229 & 0.188 & 0.219 & 0.292 & 0.479 & 0.312 \\ \hline
\multirow{5}{*}{spark} & Naive & 0.525 & 0.217 & 0.043 & 0.167 & 0.062 & 0.261 & 0.644 & 0.671 \\  
 & 1-shot & 0.287 & 0.062 & 0.042 & 0.062 & 0.016 & 0.188 & 0.292 & 0.463 \\  
 & 2-shot & 0.300 & 0.250 & 0.292 & 0.125 & 0.016 & 0.646 & 0.792 & 0.633 \\  
 & Rule Hint & 0.487 & 0.062 & 0.125 & 0.021 & 0.094 & 0.104 & 0.438 & 0.200 \\  
 & Hint Elicitation & 0.025 & 0.412 & 0.226 & 0.207 & 0.000 & 0.062 & 0.381 & 0.100 \\ \hline
\multirow{5}{*}{erniebot\_turbo} & Naive & 0.193 & 0.001 & 0.001 & 0.002 & 0.109 & 0.017 & 0.134 & 0.197 \\  
 & 1-shot & 0.212 & 0.021 & 0.021 & 0.043 & 0.250 & 0.104 & 0.083 & 0.250 \\  
 & 2-shot & 0.150 & 0.104 & 0.083 & 0.042 & 0.188 & 0.146 & 0.167 & 0.113 \\  
 & Rule Hint & 0.237 & 0.000 & 0.021 & 0.000 & 0.062 & 0.000 & 0.146 & 0.225 \\  
 & Hint Elicitation & 0.113 & 0.000 & 0.000 & 0.000 & 0.109 & 0.000 & 0.083 & 0.025 \\ 
 \bottomrule
\end{tabular}}

    \caption{Close-sourced LLMs' performance on different languages.}
    \label{tab:my_label}
\end{table}


\begin{table}[t]
    \centering
    \small
    \begin{tabular}{c|ccccccccc}
\toprule
\textbf{Model} & \textbf{Prompt} & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{SJ} & \textbf{ST} & \textbf{TD} & \textbf{TH} \\ \hline
\multirow{5}{*}{gpt4\_turbo} & Naive & 0.662 & 0.668 & 0.770 & 0.687 & 0.490 & 0.661 & 0.649 & 0.128 \\  
 & 1-shot & 0.646 & 0.762 & 0.708 & 0.808 & 0.375 & 0.438 & 0.750 & 0.438 \\  
 & 2-shot & 0.792 & 0.775 & 0.708 & 0.798 & 0.562 & 0.656 & 0.438 & 0.312 \\  
 & Rule Hint & 0.646 & 0.637 & 0.792 & 0.745 & 0.250 & 0.875 & 0.500 & 0.062 \\  
 & Hint Elicitation & 0.146 & 0.575 & 0.125 & 0.678 & 0.188 & 0.375 & 0.375 & 0.312 \\ \hline
\multirow{5}{*}{gpt4} & Naive & 0.771 & 0.821 & 0.896 & 0.798 & 0.688 & 0.719 & 0.312 & 0.312 \\  
 & 1-shot & 0.792 & 0.800 & 0.938 & 0.821 & 0.688 & 0.500 & 0.375 & 0.438 \\  
 & 2-shot & 0.750 & 0.808 & 0.979 & 0.851 & 0.812 & 0.719 & 0.438 & 0.750 \\  
 & Rule Hint & 0.771 & 0.775 & 0.896 & 0.768 & 0.250 & 0.531 & 0.625 & 0.125 \\  
 & Hint Elicitation & 0.271 & 0.562 & 0.146 & 0.635 & 0.438 & 0.469 & 0.312 & 0.312 \\ \hline
\multirow{5}{*}{minimax} & Naive & 0.271 & 0.562 & 0.792 & 0.796 & 0.145 & 0.306 & 0.250 & 0.000 \\  
 & 1-shot & 0.229 & 0.588 & 0.833 & 0.688 & 0.250 & 0.156 & 0.438 & 1.000 \\  
 & 2-shot & 0.354 & 0.600 & 0.896 & 0.639 & 0.438 & 0.250 & 0.125 & 1.000 \\  
 & Rule Hint & 0.083 & 0.525 & 0.938 & 0.683 & 0.125 & 0.219 & 0.438 & 0.000 \\  
 & Hint Elicitation & 0.188 & 0.375 & 0.000 & 0.462 & 0.000 & 0.188 & 0.375 & 0.125 \\ \hline
\multirow{5}{*}{spark} & Naive & 0.354 & 0.362 & 0.833 & 0.313 & 0.000 & 0.094 & 0.000 & 0.500 \\  
 & 1-shot & 0.062 & 0.100 & 0.625 & 0.207 & 0.000 & 0.000 & 0.250 & 0.250 \\  
 & 2-shot & 0.417 & 0.212 & 0.896 & 0.367 & 0.062 & 0.000 & 0.500 & 0.688 \\  
 & Rule Hint & 0.042 & 0.150 & 0.854 & 0.173 & 0.062 & 0.062 & 0.062 & 0.125 \\  
 & Hint Elicitation & 0.021 & 0.145 & 0.261 & 0.188 & 0.000 & 0.000 & 0.000 & 0.125 \\ \hline
\multirow{5}{*}{erniebot\_turbo} & Naive & 0.018 & 0.145 & 0.249 & 0.088 & 0.010 & 0.087 & 0.036 & 0.009 \\  
 & 1-shot & 0.062 & 0.163 & 0.125 & 0.184 & 0.000 & 0.062 & 0.250 & 0.000 \\  
 & 2-shot & 0.021 & 0.100 & 0.208 & 0.144 & 0.250 & 0.000 & 0.125 & 0.250 \\  
 & Rule Hint & 0.042 & 0.138 & 0.208 & 0.120 & 0.000 & 0.031 & 0.000 & 0.000 \\  
 & Hint Elicitation & 0.000 & 0.125 & 0.042 & 0.029 & 0.000 & 0.125 & 0.000 & 0.000 \\ 
 \bottomrule
\end{tabular}

\caption{Close-sourced LLMs' performance on different tasks.}
\label{tab:}
\end{table}


==> overall_performance_tables.03.tex <==
\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cccccccc|c}
\hline
\textbf{Model} & \textbf{Prompt} & \textbf{JSON} & \textbf{LaTeX} & \textbf{Markdown} & \textbf{ORG} & \textbf{SQL} & \textbf{Tree} & \textbf{XML} & \textbf{YAML} & \textbf{all} \\ \hline
\multirow{8}{*}{erniebot\_turbo} & Base & 0.274 & 0.002 & 0.000 & 0.000 & 0.130 & 0.026 & 0.143 & 0.244 & 0.125 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & -0.080 & -0.001 & +0.001 & +0.002 & -0.021 & -0.009 & -0.009 & -0.047 & -0.026 \\
 & 1-shot & 0.250 & 0.000 & 0.042 & 0.087 & 0.219 & 0.125 & 0.083 & 0.250 & 0.152 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & -0.037 & +0.021 & -0.021 & -0.043 & +0.031 & -0.021 & +0.000 & +0.000 & -0.009 \\
 & 2-shot & 0.125 & 0.125 & 0.125 & 0.083 & 0.219 & 0.208 & 0.167 & 0.050 & 0.134 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & -0.021 & -0.042 & -0.042 & -0.031 & -0.062 & +0.000 & +0.062 & -0.006 \\
 & Rule Hint & 0.325 & 0.000 & 0.000 & 0.000 & 0.094 & 0.000 & 0.125 & 0.325 & 0.138 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & -0.087 & +0.000 & +0.021 & +0.000 & -0.031 & +0.000 & +0.021 & -0.100 & -0.032 \\ \hline
\multirow{8}{*}{minimax} & Base & 0.775 & 0.583 & 0.417 & 0.292 & 0.442 & 0.208 & 0.583 & 0.700 & 0.466 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.050 & +0.000 & +0.021 & +0.021 & -0.269 & -0.042 & +0.021 & -0.025 & -0.184 \\
 & 1-shot & 0.800 & 0.500 & 0.583 & 0.500 & 0.375 & 0.500 & 0.625 & 0.850 & 0.616 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & -0.013 & -0.042 & -0.021 & -0.062 & +0.000 & +0.021 & +0.021 & -0.100 & -0.028 \\
 & 2-shot & 0.900 & 0.583 & 0.542 & 0.542 & 0.500 & 0.458 & 0.625 & 0.825 & 0.651 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & -0.050 & -0.062 & -0.125 & -0.104 & -0.031 & -0.021 & -0.083 & -0.037 & -0.060 \\
 & Rule Hint & 0.775 & 0.375 & 0.542 & 0.500 & 0.406 & 0.167 & 0.667 & 0.625 & 0.530 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & +0.062 & -0.042 & -0.062 & -0.031 & +0.000 & +0.062 & +0.025 & +0.006 \\ \hline
\multirow{8}{*}{spark} & Base & 0.400 & 0.208 & 0.043 & 0.125 & 0.031 & 0.292 & 0.636 & 0.575 & 0.306 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.125 & +0.000 & +0.000 & +0.042 & +0.031 & -0.043 & +0.022 & +0.089 & +0.044 \\
 & 1-shot & 0.275 & 0.083 & 0.042 & 0.042 & 0.031 & 0.042 & 0.333 & 0.375 & 0.172 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.013 & -0.021 & +0.000 & +0.021 & -0.016 & +0.146 & -0.042 & +0.087 & +0.026 \\
 & 2-shot & 0.300 & 0.250 & 0.417 & 0.125 & 0.000 & 0.667 & 0.667 & 0.625 & 0.379 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.000 & -0.125 & +0.000 & +0.016 & -0.021 & +0.125 & +0.000 & +0.000 \\
 & Rule Hint & 0.425 & 0.042 & 0.083 & 0.000 & 0.000 & 0.083 & 0.417 & 0.075 & 0.151 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.062 & +0.021 & +0.042 & +0.021 & +0.094 & +0.021 & +0.021 & +0.125 & +0.058 \\ \hline
\multirow{8}{*}{gpt4} & Base & 1.000 & 0.833 & 0.708 & 0.435 & 0.781 & 0.417 & 0.917 & 0.925 & 0.784 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +1.000 & +0.667 & +0.667 & +0.565 & +0.719 & +0.375 & +0.875 & +0.875 & +0.749 \\
 & 1-shot & 0.950 & 0.667 & 0.708 & 0.783 & 0.688 & 0.542 & 0.792 & 0.975 & 0.789 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.875 & +0.682 & +0.625 & +0.739 & +0.656 & +0.500 & +0.833 & +0.925 & +0.751 \\
 & 2-shot & 0.950 & 0.792 & 0.652 & 0.750 & 0.875 & 0.542 & 0.875 & 0.975 & 0.827 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.950 & +0.750 & +0.783 & +0.708 & +0.750 & +0.625 & +0.833 & +0.925 & +0.810 \\
 & Rule Hint & 0.975 & 0.667 & 0.652 & 0.500 & 0.656 & 0.458 & 0.833 & 0.950 & 0.745 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.950 & +0.583 & +0.542 & +0.542 & +0.500 & +0.375 & +0.875 & +0.950 & +0.698 \\ \hline
\multirow{8}{*}{gpt4\_turbo} & Base & 0.876 & 0.613 & 0.569 & 0.518 & 0.649 & 0.508 & 0.804 & 0.824 & 0.693 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & -0.060 & -0.039 & -0.049 & -0.068 & -0.014 & -0.070 & -0.016 & -0.032 & -0.042 \\
 & 1-shot & 0.925 & 0.667 & 0.625 & 0.625 & 0.594 & 0.583 & 0.708 & 0.825 & 0.716 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & -0.025 & +0.042 & +0.021 & +0.021 & -0.031 & -0.021 & +0.021 & +0.013 & +0.002 \\
 & 2-shot & 0.875 & 0.625 & 0.667 & 0.750 & 0.688 & 0.542 & 0.750 & 0.925 & 0.750 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & +0.062 & +0.000 & -0.042 & +0.000 & -0.062 & -0.042 & -0.050 & -0.013 \\
 & Rule Hint & 0.825 & 0.625 & 0.625 & 0.500 & 0.781 & 0.292 & 0.708 & 0.875 & 0.685 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & -0.021 & -0.042 & -0.062 & -0.031 & -0.021 & +0.083 & +0.013 & -0.004 \\ \hline
\end{tabular}}
\caption{Close-sourced LLMs' performance on different languages.}
\label{tab:api_on_language}
\end{table}

\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cccccccc|c}
\hline
\textbf{Model} & \textbf{Prompt} & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{SJ} & \textbf{ST} & \textbf{TD} & \textbf{TH} & \textbf{all} \\ \hline
\multirow{8}{*}{erniebot\_turbo} & Base & 0.028 & 0.223 & 0.232 & 0.113 & 0.005 & 0.111 & 0.054 & 0.018 & 0.125 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.008 & +0.067 & +0.266 & +0.062 & +0.014 & +0.062 & +0.018 & +0.000 & +0.072 \\
 & 1-shot & 0.125 & 0.200 & 0.083 & 0.194 & 0.000 & 0.000 & 0.250 & 0.000 & 0.152 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.125 & +0.167 & +0.173 & +0.000 & +0.125 & +0.250 & +0.000 & 0.134 \\
 & 2-shot & 0.042 & 0.100 & 0.042 & 0.183 & 0.250 & 0.000 & 0.250 & 0.250 & 0.134 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.100 & +0.375 & +0.106 & +0.250 & +0.000 & +0.000 & +0.250 & +0.121 \\
 & Rule Hint & 0.083 & 0.200 & 0.250 & 0.144 & 0.000 & 0.062 & 0.000 & 0.000 & 0.138 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.075 & +0.167 & +0.096 & +0.000 & +0.000 & +0.000 & +0.000 & +0.073 \\ \hline
\multirow{8}{*}{minimax} & Base & 0.250 & 0.575 & 0.750 & 0.845 & 0.131 & 0.330 & 0.375 & 0.000 & 0.466 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.292 & +0.550 & +0.833 & +0.673 & +0.170 & +0.242 & +0.125 & +0.000 & +0.390 \\
 & 1-shot & 0.292 & 0.675 & 0.917 & 0.683 & 0.250 & 0.188 & 0.375 & 1.000 & 0.616 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.167 & +0.500 & +0.750 & +0.692 & +0.250 & +0.125 & +0.500 & +1.000 & +0.560 \\
 & 2-shot & 0.417 & 0.700 & 0.917 & 0.702 & 0.500 & 0.312 & 0.125 & 1.000 & 0.651 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.292 & +0.500 & +0.875 & +0.577 & +0.375 & +0.188 & +0.125 & +1.000 & +0.530 \\
 & Rule Hint & 0.083 & 0.550 & 0.917 & 0.654 & 0.125 & 0.250 & 0.500 & 0.000 & 0.530 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.083 & +0.500 & +0.958 & +0.712 & +0.125 & +0.188 & +0.375 & +0.000 & +0.543 \\ \hline
\multirow{8}{*}{spark} & Base & 0.292 & 0.275 & 0.833 & 0.267 & 0.000 & 0.062 & 0.000 & 0.500 & 0.306 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.417 & +0.450 & +0.833 & +0.360 & +0.000 & +0.125 & +0.000 & +0.500 & +0.398 \\
 & 1-shot & 0.000 & 0.125 & 0.625 & 0.183 & 0.000 & 0.000 & 0.000 & 0.125 & 0.172 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.125 & +0.075 & +0.625 & +0.231 & +0.000 & +0.000 & +0.500 & +0.375 & +0.224 \\
 & 2-shot & 0.375 & 0.225 & 0.917 & 0.365 & 0.000 & 0.000 & 0.500 & 0.750 & 0.379 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.458 & +0.200 & +0.875 & +0.369 & +0.125 & +0.000 & +0.500 & +0.625 & +0.381 \\
 & Rule Hint & 0.083 & 0.050 & 0.708 & 0.135 & 0.000 & 0.000 & 0.000 & 0.000 & 0.151 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.250 & +1.000 & +0.212 & +0.125 & +0.125 & +0.125 & +0.250 & +0.267 \\ \hline
\multirow{8}{*}{gpt4} & Base & 0.792 & 0.795 & 0.917 & 0.827 & 0.750 & 0.750 & 0.250 & 0.375 & 0.784 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.750 & +0.846 & +0.875 & +0.769 & +0.625 & +0.688 & +0.375 & +0.250 & +0.749 \\
 & 1-shot & 0.875 & 0.800 & 0.917 & 0.840 & 0.750 & 0.500 & 0.375 & 0.500 & 0.789 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.708 & +0.800 & +0.958 & +0.802 & +0.625 & +0.500 & +0.375 & +0.375 & +0.751 \\
 & 2-shot & 0.792 & 0.821 & 0.958 & 0.846 & 1.000 & 0.750 & 0.500 & 0.625 & 0.827 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.708 & +0.795 & +1.000 & +0.856 & +0.625 & +0.688 & +0.375 & +0.875 & +0.810 \\
 & Rule Hint & 0.833 & 0.800 & 0.917 & 0.757 & 0.500 & 0.562 & 0.750 & 0.125 & 0.745 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.708 & +0.750 & +0.875 & +0.779 & +0.000 & +0.500 & +0.500 & +0.125 & +0.698 \\ \hline
\multirow{8}{*}{gpt4\_turbo} & Base & 0.712 & 0.698 & 0.778 & 0.745 & 0.457 & 0.591 & 0.714 & 0.185 & 0.693 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.611 & +0.638 & +0.762 & +0.628 & +0.527 & +0.746 & +0.583 & +0.071 & +0.626 \\
 & 1-shot & 0.667 & 0.775 & 0.708 & 0.788 & 0.375 & 0.500 & 0.750 & 0.375 & 0.716 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.625 & +0.750 & +0.708 & +0.827 & +0.375 & +0.375 & +0.750 & +0.500 & +0.720 \\
 & 2-shot & 0.833 & 0.750 & 0.750 & 0.808 & 0.500 & 0.688 & 0.500 & 0.375 & 0.750 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.750 & +0.800 & +0.667 & +0.788 & +0.625 & +0.625 & +0.375 & +0.250 & +0.724 \\
 & Rule Hint & 0.667 & 0.600 & 0.708 & 0.769 & 0.250 & 0.938 & 0.500 & 0.125 & 0.685 \\
 & \textit{\multicolumn{1}{r}{+CoT}} & +0.625 & +0.675 & +0.875 & +0.721 & +0.250 & +0.812 & +0.500 & +0.000 & +0.677 \\ \hline
\end{tabular}}
\caption{Close-sourced LLMs' performance on different tasks.}
\label{tab:api_on_task}
\end{table}



\begin{table}[h!]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{c|c|cccccccc|c}
\hline
\textbf{Model} & \textbf{Prompt} & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{SJ} & \textbf{ST} & \textbf{TD} & \textbf{TH} & \textbf{all} \\ \hline
\multirow{8}{*}{erniebot\_turbo} & \cellcolor{lightblue}Base & \cellcolor{lightblue}0.028 & \cellcolor{lightblue}0.223 & \cellcolor{lightblue}0.232 & \cellcolor{lightblue}0.113 & \cellcolor{lightblue}0.005 & \cellcolor{lightblue}0.111 & \cellcolor{lightblue}0.054 & \cellcolor{lightblue}0.018 & \cellcolor{lightblue}0.125 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.008 & \cellcolor{darkblue!8}+0.067 & \cellcolor{darkblue!8}+0.266 & \cellcolor{darkblue!8}+0.062 & \cellcolor{darkblue!8}+0.014 & \cellcolor{darkblue!8}+0.062 & \cellcolor{darkblue!8}+0.018 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.072 \\
 & \cellcolor{lightblue}1-shot & \cellcolor{lightblue}0.125 & \cellcolor{lightblue}0.200 & \cellcolor{lightblue}0.083 & \cellcolor{lightblue}0.194 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.152 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.167 & \cellcolor{darkblue!8}+0.173 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}0.134 \\
 & \cellcolor{lightblue}2-shot & \cellcolor{lightblue}0.042 & \cellcolor{lightblue}0.100 & \cellcolor{lightblue}0.042 & \cellcolor{lightblue}0.183 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.134 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.100 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.106 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.121 \\
 & \cellcolor{lightblue}Rule Hint & \cellcolor{lightblue}0.083 & \cellcolor{lightblue}0.200 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.144 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.062 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.138 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.075 & \cellcolor{darkblue!8}+0.167 & \cellcolor{darkblue!8}+0.096 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.073 \\ \hline
\multirow{8}{*}{minimax} & \cellcolor{lightblue}Base & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.575 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.845 & \cellcolor{lightblue}0.131 & \cellcolor{lightblue}0.330 & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.466 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.292 & \cellcolor{darkblue!8}+0.550 & \cellcolor{darkblue!8}+0.833 & \cellcolor{darkblue!8}+0.673 & \cellcolor{darkblue!8}+0.170 & \cellcolor{darkblue!8}+0.242 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.390 \\
 & \cellcolor{lightblue}1-shot & \cellcolor{lightblue}0.292 & \cellcolor{lightblue}0.675 & \cellcolor{lightblue}0.917 & \cellcolor{lightblue}0.683 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.188 & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}1.000 & \cellcolor{lightblue}0.616 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.167 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.750 & \cellcolor{darkblue!8}+0.692 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+1.000 & \cellcolor{darkblue!8}+0.560 \\
 & \cellcolor{lightblue}2-shot & \cellcolor{lightblue}0.417 & \cellcolor{lightblue}0.700 & \cellcolor{lightblue}0.917 & \cellcolor{lightblue}0.702 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.312 & \cellcolor{lightblue}0.125 & \cellcolor{lightblue}1.000 & \cellcolor{lightblue}0.651 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.292 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.875 & \cellcolor{darkblue!8}+0.577 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.188 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+1.000 & \cellcolor{darkblue!8}+0.530 \\
 & \cellcolor{lightblue}Rule Hint & \cellcolor{lightblue}0.083 & \cellcolor{lightblue}0.550 & \cellcolor{lightblue}0.917 & \cellcolor{lightblue}0.654 & \cellcolor{lightblue}0.125 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.530 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.083 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.958 & \cellcolor{darkblue!8}+0.712 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.188 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.543 \\ \hline
\multirow{8}{*}{spark} & \cellcolor{lightblue}Base & \cellcolor{lightblue}0.292 & \cellcolor{lightblue}0.275 & \cellcolor{lightblue}0.833 & \cellcolor{lightblue}0.267 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.062 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.306 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.417 & \cellcolor{darkblue!8}+0.450 & \cellcolor{darkblue!8}+0.833 & \cellcolor{darkblue!8}+0.360 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.398 \\
 & \cellcolor{lightblue}1-shot & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.125 & \cellcolor{lightblue}0.625 & \cellcolor{lightblue}0.183 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.125 & \cellcolor{lightblue}0.172 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.075 & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.231 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.224 \\
 & \cellcolor{lightblue}2-shot & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}0.225 & \cellcolor{lightblue}0.917 & \cellcolor{lightblue}0.365 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.379 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.458 & \cellcolor{darkblue!8}+0.200 & \cellcolor{darkblue!8}+0.875 & \cellcolor{darkblue!8}+0.369 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.381 \\
 & \cellcolor{lightblue}Rule Hint & \cellcolor{lightblue}0.083 & \cellcolor{lightblue}0.050 & \cellcolor{lightblue}0.708 & \cellcolor{lightblue}0.135 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.000 & \cellcolor{lightblue}0.151 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+1.000 & \cellcolor{darkblue!8}+0.212 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.267 \\ \hline
\multirow{8}{*}{gpt4} & \cellcolor{lightblue}Base & \cellcolor{lightblue}0.792 & \cellcolor{lightblue}0.795 & \cellcolor{lightblue}0.917 & \cellcolor{lightblue}0.827 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}0.784 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.750 & \cellcolor{darkblue!8}+0.846 & \cellcolor{darkblue!8}+0.875 & \cellcolor{darkblue!8}+0.769 & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.688 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.749 \\
 & \cellcolor{lightblue}1-shot & \cellcolor{lightblue}0.875 & \cellcolor{lightblue}0.800 & \cellcolor{lightblue}0.917 & \cellcolor{lightblue}0.840 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.789 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.708 & \cellcolor{darkblue!8}+0.800 & \cellcolor{darkblue!8}+0.958 & \cellcolor{darkblue!8}+0.802 & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.751 \\
 & \cellcolor{lightblue}2-shot & \cellcolor{lightblue}0.792 & \cellcolor{lightblue}0.821 & \cellcolor{lightblue}0.958 & \cellcolor{lightblue}0.846 & \cellcolor{lightblue}1.000 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.625 & \cellcolor{lightblue}0.827 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.708 & \cellcolor{darkblue!8}+0.795 & \cellcolor{darkblue!8}+1.000 & \cellcolor{darkblue!8}+0.856 & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.688 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.875 & \cellcolor{darkblue!8}+0.810 \\
 & \cellcolor{lightblue}Rule Hint & \cellcolor{lightblue}0.833 & \cellcolor{lightblue}0.800 & \cellcolor{lightblue}0.917 & \cellcolor{lightblue}0.757 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.562 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.125 & \cellcolor{lightblue}0.745 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.708 & \cellcolor{darkblue!8}+0.750 & \cellcolor{darkblue!8}+0.875 & \cellcolor{darkblue!8}+0.779 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.125 & \cellcolor{darkblue!8}+0.698 \\ \hline
\multirow{8}{*}{gpt4\_turbo} & \cellcolor{lightblue}Base & \cellcolor{lightblue}0.712 & \cellcolor{lightblue}0.698 & \cellcolor{lightblue}0.778 & \cellcolor{lightblue}0.745 & \cellcolor{lightblue}0.457 & \cellcolor{lightblue}0.591 & \cellcolor{lightblue}0.714 & \cellcolor{lightblue}0.185 & \cellcolor{lightblue}0.693 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.611 & \cellcolor{darkblue!8}+0.638 & \cellcolor{darkblue!8}+0.762 & \cellcolor{darkblue!8}+0.628 & \cellcolor{darkblue!8}+0.527 & \cellcolor{darkblue!8}+0.746 & \cellcolor{darkblue!8}+0.583 & \cellcolor{darkblue!8}+0.071 & \cellcolor{darkblue!8}+0.626 \\
 & \cellcolor{lightblue}1-shot & \cellcolor{lightblue}0.667 & \cellcolor{lightblue}0.775 & \cellcolor{lightblue}0.708 & \cellcolor{lightblue}0.788 & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}0.716 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.750 & \cellcolor{darkblue!8}+0.708 & \cellcolor{darkblue!8}+0.827 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.750 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.720 \\
 & \cellcolor{lightblue}2-shot & \cellcolor{lightblue}0.833 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.750 & \cellcolor{lightblue}0.808 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.688 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.375 & \cellcolor{lightblue}0.750 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.750 & \cellcolor{darkblue!8}+0.800 & \cellcolor{darkblue!8}+0.667 & \cellcolor{darkblue!8}+0.788 & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.375 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.724 \\
 & \cellcolor{lightblue}Rule Hint & \cellcolor{lightblue}0.667 & \cellcolor{lightblue}0.600 & \cellcolor{lightblue}0.708 & \cellcolor{lightblue}0.769 & \cellcolor{lightblue}0.250 & \cellcolor{lightblue}0.938 & \cellcolor{lightblue}0.500 & \cellcolor{lightblue}0.125 & \cellcolor{lightblue}0.685 \\
 & \cellcolor{darkblue!8}+CoT & \cellcolor{darkblue!8}+0.625 & \cellcolor{darkblue!8}+0.675 & \cellcolor{darkblue!8}+0.875 & \cellcolor{darkblue!8}+0.721 & \cellcolor{darkblue!8}+0.250 & \cellcolor{darkblue!8}+0.812 & \cellcolor{darkblue!8}+0.500 & \cellcolor{darkblue!8}+0.000 & \cellcolor{darkblue!8}+0.677 \\ \hline
\end{tabular}}
\caption{Close-sourced LLMs' performance on different tasks.}
\label{tab:api_on_task}
\end{table}




% \begin{table}[h!]
% \centering
% \begin{tabular}{c|l|cccccccc|c}
% \hline
% \textbf{Model} & \textbf{Prompt} & \textbf{JSON} & \textbf{LaTeX} & \textbf{Markdown} & \textbf{ORG} & \textbf{SQL} & \textbf{Tree} & \textbf{XML} & \textbf{YAML} & \textbf{all} \\ \hline
% \multirow{8}{*}{erniebot\_turbo} & Base & 0.274 & 0.002 & 0.000 & 0.000 & 0.130 & 0.026 & 0.143 & 0.244 & 0.125 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & -0.080 & -0.001 & +0.001 & +0.002 & -0.021 & -0.009 & -0.009 & -0.047 & -0.026 \\
%  & 1-shot & 0.250 & 0.000 & 0.042 & 0.087 & 0.219 & 0.125 & 0.083 & 0.250 & 0.152 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & -0.037 & +0.021 & -0.021 & -0.043 & +0.031 & -0.021 & +0.000 & +0.000 & -0.009 \\
%  & 2-shot & 0.125 & 0.125 & 0.125 & 0.083 & 0.219 & 0.208 & 0.167 & 0.050 & 0.134 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & -0.021 & -0.042 & -0.042 & -0.031 & -0.062 & +0.000 & +0.062 & -0.006 \\
%  & Rule Hint & 0.325 & 0.000 & 0.000 & 0.000 & 0.094 & 0.000 & 0.125 & 0.325 & 0.138 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & -0.087 & +0.000 & +0.021 & +0.000 & -0.031 & +0.000 & +0.021 & -0.100 & -0.032 \\ \hline
% \multirow{8}{*}{minimax} & Base & 0.775 & 0.583 & 0.417 & 0.292 & 0.442 & 0.208 & 0.583 & 0.700 & 0.466 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.050 & +0.000 & +0.021 & +0.021 & -0.269 & -0.042 & +0.021 & -0.025 & -0.184 \\
%  & 1-shot & 0.800 & 0.500 & 0.583 & 0.500 & 0.375 & 0.500 & 0.625 & 0.850 & 0.616 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & -0.013 & -0.042 & -0.021 & -0.062 & +0.000 & +0.021 & +0.021 & -0.100 & -0.028 \\
%  & 2-shot & 0.900 & 0.583 & 0.542 & 0.542 & 0.500 & 0.458 & 0.625 & 0.825 & 0.651 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & -0.050 & -0.062 & -0.125 & -0.104 & -0.031 & -0.021 & -0.083 & -0.037 & -0.060 \\
%  & Rule Hint & 0.775 & 0.375 & 0.542 & 0.500 & 0.406 & 0.167 & 0.667 & 0.625 & 0.530 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & +0.062 & -0.042 & -0.062 & -0.031 & +0.000 & +0.062 & +0.025 & +0.006 \\ \hline
% \multirow{8}{*}{spark} & Base & 0.400 & 0.208 & 0.043 & 0.125 & 0.031 & 0.292 & 0.636 & 0.575 & 0.306 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.125 & +0.000 & +0.000 & +0.042 & +0.031 & -0.043 & +0.022 & +0.089 & +0.044 \\
%  & 1-shot & 0.275 & 0.083 & 0.042 & 0.042 & 0.031 & 0.042 & 0.333 & 0.375 & 0.172 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.013 & -0.021 & +0.000 & +0.021 & -0.016 & +0.146 & -0.042 & +0.087 & +0.026 \\
%  & 2-shot & 0.300 & 0.250 & 0.417 & 0.125 & 0.000 & 0.667 & 0.667 & 0.625 & 0.379 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.000 & -0.125 & +0.000 & +0.016 & -0.021 & +0.125 & +0.000 & +0.000 \\
%  & Rule Hint & 0.425 & 0.042 & 0.083 & 0.000 & 0.000 & 0.083 & 0.417 & 0.075 & 0.151 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.062 & +0.021 & +0.042 & +0.021 & +0.094 & +0.021 & +0.021 & +0.125 & +0.058 \\ \hline
% \multirow{8}{*}{gpt4} & Base & 1.000 & 0.833 & 0.708 & 0.435 & 0.781 & 0.417 & 0.917 & 0.925 & 0.784 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +1.000 & +0.667 & +0.667 & +0.565 & +0.719 & +0.375 & +0.875 & +0.875 & +0.749 \\
%  & 1-shot & 0.950 & 0.667 & 0.708 & 0.783 & 0.688 & 0.542 & 0.792 & 0.975 & 0.789 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.875 & +0.682 & +0.625 & +0.739 & +0.656 & +0.500 & +0.833 & +0.925 & +0.751 \\
%  & 2-shot & 0.950 & 0.792 & 0.652 & 0.750 & 0.875 & 0.542 & 0.875 & 0.975 & 0.827 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.950 & +0.750 & +0.783 & +0.708 & +0.750 & +0.625 & +0.833 & +0.925 & +0.810 \\
%  & Rule Hint & 0.975 & 0.667 & 0.652 & 0.500 & 0.656 & 0.458 & 0.833 & 0.950 & 0.745 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.950 & +0.583 & +0.542 & +0.542 & +0.500 & +0.375 & +0.875 & +0.950 & +0.698 \\ \hline
% \multirow{8}{*}{gpt4\_turbo} & Base & 0.876 & 0.613 & 0.569 & 0.518 & 0.649 & 0.508 & 0.804 & 0.824 & 0.693 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & -0.060 & -0.039 & -0.049 & -0.068 & -0.014 & -0.070 & -0.016 & -0.032 & -0.042 \\
%  & 1-shot & 0.925 & 0.667 & 0.625 & 0.625 & 0.594 & 0.583 & 0.708 & 0.825 & 0.716 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & -0.025 & +0.042 & +0.021 & +0.021 & -0.031 & -0.021 & +0.021 & +0.013 & +0.002 \\
%  & 2-shot & 0.875 & 0.625 & 0.667 & 0.750 & 0.688 & 0.542 & 0.750 & 0.925 & 0.750 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & +0.062 & +0.000 & -0.042 & +0.000 & -0.062 & -0.042 & -0.050 & -0.013 \\
%  & Rule Hint & 0.825 & 0.625 & 0.625 & 0.500 & 0.781 & 0.292 & 0.708 & 0.875 & 0.685 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.025 & -0.021 & -0.042 & -0.062 & -0.031 & -0.021 & +0.083 & +0.013 & -0.004 \\ \hline
% \end{tabular}
% \caption{Close-sourced LLMs' performance on different languages.}
% \label{tab:api_on_language}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{c|l|cccccccc|c}
% \hline
% \textbf{Model} & \textbf{Prompt} & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{SJ} & \textbf{ST} & \textbf{TD} & \textbf{TH} & \textbf{all} \\ \hline
% \multirow{8}{*}{erniebot\_turbo} & Base & 0.028 & 0.223 & 0.232 & 0.113 & 0.005 & 0.111 & 0.054 & 0.018 & 0.125 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.008 & +0.067 & +0.266 & +0.062 & +0.014 & +0.062 & +0.018 & +0.000 & +0.072 \\
%  & 1-shot & 0.125 & 0.200 & 0.083 & 0.194 & 0.000 & 0.000 & 0.250 & 0.000 & 0.152 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.125 & +0.167 & +0.173 & +0.000 & +0.125 & +0.250 & +0.000 & 0.134 \\
%  & 2-shot & 0.042 & 0.100 & 0.042 & 0.183 & 0.250 & 0.000 & 0.250 & 0.250 & 0.134 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.100 & +0.375 & +0.106 & +0.250 & +0.000 & +0.000 & +0.250 & +0.121 \\
%  & Rule Hint & 0.083 & 0.200 & 0.250 & 0.144 & 0.000 & 0.062 & 0.000 & 0.000 & 0.138 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.075 & +0.167 & +0.096 & +0.000 & +0.000 & +0.000 & +0.000 & +0.073 \\ \hline
% \multirow{8}{*}{minimax} & Base & 0.250 & 0.575 & 0.750 & 0.845 & 0.131 & 0.330 & 0.375 & 0.000 & 0.466 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.292 & +0.550 & +0.833 & +0.673 & +0.170 & +0.242 & +0.125 & +0.000 & +0.390 \\
%  & 1-shot & 0.292 & 0.675 & 0.917 & 0.683 & 0.250 & 0.188 & 0.375 & 1.000 & 0.616 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.167 & +0.500 & +0.750 & +0.692 & +0.250 & +0.125 & +0.500 & +1.000 & +0.560 \\
%  & 2-shot & 0.417 & 0.700 & 0.917 & 0.702 & 0.500 & 0.312 & 0.125 & 1.000 & 0.651 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.292 & +0.500 & +0.875 & +0.577 & +0.375 & +0.188 & +0.125 & +1.000 & +0.530 \\
%  & Rule Hint & 0.083 & 0.550 & 0.917 & 0.654 & 0.125 & 0.250 & 0.500 & 0.000 & 0.530 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.083 & +0.500 & +0.958 & +0.712 & +0.125 & +0.188 & +0.375 & +0.000 & +0.543 \\ \hline
% \multirow{8}{*}{spark} & Base & 0.292 & 0.275 & 0.833 & 0.267 & 0.000 & 0.062 & 0.000 & 0.500 & 0.306 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.417 & +0.450 & +0.833 & +0.360 & +0.000 & +0.125 & +0.000 & +0.500 & +0.398 \\
%  & 1-shot & 0.000 & 0.125 & 0.625 & 0.183 & 0.000 & 0.000 & 0.000 & 0.125 & 0.172 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.125 & +0.075 & +0.625 & +0.231 & +0.000 & +0.000 & +0.500 & +0.375 & +0.224 \\
%  & 2-shot & 0.375 & 0.225 & 0.917 & 0.365 & 0.000 & 0.000 & 0.500 & 0.750 & 0.379 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.458 & +0.200 & +0.875 & +0.369 & +0.125 & +0.000 & +0.500 & +0.625 & +0.381 \\
%  & Rule Hint & 0.083 & 0.050 & 0.708 & 0.135 & 0.000 & 0.000 & 0.000 & 0.000 & 0.151 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.000 & +0.250 & +1.000 & +0.212 & +0.125 & +0.125 & +0.125 & +0.250 & +0.267 \\ \hline
% \multirow{8}{*}{gpt4} & Base & 0.792 & 0.795 & 0.917 & 0.827 & 0.750 & 0.750 & 0.250 & 0.375 & 0.784 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.750 & +0.846 & +0.875 & +0.769 & +0.625 & +0.688 & +0.375 & +0.250 & +0.749 \\
%  & 1-shot & 0.875 & 0.800 & 0.917 & 0.840 & 0.750 & 0.500 & 0.375 & 0.500 & 0.789 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.708 & +0.800 & +0.958 & +0.802 & +0.625 & +0.500 & +0.375 & +0.375 & +0.751 \\
%  & 2-shot & 0.792 & 0.821 & 0.958 & 0.846 & 1.000 & 0.750 & 0.500 & 0.625 & 0.827 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.708 & +0.795 & +1.000 & +0.856 & +0.625 & +0.688 & +0.375 & +0.875 & +0.810 \\
%  & Rule Hint & 0.833 & 0.800 & 0.917 & 0.757 & 0.500 & 0.562 & 0.750 & 0.125 & 0.745 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.708 & +0.750 & +0.875 & +0.779 & +0.000 & +0.500 & +0.500 & +0.125 & +0.698 \\ \hline
% \multirow{8}{*}{gpt4\_turbo} & Base & 0.712 & 0.698 & 0.778 & 0.745 & 0.457 & 0.591 & 0.714 & 0.185 & 0.693 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.611 & +0.638 & +0.762 & +0.628 & +0.527 & +0.746 & +0.583 & +0.071 & +0.626 \\
%  & 1-shot & 0.667 & 0.775 & 0.708 & 0.788 & 0.375 & 0.500 & 0.750 & 0.375 & 0.716 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.625 & +0.750 & +0.708 & +0.827 & +0.375 & +0.375 & +0.750 & +0.500 & +0.720 \\
%  & 2-shot & 0.833 & 0.750 & 0.750 & 0.808 & 0.500 & 0.688 & 0.500 & 0.375 & 0.750 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.750 & +0.800 & +0.667 & +0.788 & +0.625 & +0.625 & +0.375 & +0.250 & +0.724 \\
%  & Rule Hint & 0.667 & 0.600 & 0.708 & 0.769 & 0.250 & 0.938 & 0.500 & 0.125 & 0.685 \\
%  & \textit{\multicolumn{1}{r}{+CoT}} & +0.625 & +0.675 & +0.875 & +0.721 & +0.250 & +0.812 & +0.500 & +0.000 & +0.677 \\ \hline
% \end{tabular}
% \caption{Close-sourced LLMs' performance on different tasks.}
% \label{tab:api_on_task}
% \end{table}



==> overall_performance_tables.04.tex <==

\definecolor{lightblue}{RGB}{173, 216, 230}
\definecolor{lightgreen}{RGB}{144, 238, 144}
\definecolor{lightyellow}{RGB}{255, 255, 224}
\definecolor{lightred}{RGB}{255, 182, 193}
\definecolor{lightpurple}{RGB}{216, 191, 216}

\definecolor{darkblue}{RGB}{123, 166, 180}   
\definecolor{darkgreen}{RGB}{94, 188, 94}    
\definecolor{darkyellow}{RGB}{245, 245, 184} 
\definecolor{darkred}{RGB}{205, 132, 143}    
\definecolor{darkpurple}{RGB}{166, 141, 166} 



% \setlength\tabcolsep{5.7pt}


\begin{table}[t]
\centering
% \tiny
{\fontsize{8pt}{9.6pt}\selectfont
% \resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Prompt} & \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{Tab.} & \textbf{Tree} & \textbf{XML} & \textbf{YAML} & \textbf{all} \\ 
\midrule
\multirow{4}{*}{Ernie-turbo} & \cellcolor{darkblue!25}Base & \cellcolor{lightblue!25}27.4 & \cellcolor{lightblue!25}0.2 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}13.0 & \cellcolor{lightblue!25}2.6 & \cellcolor{lightblue!25}14.3 & \cellcolor{lightblue!25}24.4 & \cellcolor{darkblue!25}12.5 \\
& \cellcolor{darkblue!25}CoT & \cellcolor{lightblue!25}19.4 & \cellcolor{lightblue!25}0.1 & \cellcolor{lightblue!25}0.1 & \cellcolor{lightblue!25}0.2 & \cellcolor{lightblue!25}10.9 & \cellcolor{lightblue!25}1.5 & \cellcolor{lightblue!25}13.4 & \cellcolor{lightblue!25}19.7 & \cellcolor{darkblue!25}9.9 \\
 & \cellcolor{darkblue!25}1-shot & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}4.2 & \cellcolor{lightblue!25}8.7 & \cellcolor{lightblue!25}21.9 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}25.0 & \cellcolor{darkblue!25}15.2 \\
 & \cellcolor{darkblue!25}2-shot & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}21.9 & \cellcolor{lightblue!25}20.8 & \cellcolor{lightblue!25}16.7 & \cellcolor{lightblue!25}5.0 & \cellcolor{darkblue!25}13.4 \\
 & \cellcolor{darkblue!25}Rule Hint & \cellcolor{lightblue!25}32.5 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}9.4 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}32.5 & \cellcolor{darkblue!25}13.8 \\
\cdashlinelr{1-11} 
\multirow{4}{*}{Minimax} & \cellcolor{darkgreen!25}Base & \cellcolor{lightgreen!25}77.5 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}41.7 & \cellcolor{lightgreen!25}29.2 & \cellcolor{lightgreen!25}44.2 & \cellcolor{lightgreen!25}20.8 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}70.0 & \cellcolor{darkgreen!25}46.6 \\
 & \cellcolor{darkgreen!25}CoT & \cellcolor{lightgreen!25}82.5 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}43.8 & \cellcolor{lightgreen!25}31.3 & \cellcolor{lightgreen!25}17.3 & \cellcolor{lightgreen!25}16.6 & \cellcolor{lightgreen!25}60.4 & \cellcolor{lightgreen!25}62.5 & \cellcolor{darkgreen!25}28.2 \\
 & \cellcolor{darkgreen!25}1-shot & \cellcolor{lightgreen!25}80.0 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}62.5 & \cellcolor{lightgreen!25}85.0 & \cellcolor{darkgreen!25}61.6 \\
 & \cellcolor{darkgreen!25}2-shot & \cellcolor{lightgreen!25}90.0 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}54.2 & \cellcolor{lightgreen!25}54.2 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}45.8 & \cellcolor{lightgreen!25}62.5 & \cellcolor{lightgreen!25}82.5 & \cellcolor{darkgreen!25}65.1 \\
 & \cellcolor{darkgreen!25}Rule Hint & \cellcolor{lightgreen!25}77.5 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}54.2 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}40.6 & \cellcolor{lightgreen!25}16.7 & \cellcolor{lightgreen!25}66.7 & \cellcolor{lightgreen!25}62.5 & \cellcolor{darkgreen!25}53.0 \\
\cdashlinelr{1-11} 
\multirow{4}{*}{Spark} & \cellcolor{darkyellow}Base & \cellcolor{lightyellow}40.0 & \cellcolor{lightyellow}20.8 & \cellcolor{lightyellow}4.3 & \cellcolor{lightyellow}12.5 & \cellcolor{lightyellow}3.1 & \cellcolor{lightyellow}29.2 & \cellcolor{lightyellow}63.6 & \cellcolor{lightyellow}57.5 & \cellcolor{darkyellow}30.6 \\
& \cellcolor{darkyellow}CoT & \cellcolor{lightyellow}52.5 & \cellcolor{lightyellow}20.8 & \cellcolor{lightyellow}4.3 & \cellcolor{lightyellow}16.7 & \cellcolor{lightyellow}6.2 & \cellcolor{lightyellow}24.9 & \cellcolor{lightyellow}65.8 & \cellcolor{lightyellow}66.4 & \cellcolor{darkyellow}35.0 \\
 & \cellcolor{darkyellow}1-shot & \cellcolor{lightyellow}27.5 & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}3.1 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}33.3 & \cellcolor{lightyellow}37.5 & \cellcolor{darkyellow}17.2 \\
 & \cellcolor{darkyellow}2-shot & \cellcolor{lightyellow}30.0 & \cellcolor{lightyellow}25.0 & \cellcolor{lightyellow}41.7 & \cellcolor{lightyellow}12.5 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}66.7 & \cellcolor{lightyellow}66.7 & \cellcolor{lightyellow}62.5 & \cellcolor{darkyellow}37.9 \\
 & \cellcolor{darkyellow}Rule Hint & \cellcolor{lightyellow}42.5 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}41.7 & \cellcolor{lightyellow}7.5 & \cellcolor{darkyellow}15.1 \\
\cdashlinelr{1-11} 
\multirow{4}{*}{GPT4} & \cellcolor{darkred!25}Base & \cellcolor{lightred!25}97.0 & \cellcolor{lightred!25}83.3 & \cellcolor{lightred!25}70.8 & \cellcolor{lightred!25}43.5 & \cellcolor{lightred!25}78.1 & \cellcolor{lightred!25}41.7 & \cellcolor{lightred!25}91.7 & \cellcolor{lightred!25}92.5 & \cellcolor{darkred!25}78.4 \\
& \cellcolor{darkred!25}CoT & \cellcolor{lightred!25}98.4 & \cellcolor{lightred!25}66.7 & \cellcolor{lightred!25}67.8 & \cellcolor{lightred!25}56.5 & \cellcolor{lightred!25}71.9 & \cellcolor{lightred!25}37.5 & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}87.5 & \cellcolor{darkred!25}74.9 \\
 & \cellcolor{darkred!25}1-shot & \cellcolor{lightred!25}95.0 & \cellcolor{lightred!25}66.7 & \cellcolor{lightred!25}70.8 & \cellcolor{lightred!25}78.3 & \cellcolor{lightred!25}68.8 & \cellcolor{lightred!25}54.2 & \cellcolor{lightred!25}79.2 & \cellcolor{lightred!25}97.5 & \cellcolor{darkred!25}78.9 \\
 & \cellcolor{darkred!25}2-shot & \cellcolor{lightred!25}95.0 & \cellcolor{lightred!25}79.2 & \cellcolor{lightred!25}65.2 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}54.2 & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}97.5 & \cellcolor{darkred!25}82.7 \\
 & \cellcolor{darkred!25}Rule Hint & \cellcolor{lightred!25}97.5 & \cellcolor{lightred!25}66.7 & \cellcolor{lightred!25}65.2 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}65.6 & \cellcolor{lightred!25}45.8 & \cellcolor{lightred!25}83.3 & \cellcolor{lightred!25}95.0 & \cellcolor{darkred!25}74.5 \\
\cdashlinelr{1-11} 
\multirow{4}{*}{GPT4-turbo} & \cellcolor{darkpurple!25}Base & \cellcolor{lightpurple!25}87.6 & \cellcolor{lightpurple!25}61.3 & \cellcolor{lightpurple!25}56.9 & \cellcolor{lightpurple!25}51.8 & \cellcolor{lightpurple!25}64.9 & \cellcolor{lightpurple!25}50.8 & \cellcolor{lightpurple!25}80.4 & \cellcolor{lightpurple!25}82.4 & \cellcolor{darkpurple!25}69.3 \\
 & \cellcolor{darkpurple!25}CoT & \cellcolor{lightpurple!25}81.6 & \cellcolor{lightpurple!25}57.4 & \cellcolor{lightpurple!25}52.0 & \cellcolor{lightpurple!25}45.2 & \cellcolor{lightpurple!25}63.6 & \cellcolor{lightpurple!25}43.8 & \cellcolor{lightpurple!25}78.8 & \cellcolor{lightpurple!25}79.2 & \cellcolor{darkpurple!25}65.1 \\
 & \cellcolor{darkpurple!25}1-shot & \cellcolor{lightpurple!25}92.5 & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}59.4 & \cellcolor{lightpurple!25}58.3 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}82.5 & \cellcolor{darkpurple!25}71.6 \\
 & \cellcolor{darkpurple!25}2-shot & \cellcolor{lightpurple!25}87.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}68.8 & \cellcolor{lightpurple!25}54.2 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}92.5 & \cellcolor{darkpurple!25}75.0 \\
 & \cellcolor{darkpurple!25}Rule Hint & \cellcolor{lightpurple!25}82.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}78.1 & \cellcolor{lightpurple!25}29.2 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}87.5 & \cellcolor{darkpurple!25}68.5 \\
\bottomrule
\end{tabular}}
\caption{GPT-Judge Score for close-sourced LLMs' performance on different languages.}
\label{tab:api_on_language}
\vspace{-5mm}
\end{table}


\begin{table}[t]
\centering
% \tiny
{\fontsize{8pt}{9.6pt}\selectfont
\begin{tabular}{lcccccccccc}
\toprule
\multicolumn{1}{c}{\textbf{Model}} & \textbf{Prompt} & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{SJ} & \textbf{ST} & \textbf{TD} & \textbf{TH} & \textbf{all} \\ 
\midrule
\multirow{4}{*}{Ernie-turbo} & \cellcolor{darkblue!25}Base & \cellcolor{lightblue!25}2.8 & \cellcolor{lightblue!25}22.3 & \cellcolor{lightblue!25}23.2 & \cellcolor{lightblue!25}11.3 & \cellcolor{lightblue!25}0.5 & \cellcolor{lightblue!25}11.1 & \cellcolor{lightblue!25}5.4 & \cellcolor{lightblue!25}1.8 & \cellcolor{darkblue!25}12.5 \\
 & \cellcolor{darkblue!25}CoT & \cellcolor{lightblue!25}0.8 & \cellcolor{lightblue!25}6.7 & \cellcolor{lightblue!25}26.6 & \cellcolor{lightblue!25}6.2 & \cellcolor{lightblue!25}1.4 & \cellcolor{lightblue!25}6.2 & \cellcolor{lightblue!25}1.8 & \cellcolor{lightblue!25}0.0 & \cellcolor{darkblue!25}7.2 \\
 & \cellcolor{darkblue!25}1-shot & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}20.0 & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}19.4 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{darkblue!25}15.2 \\
 & \cellcolor{darkblue!25}2-shot & \cellcolor{lightblue!25}4.2 & \cellcolor{lightblue!25}10.0 & \cellcolor{lightblue!25}4.2 & \cellcolor{lightblue!25}18.3 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{darkblue!25}13.4 \\
 & \cellcolor{darkblue!25}Rule Hint & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}20.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}14.4 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}6.2 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{darkblue!25}13.8 \\
\cdashlinelr{1-11} 
\multirow{4}{*}{Minimax} & \cellcolor{darkgreen!25}Base & \cellcolor{lightgreen!25}25.0 & \cellcolor{lightgreen!25}57.5 & \cellcolor{lightgreen!25}75.0 & \cellcolor{lightgreen!25}84.5 & \cellcolor{lightgreen!25}13.1 & \cellcolor{lightgreen!25}33.0 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}0.0 & \cellcolor{darkgreen!25}46.6 \\
& \cellcolor{darkgreen!25}CoT & \cellcolor{lightgreen!25}29.2 & \cellcolor{lightgreen!25}55.4 & \cellcolor{lightgreen!25}81.6 & \cellcolor{lightgreen!25}67.3 & \cellcolor{lightgreen!25}17.1 & \cellcolor{lightgreen!25}24.2 & \cellcolor{lightgreen!25}12.8 & \cellcolor{lightgreen!25}0.0 & \cellcolor{darkgreen!25}39.1 \\
 & \cellcolor{darkgreen!25}1-shot & \cellcolor{lightgreen!25}29.2 & \cellcolor{lightgreen!25}67.5 & \cellcolor{lightgreen!25}91.7 & \cellcolor{lightgreen!25}68.3 & \cellcolor{lightgreen!25}25.0 & \cellcolor{lightgreen!25}18.8 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}98.0 & \cellcolor{darkgreen!25}61.6 \\
 & \cellcolor{darkgreen!25}2-shot & \cellcolor{lightgreen!25}41.7 & \cellcolor{lightgreen!25}70.0 & \cellcolor{lightgreen!25}91.7 & \cellcolor{lightgreen!25}70.2 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}31.2 & \cellcolor{lightgreen!25}12.5 & \cellcolor{lightgreen!25}96.7 & \cellcolor{darkgreen!25}65.1 \\
 & \cellcolor{darkgreen!25}Rule Hint & \cellcolor{lightgreen!25}8.3 & \cellcolor{lightgreen!25}55.0 & \cellcolor{lightgreen!25}91.7 & \cellcolor{lightgreen!25}65.4 & \cellcolor{lightgreen!25}12.5 & \cellcolor{lightgreen!25}25.0 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}0.0 & \cellcolor{darkgreen!25}53.0 \\
 \cdashlinelr{1-11} 
\multirow{4}{*}{Spark} & \cellcolor{darkyellow}Base & \cellcolor{lightyellow}29.2 & \cellcolor{lightyellow}27.5 & \cellcolor{lightyellow}83.3 & \cellcolor{lightyellow}26.7 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}6.2 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}50.0 & \cellcolor{darkyellow}30.6 \\
 & \cellcolor{darkyellow}CoT & \cellcolor{lightyellow}41.7 & \cellcolor{lightyellow}45.3 & \cellcolor{lightyellow}83.3 & \cellcolor{lightyellow}36.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}12.6 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}54.1 & \cellcolor{darkyellow}39.8 \\
 & \cellcolor{darkyellow}1-shot & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}12.5 & \cellcolor{lightyellow}62.5 & \cellcolor{lightyellow}18.3 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}12.5 & \cellcolor{darkyellow}17.2 \\
 & \cellcolor{darkyellow}2-shot & \cellcolor{lightyellow}37.5 & \cellcolor{lightyellow}22.5 & \cellcolor{lightyellow}91.7 & \cellcolor{lightyellow}36.5 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}50.0 & \cellcolor{lightyellow}75.0 & \cellcolor{darkyellow}37.9 \\
 & \cellcolor{darkyellow}Rule Hint & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}5.0 & \cellcolor{lightyellow}70.8 & \cellcolor{lightyellow}13.5 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{darkyellow}15.1 \\
\cdashlinelr{1-11} 
\multirow{4}{*}{GPT4} & \cellcolor{darkred!25}Base & \cellcolor{lightred!25}79.2 & \cellcolor{lightred!25}79.5 & \cellcolor{lightred!25}91.7 & \cellcolor{lightred!25}82.7 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}25.0 & \cellcolor{lightred!25}37.5 & \cellcolor{darkred!25}78.4 \\ 
& \cellcolor{darkred!25}Base & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}84.6 & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}76.9 & \cellcolor{lightred!25}62.5 & \cellcolor{lightred!25}68.8 & \cellcolor{lightred!25}37.1 & \cellcolor{lightred!25}25.8 & \cellcolor{darkred!25}74.9 \\
 & \cellcolor{darkred!25}1-shot & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}80.0 & \cellcolor{lightred!25}91.7 & \cellcolor{lightred!25}84.0 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}37.5 & \cellcolor{lightred!25}50.0 & \cellcolor{darkred!25}78.9 \\
 & \cellcolor{darkred!25}2-shot & \cellcolor{lightred!25}79.2 & \cellcolor{lightred!25}82.1 & \cellcolor{lightred!25}95.8 & \cellcolor{lightred!25}84.6 & \cellcolor{lightred!25}96.0 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}62.5 & \cellcolor{darkred!25}82.7 \\
 & \cellcolor{darkred!25}Rule Hint & \cellcolor{lightred!25}83.3 & \cellcolor{lightred!25}80.0 & \cellcolor{lightred!25}91.7 & \cellcolor{lightred!25}75.7 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}56.2 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}12.5 & \cellcolor{darkred!25}74.5 \\
\cdashlinelr{1-11} 
\multirow{4}{*}{GPT4-turbo} & \cellcolor{darkpurple!25}Base & \cellcolor{lightpurple!25}71.2 & \cellcolor{lightpurple!25}69.8 & \cellcolor{lightpurple!25}77.8 & \cellcolor{lightpurple!25}74.5 & \cellcolor{lightpurple!25}45.7 & \cellcolor{lightpurple!25}59.1 & \cellcolor{lightpurple!25}71.4 & \cellcolor{lightpurple!25}18.5 & \cellcolor{darkpurple!25}69.3 \\
 & \cellcolor{darkpurple!25}CoT & \cellcolor{lightpurple!25}61.1 & \cellcolor{lightpurple!25}63.8 & \cellcolor{lightpurple!25}76.2 & \cellcolor{lightpurple!25}62.8 & \cellcolor{lightpurple!25}52.7 & \cellcolor{lightpurple!25}74.6 & \cellcolor{lightpurple!25}58.3 & \cellcolor{lightpurple!25}7.1 & \cellcolor{darkpurple!25}62.6 \\
 & \cellcolor{darkpurple!25}1-shot & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}77.5 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}78.8 & \cellcolor{lightpurple!25}37.5 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}37.5 & \cellcolor{darkpurple!25}71.6 \\
 & \cellcolor{darkpurple!25}2-shot & \cellcolor{lightpurple!25}83.3 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}80.8 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}68.8 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}37.5 & \cellcolor{darkpurple!25}75.0 \\
 & \cellcolor{darkpurple!25}Rule Hint & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}60.0 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}76.9 & \cellcolor{lightpurple!25}25.0 & \cellcolor{lightpurple!25}93.8 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}12.5 & \cellcolor{darkpurple!25}68.5 \\
\bottomrule
\end{tabular}}
\caption{GPT-Judge Score for close-sourced LLMs' performance on different tasks.}
\label{tab:api_on_task}
\vspace{-5mm}
\end{table}





==> overall_performance_tables.05.tex <==

\definecolor{lightblue}{RGB}{173, 216, 230}
\definecolor{lightgreen}{RGB}{144, 238, 144}
\definecolor{lightyellow}{RGB}{255, 255, 224}
\definecolor{lightred}{RGB}{255, 182, 193}
\definecolor{lightpurple}{RGB}{216, 191, 216}

\definecolor{darkblue}{RGB}{123, 166, 180}   
\definecolor{darkgreen}{RGB}{94, 188, 94}    
\definecolor{darkyellow}{RGB}{245, 245, 184} 
\definecolor{darkred}{RGB}{205, 132, 143}    
\definecolor{darkpurple}{RGB}{166, 141, 166} 



% \setlength\tabcolsep{5.7pt}


% \begin{table}[t]
% \centering
% % \tiny
% {\fontsize{4pt}{9.6pt}\selectfont
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Model}} & \textbf{Prompt} & \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{CSV} & \textbf{Tree} & \textbf{XML} & \textbf{YAML} & \textbf{all} \\ 
% \midrule
% \multirow{5}{*}{Ernie-turbo} & \cellcolor{darkblue!25}Base 
% & \cellcolor{darkblue!25}CoT 
%  & \cellcolor{darkblue!25}1-shot
%  & \cellcolor{darkblue!25}2-shot 
%  & \cellcolor{darkblue!25}Rule Hint  \\
% \cdashlinelr{1-19} 
% \multirow{5}{*}{Minimax} & \cellcolor{darkgreen!25}Base  \\
%  & \cellcolor{darkgreen!25}CoT  \\
%  & \cellcolor{darkgreen!25}1-shot \\
%  & \cellcolor{darkgreen!25}2-shot \\
%  & \cellcolor{darkgreen!25}Rule Hint  \\
% \cdashlinelr{1-19} 
% \multirow{5}{*}{Spark} & \cellcolor{darkyellow}Base  \cellcolor{darkyellow}30.6 \\
% & \cellcolor{darkyellow}CoT & \cellcolor{darkyellow}35.0 \\
%  & \cellcolor{darkyellow}1-shot & \cellcolor{darkyellow}17.2 \\
%  & \cellcolor{darkyellow}2-shot & \cellcolor{darkyellow}37.9 \\
%  & \cellcolor{darkyellow}Rule Hint & \cellcolor{darkyellow}15.1 \\
% \cdashlinelr{1-19} 
% \multirow{5}{*}{GPT4} & \cellcolor{darkred!25}Base & \cellcolor{darkred!25}78.4 \\
% & \cellcolor{darkred!25}CoT & \cellcolor{darkred!25}74.9 \\
%  & \cellcolor{darkred!25}1-shot & \cellcolor{darkred!25}78.9 \\
%  & \cellcolor{darkred!25}2-shot & \cellcolor{darkred!25}82.7 \\
%  & \cellcolor{darkred!25}Rule Hint & \cellcolor{darkred!25}74.5 \\
% \cdashlinelr{1-19} 
% \bottomrule
% \end{tabular}}
% \caption{GPT-Judge Score for close-sourced LLMs' performance on different languages.}
% \label{tab:api_on_language}
% \vspace{-5mm}
% \end{table}


% \begin{table}[t]
% \centering
% % \tiny
\begin{table*}[t]
\centering
{\fontsize{6.8pt}{8.6pt}\selectfont
\setlength{\tabcolsep}{2.6pt} % 可以根据需要调整这个值
\begin{tabular}{lcccccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&
\multirow{2}{*}{\textbf{Prompt}} &
\multicolumn{8}{c}{\textbf{Languages}} &
\multicolumn{8}{c}{\textbf{Tasks}} &
\multirow{2}{*}{\textbf{all}}\\
\cline{3-10}
 \cdashlinelr{11-18} 
% \cdashlinelr{3-10} 
% \cdashlinelr{11-18} 
 && \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{CSV} & \textbf{Tree} & \textbf{XML} & \textbf{YAML}
 & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{JO} & \textbf{ST} & \textbf{ND} & \textbf{TH} &  \\ 
\midrule
\multirow{5}{*}{Ernie-turbo} & \cellcolor{darkblue!25}Base 
& \cellcolor{lightblue!25}27.4 & \cellcolor{lightblue!25}0.2 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}13.0 & \cellcolor{lightblue!25}2.6 & \cellcolor{lightblue!25}14.3 & \cellcolor{lightblue!25}24.4 
& \cellcolor{lightblue!25}2.8 & \cellcolor{lightblue!25}22.3 & \cellcolor{lightblue!25}23.2 & \cellcolor{lightblue!25}11.3 & \cellcolor{lightblue!25}0.5 & \cellcolor{lightblue!25}11.1 & \cellcolor{lightblue!25}5.4 & \cellcolor{lightblue!25}1.8 & \cellcolor{darkblue!25}12.5 \\
 & \cellcolor{darkblue!25}CoT 
 & \cellcolor{lightblue!25}19.4 & \cellcolor{lightblue!25}0.1 & \cellcolor{lightblue!25}0.1 & \cellcolor{lightblue!25}0.2 & \cellcolor{lightblue!25}10.9 & \cellcolor{lightblue!25}1.5 & \cellcolor{lightblue!25}13.4 & \cellcolor{lightblue!25}19.7 &  \cellcolor{lightblue!25}0.8 & \cellcolor{lightblue!25}6.7 & \cellcolor{lightblue!25}26.6 & \cellcolor{lightblue!25}6.2 & \cellcolor{lightblue!25}1.4 & \cellcolor{lightblue!25}6.2 & \cellcolor{lightblue!25}1.8 & \cellcolor{lightblue!25}0.0 & \cellcolor{darkblue!25}7.2 \\
 & \cellcolor{darkblue!25}1-shot  & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}4.2 & \cellcolor{lightblue!25}8.7 & \cellcolor{lightblue!25}21.9 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}25.0 
 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}20.0 & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}19.4 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{darkblue!25}15.2 \\
 & \cellcolor{darkblue!25}2-shot & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}21.9 & \cellcolor{lightblue!25}20.8 & \cellcolor{lightblue!25}16.7 & \cellcolor{lightblue!25}5.0 
 & \cellcolor{lightblue!25}4.2 & \cellcolor{lightblue!25}10.0 & \cellcolor{lightblue!25}4.2 & \cellcolor{lightblue!25}18.3 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{darkblue!25}13.4 \\
 & \cellcolor{darkblue!25}Rule Hint & \cellcolor{lightblue!25}32.5 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}9.4 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}12.5 & \cellcolor{lightblue!25}32.5 
 & \cellcolor{lightblue!25}8.3 & \cellcolor{lightblue!25}20.0 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}14.4 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}6.2 & \cellcolor{lightblue!25}0.0 & \cellcolor{lightblue!25}0.0 & \cellcolor{darkblue!25}13.8 \\
\cdashlinelr{1-19} 
\multirow{5}{*}{Minimax} & \cellcolor{darkgreen!25}Base & \cellcolor{lightgreen!25}77.5 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}41.7 & \cellcolor{lightgreen!25}29.2 & \cellcolor{lightgreen!25}44.2 & \cellcolor{lightgreen!25}20.8 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}70.0 & \cellcolor{lightgreen!25}25.0 & \cellcolor{lightgreen!25}57.5 & \cellcolor{lightgreen!25}75.0 & \cellcolor{lightgreen!25}84.5 & \cellcolor{lightgreen!25}13.1 & \cellcolor{lightgreen!25}33.0 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}0.0 & \cellcolor{darkgreen!25}46.6 \\
& \cellcolor{darkgreen!25}CoT & \cellcolor{lightgreen!25}82.5 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}43.8 & \cellcolor{lightgreen!25}31.3 & \cellcolor{lightgreen!25}17.3 & \cellcolor{lightgreen!25}16.6 & \cellcolor{lightgreen!25}60.4 & \cellcolor{lightgreen!25}62.5  & \cellcolor{lightgreen!25}29.2 & \cellcolor{lightgreen!25}55.4 & \cellcolor{lightgreen!25}81.6 & \cellcolor{lightgreen!25}67.3 & \cellcolor{lightgreen!25}17.1 & \cellcolor{lightgreen!25}24.2 & \cellcolor{lightgreen!25}12.8 & \cellcolor{lightgreen!25}0.0 & \cellcolor{darkgreen!25}39.1 \\
 & \cellcolor{darkgreen!25}1-shot & \cellcolor{lightgreen!25}80.0 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}62.5 & \cellcolor{lightgreen!25}85.0 & \cellcolor{lightgreen!25}29.2 & \cellcolor{lightgreen!25}67.5 & \cellcolor{lightgreen!25}91.7 & \cellcolor{lightgreen!25}68.3 & \cellcolor{lightgreen!25}25.0 & \cellcolor{lightgreen!25}18.8 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}\textbf{98.0} & \cellcolor{darkgreen!25}61.6 \\
 & \cellcolor{darkgreen!25}2-shot & \cellcolor{lightgreen!25}90.0 & \cellcolor{lightgreen!25}58.3 & \cellcolor{lightgreen!25}54.2 & \cellcolor{lightgreen!25}54.2 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}45.8 & \cellcolor{lightgreen!25}62.5 & \cellcolor{lightgreen!25}82.5 & \cellcolor{lightgreen!25}41.7 & \cellcolor{lightgreen!25}70.0 & \cellcolor{lightgreen!25}91.7 & \cellcolor{lightgreen!25}70.2 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}31.2 & \cellcolor{lightgreen!25}12.5 & \cellcolor{lightgreen!25}96.7 & \cellcolor{darkgreen!25}65.1 \\
 & \cellcolor{darkgreen!25}Rule Hint & \cellcolor{lightgreen!25}77.5 & \cellcolor{lightgreen!25}37.5 & \cellcolor{lightgreen!25}54.2 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}40.6 & \cellcolor{lightgreen!25}16.7 & \cellcolor{lightgreen!25}66.7 & \cellcolor{lightgreen!25}62.5 
 & \cellcolor{lightgreen!25}8.3 & \cellcolor{lightgreen!25}55.0 & \cellcolor{lightgreen!25}91.7 & \cellcolor{lightgreen!25}65.4 & \cellcolor{lightgreen!25}12.5 & \cellcolor{lightgreen!25}25.0 & \cellcolor{lightgreen!25}50.0 & \cellcolor{lightgreen!25}0.0 & \cellcolor{darkgreen!25}53.0 \\
 \cdashlinelr{1-19} 
\multirow{5}{*}{Spark} & \cellcolor{darkyellow}Base & \cellcolor{lightyellow}40.0 & \cellcolor{lightyellow}20.8 & \cellcolor{lightyellow}4.3 & \cellcolor{lightyellow}12.5 & \cellcolor{lightyellow}3.1 & \cellcolor{lightyellow}29.2 & \cellcolor{lightyellow}63.6 & \cellcolor{lightyellow}57.5 & \cellcolor{lightyellow}29.2 & \cellcolor{lightyellow}27.5 & \cellcolor{lightyellow}83.3 & \cellcolor{lightyellow}26.7 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}6.2 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}50.0 & \cellcolor{darkyellow}30.6 \\
 & \cellcolor{darkyellow}CoT & \cellcolor{lightyellow}52.5 & \cellcolor{lightyellow}20.8 & \cellcolor{lightyellow}4.3 & \cellcolor{lightyellow}16.7 & \cellcolor{lightyellow}6.2 & \cellcolor{lightyellow}24.9 & \cellcolor{lightyellow}65.8 & \cellcolor{lightyellow}66.4 & \cellcolor{lightyellow}41.7 & \cellcolor{lightyellow}45.3 & \cellcolor{lightyellow}83.3 & \cellcolor{lightyellow}36.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}12.6 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}54.1 & \cellcolor{darkyellow}39.8 \\
 & \cellcolor{darkyellow}1-shot & \cellcolor{lightyellow}27.5 & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}3.1 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}33.3 & \cellcolor{lightyellow}37.5 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}12.5 & \cellcolor{lightyellow}62.5 & \cellcolor{lightyellow}18.3 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}12.5 & \cellcolor{darkyellow}17.2 \\
 & \cellcolor{darkyellow}2-shot  & \cellcolor{lightyellow}30.0 & \cellcolor{lightyellow}25.0 & \cellcolor{lightyellow}41.7 & \cellcolor{lightyellow}12.5 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}\textbf{66.7} & \cellcolor{lightyellow}66.7 & \cellcolor{lightyellow}62.5 & \cellcolor{lightyellow}37.5 & \cellcolor{lightyellow}22.5 & \cellcolor{lightyellow}91.7 & \cellcolor{lightyellow}36.5 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}50.0 & \cellcolor{lightyellow}75.0 & \cellcolor{darkyellow}37.9 \\
 & \cellcolor{darkyellow}Rule Hint & \cellcolor{lightyellow}42.5 & \cellcolor{lightyellow}4.2 & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}41.7 & \cellcolor{lightyellow}7.5 & \cellcolor{lightyellow}8.3 & \cellcolor{lightyellow}5.0 & \cellcolor{lightyellow}70.8 & \cellcolor{lightyellow}13.5 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{lightyellow}0.0 & \cellcolor{darkyellow}15.1 \\
\cdashlinelr{1-19} 
\multirow{5}{*}{GPT4} & \cellcolor{darkred!25}Base  & \cellcolor{lightred!25}97.0 & \cellcolor{lightred!25}83.3 & \cellcolor{lightred!25}\textbf{70.8} & \cellcolor{lightred!25}43.5 & \cellcolor{lightred!25}78.1 & \cellcolor{lightred!25}41.7 & \cellcolor{lightred!25}\textbf{91.7} & \cellcolor{lightred!25}92.5& \cellcolor{lightred!25}79.2 & \cellcolor{lightred!25}79.5 & \cellcolor{lightred!25}91.7 & \cellcolor{lightred!25}82.7 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}25.0 & \cellcolor{lightred!25}37.5 & \cellcolor{darkred!25}78.4 \\ 
& \cellcolor{darkred!25}CoT & \cellcolor{lightred!25}\textbf{98.4} & \cellcolor{lightred!25}66.7 & \cellcolor{lightred!25}67.8 & \cellcolor{lightred!25}56.5 & \cellcolor{lightred!25}71.9 & \cellcolor{lightred!25}37.5 & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}\textbf{84.6} & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}76.9 & \cellcolor{lightred!25}62.5 & \cellcolor{lightred!25}68.8 & \cellcolor{lightred!25}37.1 & \cellcolor{lightred!25}25.8 & \cellcolor{darkred!25}74.9 \\
 & \cellcolor{darkred!25}1-shot & \cellcolor{lightred!25}95.0 & \cellcolor{lightred!25}66.7 & \cellcolor{lightred!25}\textbf{70.8} & \cellcolor{lightred!25}\textbf{78.3} & \cellcolor{lightred!25}68.8 & \cellcolor{lightred!25}54.2 & \cellcolor{lightred!25}79.2& \cellcolor{lightred!25}\textbf{97.5} & \cellcolor{lightred!25}\textbf{87.5} & \cellcolor{lightred!25}80.0 & \cellcolor{lightred!25}91.7 & \cellcolor{lightred!25}84.0 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}37.5 & \cellcolor{lightred!25}50.0 & \cellcolor{darkred!25}78.9 \\
 & \cellcolor{darkred!25}2-shot & \cellcolor{lightred!25}95.0 & \cellcolor{lightred!25}\textbf{79.2} & \cellcolor{lightred!25}65.2 & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}\textbf{87.5} & \cellcolor{lightred!25}54.2 & \cellcolor{lightred!25}87.5 & \cellcolor{lightred!25}\textbf{97.5} & \cellcolor{lightred!25}79.2 & \cellcolor{lightred!25}82.1 & \cellcolor{lightred!25}95.8 & \cellcolor{lightred!25}84.6 & \cellcolor{lightred!25}\textbf{96.0} & \cellcolor{lightred!25}75.0 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}62.5 & \cellcolor{darkred!25}\textbf{82.7} \\
 & \cellcolor{darkred!25}Rule Hint & \cellcolor{lightred!25}97.5 & \cellcolor{lightred!25}66.7 & \cellcolor{lightred!25}65.2 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}65.6 & \cellcolor{lightred!25}45.8 & \cellcolor{lightred!25}83.3 & \cellcolor{lightred!25}95.0 & \cellcolor{lightred!25}83.3 & \cellcolor{lightred!25}80.0 & \cellcolor{lightred!25}91.7 & \cellcolor{lightred!25}75.7 & \cellcolor{lightred!25}50.0 & \cellcolor{lightred!25}56.2 & \cellcolor{lightred!25}\textbf{75.0} & \cellcolor{lightred!25}12.5 & \cellcolor{darkred!25}74.5 \\
\cdashlinelr{1-19} 
\multirow{5}{*}{GPT4-turbo} & \cellcolor{darkpurple!25}Base & \cellcolor{lightpurple!25}87.6 & \cellcolor{lightpurple!25}61.3 & \cellcolor{lightpurple!25}56.9 & \cellcolor{lightpurple!25}51.8 & \cellcolor{lightpurple!25}64.9 & \cellcolor{lightpurple!25}50.8 & \cellcolor{lightpurple!25}80.4 & \cellcolor{lightpurple!25}82.4 &\cellcolor{lightpurple!25}71.2 & \cellcolor{lightpurple!25}69.8 & \cellcolor{lightpurple!25}77.8 & \cellcolor{lightpurple!25}74.5 & \cellcolor{lightpurple!25}45.7 & \cellcolor{lightpurple!25}59.1 & \cellcolor{lightpurple!25}71.4 & \cellcolor{lightpurple!25}18.5 & \cellcolor{darkpurple!25}69.3 \\
 & \cellcolor{darkpurple!25}CoT & \cellcolor{lightpurple!25}81.6 & \cellcolor{lightpurple!25}57.4 & \cellcolor{lightpurple!25}52.0 & \cellcolor{lightpurple!25}45.2 & \cellcolor{lightpurple!25}63.6 & \cellcolor{lightpurple!25}43.8 & \cellcolor{lightpurple!25}78.8 & \cellcolor{lightpurple!25}79.2 & \cellcolor{lightpurple!25}61.1 & \cellcolor{lightpurple!25}63.8 & \cellcolor{lightpurple!25}76.2 & \cellcolor{lightpurple!25}62.8 & \cellcolor{lightpurple!25}52.7 & \cellcolor{lightpurple!25}74.6 & \cellcolor{lightpurple!25}58.3 & \cellcolor{lightpurple!25}7.1 & \cellcolor{darkpurple!25}62.6 \\
 & \cellcolor{darkpurple!25}1-shot & \cellcolor{lightpurple!25}92.5 & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}59.4 & \cellcolor{lightpurple!25}58.3 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}82.5 & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}77.5 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}78.8 & \cellcolor{lightpurple!25}37.5 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}\textbf{75.0} & \cellcolor{lightpurple!25}37.5 & \cellcolor{darkpurple!25}71.6 \\
 & \cellcolor{darkpurple!25}2-shot & \cellcolor{lightpurple!25}87.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}68.8 & \cellcolor{lightpurple!25}54.2 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}92.5 & \cellcolor{lightpurple!25}83.3 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}75.0 & \cellcolor{lightpurple!25}80.8 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}68.8 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}37.5 & \cellcolor{darkpurple!25}75.0 \\
 & \cellcolor{darkpurple!25}Rule Hint & \cellcolor{lightpurple!25}82.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}62.5 & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}78.1 & \cellcolor{lightpurple!25}29.2 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}87.5 & \cellcolor{lightpurple!25}66.7 & \cellcolor{lightpurple!25}60.0 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}76.9 & \cellcolor{lightpurple!25}25.0 & \cellcolor{lightpurple!25}\textbf{93.8} & \cellcolor{lightpurple!25}50.0 & \cellcolor{lightpurple!25}12.5 & \cellcolor{darkpurple!25}68.5 \\
\bottomrule
\end{tabular}}
\caption{GPT-Judge Score for close-sourced LLMs' performance. Bolded text represent the best performance in the column.}
\label{tab:api_overall}
% \vspace{-5mm}
\end{table*}


\begin{table}[t]

\fontsize{6.8pt}{8.6pt}\selectfont
\begin{tabular}{lccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&\multicolumn{5}{c}{\textbf{Prompt}} \\
      & Base & CoT & 1-shot & 2-shot & Rule Hint \\
     \cline{2-6}
     Ernie-turbo & 4.9 & 2.4 & 6.7 & 7.9 & 5.5 \\
     Minimax & 31.3 & 20.7 & 40.3 & 44.3 & 35.7\\
     Spark & 16.3 & 22.4 & 10.7 & 25.3 & 11.5 \\
     GPT4 & 65.0 & 59.3 & 59.9 & 64.1 & 57.2\\
     GPT4-turbo & 54.2 & 50.7 & 49.4 & 53.8 & 49.4 \\
     \hline
     Human & 95.7 & - & - & - & -\\
     \bottomrule
\end{tabular}
\caption{Performance of all LLMs and Humans on StrucText-Eval-Hard.}
\label{tab:hard_performance}

\end{table}


==> overall_performance_tables.06.tex <==

\definecolor{lightblue}{RGB}{173, 216, 230}
\definecolor{lightpink}{RGB}{255, 182, 193}  % 修改为更接近粉色
\definecolor{lightgray}{RGB}{211, 211, 211}  % 修改为更接近灰色
\definecolor{lightgreen}{RGB}{144, 238, 144}
\definecolor{lightyellow}{RGB}{255, 255, 200}  % 调整为更亮的黄色
\definecolor{lightred}{RGB}{255, 182, 193}
\definecolor{lightpurple}{RGB}{216, 191, 216}

\definecolor{darkblue}{RGB}{123, 166, 180}  
\definecolor{darkpink}{RGB}{199, 21, 133}   % 修改为深粉色
\definecolor{darkgray}{RGB}{169, 169, 169}  % 修改为深灰色
\definecolor{darkgreen}{RGB}{94, 188, 94}    
\definecolor{darkyellow}{RGB}{218, 165, 32}   % 调整为更深的黄色
\definecolor{darkred}{RGB}{205, 92, 92}     % 这是稍微深一点的红色
\definecolor{darkpurple}{RGB}{166, 141, 166}


% \setlength\tabcolsep{5.7pt}


% \begin{table}[t]
% \centering
% % \tiny
% {\fontsize{4pt}{9.6pt}\selectfont
% % \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccccc}
% \toprule
% \multicolumn{1}{c}{\textbf{Model}} & \textbf{Prompt} & \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{CSV} & \textbf{Tree} & \textbf{XML} & \textbf{YAML} & \textbf{all} \\ 
% \midrule
% \multirow{5}{*}{Ernie} & \cellcolor{darkgreen!25}Naive 
% & \cellcolor{darkgreen!25}Self-CoT
%  & \cellcolor{darkgreen!25}1-shot
%  & \cellcolor{darkgreen!25}2-shot 
%  & \cellcolor{darkgreen!25}Rule Hint  \\
% \cdashlinelr{1-19} 
% \multirow{5}{*}{Minimax} & \cellcolor{darkgreen!25}Naive  \\
%  & \cellcolor{darkgreen!25}Self-CoT \\
%  & \cellcolor{darkgreen!25}1-shot \\
%  & \cellcolor{darkgreen!25}2-shot \\
%  & \cellcolor{darkgreen!25}Rule Hint  \\
% \cdashlinelr{1-19} 
% \multirow{5}{*}{Spark} & \cellcolor{darkyellow}Naive  \cellcolor{darkyellow}30.6 \\
% & \cellcolor{darkyellow}Self-CoT& \cellcolor{darkyellow}35.0 \\
%  & \cellcolor{darkyellow}1-shot & \cellcolor{darkyellow}17.2 \\
%  & \cellcolor{darkyellow}2-shot & \cellcolor{darkyellow}37.9 \\
%  & \cellcolor{darkyellow}Rule Hint & \cellcolor{darkyellow}15.1 \\
% \cdashlinelr{1-19} 
% \multirow{5}{*}{GPT4} & \cellcolor{darkred!25}Naive & \cellcolor{darkred!25}78.4 \\
% & \cellcolor{darkred!25}Self-CoT& \cellcolor{darkred!25}74.9 \\
%  & \cellcolor{darkred!25}1-shot & \cellcolor{darkred!25}78.9 \\
%  & \cellcolor{darkred!25}2-shot & \cellcolor{darkred!25}82.7 \\
%  & \cellcolor{darkred!25}Rule Hint & \cellcolor{darkred!25}74.5 \\
% \cdashlinelr{1-19} 
% \bottomrule
% \end{tabular}}
% \caption{GPT-Judge Score for close-sourced LLMs' performance on different languages.}
% \label{tab:api_on_language}
% \vspace{-5mm}
% \end{table}


% \begin{table}[t]
% \centering
% % \tiny
\begin{table*}[t]
\centering
{\fontsize{6.8pt}{8.6pt}\selectfont
\setlength{\tabcolsep}{2.6pt} % 可以根据需要调整这个值
\begin{tabular}{llccccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&
\multirow{2}{*}{\textbf{Prompt}} &
\multicolumn{8}{c}{\textbf{Languages}} &
\multicolumn{8}{c}{\textbf{Tasks}} &
\multirow{2}{*}{\textbf{all}}\\
\cline{3-10}
 \cdashlinelr{11-18} 
% \cdashlinelr{3-10} 
% \cdashlinelr{11-18} 
 && \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{CSV} & \textbf{Tree} & \textbf{XML} & \textbf{YAML}
 & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{JO} & \textbf{ST} & \textbf{ND} & \textbf{TH} &  \\ 
\midrule
\multirow{4}{*}{Qwen2-7B} & \cellcolor{darkblue!25}Naive & \cellcolor{lightblue!25}70.4 & \cellcolor{lightblue!25}68.8 & \cellcolor{lightblue!25}68.0 & \cellcolor{lightblue!25}54.5 & \cellcolor{lightblue!25}83.5 & \cellcolor{lightblue!25}68.9 & \cellcolor{lightblue!25}57.6 & \cellcolor{lightblue!25}68.5 & \cellcolor{lightblue!25}48.5 & \cellcolor{lightblue!25}74.2 & \cellcolor{lightblue!25}49.2 & \cellcolor{lightblue!25}72.4 & \cellcolor{lightblue!25}79.5 & \cellcolor{lightblue!25}78.4 & \cellcolor{lightblue!25}47.7 & \cellcolor{lightblue!25}93.2 & \cellcolor{darkblue!25}30.0\\
 & \cellcolor{darkblue!25}Self-CoT & \cellcolor{lightblue!25}12.8 & \cellcolor{lightblue!25}1.5 & \cellcolor{lightblue!25}1.5 & \cellcolor{lightblue!25}9.1 & \cellcolor{lightblue!25}29.0 & \cellcolor{lightblue!25}4.5 & \cellcolor{lightblue!25}3.6 & \cellcolor{lightblue!25}3.5 & \cellcolor{lightblue!25}4.5 & \cellcolor{lightblue!25}6.4 & \cellcolor{lightblue!25}6.1 & \cellcolor{lightblue!25}8.1 & \cellcolor{lightblue!25}27.3 & \cellcolor{lightblue!25}26.1 & \cellcolor{lightblue!25}2.3 & \cellcolor{lightblue!25}6.8 & \cellcolor{darkblue!25}17.2\\
 & \cellcolor{darkblue!25}PS-CoT & \cellcolor{lightblue!25}31.7 & \cellcolor{lightblue!25}31.7 & \cellcolor{lightblue!25}19.4 & \cellcolor{lightblue!25}20.1 & \cellcolor{lightblue!25}67.0 & \cellcolor{lightblue!25}36.4 & \cellcolor{lightblue!25}25.8 & \cellcolor{lightblue!25}24.9 & \cellcolor{lightblue!25}9.8 & \cellcolor{lightblue!25}19.8 & \cellcolor{lightblue!25}32.6 & \cellcolor{lightblue!25}34.1 & \cellcolor{lightblue!25}63.6 & \cellcolor{lightblue!25}60.2 & \cellcolor{lightblue!25}25.0 & \cellcolor{lightblue!25}72.7 & \cellcolor{darkblue!25}29.1\\
\cdashlinelr{2-19}
 & \cellcolor{darkblue!25}w/ Hint & \cellcolor{lightblue!25}70.8 & \cellcolor{lightblue!25}66.1 & \cellcolor{lightblue!25}66.5 & \cellcolor{lightblue!25}58.1 & \cellcolor{lightblue!25}85.2 & \cellcolor{lightblue!25}56.8 & \cellcolor{lightblue!25}55.2 & \cellcolor{lightblue!25}70.2 & \cellcolor{lightblue!25}43.9 & \cellcolor{lightblue!25}72.3 & \cellcolor{lightblue!25}43.2 & \cellcolor{lightblue!25}75.3 & \cellcolor{lightblue!25}86.4 & \cellcolor{lightblue!25}77.3 & \cellcolor{lightblue!25}45.5 & \cellcolor{lightblue!25}65.9 & \cellcolor{darkblue!25}44.0\\
\cdashlinelr{1-19}
\multirow{4}{*}{Qwen2-72B} & \cellcolor{darkpurple!25}Naive & \cellcolor{lightpurple!25}85.8 & \cellcolor{lightpurple!25}73.7 & \cellcolor{lightpurple!25}75.1 & \cellcolor{lightpurple!25}67.1 & \cellcolor{lightpurple!25}92.6 & \cellcolor{lightpurple!25}86.4 & \cellcolor{lightpurple!25}71.2 & \cellcolor{lightpurple!25}82.7 & \cellcolor{lightpurple!25}80.3 & \cellcolor{lightpurple!25}81.5 & \cellcolor{lightpurple!25}62.9 & \cellcolor{lightpurple!25}80.8 & \cellcolor{lightpurple!25}90.9 & \cellcolor{lightpurple!25}90.9 & \cellcolor{lightpurple!25}77.3 & \cellcolor{lightpurple!25}95.5 & \cellcolor{darkpurple!25}42.6\\
 & \cellcolor{darkpurple!25}Self-CoT & \cellcolor{lightpurple!25}85.4 & \cellcolor{lightpurple!25}69.9 & \cellcolor{lightpurple!25}70.8 & \cellcolor{lightpurple!25}65.2 & \cellcolor{lightpurple!25}95.5 & \cellcolor{lightpurple!25}90.2 & \cellcolor{lightpurple!25}79.5 & \cellcolor{lightpurple!25}89.7 & \cellcolor{lightpurple!25}78.8 & \cellcolor{lightpurple!25}77.1 & \cellcolor{lightpurple!25}81.1 & \cellcolor{lightpurple!25}81.7 & \cellcolor{lightpurple!25}90.9 & \cellcolor{lightpurple!25}95.5 & \cellcolor{lightpurple!25}84.1 & \cellcolor{lightpurple!25}95.5 & \cellcolor{darkpurple!25}51.0\\
 & \cellcolor{darkpurple!25}PS-CoT & \cellcolor{lightpurple!25}89.5 & \cellcolor{lightpurple!25}70.1 & \cellcolor{lightpurple!25}68.9 & \cellcolor{lightpurple!25}61.7 & \cellcolor{lightpurple!25}92.0 & \cellcolor{lightpurple!25}84.8 & \cellcolor{lightpurple!25}81.1 & \cellcolor{lightpurple!25}93.4 & \cellcolor{lightpurple!25}76.5 & \cellcolor{lightpurple!25}77.6 & \cellcolor{lightpurple!25}87.9 & \cellcolor{lightpurple!25}80.8 & \cellcolor{lightpurple!25}81.8 & \cellcolor{lightpurple!25}93.2 & \cellcolor{lightpurple!25}86.4 & \cellcolor{lightpurple!25}97.7 & \cellcolor{darkpurple!25}65.3\\
\cdashlinelr{2-19}
 & \cellcolor{darkpurple!25}w/ Hint & \cellcolor{lightpurple!25}90.0 & \cellcolor{lightpurple!25}72.5 & \cellcolor{lightpurple!25}79.1 & \cellcolor{lightpurple!25}68.6 & \cellcolor{lightpurple!25}94.9 & \cellcolor{lightpurple!25}81.1 & \cellcolor{lightpurple!25}72.7 & \cellcolor{lightpurple!25}90.8 & \cellcolor{lightpurple!25}81.1 & \cellcolor{lightpurple!25}84.0 & \cellcolor{lightpurple!25}77.3 & \cellcolor{lightpurple!25}82.4 & \cellcolor{lightpurple!25}95.5 & \cellcolor{lightpurple!25}92.0 & \cellcolor{lightpurple!25}72.7 & \cellcolor{lightpurple!25}86.4 & \cellcolor{darkpurple!25}49.4\\
\cdashlinelr{1-19}
\multirow{4}{*}{Llama-3.1-8B} & \cellcolor{darkgray!25}Naive & \cellcolor{lightgray!25}43.9 & \cellcolor{lightgray!25}64.6 & \cellcolor{lightgray!25}49.3 & \cellcolor{lightgray!25}48.3 & \cellcolor{lightgray!25}42.6 & \cellcolor{lightgray!25}50.0 & \cellcolor{lightgray!25}26.5 & \cellcolor{lightgray!25}46.9 & \cellcolor{lightgray!25}30.3 & \cellcolor{lightgray!25}49.4 & \cellcolor{lightgray!25}1.5 & \cellcolor{lightgray!25}61.0 & \cellcolor{lightgray!25}11.4 & \cellcolor{lightgray!25}45.5 & \cellcolor{lightgray!25}22.7 & \cellcolor{lightgray!25}79.5 & \cellcolor{darkgray!25}21.3\\
 & \cellcolor{darkgray!25}Self-CoT & \cellcolor{lightgray!25}52.2 & \cellcolor{lightgray!25}40.6 & \cellcolor{lightgray!25}49.2 & \cellcolor{lightgray!25}39.0 & \cellcolor{lightgray!25}66.5 & \cellcolor{lightgray!25}43.2 & \cellcolor{lightgray!25}36.6 & \cellcolor{lightgray!25}55.2 & \cellcolor{lightgray!25}40.9 & \cellcolor{lightgray!25}40.2 & \cellcolor{lightgray!25}39.7 & \cellcolor{lightgray!25}53.0 & \cellcolor{lightgray!25}77.3 & \cellcolor{lightgray!25}65.9 & \cellcolor{lightgray!25}52.3 & \cellcolor{lightgray!25}36.4 & \cellcolor{darkgray!25}48.5\\
 & \cellcolor{darkgray!25}PS-CoT & \cellcolor{lightgray!25}45.8 & \cellcolor{lightgray!25}18.7 & \cellcolor{lightgray!25}34.0 & \cellcolor{lightgray!25}32.8 & \cellcolor{lightgray!25}64.0 & \cellcolor{lightgray!25}63.1 & \cellcolor{lightgray!25}44.6 & \cellcolor{lightgray!25}41.3 & \cellcolor{lightgray!25}48.8 & \cellcolor{lightgray!25}50.5 & \cellcolor{lightgray!25}44.7 & \cellcolor{lightgray!25}32.8 & \cellcolor{lightgray!25}69.8 & \cellcolor{lightgray!25}56.8 & \cellcolor{lightgray!25}64.3 & \cellcolor{lightgray!25}62.8 & \cellcolor{darkgray!25}55.9\\
\cdashlinelr{2-19}
 & \cellcolor{darkgray!25}w/ Hint & \cellcolor{lightgray!25}44.9 & \cellcolor{lightgray!25}62.2 & \cellcolor{lightgray!25}55.9 & \cellcolor{lightgray!25}48.1 & \cellcolor{lightgray!25}29.0 & \cellcolor{lightgray!25}54.5 & \cellcolor{lightgray!25}30.5 & \cellcolor{lightgray!25}51.4 & \cellcolor{lightgray!25}31.8 & \cellcolor{lightgray!25}45.4 & \cellcolor{lightgray!25}9.1 & \cellcolor{lightgray!25}63.4 & \cellcolor{lightgray!25}2.3 & \cellcolor{lightgray!25}22.7 & \cellcolor{lightgray!25}38.6 & \cellcolor{lightgray!25}90.9 & \cellcolor{darkgray!25}26.9\\
\cdashlinelr{1-19}
\multirow{4}{*}{Llama-3.1-70B} & \cellcolor{darkgreen!25}Naive & \cellcolor{lightgreen!25}93.8 & \cellcolor{lightgreen!25}70.9 & \cellcolor{lightgreen!25}69.8 & \cellcolor{lightgreen!25}62.8 & \cellcolor{lightgreen!25}72.7 & \cellcolor{lightgreen!25}51.5 & \cellcolor{lightgreen!25}78.7 & \cellcolor{lightgreen!25}88.8 & \cellcolor{lightgreen!25}81.8 & \cellcolor{lightgreen!25}75.4 & \cellcolor{lightgreen!25}82.6 & \cellcolor{lightgreen!25}81.0 & \cellcolor{lightgreen!25}72.7 & \cellcolor{lightgreen!25}59.1 & \cellcolor{lightgreen!25}47.7 & \cellcolor{lightgreen!25}43.2 & \cellcolor{darkgreen!25}50.8\\
 & \cellcolor{darkgreen!25}Self-CoT & \cellcolor{lightgreen!25}93.6 & \cellcolor{lightgreen!25}71.4 & \cellcolor{lightgreen!25}69.7 & \cellcolor{lightgreen!25}54.8 & \cellcolor{lightgreen!25}96.0 & \cellcolor{lightgreen!25}84.1 & \cellcolor{lightgreen!25}87.1 & \cellcolor{lightgreen!25}95.9 & \cellcolor{lightgreen!25}88.6 & \cellcolor{lightgreen!25}67.9 & \cellcolor{lightgreen!25}86.4 & \cellcolor{lightgreen!25}85.7 & \cellcolor{lightgreen!25}97.7 & \cellcolor{lightgreen!25}93.2 & \cellcolor{lightgreen!25}77.3 & \cellcolor{lightgreen!25}97.7 & \cellcolor{darkgreen!25}76.7\\
 & \cellcolor{darkgreen!25}PS-CoT & \cellcolor{lightgreen!25}94.5 & \cellcolor{lightgreen!25}68.7 & \cellcolor{lightgreen!25}72.7 & \cellcolor{lightgreen!25}61.7 & \cellcolor{lightgreen!25}93.7 & \cellcolor{lightgreen!25}83.2 & \cellcolor{lightgreen!25}93.9 & \cellcolor{lightgreen!25}98.5 & \cellcolor{lightgreen!25}90.8 & \cellcolor{lightgreen!25}77.0 & \cellcolor{lightgreen!25}93.9 & \cellcolor{lightgreen!25}84.2 & \cellcolor{lightgreen!25}93.2 & \cellcolor{lightgreen!25}90.9 & \cellcolor{lightgreen!25}81.8 & \cellcolor{lightgreen!25}90.9 & \cellcolor{darkgreen!25}72.9\\
\cdashlinelr{2-19}
 & \cellcolor{darkgreen!25}w/ Hint & \cellcolor{lightgreen!25}93.6 & \cellcolor{lightgreen!25}73.9 & \cellcolor{lightgreen!25}77.4 & \cellcolor{lightgreen!25}71.6 & \cellcolor{lightgreen!25}72.7 & \cellcolor{lightgreen!25}74.2 & \cellcolor{lightgreen!25}80.4 & \cellcolor{lightgreen!25}93.6 & \cellcolor{lightgreen!25}88.6 & \cellcolor{lightgreen!25}84.9 & \cellcolor{lightgreen!25}84.1 & \cellcolor{lightgreen!25}83.5 & \cellcolor{lightgreen!25}70.5 & \cellcolor{lightgreen!25}60.2 & \cellcolor{lightgreen!25}65.9 & \cellcolor{lightgreen!25}75.0 & \cellcolor{darkgreen!25}58.4\\
\cdashlinelr{1-19}
\multirow{4}{*}{Llama-3.1-405B} & \cellcolor{darkyellow!25}Naive & \cellcolor{lightyellow!25}82.0 & \cellcolor{lightyellow!25}62.9 & \cellcolor{lightyellow!25}70.0 & \cellcolor{lightyellow!25}60.9 & \cellcolor{lightyellow!25}96.6 & \cellcolor{lightyellow!25}65.9 & \cellcolor{lightyellow!25}61.5 & \cellcolor{lightyellow!25}78.1 & \cellcolor{lightyellow!25}74.2 & \cellcolor{lightyellow!25}69.4 & \cellcolor{lightyellow!25}32.6 & \cellcolor{lightyellow!25}82.4 & \cellcolor{lightyellow!25}97.7 & \cellcolor{lightyellow!25}94.3 & \cellcolor{lightyellow!25}45.5 & \cellcolor{lightyellow!25}79.5 & \cellcolor{darkyellow!25}38.3\\
 & \cellcolor{darkyellow!25}Self-CoT & \cellcolor{lightyellow!25}87.7 & \cellcolor{lightyellow!25}62.2 & \cellcolor{lightyellow!25}74.2 & \cellcolor{lightyellow!25}62.2 & \cellcolor{lightyellow!25}95.5 & \cellcolor{lightyellow!25}75.8 & \cellcolor{lightyellow!25}78.5 & \cellcolor{lightyellow!25}90.8 & \cellcolor{lightyellow!25}87.9 & \cellcolor{lightyellow!25}73.2 & \cellcolor{lightyellow!25}63.6 & \cellcolor{lightyellow!25}83.4 & \cellcolor{lightyellow!25}100.0 & \cellcolor{lightyellow!25}90.9 & \cellcolor{lightyellow!25}59.1 & \cellcolor{lightyellow!25}88.6 & \cellcolor{darkyellow!25}67.1\\
 & \cellcolor{darkyellow!25}PS-CoT & \cellcolor{lightyellow!25}84.5 & \cellcolor{lightyellow!25}67.4 & \cellcolor{lightyellow!25}76.0 & \cellcolor{lightyellow!25}66.7 & \cellcolor{lightyellow!25}92.0 & \cellcolor{lightyellow!25}86.7 & \cellcolor{lightyellow!25}94.7 & \cellcolor{lightyellow!25}94.7 & \cellcolor{lightyellow!25}88.3 & \cellcolor{lightyellow!25}79.1 & \cellcolor{lightyellow!25}93.2 & \cellcolor{lightyellow!25}81.1 & \cellcolor{lightyellow!25}97.7 & \cellcolor{lightyellow!25}85.2 & \cellcolor{lightyellow!25}90.9 & \cellcolor{lightyellow!25}88.6 & \cellcolor{darkyellow!25}74.9\\
\cdashlinelr{2-19}
 & \cellcolor{darkyellow!25}w/ Hint & \cellcolor{lightyellow!25}85.4 & \cellcolor{lightyellow!25}68.3 & \cellcolor{lightyellow!25}75.1 & \cellcolor{lightyellow!25}66.7 & \cellcolor{lightyellow!25}98.3 & \cellcolor{lightyellow!25}70.5 & \cellcolor{lightyellow!25}74.5 & \cellcolor{lightyellow!25}87.2 & \cellcolor{lightyellow!25}74.2 & \cellcolor{lightyellow!25}78.0 & \cellcolor{lightyellow!25}59.1 & \cellcolor{lightyellow!25}84.9 & \cellcolor{lightyellow!25}97.7 & \cellcolor{lightyellow!25}97.7 & \cellcolor{lightyellow!25}50.0 & \cellcolor{lightyellow!25}84.1 & \cellcolor{darkyellow!25}46.5\\
\cdashlinelr{1-19}
\multirow{4}{*}{Mistral-7B} & \cellcolor{darkred!25}Naive & \cellcolor{lightred!25}32.5 & \cellcolor{lightred!25}42.1 & \cellcolor{lightred!25}44.9 & \cellcolor{lightred!25}40.2 & \cellcolor{lightred!25}9.1 & \cellcolor{lightred!25}4.5 & \cellcolor{lightred!25}14.8 & \cellcolor{lightred!25}33.5 & \cellcolor{lightred!25}6.1 & \cellcolor{lightred!25}30.8 & \cellcolor{lightred!25}0.0 & \cellcolor{lightred!25}47.7 & \cellcolor{lightred!25}0.0 & \cellcolor{lightred!25}6.8 & \cellcolor{lightred!25}0.0 & \cellcolor{lightred!25}0.0 & \cellcolor{darkred!25}11.3\\
 & \cellcolor{darkred!25}Self-CoT & \cellcolor{lightred!25}56.5 & \cellcolor{lightred!25}35.1 & \cellcolor{lightred!25}40.3 & \cellcolor{lightred!25}36.6 & \cellcolor{lightred!25}34.7 & \cellcolor{lightred!25}15.9 & \cellcolor{lightred!25}33.7 & \cellcolor{lightred!25}54.3 & \cellcolor{lightred!25}28.8 & \cellcolor{lightred!25}49.2 & \cellcolor{lightred!25}64.4 & \cellcolor{lightred!25}43.9 & \cellcolor{lightred!25}6.8 & \cellcolor{lightred!25}23.9 & \cellcolor{lightred!25}13.6 & \cellcolor{lightred!25}13.6 & \cellcolor{darkred!25}8.1\\
 & \cellcolor{darkred!25}PS-CoT & \cellcolor{lightred!25}43.9 & \cellcolor{lightred!25}19.7 & \cellcolor{lightred!25}22.9 & \cellcolor{lightred!25}15.6 & \cellcolor{lightred!25}14.8 & \cellcolor{lightred!25}18.2 & \cellcolor{lightred!25}34.6 & \cellcolor{lightred!25}44.1 & \cellcolor{lightred!25}18.9 & \cellcolor{lightred!25}30.6 & \cellcolor{lightred!25}56.8 & \cellcolor{lightred!25}29.1 & \cellcolor{lightred!25}22.7 & \cellcolor{lightred!25}6.8 & \cellcolor{lightred!25}13.6 & \cellcolor{lightred!25}22.7 & \cellcolor{darkred!25}19.5\\
\cdashlinelr{2-19}
 & \cellcolor{darkred!25}w/ Hint & \cellcolor{lightred!25}34.6 & \cellcolor{lightred!25}39.4 & \cellcolor{lightred!25}52.7 & \cellcolor{lightred!25}40.5 & \cellcolor{lightred!25}10.2 & \cellcolor{lightred!25}6.8 & \cellcolor{lightred!25}12.7 & \cellcolor{lightred!25}36.5 & \cellcolor{lightred!25}9.8 & \cellcolor{lightred!25}34.3 & \cellcolor{lightred!25}0.0 & \cellcolor{lightred!25}48.9 & \cellcolor{lightred!25}0.0 & \cellcolor{lightred!25}8.0 & \cellcolor{lightred!25}0.0 & \cellcolor{lightred!25}0.0 & \cellcolor{darkred!25}10.6\\


\bottomrule
\end{tabular}}
\caption{RougeL score for open sourced LLMs' performance. Bolded text represent the best performance in the column.}
\label{tab:api_overall}
\vspace{-5mm}
\end{table*}



\begin{table}[t]
\resizebox{\columnwidth}{!}{
% \fontsize{5.5pt}{5pt}\selectfont
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Prompt}} \\
      & Naive & w/ Hint & 3-Shot & Simple 3-Shot \\
     \hline
     \multirow{1}{*}{GPT-4o-Turbo}    & \cellcolor{lightblue!25}51.1 & \cellcolor{lightblue!25}54.2 & \cellcolor{lightblue!25}69.5 &\cellcolor{lightblue!25}49.7\\
     \multirow{1}{*}{GPT-4o-Mini}    & \cellcolor{lightpurple!25}39.3 & \cellcolor{lightpurple!25}47.7 & \cellcolor{lightpurple!25}65.6 &\cellcolor{lightpurple!25}39.9\\
     \multirow{1}{*}{Gemini1.5-Pro}    & \cellcolor{lightgray!25}11.2 & \cellcolor{lightgray!25}15.7 & \cellcolor{lightgray!25}53.0 &\cellcolor{lightgray!25}12.5\\
     \multirow{1}{*}{Gemini1.5-Flash}    & \cellcolor{lightgreen!25}12.9 & \cellcolor{lightgreen!25}12.9 & \cellcolor{lightgreen!25}38.3 &\cellcolor{lightgreen!25}11.9\\
     \multirow{1}{*}{GLM-4-Plus}    & \cellcolor{lightyellow!25}47.3 & \cellcolor{lightyellow!25}50.9 & \cellcolor{lightyellow!25}65.8 &\cellcolor{lightyellow!25}51.7\\
     \multirow{1}{*}{GLM-4-Flash}    & \cellcolor{lightred!25}40.9 & \cellcolor{lightred!25}47.8 & \cellcolor{lightred!25}55.2 &\cellcolor{lightred!25}41.7\\
     
     \hline
     \hline
     \multirow{1}{*}{QWen-2-7B}    & \cellcolor{lightblue!25}29.6 & \cellcolor{lightblue!25}35.0 & \cellcolor{lightblue!25}51.9 &\cellcolor{lightblue!25}30.0\\
     \multirow{1}{*}{QWen-2-72B}    & \cellcolor{lightpurple!25}42.5 & \cellcolor{lightpurple!25}45.3 & \cellcolor{lightpurple!25}61.4 &\cellcolor{lightpurple!25}36.2\\
     \multirow{1}{*}{Llama-3.1-8B}    & \cellcolor{lightgray!25}22.3 & \cellcolor{lightgray!25}26.7 & \cellcolor{lightgray!25}33.7 &\cellcolor{lightgray!25}34.2\\
     \multirow{1}{*}{Llama-3.1-70B}    & \cellcolor{lightgreen!25}45.8 & \cellcolor{lightgreen!25}56.0 & \cellcolor{lightgreen!25}58.4  &\cellcolor{lightgreen!25}50.1\\
     \multirow{1}{*}{Llama-3.1-405B}    & \cellcolor{lightyellow!25}34.4 & \cellcolor{lightyellow!25}41.7 & \cellcolor{lightyellow!25}48.7  &\cellcolor{lightyellow!25}40.6\\
     \multirow{1}{*}{Mistral-0.2-7B}    & \cellcolor{lightred!25}7.0 & \cellcolor{lightred!25}9.5 & \cellcolor{lightred!25}21.0 &\cellcolor{lightred!25}6.9 \\
     \hline
     \hline
     Human        & 92.6 & - & - &-\\
     
     \bottomrule
\end{tabular}
}
\caption{Performance of all LLMs and Humans on StrucText-Eval-Hard.}
\label{tab:hard_performance}
\vspace{-5mm}
\end{table}


% \begin{table}[t]
% \resizebox{\columnwidth}{!}{
% % \fontsize{5.5pt}{5pt}\selectfont
% \begin{tabular}{lccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Few-Shot}} & \multicolumn{5}{c}{\textbf{Prompt}} \\
%       &  & Naive & CoT & PS-CoT & w/ Hint & \textbf{Self-Hint} \\
%      \hline
%      \multirow{2}{*}{Gemini1.5-Pro}    & \cellcolor{darkblue!25}0 & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- \\
%      & \cellcolor{darkblue!25}3 & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{Gemini1.5-Pro-Flash}       & \cellcolor{darkgray!25}0 & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- \\
%      & \cellcolor{darkgray!25}3 & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{GPT4-o}        & \cellcolor{darkgreen!25}0 & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- \\
%      & \cellcolor{darkgreen!25}3 & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{GPT4-o-Mini}     & \cellcolor{darkyellow!25}0 & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- \\
%      & \cellcolor{darkyellow!25}3 & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{GLM4-Plus}          & \cellcolor{darkred!25}0 & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- \\
%      & \cellcolor{darkred!25}3 & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{GLM4-Flash}    & \cellcolor{darkpurple!25}0 & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- \\
%      & \cellcolor{darkpurple!25}3 & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- \\
%      \hline
%      \hline
%      \multirow{2}{*}{QWen-2-7B}      & \cellcolor{darkblue!25}0 & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- \\
%      & \cellcolor{darkblue!25}3 & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{QWen-2-72B}     & \cellcolor{darkgray!25}0 & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- \\
%      & \cellcolor{darkgray!25}3 & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{Llama-3.1-8B}   & \cellcolor{darkgreen!25}0 & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- \\
%      & \cellcolor{darkgreen!25}3 & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{Llama-3.1-70B}  & \cellcolor{darkyellow!25}0 & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- \\
%      & \cellcolor{darkyellow!25}3 & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{Llama-3.1-405B} & \cellcolor{darkred!25}0 & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- \\
%      & \cellcolor{darkred!25}3 & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- \\
%     \cdashlinelr{1-7} 
%      \multirow{2}{*}{Mistral0.2-7B}  & \cellcolor{darkpurple!25}0 & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- \\
%      & \cellcolor{darkpurple!25}3 & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- \\
%      \hline
%      \hline
%      Human        & - & 95.7 & - & - & - & - \\
     
%      \bottomrule
% \end{tabular}
% }
% \caption{Performance of all LLMs and Humans on StrucText-Eval-Hard.}
% \label{tab:hard_performance}

% \end{table}




% \begin{table*}[t]
% \centering
% {\fontsize{6.8pt}{8.6pt}\selectfont
% \setlength{\tabcolsep}{2.6pt}
% \begin{tabular}{lcccccccccccccccccc}
% \toprule
% \multirow{2}{*}{\textbf{Model}}&
% \multirow{2}{*}{\textbf{Prompt}} &
% \multicolumn{8}{c}{\textbf{Languages}} &
% \multicolumn{8}{c}{\textbf{Tasks}} &
% \multirow{2}{*}{\textbf{all}}\\
% \cline{3-10}
%  \cdashlinelr{11-18} 
 
%  && \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{CSV} & \textbf{Tree} & \textbf{XML} & \textbf{YAML}
%  & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{JO} & \textbf{ST} & \textbf{ND} & \textbf{TH} &  \\ 
% \midrule

% \multirow{2}{*}{GPT-4o} & \cellcolor{darkblue!25}Naive 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{darkblue!25}- \\

% & \cellcolor{darkblue!25}3-Shot 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{darkblue!25}- \\

% \cdashlinelr{1-19} 
% \multirow{2}{*}{GPT-4o-Mini} & \cellcolor{darkpurple!25}Naive 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{darkpurple!25}- \\

% & \cellcolor{darkpurple!25}3-Shot 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{darkpurple!25}- \\

% \cdashlinelr{1-19} 

% \multirow{2}{*}{Gemini-1.5-Pro} & \cellcolor{darkgray!25}Naive 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{darkgray!25}- \\

% & \cellcolor{darkgray!25}3-Shot 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{darkgray!25}- \\

% \cdashlinelr{1-19} 
% \multirow{2}{*}{Gemini-1.5-Pro-Flash} & \cellcolor{darkgreen!25}Naive 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{darkgreen!25}- \\

% & \cellcolor{darkgreen!25}3-Shot 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{darkgreen!25}- \\

% \cdashlinelr{1-19} 

% \multirow{2}{*}{GLM-4-Plus} & \cellcolor{darkyellow!25}Naive 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{darkyellow!25}- \\

% & \cellcolor{darkyellow!25}3-Shot 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{darkyellow!25}- \\
% \cdashlinelr{1-19} 

% \multirow{2}{*}{GLM-4-Flash} & \cellcolor{darkred!25}Naive 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{darkred!25}- \\

% & \cellcolor{darkred!25}3-Shot 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{darkred!25}- \\

% \hline
% \hline


% \multirow{2}{*}{QWen-2-7B} & \cellcolor{darkblue!25}Naive 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{darkblue!25}- \\

% & \cellcolor{darkblue!25}3-Shot 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- 
% & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{lightblue!25}- & \cellcolor{darkblue!25}- \\

% \cdashlinelr{1-19} 
% \multirow{2}{*}{QWen-2-72B} & \cellcolor{darkpurple!25}Naive 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{darkpurple!25}- \\

% & \cellcolor{darkpurple!25}3-Shot 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- 
% & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{lightpurple!25}- & \cellcolor{darkpurple!25}- \\

% \cdashlinelr{1-19} 

% \multirow{2}{*}{Llama-3.1-8B} & \cellcolor{darkgray!25}Naive 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{darkgray!25}- \\

% & \cellcolor{darkgray!25}3-Shot 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- 
% & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{lightgray!25}- & \cellcolor{darkgray!25}- \\

% \cdashlinelr{1-19} 
% \multirow{2}{*}{Llama-3.1-70B} & \cellcolor{darkgreen!25}Naive 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{darkgreen!25}- \\

% & \cellcolor{darkgreen!25}3-Shot 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- 
% & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{lightgreen!25}- & \cellcolor{darkgreen!25}- \\

% \cdashlinelr{1-19} 

% \multirow{2}{*}{Llama-3.1-405B} & \cellcolor{darkyellow!25}Naive 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{darkyellow!25}- \\

% & \cellcolor{darkyellow!25}3-Shot 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- 
% & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{lightyellow!25}- & \cellcolor{darkyellow!25}- \\
% \cdashlinelr{1-19} 

% \multirow{2}{*}{Mistral-0.2-7B} & \cellcolor{darkred!25}Naive 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{darkred!25}- \\

% & \cellcolor{darkred!25}3-Shot 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- 
% & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{lightred!25}- & \cellcolor{darkred!25}- \\

% \bottomrule
% \end{tabular}}
% \caption{GPT-Judge Score for close-sourced LLMs' performance. Bolded text represent the best performance in the column.}
% \label{tab:hard_performance}

% \end{table*}


==> performance_EM_tables.tex <==

\definecolor{lightblue}{RGB}{173, 216, 230}
\definecolor{lightgreen}{RGB}{144, 238, 144}
\definecolor{lightyellow}{RGB}{255, 255, 224}
\definecolor{lightred}{RGB}{255, 182, 193}
\definecolor{lightpurple}{RGB}{216, 191, 216}

\definecolor{darkblue}{RGB}{123, 166, 180}   
\definecolor{darkgreen}{RGB}{94, 188, 94}    
\definecolor{darkyellow}{RGB}{245, 245, 184} 
\definecolor{darkred}{RGB}{205, 132, 143}    
\definecolor{darkpurple}{RGB}{166, 141, 166} 



\begin{table}[t]
\centering
{\fontsize{6.8pt}{8.6pt}\selectfont
\setlength{\tabcolsep}{2.6pt} % 可以根据需要调整这个值
\begin{tabular}{lcccccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&
\multirow{2}{*}{\textbf{Prompt}} &
\multicolumn{8}{c}{\textbf{Languages}} &
\multicolumn{8}{c}{\textbf{Tasks}} &
\multirow{2}{*}{\textbf{all}}\\
\cline{3-10}
 \cdashlinelr{11-18} 
% \cdashlinelr{3-10} 
% \cdashlinelr{11-18} 
 && \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{CSV} & \textbf{Tree} & \textbf{XML} & \textbf{YAML}
 & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{JO} & \textbf{ST} & \textbf{ND} & \textbf{TH} &  \\ 
\midrule
\multirow{5}{*}{Ernie-turbo} & Base 
& 27.4 & 0.2 & 0.0 & 0.0 & 13.0 & 2.6 & 14.3 & 24.4 
& 2.8 & 22.3 & 23.2 & 11.3 & 0.5 & 11.1 & 5.4 & 1.8 & 12.5 \\
 & CoT 
 & 19.4 & 0.1 & 0.1 & 0.2 & 10.9 & 1.5 & 13.4 & 19.7 &  0.8 & 6.7 & 26.6 & 6.2 & 1.4 & 6.2 & 1.8 & 0.0 & 7.2 \\
 & 1-shot  & 25.0 & 0.0 & 4.2 & 8.7 & 21.9 & 12.5 & 8.3 & 25.0 
 & 12.5 & 20.0 & 8.3 & 19.4 & 0.0 & 0.0 & 25.0 & 0.0 & 15.2 \\
 & 2-shot & 12.5 & 12.5 & 12.5 & 8.3 & 21.9 & 20.8 & 16.7 & 5.0 
 & 4.2 & 10.0 & 4.2 & 18.3 & 25.0 & 0.0 & 25.0 & 25.0 & 13.4 \\
 & Rule Hint & 32.5 & 0.0 & 0.0 & 0.0 & 9.4 & 0.0 & 12.5 & 32.5 
 & 8.3 & 20.0 & 25.0 & 14.4 & 0.0 & 6.2 & 0.0 & 0.0 & 13.8 \\
\cdashlinelr{1-19} 
\multirow{5}{*}{Minimax} & Base & 77.5 & 58.3 & 41.7 & 29.2 & 44.2 & 20.8 & 58.3 & 70.0 & 25.0 & 57.5 & 75.0 & 84.5 & 13.1 & 33.0 & 37.5 & 0.0 & 46.6 \\
& CoT & 82.5 & 58.3 & 43.8 & 31.3 & 17.3 & 16.6 & 60.4 & 62.5  & 29.2 & 55.4 & 81.6 & 67.3 & 17.1 & 24.2 & 12.8 & 0.0 & 39.1 \\
 & 1-shot & 80.0 & 50.0 & 58.3 & 50.0 & 37.5 & 50.0 & 62.5 & 85.0 & 29.2 & 67.5 & 91.7 & 68.3 & 25.0 & 18.8 & 37.5 & 98.0 & 61.6 \\
 & 2-shot & 90.0 & 58.3 & 54.2 & 54.2 & 50.0 & 45.8 & 62.5 & 82.5 & 41.7 & 70.0 & 91.7 & 70.2 & 50.0 & 31.2 & 12.5 & 96.7 & 65.1 \\
 & Rule Hint & 77.5 & 37.5 & 54.2 & 50.0 & 40.6 & 16.7 & 66.7 & 62.5 
 & 8.3 & 55.0 & 91.7 & 65.4 & 12.5 & 25.0 & 50.0 & 0.0 & 53.0 \\
 \cdashlinelr{1-19} 
\multirow{5}{*}{Spark} & Base & 40.0 & 20.8 & 4.3 & 12.5 & 3.1 & 29.2 & 63.6 & 57.5 & 29.2 & 27.5 & 83.3 & 26.7 & 0.0 & 6.2 & 0.0 & 50.0 & 30.6 \\
 & CoT & 52.5 & 20.8 & 4.3 & 16.7 & 6.2 & 24.9 & 65.8 & 66.4 & 41.7 & 45.3 & 83.3 & 36.0 & 0.0 & 12.6 & 0.0 & 54.1 & 39.8 \\
 & 1-shot & 27.5 & 8.3 & 4.2 & 4.2 & 3.1 & 4.2 & 33.3 & 37.5 & 0.0 & 12.5 & 62.5 & 18.3 & 0.0 & 0.0 & 0.0 & 12.5 & 17.2 \\
 & 2-shot  & 30.0 & 25.0 & 41.7 & 12.5 & 0.0 & 66.7 & 66.7 & 62.5 & 37.5 & 22.5 & 91.7 & 36.5 & 0.0 & 0.0 & 50.0 & 75.0 & 37.9 \\
 & Rule Hint & 42.5 & 4.2 & 8.3 & 0.0 & 0.0 & 8.3 & 41.7 & 7.5 & 8.3 & 5.0 & 70.8 & 13.5 & 0.0 & 0.0 & 0.0 & 0.0 & 15.1 \\
\cdashlinelr{1-19} 
\multirow{5}{*}{GPT4} & Base  & 97.0 & 83.3 & 70.8 & 43.5 & 78.1 & 41.7 & 91.7 & 92.5& 79.2 & 79.5 & 91.7 & 82.7 & 75.0 & 75.0 & 25.0 & 37.5 & 78.4 \\ 
& CoT & 98.4 & 66.7 & 67.8 & 56.5 & 71.9 & 37.5 & 87.5 & 87.5 & 75.0 & 84.6 & 87.5 & 76.9 & 62.5 & 68.8 & 37.1 & 25.8 & 74.9 \\
 & 1-shot & 95.0 & 66.7 & 70.8 & 78.3 & 68.8 & 54.2 & 79.2 & 97.5 & 87.5 & 80.0 & 91.7 & 84.0 & 75.0 & 50.0 & 37.5 & 50.0 & 78.9 \\
 & 2-shot & 95.0 & 79.2 & 65.2 & 75.0 & 87.5 & 54.2 & 87.5 & 97.5 & 79.2 & 82.1 & 95.8 & 84.6 & 96.0 & 75.0 & 50.0 & 62.5 & 82.7 \\
 & Rule Hint & 97.5 & 66.7 & 65.2 & 50.0 & 65.6 & 45.8 & 83.3 & 95.0 & 83.3 & 80.0 & 91.7 & 75.7 & 50.0 & 56.2 & 75.0 & 12.5 & 74.5 \\
\cdashlinelr{1-19} 
\multirow{5}{*}{GPT4-turbo} & Base & 87.6 & 61.3 & 56.9 & 51.8 & 64.9 & 50.8 & 80.4 & 82.4 &71.2 & 69.8 & 77.8 & 74.5 & 45.7 & 59.1 & 71.4 & 18.5 & 69.3 \\
 & CoT & 81.6 & 57.4 & 52.0 & 45.2 & 63.6 & 43.8 & 78.8 & 79.2 & 61.1 & 63.8 & 76.2 & 62.8 & 52.7 & 74.6 & 58.3 & 7.1 & 62.6 \\
 & 1-shot & 92.5 & 66.7 & 62.5 & 62.5 & 59.4 & 58.3 & 70.8 & 82.5 & 66.7 & 77.5 & 70.8 & 78.8 & 37.5 & 50.0 & 75.0 & 37.5 & 71.6 \\
 & 2-shot & 87.5 & 62.5 & 66.7 & 75.0 & 68.8 & 54.2 & 75.0 & 92.5 & 83.3 & 75.0 & 75.0 & 80.8 & 50.0 & 68.8 & 50.0 & 37.5 & 75.0 \\
 & Rule Hint & 82.5 & 62.5 & 62.5 & 50.0 & 78.1 & 29.2 & 70.8 & 87.5 & 66.7 & 60.0 & 70.8 & 76.9 & 25.0 & 93.8 & 50.0 & 12.5 & 68.5 \\
\bottomrule
\end{tabular}}
\caption{Exact Match Score for close-sourced LLMs' performance.}
\label{tab:em_api_overall}
\vspace{-5mm}
\end{table}





==> performance_RougeL_tables.tex <==

\definecolor{lightblue}{RGB}{173, 216, 230}
\definecolor{lightgreen}{RGB}{144, 238, 144}
\definecolor{lightyellow}{RGB}{255, 255, 224}
\definecolor{lightred}{RGB}{255, 182, 193}
\definecolor{lightpurple}{RGB}{216, 191, 216}

\definecolor{darkblue}{RGB}{123, 166, 180}   
\definecolor{darkgreen}{RGB}{94, 188, 94}    
\definecolor{darkyellow}{RGB}{245, 245, 184} 
\definecolor{darkred}{RGB}{205, 132, 143}    
\definecolor{darkpurple}{RGB}{166, 141, 166} 



\begin{table}[t]
\centering
{\fontsize{6.8pt}{8.6pt}\selectfont
\setlength{\tabcolsep}{2.6pt} % 可以根据需要调整这个值
\begin{tabular}{lcccccccccccccccccc}
\toprule
\multirow{2}{*}{\textbf{Model}}&
\multirow{2}{*}{\textbf{Prompt}} &
\multicolumn{8}{c}{\textbf{Languages}} &
\multicolumn{8}{c}{\textbf{Tasks}} &
\multirow{2}{*}{\textbf{all}}\\
\cline{3-10}
 \cdashlinelr{11-18} 
% \cdashlinelr{3-10} 
% \cdashlinelr{11-18} 
 && \textbf{JSON} & \textbf{LaTeX} & \textbf{Md.} & \textbf{ORG} & \textbf{CSV} & \textbf{Tree} & \textbf{XML} & \textbf{YAML}
 & \textbf{PC} & \textbf{PW} & \textbf{SY} & \textbf{TR} & \textbf{JO} & \textbf{ST} & \textbf{ND} & \textbf{TH} &  \\ 
\midrule
Ernie-Turbo&Base&1.30 & 1.40 & 1.00 & 0.90 & 1.00 & 0.50 & 4.00 & 7.00 & 0.10 & 0.60 & 0.00 & 4.70 & 0.20 & 1.20 & 0.70 & 0.70 & 2.40 \\
Ernie-Turbo&CoT&1.10 & 1.20 & 0.90 & 0.90 & 1.20 & 0.90 & 2.00 & 5.70 & 0.10 & 1.10 & 0.00 & 7.20 & 1.50 & 3.10 & 3.00 & 2.30 & 2.00 \\
Ernie-Turbo&1-shot&11.00 & 16.90 & 19.60 & 17.00 & 3.10 & 1.40 & 1.30 & 12.20 & 0.80 & 13.80 & 0.00 & 16.90 & 1.20 & 0.90 & 2.00 & 0.70 & 10.20 \\
Ernie-Turbo&2-shot&7.00 & 24.60 & 21.70 & 17.50 & 3.10 & 1.60 & 8.60 & 7.50 & 0.40 & 16.80 & 0.00 & 16.50 & 2.90 & 0.20 & 2.20 & 1.70 & 10.60 \\
Ernie-Turbo&Rule Hint&2.50 & 6.60 & 8.00 & 9.20 & 0.90 & 0.70 & 1.40 & 4.00 & 0.00 & 7.80 & 0.00 & 5.50 & 0.20 & 0.90 & 1.30 & 0.60 & 3.90 \\
   \cdashlinelr{1-19} 
Minimax&Base&16.20 & 39.60 & 34.30 & 31.80 & 6.10 & 2.50 & 5.90 & 19.30 & 2.70 & 25.60 & 4.10 & 19.60 & 1.70 & 4.80 & 4.70 & 0.00 & 9.50 \\
Minimax&CoT&15.50 & 37.90 & 33.80 & 29.90 & 2.30 & 2.20 & 5.70 & 18.20 & 6.20 & 47.30 & 8.40 & 46.60 & 3.60 & 8.30 & 6.30 & 0.00 & 6.60 \\
Minimax&1-shot&19.50 & 33.30 & 33.10 & 32.80 & 6.30 & 4.30 & 14.10 & 23.90 & 3.10 & 30.70 & 4.40 & 30.40 & 3.30 & 4.20 & 4.70 & 6.90 & 20.50 \\
Minimax&2-shot&23.60 & 38.50 & 34.80 & 35.50 & 8.60 & 3.70 & 13.30 & 25.30 & 4.40 & 32.80 & 3.40 & 34.00 & 6.70 & 6.10 & 1.60 & 6.90 & 22.60 \\
Minimax&Rule Hint&12.90 & 18.10 & 19.80 & 20.80 & 2.20 & 0.60 & 5.10 & 11.70 & 0.00 & 16.70 & 3.60 & 17.40 & 0.40 & 1.30 & 1.90 & 0.00 & 11.20 \\
   \cdashlinelr{1-19} 
Spark&Base&0.40 & 0.20 & 9.30 & 0.20 & 0.20 & 0.00 & 0.10 & 0.50 & 0.00 & 4.40 & 0.10 & 0.90 & 0.40 & 0.10 & 0.10 & 0.10 & 1.20 \\
Spark&CoT&0.40 & 0.20 & 6.10 & 0.20 & 0.20 & 0.00 & 0.10 & 0.50 & 0.00 & 6.00 & 0.20 & 1.50 & 0.60 & 0.20 & 0.10 & 0.10 & 0.90 \\
Spark&1-shot&4.10 & 2.00 & 1.40 & 8.50 & 0.10 & 0.10 & 0.30 & 2.00 & 0.00 & 4.90 & 0.50 & 3.20 & 0.00 & 0.00 & 0.20 & 0.20 & 2.30 \\
Spark&2-shot&1.00 & 0.50 & 0.50 & 0.60 & 0.40 & 0.10 & 0.20 & 1.10 & 0.00 & 0.60 & 0.10 & 1.00 & 0.00 & 0.10 & 0.10 & 0.10 & 0.60 \\
Spark&Rule Hint&0.40 & 1.20 & 1.00 & 4.00 & 0.30 & 0.10 & 0.70 & 1.30 & 0.00 & 2.60 & 0.20 & 1.20 & 0.30 & 0.30 & 0.10 & 0.10 & 1.00 \\
   \cdashlinelr{1-19} 
GPT4&Base&19.70 & 41.20 & 38.70 & 38.00 & 11.50 & 3.90 & 10.70 & 21.60 & 7.00 & 29.90 & 2.10 & 33.00 & 9.40 & 13.60 & 3.10 & 2.60 & 22.30 \\
GPT4&CoT&18.40 & 39.90 & 38.50 & 39.60 & 7.20 & 4.40 & 8.60 & 20.70 & 6.20 & 30.80 & 2.10 & 31.50 & 0.90 & 9.90 & 4.70 & 2.00 & 21.20 \\
GPT4&1-shot&22.80 & 38.50 & 35.50 & 38.90 & 11.30 & 5.50 & 18.50 & 26.00 & 9.40 & 34.30 & 4.00 & 34.50 & 10.00 & 9.80 & 4.70 & 3.40 & 23.90 \\
GPT4&2-shot&23.10 & 38.70 & 38.20 & 36.70 & 14.40 & 5.40 & 17.50 & 26.30 & 8.40 & 35.10 & 3.40 & 34.60 & 13.30 & 14.50 & 6.20 & 4.30 & 24.60 \\
GPT4&Rule Hint&13.50 & 22.20 & 21.20 & 23.80 & 3.20 & 1.80 & 5.00 & 13.70 & 2.70 & 19.10 & 2.20 & 19.20 & 1.60 & 2.70 & 2.90 & 0.40 & 12.70 \\
   \cdashlinelr{1-19} 
GPT4-Turbo&Base&10.70 & 35.10 & 34.10 & 32.30 & 2.90 & 1.80 & 8.90 & 15.90 & 1.40 & 23.70 & 1.60 & 26.10 & 1.30 & 2.40 & 2.50 & 0.90 & 16.20 \\
GPT4-Turbo&CoT&8.70 & 31.40 & 30.00 & 27.30 & 2.00 & 1.50 & 7.80 & 13.80 & 2.30 & 45.40 & 3.10 & 43.60 & 2.30 & 3.80 & 4.20 & 1.60 & 13.90 \\
GPT4-Turbo&1-shot&21.30 & 35.90 & 35.50 & 36.70 & 8.70 & 5.90 & 17.90 & 25.00 & 7.50 & 33.20 & 1.50 & 33.70 & 1.50 & 9.40 & 8.20 & 2.50 & 22.80 \\
GPT4-Turbo&2-shot&21.70 & 37.50 & 36.30 & 36.70 & 11.10 & 5.10 & 16.90 & 25.30 & 8.50 & 33.40 & 1.50 & 34.10 & 1.90 & 14.00 & 5.00 & 2.10 & 23.30 \\
GPT4-Turbo&Rule Hint&9.70 & 20.70 & 21.90 & 21.90 & 2.00 & 0.60 & 3.70 & 12.20 & 0.70 & 16.70 & 1.60 & 17.40 & 1.50 & 2.00 & 1.20 & 0.20 & 11.10 \\

\bottomrule
\end{tabular}}
\caption{RougeL Score for close-sourced LLMs' performance.}
\label{tab:rougel_api_overall}
\vspace{-5mm}
\end{table}





==> plotdata/GPTJUDGEForFT.tex <==
% acc for model base_finetune is 0.9956896551724138
% acc for model fewshot_finetune is 0.9870689655172413
% acc for model mixrulehint_finetune is 0.9913793103448276
% acc for model mix_finetune is 0.9913793103448276
% acc for model rulehint_finetune is 0.978448275862069

% draw a bar graph in tikz:

\begin{figure}
  \center
\begin{tikzpicture}
\begin{axis}[
    ybar=2*\pgflinewidth,
    % height=\textwidth,
    symbolic x coords={Pretrain, Base,2-Shot,RH Mix,Mix,RH},
    ylabel = {GPTJudge Acc.},
    xtick=data,
    enlarge y limits={upper, value=0.15},
    ymin=0,
    nodes near coords,
    nodes near coords align={vertical},
    nodes near coords style={rotate=90, anchor=west}
]


\addplot[style={lightgray,fill=lightgray,mark=none, text=black}] coordinates {
  (Pretrain,0.06465517241379311)
   (Base,0.5043103448275862)
   (2-Shot,0.2413793103448276)
   (RH Mix,0.47413793103448276)
   (Mix,0.3146551724137931)
   (RH,0.04310344827586207)
};
\addplot[red,sharp plot,update limits=false] coordinates { ([normalized]-2,0.06465517241379311) ([normalized]6.5,0.06465517241379311) };

\end{axis}
\end{tikzpicture}
\caption{GPTJudge Acc. Fine-tuned on Various Dataset. Score before finetune marked by red line.}
\label{fig:judgeftmethod}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:

% yehaoning@WIN-6OHPAKJ9FU2 MINGW64 /f/yhn/LLaMA-Factory (main)
% $ cat ../LLMStructure/log.txt | grep acc|grep "for model"
% acc for model base_finetune is 0.5043103448275862
% acc for model fewshot_finetune is 0.2413793103448276
% acc for model mixrulehint_finetune is 0.47413793103448276
% acc for model mix_finetune is 0.3146551724137931
% acc for model rulehint_finetune is 0.04310344827586207
% acc for model before_finetune is 0.06465517241379311


==> plotdata/GPTJudgeForAPIDetailed.tex <==
% HEATMAP
\def\cellsize{10mm}
\def\scalerate{0.6}
\newcommand{\heatmap}[2]{
  \begin{subfigure}[b]{0.5\textwidth}
    \begin{tikzpicture}
      [scale=\scalerate, every node/.style={transform shape}]
      \foreach \y [count=\n] in {#1} {
        \foreach \x [count=\m] in \y {% heatmap tiles
          \pgfmathsetmacro{\colorpercentage}{100*\x}
          \node[fill=rred!\colorpercentage!bblue, minimum size=\cellsize, text=white] at (\m,-\n) {\x};
        }
      }
      % column labels
      \foreach \x [count=\m] in {SPARK*, SPARK, MINIMAX*, MINIMAX, ERNIE*, ERNIE, \textbf{GPT4*}, \textbf{GPT4}, GPT4*, GPT4} {
        \node[minimum size=\cellsize] at (\m, 0) {\tiny{\x}};
      }
      % row labels
      \foreach \a [count=\i] in {2shot, 1shot, rulehint$^{+}$, base} {
        \node[minimum size=\cellsize] at (0,-\i) {\tiny{\a}};
      }

      % \node [align=flush center,text width=8cm] at (5,-5)
      % {#2};% in-pic caption https://tex.stackexchange.com/a/24010
    \end{tikzpicture}
    \caption{#2} % \label{fig:y equals x}
  \end{subfigure}
  \hfill
}
% HEATMAP https://tikz.net/heatmap/
%
\begin{figure}
\heatmap{
{0.625,0.667,0.417,0.458,0.083,0.208,0.417,0.542,0.625,0.542},
{0.333,0.042,0.542,0.500,0.083,0.125,0.542,0.583,0.500,0.542},
{0.125,0.083,0.167,0.167,0.000,0.000,0.250,0.292,0.375,0.458},
{0.227,0.292,0.125,0.208,0.042,0.042,0.375,0.542,0.375,0.417},
}{GPTJudge Acc Tree}
\heatmap{
{0.031,0.000,0.438,0.500,0.156,0.219,0.688,0.688,0.750,0.875},
{0.000,0.031,0.375,0.375,0.281,0.219,0.531,0.594,0.656,0.688},
{0.188,0.000,0.344,0.406,0.031,0.094,0.719,0.781,0.500,0.656},
{0.094,0.031,0.406,0.438,0.094,0.062,0.688,0.688,0.719,0.781},
}{GPTJudge Acc Tabular}
\heatmap{
{0.300,0.300,0.800,0.900,0.175,0.125,0.925,0.875,0.950,0.950},
{0.300,0.275,0.775,0.800,0.175,0.250,0.875,0.925,0.875,0.950},
{0.550,0.425,0.825,0.775,0.150,0.325,0.875,0.825,0.950,0.975},
{0.650,0.400,0.875,0.775,0.150,0.200,0.800,0.850,1.000,1.000},
}{GPTJudge Acc JSON}
\heatmap{
{0.641,0.625,0.750,0.825,0.175,0.050,0.825,0.925,0.925,0.975},
{0.550,0.375,0.650,0.850,0.250,0.250,0.850,0.825,0.925,0.975},
{0.325,0.075,0.675,0.625,0.125,0.325,0.900,0.875,0.950,0.950},
{0.769,0.575,0.650,0.700,0.150,0.175,0.800,0.850,0.875,0.925},
}{GPTJudge Acc YAML}
\heatmap{
{0.917,0.667,0.458,0.625,0.167,0.167,0.667,0.750,0.833,0.875},
{0.250,0.333,0.667,0.625,0.083,0.083,0.750,0.708,0.833,0.792},
{0.458,0.417,0.792,0.667,0.167,0.125,0.875,0.708,0.875,0.833},
{0.652,0.636,0.625,0.583,0.042,0.083,0.708,0.833,0.875,0.917},
}{GPTJudge Acc XML}
\heatmap{
{0.167,0.417,0.292,0.542,0.042,0.125,0.667,0.667,0.783,0.652},
{0.042,0.042,0.542,0.583,0.000,0.042,0.667,0.625,0.625,0.708},
{0.167,0.083,0.458,0.542,0.042,0.000,0.542,0.625,0.542,0.652},
{0.042,0.043,0.458,0.417,0.000,0.000,0.458,0.542,0.667,0.708},
}{GPTJudge Acc Markdown}
\heatmap{
{0.125,0.125,0.333,0.542,0.000,0.083,0.667,0.750,0.708,0.750},
{0.083,0.042,0.375,0.500,0.000,0.087,0.667,0.625,0.739,0.783},
{0.042,0.000,0.375,0.500,0.000,0.000,0.375,0.500,0.542,0.500},
{0.208,0.125,0.333,0.292,0.042,0.000,0.208,0.500,0.565,0.435},
}{GPTJudge Acc ORG}
\heatmap{
{0.250,0.250,0.458,0.583,0.083,0.125,0.750,0.625,0.750,0.792},
{0.042,0.083,0.417,0.500,0.042,0.000,0.750,0.667,0.682,0.667},
{0.083,0.042,0.500,0.375,0.000,0.000,0.583,0.625,0.583,0.667},
{0.227,0.208,0.583,0.583,0.000,0.043,0.542,0.667,0.667,0.833},
}{GPTJudge Acc LaTeX}
\caption{API Test Original Data}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:

% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for Tree }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.625,0.667,0.417,0.458,0.083,0.208,0.417,0.542,0.625,0.542
% 0.125,0.083,0.167,0.167,0.000,0.000,0.250,0.292,0.375,0.458
% 0.125,0.000,0.167,0.417,0.000,0.000,0.458,0.125,0.208,0.375
% 0.227,0.292,0.125,0.208,0.042,0.042,0.375,0.542,0.375,0.417
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for SQL }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.031,0.000,0.438,0.500,0.156,0.219,0.688,0.688,0.750,0.875
% 0.188,0.000,0.344,0.406,0.031,0.094,0.719,0.781,0.500,0.656
% 0.000,0.000,0.250,0.188,0.094,0.125,0.469,0.406,0.406,0.625
% 0.094,0.031,0.406,0.438,0.094,0.062,0.688,0.688,0.719,0.781
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for JSON }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.300,0.300,0.800,0.900,0.175,0.125,0.925,0.875,0.950,0.950
% 0.550,0.425,0.825,0.775,0.150,0.325,0.875,0.825,0.950,0.975
% 0.050,0.000,0.350,0.325,0.150,0.075,0.500,0.600,0.475,0.550
% 0.650,0.400,0.875,0.775,0.150,0.200,0.800,0.850,1.000,1.000
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for YAML }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.641,0.625,0.750,0.825,0.175,0.050,0.825,0.925,0.925,0.975
% 0.325,0.075,0.675,0.625,0.125,0.325,0.900,0.875,0.950,0.950
% 0.125,0.075,0.250,0.375,0.050,0.000,0.575,0.450,0.425,0.650
% 0.769,0.575,0.650,0.700,0.150,0.175,0.800,0.850,0.875,0.925
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for XML }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.917,0.667,0.458,0.625,0.167,0.167,0.667,0.750,0.833,0.875
% 0.458,0.417,0.792,0.667,0.167,0.125,0.875,0.708,0.875,0.833
% 0.435,0.333,0.292,0.667,0.042,0.125,0.417,0.667,0.292,0.583
% 0.652,0.636,0.625,0.583,0.042,0.083,0.708,0.833,0.875,0.917
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for Markdown }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.167,0.417,0.292,0.542,0.042,0.125,0.667,0.667,0.783,0.652
% 0.167,0.083,0.458,0.542,0.042,0.000,0.542,0.625,0.542,0.652
% 0.389,0.067,0.167,0.292,0.000,0.000,0.417,0.500,0.375,0.417
% 0.042,0.043,0.458,0.417,0.000,0.000,0.458,0.542,0.667,0.708
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for ORG }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.125,0.125,0.333,0.542,0.000,0.083,0.667,0.750,0.708,0.750
% 0.042,0.000,0.375,0.500,0.000,0.000,0.375,0.500,0.542,0.500
% 0.231,0.250,0.167,0.208,0.000,0.000,0.333,0.292,0.375,0.625
% 0.208,0.125,0.333,0.292,0.042,0.000,0.208,0.500,0.565,0.435
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for LaTeX }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.250,0.250,0.458,0.583,0.083,0.125,0.750,0.625,0.750,0.792
% 0.083,0.042,0.500,0.375,0.000,0.000,0.583,0.625,0.583,0.667
% 0.471,0.333,0.417,0.667,0.000,0.000,0.750,0.750,0.708,0.708
% 0.227,0.208,0.583,0.583,0.000,0.043,0.542,0.667,0.667,0.833
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}


==> plotdata/GPTJudgeForAPIMethod.tex <==

% todo: refactor the logic to draw the heatmap
\def\rows{SPARK*, SPARK, MINIMAX*, MINIMAX, ERNIE*, ERNIE, \textbf{GPT4*}, \textbf{GPT4}, GPT4*, GPT4}
\def\cols{2shot, 1shot, rulehint$^{+}$, base}
\newcommand{\methodheatmap}[1]{
\begin{tikzpicture}
  [scale=\ratio, every node/.style={transform shape}]
  \foreach \y [count=\n] in #1 {

    \foreach \x [count=\m] in \y {% heatmap tiles
      \pgfmathsetmacro{\colorpercentage}{100*\x}
%      \pgfmathsetmacro{\xpos}{(\ratio * \m)}

      \node[fill=rred!\colorpercentage!bblue, minimum size=\cellsize, text=white] at (\m,-\n) {\x};
    }
  }
  % row labels
  \foreach \x [count=\m] in \rows {
%    \pgfmathsetmacro{\xpos}{(\ratio * \m)}
    \node at (\m, 0) {\tiny{\x}};
  }
  % column labels
  \foreach \a [count=\i] in \cols {
    \node at (0,-\i) {\tiny{\a}};
  }
\end{tikzpicture}
}

\def\cellsize{11mm}
\def\ratio{1.1}
\begin{figure}
  \centering
%   \methodheatmap{{
%     {0.382,0.379,0.530,0.651,0.121,0.134,0.724,0.750,0.809,0.826},
%     {0.224,0.172,0.560,0.616,0.134,0.151,0.720,0.716,0.750,0.788},
%     {0.267,0.151,0.543,0.530,0.073,0.138,0.677,0.685,0.698,0.744},
%     {0.398,0.307,0.539,0.530,0.078,0.091,0.608,0.707,0.748,0.782},
% %    {0.398,0.307,0.539,0.530,0.078,0.091,0.608,0.707,0.748,0.782},
%   }}

% \definecolor{rred}{HTML}{d43e4f}
% \definecolor{ppurple}{HTML}{5e4fa2}
% \definecolor{ccyan}{HTML}{67c1a5}
% \definecolor{ggreen}{HTML}{acdda5}
% \definecolor{llime}{HTML}{e6f598}
% \definecolor{yyellow}{HTML}{ffffbf}
% \definecolor{llightorange}{HTML}{fdae61}
% \definecolor{bblue}{HTML}{3287bd}
% \definecolor{oorange}{HTML}{f46e43}
\begin{tikzpicture}
\begin{axis}[
    % width  = \textwidth,
    ymin=0,
    bar width=3pt,
    ybar=2*\pgflinewidth,
    symbolic x coords={2shot, 1shot, rulehint$^{+}$, base},
    % ymajorgrids = true,
    enlarge x limits=0.15,
    ylabel = {GPTJudge Acc.},
    xtick=data,
    % nodes near coords,
    % nodes near coords align={vertical},
    % nodes near coords/.append style={/pgf/number format/.cd,fixed,precision=10},
    legend style={
      at={(1.05,1.00)},
      anchor=north west,
      column sep=0.5ex}
]
\addplot[style={rred,fill=rred,mark=none}] coordinates {
  (2shot,         0.382)
  (1shot,         0.224)
  (rulehint$^{+}$,0.267)
  (base,          0.398)
};
\addplot[style={rrred,fill=rrred,mark=none}] coordinates {
  (2shot,         0.379)
  (1shot,         0.172)
  (rulehint$^{+}$,0.151)
  (base,          0.307)
};
\addplot[style={bblue,fill=bblue,mark=none}] coordinates {
  (2shot,         0.530)
  (1shot,         0.560)
  (rulehint$^{+}$,0.543)
  (base,          0.539)
};
\addplot[style={bbblue,fill=bbblue,mark=none}] coordinates {
  (2shot,         0.651)
  (1shot,         0.616)
  (rulehint$^{+}$,0.530)
  (base,          0.530)
};
\addplot[style={ppurple,fill=ppurple,mark=none}] coordinates {
  (2shot,         0.121)
  (1shot,         0.134)
  (rulehint$^{+}$,0.073)
  (base,          0.078)
};
\addplot[style={pppurple,fill=pppurple,mark=none}] coordinates {
  (2shot,         0.134)
  (1shot,         0.151)
  (rulehint$^{+}$,0.138)
  (base,          0.091)
};
\addplot[style={ggreen,fill=ggreen,mark=none}] coordinates {
  (2shot,         0.724)
  (1shot,         0.720)
  (rulehint$^{+}$,0.677)
  (base,          0.608)
};
\addplot[style={gggreen,fill=gggreen,mark=none}] coordinates {
  (2shot,         0.750)
  (1shot,         0.716)
  (rulehint$^{+}$,0.685)
  (base,          0.707)
};
\addplot[style={ccyan,fill=ccyan,mark=none}] coordinates {
  (2shot,         0.809)
  (1shot,         0.750)
  (rulehint$^{+}$,0.698)
  (base,          0.748)
};
\addplot[style={cccyan,fill=cccyan,mark=none}] coordinates {
  (2shot,         0.826)
  (1shot,         0.788)
  (rulehint$^{+}$,0.744)
  (base,          0.782)
};
\legend{SPARK*, SPARK, MINIMAX*, MINIMAX, ERNIE*, ERNIE, GPT4-turbo*, GPT4-turbo, GPT4*, GPT4}
\end{axis}
\end{tikzpicture}
\caption{GPTJudge Acc. for API Test. Prompt w/ Hint Eliciting in ~\autoref{fig:framework_hint} marked by *}
\label{fig:judgeapimethod}
\end{figure}

\def\cols{base}
\def\rows{\textit{SPARK}, SPARK, \textit{MINIMAX}, MINIMAX, \textit{ERNIE}, ERNIE, \textbf{\textit{GPT4}}, \textbf{GPT4}, \textit{GPT4}, GPT4}

\def\cellsize{11mm}
\def\ratio{1.1}




\newif\ifsimplehard
\simplehardfalse
\ifsimplehard
\begin{figure}
  \centering
%   \methodheatmap{{
%     % {0.405,0.353,0.759,0.543,0.172,0.095,0.862,0.638,0.912,0.741},
%     % {0.198,0.147,0.724,0.509,0.216,0.086,0.836,0.595,0.894,0.690},
%     % {0.147,0.155,0.603,0.457,0.181,0.095,0.776,0.595,0.817,0.672},
%     {0.349,0.266,0.569,0.491,0.121,0.061,0.681,0.733,0.815,0.750},
% %    {0.398,0.307,0.539,0.530,0.078,0.091,0.608,0.707,0.748,0.782},
%   }}
\begin{tikzpicture}
\begin{axis}[
    % width  = 0.5\textwidth,
    ymin=0,
    bar width=12pt,
    ybar=2*\pgflinewidth,
    symbolic x coords={Hard, Simple},
    % ymajorgrids = true,
    enlarge x limits=0.45,
    ylabel = {GPTJudge Acc.},
    xtick=data,
    % nodes near coords,
    % nodes near coords align={vertical},
    % nodes near coords/.append style={/pgf/number format/.cd,fixed,precision=10},
    legend style={
      at={(1.05,1.00)},
      anchor=north west,
      column sep=1ex}
]
\addplot[style={rred,fill=rred,mark=none}] coordinates {
  (Hard,         0.266)
  (Simple,       0.349)
};
\addplot[style={bblue,fill=bblue,mark=none}] coordinates {
  (Hard,         0.491)
  (Simple,       0.569)
};
\addplot[style={ppurple,fill=ppurple,mark=none}] coordinates {
  (Hard,         0.061)
  (Simple,       0.121)
};
\addplot[style={ggreen,fill=ggreen,mark=none}] coordinates {
  (Hard,         0.733)
  (Simple,       0.681)
};
\addplot[style={ccyan,fill=ccyan,mark=none}] coordinates {
  (Hard,         0.750)
  (Simple,       0.815)
};
\legend{SPARK, MINIMAX, ERNIE, \textbf{GPT4}, GPT4}
\end{axis}
\end{tikzpicture}
\caption{GPTJudge Acc. API Test. Hard v.s., Simple.}
\label{fig:judgeapimethodcmpsimplehard}
\end{figure}
\fi

% Avg input file len is 532.1379310344828 bytes SIMPLE
% Avg input file len is 1534.6637931034484 bytes Hard

% \begin{figure}
%   \centering
%   \methodheatmap{{
%     {     ,0.405,     ,0.759,     ,0.172,     ,0.862,     ,0.912},
%     {     ,0.198,     ,0.724,     ,0.216,     ,0.836,     ,0.894},
%     {     ,0.147,     ,0.603,     ,0.181,     ,0.776,     ,0.817},
%     {     ,0.349,     ,0.569,     ,0.121,     ,0.681,     ,0.815},
% %    {0.398,0.307,0.539,0.530,0.078,0.091,0.608,0.707,0.748,0.782},
%   }}
% \caption{GPTJudge Acc. API Test. Simple Data}
% \label{fig:judgeapimethodsimple}
% \end{figure}

% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for Tree }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.625,0.667,0.417,0.458,0.083,0.208,0.417,0.542,0.625,0.542
% 0.125,0.083,0.167,0.167,0.000,0.000,0.250,0.292,0.375,0.458
% 0.125,0.000,0.167,0.417,0.000,0.000,0.458,0.125,0.208,0.375
% 0.227,0.292,0.125,0.208,0.042,0.042,0.375,0.542,0.375,0.417
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for SQL }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.031,0.000,0.438,0.500,0.156,0.219,0.688,0.688,0.750,0.875
% 0.188,0.000,0.344,0.406,0.031,0.094,0.719,0.781,0.500,0.656
% 0.000,0.000,0.250,0.188,0.094,0.125,0.469,0.406,0.406,0.625
% 0.094,0.031,0.406,0.438,0.094,0.062,0.688,0.688,0.719,0.781
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for JSON }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.300,0.300,0.800,0.900,0.175,0.125,0.925,0.875,0.950,0.950
% 0.550,0.425,0.825,0.775,0.150,0.325,0.875,0.825,0.950,0.975
% 0.050,0.000,0.350,0.325,0.150,0.075,0.500,0.600,0.475,0.550
% 0.650,0.400,0.875,0.775,0.150,0.200,0.800,0.850,1.000,1.000
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for YAML }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.641,0.625,0.750,0.825,0.175,0.050,0.825,0.925,0.925,0.975
% 0.325,0.075,0.675,0.625,0.125,0.325,0.900,0.875,0.950,0.950
% 0.125,0.075,0.250,0.375,0.050,0.000,0.575,0.450,0.425,0.650
% 0.769,0.575,0.650,0.700,0.150,0.175,0.800,0.850,0.875,0.925
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for XML }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.917,0.667,0.458,0.625,0.167,0.167,0.667,0.750,0.833,0.875
% 0.458,0.417,0.792,0.667,0.167,0.125,0.875,0.708,0.875,0.833
% 0.435,0.333,0.292,0.667,0.042,0.125,0.417,0.667,0.292,0.583
% 0.652,0.636,0.625,0.583,0.042,0.083,0.708,0.833,0.875,0.917
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for Markdown }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.167,0.417,0.292,0.542,0.042,0.125,0.667,0.667,0.783,0.652
% 0.167,0.083,0.458,0.542,0.042,0.000,0.542,0.625,0.542,0.652
% 0.389,0.067,0.167,0.292,0.000,0.000,0.417,0.500,0.375,0.417
% 0.042,0.043,0.458,0.417,0.000,0.000,0.458,0.542,0.667,0.708
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for ORG }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.125,0.125,0.333,0.542,0.000,0.083,0.667,0.750,0.708,0.750
% 0.042,0.000,0.375,0.500,0.000,0.000,0.375,0.500,0.542,0.500
% 0.231,0.250,0.167,0.208,0.000,0.000,0.333,0.292,0.375,0.625
% 0.208,0.125,0.333,0.292,0.042,0.000,0.208,0.500,0.565,0.435
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for LaTeX }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.250,0.250,0.458,0.583,0.083,0.125,0.750,0.625,0.750,0.792
% 0.083,0.042,0.500,0.375,0.000,0.000,0.583,0.625,0.583,0.667
% 0.471,0.333,0.417,0.667,0.000,0.000,0.750,0.750,0.708,0.708
% 0.227,0.208,0.583,0.583,0.000,0.043,0.542,0.667,0.667,0.833
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}

% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for Tree }
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.625,0.667,0.417,0.458,0.083,0.208,0.417,0.542,0.625,0.542
% 0.333,0.042,0.542,0.500,0.083,0.125,0.542,0.583,0.500,0.542
% 0.125,0.083,0.167,0.167,0.000,0.000,0.250,0.292,0.375,0.458
% 0.227,0.292,0.125,0.208,0.042,0.042,0.375,0.542,0.375,0.417
% \end{tabular}
% }
% \end{center}
% \end{table}
% \end{frame}
% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for SQL }
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.031,0.000,0.438,0.500,0.156,0.219,0.688,0.688,0.750,0.875
% 0.000,0.031,0.375,0.375,0.281,0.219,0.531,0.594,0.656,0.688
% 0.188,0.000,0.344,0.406,0.031,0.094,0.719,0.781,0.500,0.656
% 0.094,0.031,0.406,0.438,0.094,0.062,0.688,0.688,0.719,0.781
% \end{tabular}
% }
% \end{center}
% \end{table}
% \end{frame}
% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for JSON }
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.300,0.300,0.800,0.900,0.175,0.125,0.925,0.875,0.950,0.950
% 0.300,0.275,0.775,0.800,0.175,0.250,0.875,0.925,0.875,0.950
% 0.550,0.425,0.825,0.775,0.150,0.325,0.875,0.825,0.950,0.975
% 0.650,0.400,0.875,0.775,0.150,0.200,0.800,0.850,1.000,1.000
% \end{tabular}
% }
% \end{center}
% \end{table}
% \end{frame}
% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for YAML }
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.641,0.625,0.750,0.825,0.175,0.050,0.825,0.925,0.925,0.975
% 0.550,0.375,0.650,0.850,0.250,0.250,0.850,0.825,0.925,0.975
% 0.325,0.075,0.675,0.625,0.125,0.325,0.900,0.875,0.950,0.950
% 0.769,0.575,0.650,0.700,0.150,0.175,0.800,0.850,0.875,0.925
% \end{tabular}
% }
% \end{center}
% \end{table}
% \end{frame}
% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for XML }
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.917,0.667,0.458,0.625,0.167,0.167,0.667,0.750,0.833,0.875
% 0.250,0.333,0.667,0.625,0.083,0.083,0.750,0.708,0.833,0.792
% 0.458,0.417,0.792,0.667,0.167,0.125,0.875,0.708,0.875,0.833
% 0.652,0.636,0.625,0.583,0.042,0.083,0.708,0.833,0.875,0.917
% \end{tabular}
% }
% \end{center}
% \end{table}
% \end{frame}
% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for Markdown }
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.167,0.417,0.292,0.542,0.042,0.125,0.667,0.667,0.783,0.652
% 0.042,0.042,0.542,0.583,0.000,0.042,0.667,0.625,0.625,0.708
% 0.167,0.083,0.458,0.542,0.042,0.000,0.542,0.625,0.542,0.652
% 0.042,0.043,0.458,0.417,0.000,0.000,0.458,0.542,0.667,0.708
% \end{tabular}
% }
% \end{center}
% \end{table}
% \end{frame}
% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for ORG }
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.125,0.125,0.333,0.542,0.000,0.083,0.667,0.750,0.708,0.750
% 0.083,0.042,0.375,0.500,0.000,0.087,0.667,0.625,0.739,0.783
% 0.042,0.000,0.375,0.500,0.000,0.000,0.375,0.500,0.542,0.500
% 0.208,0.125,0.333,0.292,0.042,0.000,0.208,0.500,0.565,0.435
% \end{tabular}
% }
% \end{center}
% \end{table}
% \end{frame}
% \begin{frame}
% \begin{table}[htbp!]
% \caption{GPT Judge for LaTeX}
% \begin{center}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{r|lllllllllll}
% \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% \\\hline
% 0.250,0.250,0.458,0.583,0.083,0.125,0.750,0.625,0.750,0.792
% 0.042,0.083,0.417,0.500,0.042,0.000,0.750,0.667,0.682,0.667
% 0.083,0.042,0.500,0.375,0.000,0.000,0.583,0.625,0.583,0.667
% 0.227,0.208,0.583,0.583,0.000,0.043,0.542,0.667,0.667,0.833
% \end{tabular}}
% \end{center}
% \end{table}
% \end{frame}
% ===============
% 0.382,0.379,0.530,0.651,0.121,0.134,0.724,0.750,0.809,0.826
% 0.224,0.172,0.560,0.616,0.134,0.151,0.720,0.716,0.750,0.788
% 0.267,0.151,0.543,0.530,0.073,0.138,0.677,0.685,0.698,0.744
% 0.398,0.307,0.539,0.530,0.078,0.091,0.608,0.707,0.748,0.782

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> plotdata/GPTJudgeForAPIType.tex <==
\newcommand{\typeheatmap}[1]{
\begin{tikzpicture}
  [scale=\ratio, every node/.style={transform shape}]
  \foreach \y [count=\n] in #1 {
    \foreach \x [count=\m] in \y {% heatmap tiles
      \pgfmathsetmacro{\colorpercentage}{100*\x}
      \pgfmathsetmacro{\xpos}{(\ratio * \m)}
      \node[fill=rred!\colorpercentage!bblue, minimum size=\cellsize, text=white] at (\xpos,-\n) {\x};
    }
  }
  % column labels
  \foreach \x [count=\m] in {SPARK*, SPARK, MINIMAX*, MINIMAX, ERNIE*, ERNIE, \textbf{GPT4*}, \textbf{GPT4}, GPT4*, GPT4} {
    \pgfmathsetmacro{\xpos}{(\ratio * \m)}
    \node[minimum size=\cellsize] at (\xpos, 0) {\tiny{\x}};
  }
  % row labels
  \foreach \a [count=\i] in {Tree, Tabular, JSON, YAML, XML, Markdown, ORG, LaTeX} {
    \node[minimum size=\cellsize] at (0,-\i) {\tiny{\a}};
  }
\end{tikzpicture}
}
\def\cellsize{11mm}
\def\ratio{1.1}
\begin{figure}
  \centering
  % \typeheatmap{{
  %   {0.227,0.292,0.125,0.208,0.042,0.042,0.375,0.542,0.375,0.417},
  %   {0.094,0.031,0.406,0.438,0.094,0.062,0.688,0.688,0.719,0.781},
  %   {0.650,0.400,0.875,0.775,0.150,0.200,0.800,0.850,1.000,1.000},
  %   {0.769,0.575,0.650,0.700,0.150,0.175,0.800,0.850,0.875,0.925},
  %   {0.652,0.636,0.625,0.583,0.042,0.083,0.708,0.833,0.875,0.917},
  %   {0.042,0.043,0.458,0.417,0.000,0.000,0.458,0.542,0.667,0.708},
  %   {0.208,0.125,0.333,0.292,0.042,0.000,0.208,0.500,0.565,0.435},
  %   {0.227,0.208,0.583,0.583,0.000,0.043,0.542,0.667,0.667,0.833},
  \resizebox{0.75\textwidth}{!}{%
\begin{tikzpicture}
\begin{axis}[
    width  = \textwidth,
    ymin=0,
    ymax=1,
    bar width=3pt,
    ybar=2*\pgflinewidth,
    symbolic x coords={Tree, Tabular, JSON, YAML, XML, Markdown, ORG, LaTeX},
    % ymajorgrids = true,
    % enlarge x limits=0.10,
    ylabel = {GPTJudge Acc.},
    xtick=data,
    % nodes near coords,
    % nodes near coords align={vertical},
    % nodes near coords/.append style={/pgf/number format/.cd,fixed,precision=10},
    legend style={
      at={(1.05,1.00)},
      anchor=north west,
      column sep=0.5ex}
]
\addplot[style={rred,fill=rred,mark=none}] coordinates {
(Tree,         0.227)
(Tabular,         0.094)
(JSON,         0.65)
(YAML,         0.769)
(XML,         0.652)
(Markdown,         0.042)
(ORG,         0.208)
(LaTeX,         0.227)
};
\addplot[style={rrred,fill=rrred,mark=none}] coordinates {
(Tree,         0.292)
(Tabular,         0.031)
(JSON,         0.4)
(YAML,         0.575)
(XML,         0.636)
(Markdown,         0.043)
(ORG,         0.125)
(LaTeX,         0.208)
};
\addplot[style={bblue,fill=bblue,mark=none}] coordinates {
(Tree,         0.125)
(Tabular,         0.406)
(JSON,         0.875)
(YAML,         0.65)
(XML,         0.625)
(Markdown,         0.458)
(ORG,         0.333)
(LaTeX,         0.583)
};
\addplot[style={bbblue,fill=bbblue,mark=none}] coordinates {
(Tree,         0.208)
(Tabular,         0.438)
(JSON,         0.775)
(YAML,         0.7)
(XML,         0.583)
(Markdown,         0.417)
(ORG,         0.292)
(LaTeX,         0.583)
};
\addplot[style={ppurple,fill=ppurple,mark=none}] coordinates {
(Tree,         0.042)
(Tabular,         0.094)
(JSON,         0.15)
(YAML,         0.15)
(XML,         0.042)
(Markdown,         0.0)
(ORG,         0.042)
(LaTeX,         0.0)
};
\addplot[style={pppurple,fill=pppurple,mark=none}] coordinates {
(Tree,         0.042)
(Tabular,         0.062)
(JSON,         0.2)
(YAML,         0.175)
(XML,         0.083)
(Markdown,         0.0)
(ORG,         0.0)
(LaTeX,         0.043)
};
\addplot[style={ggreen,fill=ggreen,mark=none}] coordinates {
(Tree,         0.375)
(Tabular,         0.688)
(JSON,         0.8)
(YAML,         0.8)
(XML,         0.708)
(Markdown,         0.458)
(ORG,         0.208)
(LaTeX,         0.542)
};
\addplot[style={gggreen,fill=gggreen,mark=none}] coordinates {
(Tree,         0.542)
(Tabular,         0.688)
(JSON,         0.85)
(YAML,         0.85)
(XML,         0.833)
(Markdown,         0.542)
(ORG,         0.5)
(LaTeX,         0.667)
};
\addplot[style={ccyan,fill=ccyan,mark=none}] coordinates {
(Tree,         0.375)
(Tabular,         0.719)
(JSON,         1.0)
(YAML,         0.875)
(XML,         0.875)
(Markdown,         0.667)
(ORG,         0.565)
(LaTeX,         0.667)
};
\addplot[style={cccyan,fill=cccyan,mark=none}] coordinates {
(Tree,         0.417)
(Tabular,         0.781)
(JSON,         1.0)
(YAML,         0.925)
(XML,         0.917)
(Markdown,         0.708)
(ORG,         0.435)
(LaTeX,         0.833)
};
% \addplot[red,sharp plot,update limits=false] coordinates { ([normalized]-1,1.0) ([normalized]9,1.0) };
\legend{SPARK*, SPARK, MINIMAX*, MINIMAX, ERNIE*, ERNIE, GPT4-turbo*, GPT4-turbo, GPT4*, GPT4}
\end{axis}
\end{tikzpicture}
}
\caption{API Test, Base Dataset. Prompt w/ Hint Eliciting in ~\autoref{fig:framework_hint} marked by *}
\label{fig:judgeapitype}
\end{figure}

% \begin{figure}
%   \centering
%   \typeheatmap{{
%     {0.273,0.083,0.000,0.083,0.000,0.000,0.250,0.500,0.250,0.333},
%     {0.062,0.000,0.438,0.438,0.125,0.062,0.625,0.812,0.625,0.750},
%     {0.600,0.200,0.800,0.700,0.050,0.100,0.850,0.900,1.000,1.000},
%     {0.789,0.550,0.750,0.750,0.150,0.150,0.850,0.950,0.900,1.000},
%     {0.667,0.818,0.667,0.667,0.083,0.000,0.667,1.000,0.917,0.917},
%     {0.000,0.091,0.333,0.333,0.000,0.000,0.333,0.417,0.583,0.583},
%     {0.083,0.083,0.333,0.250,0.000,0.000,0.083,0.417,0.417,0.333},
%     {0.100,0.250,0.417,0.417,0.000,0.091,0.500,0.583,0.500,0.750},
%   }}
% \caption{API Test, Base Dataset. Hard}
% \label{fig:judgeapitypehard}
% \end{figure}

% \begin{figure}
%   \centering
%   \typeheatmap{{
%     {0.182,0.500,0.250,0.333,0.083,0.083,0.500,0.583,0.500,0.500},
%     {0.125,0.062,0.375,0.438,0.062,0.062,0.750,0.562,0.812,0.812},
%     {0.700,0.600,0.950,0.850,0.250,0.300,0.750,0.800,1.000,1.000},
%     {0.750,0.600,0.550,0.650,0.150,0.200,0.750,0.750,0.850,0.850},
%     {0.636,0.455,0.583,0.500,0.000,0.167,0.750,0.667,0.833,0.917},
%     {0.083,0.000,0.583,0.500,0.000,0.000,0.583,0.667,0.750,0.833},
%     {0.333,0.167,0.333,0.333,0.083,0.000,0.333,0.583,0.727,0.545},
%     {0.333,0.167,0.750,0.750,0.000,0.000,0.583,0.750,0.833,0.917},
%   }}
% \caption{API Test, Base Dataset. Simple}
% \label{fig:judgeapitypesimple}
% \end{figure}

% \heatmap{GPTJudge Acc}


% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for Tree }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.625,0.667,0.417,0.458,0.083,0.208,0.417,0.542,0.625,0.542
% 0.125,0.083,0.167,0.167,0.000,0.000,0.250,0.292,0.375,0.458
% 0.125,0.000,0.167,0.417,0.000,0.000,0.458,0.125,0.208,0.375
% 0.227,0.292,0.125,0.208,0.042,0.042,0.375,0.542,0.375,0.417
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for SQL }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.031,0.000,0.438,0.500,0.156,0.219,0.688,0.688,0.750,0.875
% 0.188,0.000,0.344,0.406,0.031,0.094,0.719,0.781,0.500,0.656
% 0.000,0.000,0.250,0.188,0.094,0.125,0.469,0.406,0.406,0.625
% 0.094,0.031,0.406,0.438,0.094,0.062,0.688,0.688,0.719,0.781
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for JSON }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.300,0.300,0.800,0.900,0.175,0.125,0.925,0.875,0.950,0.950
% 0.550,0.425,0.825,0.775,0.150,0.325,0.875,0.825,0.950,0.975
% 0.050,0.000,0.350,0.325,0.150,0.075,0.500,0.600,0.475,0.550
% 0.650,0.400,0.875,0.775,0.150,0.200,0.800,0.850,1.000,1.000
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for YAML }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.641,0.625,0.750,0.825,0.175,0.050,0.825,0.925,0.925,0.975
% 0.325,0.075,0.675,0.625,0.125,0.325,0.900,0.875,0.950,0.950
% 0.125,0.075,0.250,0.375,0.050,0.000,0.575,0.450,0.425,0.650
% 0.769,0.575,0.650,0.700,0.150,0.175,0.800,0.850,0.875,0.925
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for XML }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.917,0.667,0.458,0.625,0.167,0.167,0.667,0.750,0.833,0.875
% 0.458,0.417,0.792,0.667,0.167,0.125,0.875,0.708,0.875,0.833
% 0.435,0.333,0.292,0.667,0.042,0.125,0.417,0.667,0.292,0.583
% 0.652,0.636,0.625,0.583,0.042,0.083,0.708,0.833,0.875,0.917
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for Markdown }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.167,0.417,0.292,0.542,0.042,0.125,0.667,0.667,0.783,0.652
% 0.167,0.083,0.458,0.542,0.042,0.000,0.542,0.625,0.542,0.652
% 0.389,0.067,0.167,0.292,0.000,0.000,0.417,0.500,0.375,0.417
% 0.042,0.043,0.458,0.417,0.000,0.000,0.458,0.542,0.667,0.708
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for ORG }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.125,0.125,0.333,0.542,0.000,0.083,0.667,0.750,0.708,0.750
% 0.042,0.000,0.375,0.500,0.000,0.000,0.375,0.500,0.542,0.500
% 0.231,0.250,0.167,0.208,0.000,0.000,0.333,0.292,0.375,0.625
% 0.208,0.125,0.333,0.292,0.042,0.000,0.208,0.500,0.565,0.435
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}
% % \begin{frame}
% % \begin{table}[htbp!]
% % \caption{GPT Judge for LaTeX }
% % \begin{center}
% % \resizebox{\textwidth}{!}{
% % \begin{tabular}{r|lllllllllll}
% % \multicolumn{1}{c}{\bf Benchmark}&\multicolumn{1}{c}{\bf spark engi}&\multicolumn{1}{c}{\bf spark base}&\multicolumn{1}{c}{\bf minimax engi}&\multicolumn{1}{c}{\bf minimax base}&\multicolumn{1}{c}{\bf baidu erniebot turbo engi}&\multicolumn{1}{c}{\bf baidu erniebot turbo base}&\multicolumn{1}{c}{\bf gpt4xhs engi}&\multicolumn{1}{c}{\bf gpt4xhs base}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo engi}&\multicolumn{1}{c}{\bf gpt4xhs base non turbo base}
% % \\\hline
% 0.250,0.250,0.458,0.583,0.083,0.125,0.750,0.625,0.750,0.792
% 0.083,0.042,0.500,0.375,0.000,0.000,0.583,0.625,0.583,0.667
% 0.471,0.333,0.417,0.667,0.000,0.000,0.750,0.750,0.708,0.708
% 0.227,0.208,0.583,0.583,0.000,0.043,0.542,0.667,0.667,0.833
% % \end{tabular}
% % }
% % \end{center}
% % \end{table}
% % \end{frame}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/00.Checklist.tex <==

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Sec.~\ref{sec:intro}}
  \item Did you describe the limitations of your work?
    \answerYes{See Sec.~\ref{sec:limitation}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Sec.~\ref{sec:ethical}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{See Sec.~\ref{sec:ethical}}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Sec.~\ref{sec:datasetconstr}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sec.~\ref{sec:setup} and Sec.~\ref{ap:setting}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Sec.~\ref{ap:setting}}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Sec.~\ref{ap:setting}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Sec.~\ref{sec:setup}}
  \item Did you mention the license of the assets?
    \answerYes{See Sec.~\ref{sec:setup}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See \url{https://github.com/YHN-ice/StructBench}}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See Sec.~\ref{sec:datasetconstr}}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Sec.~\ref{sec:ethical}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Sec.~\ref{ap:manual}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerYes{See Sec.~\ref{ap:manual}}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See Sec.~\ref{ap:manual}}
\end{enumerate}

\end{enumerate}

==> texs/02.RelatedWork.04.tex <==
\begin{figure*}[t]

\centering
\fontsize{9pt}{8.6pt}\selectfont
  \begin{forest}
    for tree={
      align=center,
      % font=\sffamily,
      edge+={thick, -{Stealth[]}},
      l sep'+=10pt,
      fork sep'=10pt,
    },
    forked edges,
    if level=0{
      inner xsep=0pt,
      tikz={\draw [thick] (.children first) -- (.children last);}
    }{},
    [Structure-Rich Texts
      % [Abstract Data Structure [Tree]]
      [Structured Data 
      [Tabular [CSV]]
      [Tree [Custom Language]]]
      [Semi-Structured Data
        [Object Notation
          [JSON]
          [YAML]
          [XML]
        ]
        [Markup Language
          [Markdown]
          [LaTeX]
          [Org]
        ]
      ]
    ]
  \end{forest}
  
\caption{Taxonomy of Structure-Rich Texts covered in StrucText-Eval.}
\label{fig:taxonomy}
\vspace{-5mm}
\end{figure*}


\subsection{Structural Text Understanding Enhanced Models}

Previous explorations over structural information focused on tasks related to programming languages and graphs. 
\cite{mou2016convolutional} built a tree-based convolutional neural network that outperformed language models on functionality classification tasks and pattern detection tasks over programming languages. % functionality classification, pattern detection
\cite{wang2020detecting} outperformed state of the art~(SOTA) on code clone detection benchmarks, applying graph neural networks on abstract syntax trees~(ASTs) representation augmented by control and data flow edges, which is different in architecture from language models curated for natural language tasks. 
\cite{zhou2019devign} built a graph neural network over rich node representations of code and gained SOTA on vulnerability identification in 4 large-scaled open-source C projects. 
\cite{perozzi2024let} proposed a dedicated graph neural network~(GNN) to encode graph into embedding space of LLMs, and used LLMs as an decoder to solve the graph tasks in GraphQA~\cite{fatemi2023talk}.
\cite{chen2023exploring} explored LLMs' potential in learning graphs, focusing on node classification tasks, using LLMs as enhancers for GNN predictor and directly as predictor.
\cite{chen2024beyond} disclosed the employment of formats other than natural language in CoT reasoning and multi-agent communication significantly enhances model performance while also decreasing token usage on reasoning tasks.


\subsection{Structural Text Understanding Evaluation Datasets}

The similar datasets dedicating to structure information understanding are scarce.
GraphQA~\cite{fatemi2023talk} is a benchmark for assessing LLMs on reasoning over graph data, composed of 7 simple graph tasks, with exploration on methods in encoding graph-structured data as text.
Struc-Bench~\cite{tang2023struc} collect data from open source to evaluate if LLM can generate complex structured tabular text.
\cite{sui2024table} consists of 8 tasks on table-formatted input texts, i.e., input data organized in row-column structures, with studying in input design and prompt enhancement.
\cite{pasupat2015compositional} exposed a dataset of 22,033 complex questions on Wikipedia tables and proposed a parsing algorithm for answering complex questions on semi-structured tables.
For tabular data, \cite{SHWARTZZIV202284} showed that deep models were not a good solution; \cite{NEURIPS2021_9d86d83f} designed two specialized baseline architecture for tabular data and concluded that universally superior solution does not exist.
\cite{wang2024can} is another graph-based problem solving benchmark, with graph structure described with natural language.
\cite{fatemi2023talk} and \cite{sui2024table} include comparison of encoding methods for structure information, i.e., graphs and tables, respectively, showing that LLMs performance varies on different encodings and the relatively vacancy on LLM's understanding of structure-rich texts input.


Our dataset diverges from previous work in two significant ways.
Firstly, our tasks exclusively concentrate on analyzing structural information and executing dependent inference, unlike prior approaches~\cite{mou2016convolutional, zhou2019devign} that employ structural data primarily as an auxiliary tool for classification or semantic comprehension.
StrucText-Eval focus on symbolic structure by erasing content semantics from input texts, preserving only structural details, which renders the texts semantically obscure and the tasks semantically agnostic.
Secondly, our benchmark extends beyond traditional graph reasoning and table information retrieval to include a broader spectrum of structure-rich text types.
It also incorporates comprehensive structure-based inference tasks that are tailored to specific input formats.


==> texs/02.RelatedWork.05.tex <==
\begin{figure*}[t]

\centering
\fontsize{9pt}{8.6pt}\selectfont
  \begin{forest}
    for tree={
      align=center,
      % font=\sffamily,
      edge+={thick, -{Stealth[]}},
      l sep'+=10pt,
      fork sep'=10pt,
    },
    forked edges,
    if level=0{
      inner xsep=0pt,
      tikz={\draw [thick] (.children first) -- (.children last);}
    }{},
    [Structure-Rich Texts
      % [Abstract Data Structure [Tree]]
      [Structured Data 
      [Tabular [CSV]]
      [Tree [Custom Language]]]
      [Semi-Structured Data
        [Object Notation
          [JSON]
          [YAML]
          [XML]
        ]
        [Markup Language
          [Markdown]
          [LaTeX]
          [Org]
        ]
      ]
    ]
  \end{forest}
  
\caption{Taxonomy of Structure-Rich Texts covered in StrucText-Eval.}
\label{fig:taxonomy}
\vspace{-5mm}
\end{figure*}

\subsection{Structural Text Understanding Enhancements}

Recent efforts to enhance LLMs have focused on integrating external structures such as graphs, tool flows, and cross-domain representations to improve reasoning capabilities across various tasks.
For instance, ControlLLM utilizes tool graphs to decompose complex multimodal tasks, resulting in enhanced performance on image and audio processing tasks by leveraging the topological dependencies of tools \cite{1.pdf}.
Graph-based models like GraphGPT and BooG have shown promising results, with the former improving generalization across node classification and molecular tasks via graph instruction tuning \cite{7.pdf, 14.pdf}, while the latter employs virtual supernodes to unify graph structures across domains, fostering cross-domain task transferability \cite{2.pdf}.
Additionally, methods like RC2R demonstrate the effective combination of knowledge graphs and LLMs for domain-specific causal reasoning, particularly in financial risk propagation tasks \cite{4.pdf}.
These advancements highlight the benefits of embedding structural elements—ranging from graph architectures to domain-specific knowledge graphs—within LLM frameworks to improve task-specific inference and reasoning.

\subsection{Structural Text Understanding Evaluation}

Evaluating LLMs' ability to understand structured data has become increasingly critical, though benchmarks remain limited. GraphQA and Struc-Bench are key datasets that assess LLMs' reasoning over graph-structured data and tabular text, respectively, illustrating the models' varying capabilities based on input encoding \cite{fatemi2023talk, tang2023struc}.
More specialized benchmarks, such as TEMPTABQA, evaluate temporal reasoning in tabular data, while TableLLM tests LLMs' proficiency in handling complex document-based table manipulation tasks \cite{12.pdf, 20.pdf}. Other works, such as the evaluation of knowledge graph-based reasoning in complex time-series QA systems (JMFRN) \cite{5.pdf}, and privacy-oriented graph tasks in GHRatio \cite{3.pdf}, further explore how LLMs handle intricate, structure-rich information, shedding light on their performance across different structured data formats.


Our work diverges from prior research by focusing exclusively on structure-based inference, deliberately removing semantic content to challenge LLMs to reason purely from structural patterns. Unlike previous approaches that use structural data as supplementary input for classification or semantic tasks \cite{pasupat2015compositional, sui2024table}, we design tasks that are semantically agnostic, requiring models to infer meaning solely from symbolic structures. Moreover, while earlier benchmarks emphasize graph reasoning or tabular information retrieval, our work extends to a broader spectrum of structure-rich text types, encompassing a wider variety of input formats and more complex dependency-based inference tasks.

% \subsection{Structural Text Understanding Enhanced Models}
% Existing research on enhancing LLMs with structural understanding spans several domains, primarily focusing on improving LLMs' ability to handle tasks related to graph-structured data and structured reasoning.

% One prominent approach involves augmenting LLMs with external tools or structures.
% Frameworks like ControlLLM leverage tool graphs for complex multimodal tasks, effectively breaking down tasks into subproblems and enhancing LLMs' reasoning through structured topologies \cite{1.pdf}. 
% Models like GraphGPT use graph-based instruction tuning to refine LLMs' understanding of graph data, improving their generalization across tasks such as node classification and molecular data analysis \cite{7.pdf, 14.pdf}.
% Another significant line of research introduces new representations of graph structures, such as the use of virtual supernodes in BooG models, which facilitate cross-domain graph tasks by unifying structural patterns \cite{2.pdf}.
% Efforts to enhance task-specific capabilities, such as financial risk inference (RC2R), combine knowledge graphs with causal reasoning to aid in complex decision-making processes \cite{4.pdf}. This highlights the increasing trend of integrating external domain-specific structures, like financial knowledge graphs, to improve LLM performance across various fields.

% These advancements illustrate that incorporating structural elements, whether through external graphs, graph-based pretraining, or structured task formats, significantly boosts LLMs' performance across domains like programming, molecular science, and financial analysis \cite{mou2016convolutional, wang2020detecting, zhou2019devign}.

% \subsection{Structural Text Understanding Evaluation Datasets}
% The development of evaluation benchmarks tailored to assessing LLMs' understanding of structured data has also progressed significantly, though such datasets remain relatively scarce compared to natural language benchmarks. One of the earliest efforts, GraphQA, evaluates LLMs' reasoning over graph data using simple graph tasks, while later benchmarks, such as Struc-Bench, broaden the scope to complex structured tabular text \cite{fatemi2023talk, tang2023struc}. These datasets explore how well LLMs encode and reason about structure-rich information, showing variations in performance based on different encoding techniques.

% More recent efforts, such as TableLLM and TEMPTABQA, push the boundaries of structured reasoning by introducing time-sensitive tasks and document-level table manipulation challenges \cite{20.pdf, 12.pdf}. These works emphasize the need for robust handling of structured inputs beyond traditional graphs and tables, incorporating more intricate data sources like knowledge graphs, semi-structured tables, and even hybrid data formats.

% Our work diverges from these earlier benchmarks by focusing exclusively on structural information, removing semantic content to challenge LLMs' ability to infer solely from structural patterns. This positions our dataset as distinct from prior approaches, which predominantly utilize structural data as an auxiliary feature for tasks like classification or question answering \cite{pasupat2015compositional, sui2024table}. Our tasks emphasize symbolic structures, requiring models to perform semantically agnostic reasoning, which has not been extensively addressed in the current body of research.


% \subsection{Structural Text Understanding Enhanced Models}

% Previous explorations over structural information focused on tasks related to programming languages and graphs. 
% \cite{mou2016convolutional} built a tree-based convolutional neural network that outperformed language models on functionality classification tasks and pattern detection tasks over programming languages. % functionality classification, pattern detection
% \cite{wang2020detecting} outperformed state of the art~(SOTA) on code clone detection benchmarks, applying graph neural networks on abstract syntax trees~(ASTs) representation augmented by control and data flow edges, which is different in architecture from language models curated for natural language tasks. 
% \cite{zhou2019devign} built a graph neural network over rich node representations of code and gained SOTA on vulnerability identification in 4 large-scaled open-source C projects. 
% \cite{perozzi2024let} proposed a dedicated graph neural network~(GNN) to encode graph into embedding space of LLMs, and used LLMs as an decoder to solve the graph tasks in GraphQA~\cite{fatemi2023talk}.
% \cite{chen2023exploring} explored LLMs' potential in learning graphs, focusing on node classification tasks, using LLMs as enhancers for GNN predictor and directly as predictor.
% \cite{chen2024beyond} disclosed the employment of formats other than natural language in CoT reasoning and multi-agent communication significantly enhances model performance while also decreasing token usage on reasoning tasks.


% \subsection{Structural Text Understanding Evaluation Datasets}

% The similar datasets dedicating to structure information understanding are scarce.
% GraphQA~\cite{fatemi2023talk} is a benchmark for assessing LLMs on reasoning over graph data, composed of 7 simple graph tasks, with exploration on methods in encoding graph-structured data as text.
% Struc-Bench~\cite{tang2023struc} collect data from open source to evaluate if LLM can generate complex structured tabular text.
% \cite{sui2024table} consists of 8 tasks on table-formatted input texts, i.e., input data organized in row-column structures, with studying in input design and prompt enhancement.
% \cite{pasupat2015compositional} exposed a dataset of 22,033 complex questions on Wikipedia tables and proposed a parsing algorithm for answering complex questions on semi-structured tables.
% For tabular data, \cite{SHWARTZZIV202284} showed that deep models were not a good solution; \cite{NEURIPS2021_9d86d83f} designed two specialized baseline architecture for tabular data and concluded that universally superior solution does not exist.
% \cite{wang2024can} is another graph-based problem solving benchmark, with graph structure described with natural language.
% \cite{fatemi2023talk} and \cite{sui2024table} include comparison of encoding methods for structure information, i.e., graphs and tables, respectively, showing that LLMs performance varies on different encodings and the relatively vacancy on LLM's understanding of structure-rich texts input.


% Our dataset diverges from previous work in two significant ways.
% Firstly, our tasks exclusively concentrate on analyzing structural information and executing dependent inference, unlike prior approaches~\cite{mou2016convolutional, zhou2019devign} that employ structural data primarily as an auxiliary tool for classification or semantic comprehension.
% StrucText-Eval focus on symbolic structure by erasing content semantics from input texts, preserving only structural details, which renders the texts semantically obscure and the tasks semantically agnostic.
% Secondly, our benchmark extends beyond traditional graph reasoning and table information retrieval to include a broader spectrum of structure-rich text types.
% It also incorporates comprehensive structure-based inference tasks that are tailored to specific input formats.


==> texs/031.Method.tex <==
我们提出SumShot来增强大语言模型对于结构化数据理解的能力。
SumShot的思路来源于对训练数据、或者其他类型的标注数据的总结，并将总结用于下游的推理过程中。

目前有其他工作也使用LLM来总结已有内容，从而进行Inductive Reasoning。
如图~\ref{}所示，SumShot的特点在于，对于复杂的问题，可以通过总结简单的few-Shot，从而在推理时以更少量的token达到较好的效果。
更进一步，SumShot可以通过总结若干不同的Demonstraion，从而在推理时可以以相同量的token包含很多的信息，从而得到更好的效果。


==> texs/04.ExperimentSetup.04.tex <==
To evaluate LLMs' current capability of processing structure-rich text and executing dependent inference, we conducted a series of experiments using StrucText-Eval in various settings.
Our study utilizes both prompt-based and finetuning methods to analyze the performance variations.




\subsection{Models}

We tested six Open-Source LLMs in both StrucText-Eval Test and Test-Hard Suite, we use the short name (in the bracket) of these LLMs in the experiments:
\textbf{Qwen/Qwen2-7B-Instruct} (Qwen-2-7B),
\textbf{Qwen/Qwen2-72B-Instruct} (Qwen-2-72B),
\textbf{meta-llama/Meta-Llama-3.1-8B-Instruct} (Llama-3.1-8B),
\textbf{meta-llama/Meta-Llama-3.1-72B-Instruct} (Llama-3.1-70B),
\textbf{meta-llama/Meta-Llama-3.1-405B-Instruct}  (Llama-3.1-405B),
\textbf{mistralai/Mistral-7B-Instruct-v0.2} (Mistral-0.2-7B)

Considering the huge expense in using API-based model, we only tested six Close-Source LLMs in StrucText-Eval-Hard:
% \textbf{o1-preview-2024-09-12} (o1-preview),
% \textbf{o1-mini-2024-09-12} (o1-mini),
\textbf{gpt-4o-2024-08-06} (gpt-4o),
\textbf{gpt-4o-mini-2024-07-18} (gpt-4o-mini),
\textbf{gemini-1.5-pro}(gemini-1.5-pro),
\textbf{gemini-1.5-flash}(gemini-1.5-flash),
\textbf{GLM-4-Plus} (glm-4-plus),
\textbf{GLM-4-Flash} (glm-4-flash).

% The prompt and the setting of all llms are listed in Appendix~\ref{ap:setting}



% We tested five Close-Source LLMs accessed through public APIs: \textbf{GPT4}, \textbf{GPT4 Turbo}, \textbf{MINIMAX}, \textbf{SPARK}, and \textbf{ERNIE}.
% Besides these API-Based models, we also finetuned \textbf{Llama-7B-v1} under several conditions with partially frozen parameters.
% The API calling and finetuning setting is listed in Appendix~\ref{ap:setting}.




\subsection{Prompt-based Method}
We also evaluated the impact of different prompt designs on the performance of LLMs by utilizing six distinct prompt configurations in the main experiments.
% Additional prompt methods are provided in Table~\ref{tab:other_metrics} in the Appendix, and the 
Detailed implementation of these prompts can be found in Sec.~\ref{ap:prompt} in the Appendix.
The six primary prompt settings are as follows:

\texttt{\textbf{Naive}}: This configuration involves a straightforward input of ``Context'', ``Question'', and ``Options'' into the LLMs to generate responses.
\texttt{\textbf{Self-Chain-of-Thought (Self-CoT)}}~\cite{kojima2022large}: This approach incorporates a step-by-step reasoning prompt to guide the model through logical reasoning.
\texttt{\textbf{Plan-and-Solve CoT (PS-CoT)}}~\cite{wang2023plan}: This method emphasizes problem decomposition before solving, encouraging the model to first break down the problem before generating a solution.
\texttt{\textbf{With Hint (w/ hint)}}: In this setting, manually curated hints are provided to the model to observe its performance when additional information is injected. 
Since this approach introduces supplementary data, it is delineated by a dashed line from other methods in Table~\ref{tab:api_overall}.
\texttt{\textbf{Few-Shot Demonstration}}: involves appending few training data directly to the prompt. 
The \texttt{\textbf{Simple Few-Shot Demonstration}}: uses only the shortest examples from the training set as few-shot demonstrations.


% We assessed the influence of prompt design on LLM performance by employing four distinct prompt settings in the main content, and some other prompt method can be found in Tab.~\ref{tab:more_experiment} in the Appendix. and the detailed implementation of these prompts can be found in Tab.~\ref{tab:prompt} in the Appendix.
% \texttt{\textbf{Naive}}, which simply inputs ``Context'', ``Question'', and ``Options'' into LLMs for answers.
% \texttt{\textbf{Self-Chain-of-Thought}} (Self-CoT)~\cite{kojima2022large}, applying a step-by-step reasoning prompt.
% \texttt{\textbf{Plan-and-Solve CoT (PS-CoT)}}~\cite{wang2023plan}, focusing on problem deconstruction before solution.
% \texttt{\textbf{With Hint (w/ hint)}}, 主要是将人工总结的提示注入给模型，观察模型的表现结果。考虑到这个方法注入了额外的信息，所以表~\ref{tab:api_overall}中用额外的虚线与其他方法进行分割

% 在图~\ref{plot}和表~\ref{}中，我们还使用了Few-Shot Demontration。
% 这个方法是将训练集中的数据直接拼接到Prompt里。
% 其中Simple Few-Shot Demonstration只使用了训练集中长度最短的数据用作Demonstraion。


\subsection{Evaluation Method}
We use the RougeL metric~\cite{lin2004rouge} to assess the degree of character-level similarity between model outputs in the main content of this paper.
In certain cases, the task requires the LLM to generate the entire reasoning path leading to the answer, which result in high RougeL scores.
So we assign a score of 0 if the RougeL score falls below 0.75.

Additionally, we present the results of other evaluation metrics, including LLM-as-Judge-Score~\cite{zheng2023judging}, BLEU~\cite{papineni2002bleu}, and Exact Match, in Tab.~\ref{tab:other_metrics} in the appendix.
Furthermore, we conduct a consistency analysis across these metrics in comparison with human judgments, as shown in Fig.~\ref{fig:cor_metrics}.




==> texs/07.App.Statistics.01.tex <==

The detailed statistic information about StrucText-Eval is illustrated in Tab.~\ref{tab:statistic}.

\input{benchmark_statistic}



% \subsection{Experimental Data}
% \input{./data_tabs.tex}


% \subsection{Comparation on GPT Judged Accuracy of LLMs}\label{ap:bargraphs}
% \input{bargraph.tex}
% \input{plotdata/GPTJudgeForAPIDetailed.tex}
% \subsection{Sample of Input and Tasks}\label{ap:samples}
% \input{./input_sample.tex}




==> texs/12.App.DetailEvaluation.01.tex <==


% The Exact Match~(EM) Score is illustrated in Tab.~\ref{tab:em_api_overall}.
The RougeL Score is illustrated in Tab.~\ref{tab:rougel_api_overall}.


% \input{performance_EM_tables}
\input{performance_RougeL_tables}

==> texs/old_version/01.Introduction.02.tex <==
The landscape of machine learning and artificial intelligence is rapidly transforming with the emergence of intelligent agents acting as information middleware.
These agents, often tasked with executing commands on behalf of humans, operate within a milieu dominated by machine-generated texts.
Machine-generated texts, which serve as carriers for data flow between programs, are typically stored, transmitted, and processed in formats rich in structure formed by tags and mark-ups.
This paradigm shift necessitates a profound understanding of Large Language Models’ (LLMs) capabilities in processing and interpreting structure-rich texts.
Our study introduces an innovative benchmark designed to evaluate LLMs’ proficiency in this realm, marking a significant stride in the field of structured text processing and knowledge inference.

Firstly, the advent of intelligent agents as intermediaries in information processing underscores the critical need for LLMs to adeptly handle texts generated by machines, which are often structured and require nuanced understanding for effective machine-to-machine communication.

Secondly, there is a discernible gap in the existing benchmarks and datasets concerning the diversity and complexity of structured texts.
Traditional datasets are predominantly centered around codebases and fail to fully represent the intricate structures prevalent in texts intended for machine comprehension.

The rapid increase in complex, structured texts necessitates a dedicated benchmark for evaluating machines' ability to understand and generate such content. This benchmark addresses a critical gap in current methodologies, catering to the evolving needs of machine-to-machine communication and structured data processing.

The primary goal of our research is to build a benchmark evaluating LLMs in the context of texts integral to intelligent agents’ workflows.
We assess model capabilities by posing questions based on structured text inputs that are syntactically correct but semantically null and void, imposing a challenge for models in discerning structure for meaning.
We conducted assessment on a range of LLMs, and compared their performance on different categories of tasks.
Furthermore, we fine-tuned 3 models with our datasets in hope of enhanced machine comprehension on structured texts.

We searched vastly structured texts that have well-documented syntax and are widely used in industry and academies, e.g., JSON, YAML, LaTeX.
We include both fully-structured and half-structured data to enrich the diversity of our dataset.
For each class of texts, we designed 3-5 tasks that are structure-related, some of which are specific to their classification.

Based on the syntax and rules for construction, we randomly generate the input texts, and procedurally generate the corresponding tasks data in the meantime.

% 人类为什么会需要使用结构化的表达？【往逻辑表达和规则那里去靠】
% 理解结构化的表达对于LLM意味着什么？【理解结构化的形式、更清晰的人类逻辑，以及人类规则】

% 结构化的文字表达方式是人类进行逻辑表达和规则理解的重要工具，它能够提升思想的清晰度和准确度，同时也有助于规则的明确和遵守。简言之，这种表达方式对于有效的沟通、理解和合作具有至关重要的作用。

人类使用结构化的文字表达方式，旨在清晰、准确地表达思想和观点，以及理解和应用逻辑规则。
这些结构化的文字表达方式，因为包含了严格的语法规则，所以可以通过严格且清晰的逻辑来帮助其他人理解表达的内容。
例如，文章的段落结构和特定的文本结构如Markdown，可以帮助作者按照一定的逻辑顺序呈现信息，使读者更容易理解作者的观点和论据。

评估大语言模型（LLM）理解结构化文字表达的能力，对于其准确理解和回应用户请求具有重要意义。
这包括LLM对自然文本逻辑表达的理解能力，以及对自然文本中的规则，包括语法规则和社会文化规则的理解能力。
这种评估可以揭示LLM的能力和限制，为其持续改进和优化提供依据，以更好地服务于人类社会。

目前的语言模型在结构化文本的理解上有哪些缺陷？
这些缺陷的本质是源于模型对于结构形式的理解和规则的理解不足。
评估和改善这些缺陷非常重要。

为了有效地评估这些缺陷，我们设计了Structure-Rich Text Benchmark。
如表~\ref{sample-table}所示，我们的Benchmark中包含了xxx个任务。
针对每个具体的任务，我们都设计了一个能够根据一定的规则自动化生成结构数据的方法。
每条规则包含了xxx和xxx，以及xxx。
每个任务平均有xxx个规则，然后将这些规则进行随机组合，并生成最后benchmark的数据。

同时为了有效地改善这些缺陷，我们做了怎样的训练。
我们利用了课程学习的思想，将规则的描述和使用规则的描述进行组合，并输入给模型进行训练。
同时，我们还要求模型能够为每个sample生成合理的解释。
通过这样的方式，LLM不仅能够理解格式化文本，更能够理解格式化文本背后所表示的逻辑和规则。

最后，根据我们的评估结果，我们发现xxxx。

\subsection{Contribution}
\begin{itemize}
    \item We first thoroughly evaluated the LLMs' ability to understand and manipulate structure-rich texts.
	\item We present a taxonomy for structured texts and designed structure-related tasks for each class.
	\item With a total of 8 text classes and 3-5 tasks for each class, we present 29 structure-specific tasks and 580 samples for our benchmark dataset.
	\item We also tested 4 LLMs and present the results under different metrics for assessment.
\end{itemize}


需要写的内容
1. 目前LLM在理解结构化文本上的缺陷
2. Benchmark是如何构建
    Tree
    Tabular
    Json
    YAML
    XML
    MarkDown
    Org
    Latex
    - Input
    - Output
    - Instruction
    - Explanation
3. 如何增强LLM对于结构化文本的理解能力
    - 课程学习怎么搞
    - Explanation怎么弄
    - 其他的一些小trick
4. 实验结果
    - Overall Experiments
        - API-based 大模型在benchmark上的效果
        - open source LLM在benchmark上的效果
        - 拿benchmark直接train出来的模型的效果
        - 我们方法train出来的LLM在benchmark上的效果
    - Detailed Experiments
        - Few shot Demonstration的测试结果
        - 保证OOD设定下的测试结果
        - Model Performance和xxx之间的关系：
            - Input Length
            - 
    - Case Study
        - 不同大模型生成的case以及explanation
        - 



==> texs/old_version/01.Introduction.03.tex <==
% GOTO Intro
\gzh{I reformalize the background of your paper, the first three paragraphs may be stored into another tex file, but don't need to show up in Intro any more.
You need to fill the blue text in the following content.
btw, you may read the introduction of our paper: DetectBench.
You may borrow the structure of Introduction in DetectBench.%\url{https://www.overleaf.com/7951644528gcrgjdgpsqfv#0adf4f}
}


Deep neural networks, as a modern implementation of the connectionist approach, are well suited for natural language processing, where probabilistic language models are prominent~\citep{thomas2008connectionist, bengio2000neural}.
In contrast, symbolism represents another facet of artificial general intelligence~(AGI), arguing that symbolic thought is essential for human beings to ``generalize most broadly''~\citep{goertzel2014artificial}.
Given the contrasting paradigms of AGI, investigating how deep learning models can adapt to symbolic computation is a critical challenge.
This touches on the fundamental question of whether probabilistic models for stochastic tasks can effectively manage the systematic and deterministic reasoning necessary for symbolic manipulation and processing.
Text structured as Tree, Table, JSON, YAML, XML, Markdown, LaTeX and Org formats consists of formation and inference rules that express logical relationships more unambiguously compared to natural languages.
These structures represent a less rigorous form of the symbol systems mentioned above and serve as an ideal medium for evaluating the problem.

Structure-rich text\footnote{structure-rich text and structured text are used interchangeably hereafter} also serves as a key component of a series of web services, e.g., REST, JSON-RPC, XML-bsed data exchange protocol~(e.g., SOAP), and service process definition language(e.g., WSDL), of higier-order services that utilize disparate inter-operating services to automate complex tasks, e.g., travel planning and advanced information retrieval~(\citet{masse2011rest, 8385157, 8603059, de2013eve, box2000simple, christensen2001web, samsel2013web, papazoglou2004survey, dustdar2005survey, 8603059}).
Additionally, structured texts is critical for the functionality of web-based agents that operating across diverse host platforms and languages, frequently encountering data from a wide array of sources presented in structure-rich text, a diversity stemming from varied communication protocols, with Retrieval-Augmented Generation (RAG) being a typical example~(\citet{8603059, de2013eve, lewis2020retrieval}).

\gzh{This paragraph should talk about: Why Structured Text is important.
However, I think ``Formal System'' and ``Web-Based Intelligent Agents'' is not sharp enough.
Can you write some thing else to stress that Structured Text is important.}
\yhn{Formal system and web-based agents are the best justification I can think of.}

Large Language Models (LLMs) have demonstrated exceptional capability across various natural language tasks, e.g., question answering, information retrieval, summarization, sentiment analysis, and toxicity detection~\citep{liang2022holistic}. \gzh{LLM is powerfull} \yhn{added examples from HELM}

For discerning the use of terminology in this work, a task is decomposed as three parts, {\color{red}input texts}, {\color{blue} instruction/question}, and {\color{cyan}answer} as following.
\begin{quote}
  \texttt{user:}

  \quad {\color{blue} Summarize this article:}

  \quad {\color{red}A long time ago, there is a fox ...}

  \texttt{AI:}

  \quad {\color{cyan} This article is about ...}
\end{quote}

% However, their proficiency in interpreting structured texts remains less understood.
\gzh{LLM fall short in structured text understanding + What is structured text} \yhn{What is strucutred text is answered in the first paragraph. The ``fall-short'' is merged to the following sentence.}

As probabilistic models, LLMs excel in processing the stochastic nature of natural language by predicting token sequences, but their effectiveness in symbolic computation based on strict rules and logical relationships is still an open question as stated above~\citep{bengio2000neural, ney1994structuring}. \gzh{Why LLM cannot handle this task?} \yhn{callback to the first paragraph, added reference to language model being probabilistic}


% Existing benchmarks, such as those introduced by Fatemi et al. (2023) and Sui et al. (2024), primarily cater to natural language inputs or a constrained selection of structured input types, notably graphs or tables. This limitation misaligns with the real-world applications and the extensive array of structure-rich text types encountered by Large Language Models (LLMs). Furthermore, current methodologies leverage structural information through the creation of task-specific input designs or architectures, as noted by Perozzi et al. (2024) and Sui et al. (2024), yet this strategy may not fully capture the complexity or diversity of real-world structured data.

Existing benchmarks, such as those presented by \cite{fatemi2023talk, perozzi2024let, sui2024table}, predominantly focus on natural language inputs or provide a limited array of structured input text, which primarily centered around graphs or tables. \gzh{Is this the only shortcommings of other works?}. \yhn{another added at the end of this paragraph.}
This limited structure diversity diverges from \sout{the real-world applications\gzh{Why?} \yhn{Deleted} of Large Language Models (LLMs) and} the diverse, structure-rich text used in office environments, such as Markdown and LaTeX, thereby offering a skewed representation of practical LLM use cases.
As a consequence of limited scope, they leave the symbolic, semantically agnostic nature shared by these structured texts untouched, which is emphasize by erasing content semantics through randomized generation method discussed immediately.
Besides dataset, current methods cope with structural tasks by developing task-specific input designs or model architectures~(\cite{perozzi2024let, sui2024table}), leading to an specific dependent approach with limited generalizability.

\gzh{I don't read the following Introduction, for it seems unfinished.}


In response, we introduce the \textbf{\textit{Struct}}ure-Rich Text \textbf{\textit{Bench}}mark~(\textbf{StructBench}), a comprehensive benchmark designed to assess LLMs' proficiency in deciphering structures embedded in input text.
StructBench aims to determine whether LLMs are capable of understanding raw structural tags, executing logic inference based on the decoded semantic of these symbols, and constructing their responses conforming instruction requirements.
The experiments demonstrate that StructBench presents a combined challenge of structure understanding and inference, and while human beings perform well on these questions, leading LLMs struggle to answer them accurately.

\sout{TODO START

What is currently being done in academia.
What are their shortcomings.
(A super refined version of Related Work)

TODO END} \yhn{done in the paragraph ``Existing benchmarks...''}

% 我们的Benchmark中包含了xxx个任务，针对每个具体的任务，我们都设计了一个能够根据一定的规则自动化生成结构数据的方法。
% 每个任务生成了多少数据，总共有多少数据
StructBench comprises 6032 QAs for 29 structure-targeted tasks (208 QAs per tasks) across 8 input texts.
For each task, we derived question and answer using rule-based procedure.
% 一句话介绍生成文本规则和生成答案的规则
We designed rules\footnote{a small subset of the syntax for respective input format} for input text generation where the content is randomly selected from a finite alphabet~(\ref{ap:rules}), and deterministic procedures to carve out the answer.

\sout{StructBench addresses the evaluation of LLMs in understanding the structural information of input texts and executing symbolic computation and manipulation, focusing on structural understanding and logical inference.}\yhn{deleted. dup with ``StructBench aims to determin...''}


% \subsection{Contribution} 先不着急改这里
\begin{itemize}
    \item We first thoroughly evaluated the LLMs' ability to understand and manipulate structure-rich texts.
	\item We present a taxonomy for structured texts and designed structure-related tasks for each class. With a total of 8 text classes and 3-5 tasks for each class, we present 29 structure-specific tasks and 580 samples for our benchmark dataset.
	\item We also tested 5 LLMs and present the results under different prompt methods for assessment.
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/01.Introduction.04.tex <==

\gzh{I change the order of the first two paragraphs.
I think the description to the task is more important than why LLM can't handle this task.}



Structure-rich text is composed of semantic content and reserved syntactical symbols, such as tables, LaTeX, and graph defined by nodes and edge set. Structure-rich text\footnote{structure-rich text and structure-rich text are \blue{used interchangeably hereafter}\gzh{Don't do that! Make your term and writing consistent!}\yhn{replaced ``structured text'' with ``structure-rich text'' as in the title}} also serves as a key component of a series of web services, e.g., REST~\citep{masse2011rest, 8385157}, JSON-RPC~\citep{samsel2013web}, XML-based data exchange protocol~(e.g., SOAP~\citep{box2000simple}), and service process definition language(e.g., WSDL~\citep{christensen2001web})\gzh{place the citations directly behind these key components}, and higher-order services ~\citep{8603059, de2013eve, papazoglou2004survey, dustdar2005survey}.\gzh{This sentence is so long, delete some of the cases.}\yhn{refactored}
Additionally, structure-rich texts is critical for the functionality of web-based agents that operating across diverse host platforms and languages, frequently encountering data from a wide array of sources presented in structure-rich text, a diversity stemming from varied communication protocols, with Retrieval-Augmented Generation (RAG) being a typical example~(\citet{8603059, de2013eve, lewis2020retrieval}).

\gzh{You may need to simply define what is ``structure text'' or ``structure-rich text''.
The following paragraphs talk about "trees" and "graphs" and I would like to know why these two types are structural and what other types are there?}
\yhn{added as the first sentence of first paragraph}


Large language models~(LLMs)\gzh{Don't start from the topic that so far away, just start from LLM, directly tell the readers why LLM cannot handle structure text benchmark.
And here is the technique: you need to stress the main part of your research repetitively in your paper, and you need to place the most important view in front of other content.
Like: if you want say that ``deep model cannot handle structure text for xxx reason. llm is one type of deep model, so llm cannot either'', you should direct write ``llm cannot handle structure text for xxx reason.''.
Because llm but not deep model is part of your reasearch, and llm cannot handle structure text is an important view.}\yhn{changed to LLM}, as a modern implementation of the connectionist approach~\citep{thomas2008connectionist}, excel in processing the stochastic nature~\citep{ney1994structuring} of natural language by predicting token sequences, where probabilistic models are prominent~\citep{bengio2000neural}.
Specifically, LLMs have demonstrated exceptional capability across various natural language tasks, e.g., question answering, information retrieval, summarization, sentiment analysis, and toxicity detection~\citep{liang2022holistic}.


In contrast, symbolism represents another facet of artificial general intelligence~(AGI), arguing that symbolic thought is essential for human beings to ``generalize most broadly''~\citep{goertzel2014artificial}.
As probabilistic models, LLMs' effectiveness in symbolic computation based on strict rules and logical relationships is still an open question~\citep{bengio2000neural}.
Given the contrasting paradigms of AGI, investigating how deep learning models can adapt to symbolic computation is a critical challenge.
This touches on the fundamental question of whether probabilistic models for stochastic tasks can effectively manage the systematic and deterministic reasoning necessary for symbolic manipulation and processing.
Text structured as Tree, Table, JSON, YAML, XML, Markdown, LaTeX and Org formats consists of formation and inference rules that express logical relationships more unambiguously compared to natural languages.
These structures represent a less rigorous form of the symbol systems mentioned above and serve as an ideal medium for evaluating the problem.

\gzh{This paragraph should be refined into the Second paragraph}\yhn{moved to the end of 2nd paragraph}
\sout{Large Language Models (LLMs) have demonstrated exceptional capability across various natural language tasks, e.g., question answering, information retrieval, summarization, sentiment analysis, and toxicity detection~ citep liang2022holistic .}

\gzh{This paragarph should be placed in the Dataset Consturction Section or Experiment Section, but not in Introduction.
Introduciton should consist of mostly free-text to stress the importance of your research question, describe briefly about how you handle this question, and what's your conclusion or discovery.} \yhn{moved to the beginning of sec3}

% However, their proficiency in interpreting structure-rich texts remains less understood.
\gzh{This paragraph should also be refined into the Second paragraph}\yhn{split into the good side and down side, good side put into 2nd paragraph(1st sentence), down side put into 3nd paragraph(``As probabilistic ...'')}
\sout{As probabilistic models, LLMs excel in processing the stochastic nature of natural language by predicting token sequences, but their effectiveness in symbolic computation based on strict rules and logical relationships is still an open question as stated above~ citep bengio2000neural, ney1994structuring.}

% Existing benchmarks, such as those introduced by Fatemi et al. (2023) and Sui et al. (2024), primarily cater to natural language inputs or a constrained selection of structured input types, notably graphs or tables. This limitation misaligns with the real-world applications and the extensive array of structure-rich text types encountered by Large Language Models (LLMs). Furthermore, current methodologies leverage structural information through the creation of task-specific input designs or architectures, as noted by Perozzi et al. (2024) and Sui et al. (2024), yet this strategy may not fully capture the complexity or diversity of real-world structured data.


Existing benchmarks, such as those presented by \cite{fatemi2023talk, perozzi2024let, sui2024table}, focus on natural language inputs or provide a limited array of structure-rich text, such as graphs or tables. \gzh{Blue words are so vague. Be more precise.}\yhn{deleted}
This limited structure diversity diverges from the diverse structure-rich texts used in office environment, such as Markdown and LaTeX, thereby offering a skewed representation of practical LLM use cases.
As a consequence of limited scope, they leave the symbolic, semantically agnostic nature shared by these structure-rich texts untouched, which is emphasized in this work by erasing content semantics through randomized generation method\gzh{Don't that rush, your writing need to focus on the topic of the paragraph. Don't mention what the other paragraphs will contain.}.
Besides dataset, current methods cope with structural tasks by developing task-specific input designs or model architectures~(\cite{perozzi2024let, sui2024table}), leading to task dependent approach with limited generalizability.
\gzh{I have a concern, the only shortage of the existing benchmarks is they only contained limited type of structure?
}\yhn{It's ``they leave the symbolic, semantically agnostic nature shared by these structure-rich texts untouched''}


In response, we introduce the \textbf{\textit{Struct}}ure-Rich Text \textbf{\textit{Bench}}mark~(\textbf{StructBench}), a comprehensive benchmark designed to assess LLMs' proficiency in deciphering structures embedded in input text.
StructBench aims to determine whether LLMs are capable of understanding raw structural tags, executing logic inference based on the decoded semantic of these symbols, and constructing their responses conforming instruction requirements.
\gzh{The first two sentences are good.
But the last sentence should be placed behind the next paragraph}\yhn{moved}
StructBench comprises 6032 samples\gzh{use ``questions'' or ``samples'' but not QAs}\yhn{replaced} for 29 structure-targeted tasks \gzh{It's not important, you may delete it.}\yhn{removed} across 8 structure-rich texts\gzh{even I know your research, i am confused by ``input texts''. You may change a word.}.
The structure-rich texts in StructBench are generated systematically by rules~(\ref{ap:rules}) with contents randomly selected from a finite alphabet.
The question-answer pairs are derived using deterministic rule-based procedure.
\gzh{You did introduce the generation in one sentence.
But the writing style make it more like a part of a detail description (as if the description is cut in half) but not a general description.
You may consider the following style:
``
The questions within StructBench is generated by the manually written rules.
''
}\yhn{refactored}

\gzh{You lack of a paragraph to give the conclusion or the discovery of your research.
You may combine the last two paragraph into one, then add another one to talk about the experiments and the conclusion.
}\yhn{merged. added conclusion and experiments below}

The experiments demonstrate that StructBench presents a combined challenge of structure understanding and inference, and while human beings perform well on these questions, leading LLMs struggle to answer them accurately, revealing restricted generalizability.
Moreover, fine-tuning adapts poorly to structure inference tasks and offers limited performance enhancement, whereas few-shot learning demonstrates promising improvement compared to other prompt engineering methods, including Chain-of-Thought~(CoT).
In conclusion, LLMs exhibit low performance and little generalizability on structure inference tasks in StructBench, which is not adequately addressed through fine-tuning or prompt engineering, necessitating more attention on these symbolic tasks and alternative strategies to achieve broader generalizability. The contribution of our work is summarized as follow:

% \subsection{Contribution} 先不着急改这里

\gzh{I haven't read the contribution yet because it can be changed at last.
But you have to add that paragraph before the itemized contribution:
`` the contribution of our work is summarized as follow:''
} \yhn{added}
\begin{itemize}
    \item We first thoroughly evaluated the LLMs' ability to understand and manipulate structure-rich texts.
	\item We present a taxonomy for structure-rich texts and designed structure-related tasks for each class. With a total of 8 text classes and 3-5 tasks for each class, we present 29 structure-specific tasks and 580 samples for our benchmark dataset.
	\item We also tested 5 LLMs and present the results under different prompt methods for assessment.
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/01.Introduction.05.tex <==


Structure-rich text is composed of semantic content and reserved syntactical symbols, such as tables, LaTeX, and graph defined by nodes and edge set. Structure-rich text also serves as a key component of a series of web services, e.g., REST~\citep{masse2011rest, 8385157}, JSON-RPC~\citep{samsel2013web}, XML-based data exchange protocol~(e.g., SOAP~\citep{box2000simple}), and service process definition language(e.g., WSDL~\citep{christensen2001web}), and higher-order services ~\citep{8603059, de2013eve, papazoglou2004survey, dustdar2005survey}.
Additionally, structure-rich texts is critical for the functionality of web-based agents that operating across diverse host platforms and languages, frequently encountering data from a wide array of sources presented in structure-rich text, a diversity stemming from varied communication protocols, with Retrieval-Augmented Generation (RAG) being a typical example~(\citet{8603059, de2013eve, lewis2020retrieval}).




Large language models~(LLMs), as a modern implementation of the connectionist approach~\citep{thomas2008connectionist}, excel in processing the stochastic nature~\citep{ney1994structuring} of natural language by predicting token sequences, where probabilistic models are prominent~\citep{bengio2000neural}.
Specifically, LLMs have demonstrated exceptional capability across various natural language tasks, e.g., question answering, information retrieval, summarization, sentiment analysis, and toxicity detection~\citep{liang2022holistic}.


In contrast, symbolism represents another facet of artificial general intelligence~(AGI), arguing that symbolic thought is essential for human beings to ``generalize most broadly''~\citep{goertzel2014artificial}.
As probabilistic models, LLMs' effectiveness in symbolic computation based on strict rules and logical relationships is still an open question~\citep{bengio2000neural}.
Given the contrasting paradigms of AGI, investigating how deep learning models can adapt to symbolic computation is a critical challenge.
This touches on the fundamental question of whether probabilistic models for stochastic tasks can effectively manage the systematic and deterministic reasoning necessary for symbolic manipulation and processing.
Text structured as Tree, Table, JSON, YAML, XML, Markdown, LaTeX and Org formats consists of formation and inference rules that express logical relationships more unambiguously compared to natural languages.
These structures represent a less rigorous form of the symbol systems mentioned above and serve as an ideal medium for evaluating the problem.






Existing benchmarks, such as those presented by \cite{fatemi2023talk, perozzi2024let, sui2024table}, focus on natural language inputs or provide a limited array of structure-rich text, such as graphs or tables. 
This limited structure diversity diverges from the diverse structure-rich texts used in office environment, such as Markdown and LaTeX, thereby offering a skewed representation of practical LLM use cases.
As a consequence of limited scope, they leave the symbolic, semantically agnostic nature shared by these structure-rich texts untouched, which is emphasized in this work by erasing content semantics through randomized generation method.
Besides dataset, current methods cope with structural tasks by developing task-specific input designs or model architectures~(\cite{perozzi2024let, sui2024table}), leading to task dependent approach with limited generalizability.



In response, we introduce the \textbf{\textit{Struct}}ure-Rich Text \textbf{\textit{Bench}}mark~(\textbf{StructBench}), a comprehensive benchmark designed to assess LLMs' proficiency in deciphering structures embedded in input text.
StructBench aims to determine whether LLMs are capable of understanding raw structural tags, executing logic inference based on the decoded semantic of these symbols, and constructing their responses conforming instruction requirements.
StructBench comprises 6032 samples for 29 structure-targeted tasks  across 8 structure-rich texts.
The structure-rich texts in StructBench are generated systematically by rules~(\autoref{ap:rules}) with contents randomly selected from a finite alphabet.
The question-answer pairs are derived using deterministic rule-based procedure.



The experiments demonstrate that StructBench presents a combined challenge of structure understanding and inference, and while human beings perform well on these questions, leading LLMs struggle to answer them accurately, revealing restricted generalizability.
Moreover, fine-tuning adapts poorly to structure inference tasks and offers limited performance enhancement, whereas few-shot learning demonstrates promising improvement compared to other prompt engineering methods, including Chain-of-Thought~(CoT).
In conclusion, LLMs exhibit low performance and little generalizability on structure inference tasks in StructBench, which is not adequately addressed through fine-tuning or prompt engineering, necessitating more attention on these symbolic tasks and alternative strategies to achieve broader generalizability. The contribution of our work is summarized as follow:

% \subsection{Contribution} 先不着急改这里


\begin{itemize}
    \item We first thoroughly evaluated the LLMs' ability to understand and manipulate structure-rich texts.
	\item We present a taxonomy for structure-rich texts and designed structure-related tasks for each class. With a total of 8 text classes and 3-5 tasks for each class, we present 29 structure-specific tasks and 580 samples for our benchmark dataset.
	\item We also tested 5 LLMs and present the results under different prompt methods for assessment.
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/01.Introduction.06.tex <==


% Structure-rich text is composed of semantic content and reserved syntactical symbols, such as tables, LaTeX, and graph defined by nodes and edge set. Structure-rich text also serves as a key component of a series of web services, e.g., REST~\citep{masse2011rest, 8385157}, JSON-RPC~\citep{samsel2013web}, XML-based data exchange protocol~(e.g., SOAP~\citep{box2000simple}), and service process definition language(e.g., WSDL~\citep{christensen2001web}), and higher-order services ~\citep{8603059, de2013eve, papazoglou2004survey, dustdar2005survey}.
% Additionally, structure-rich texts is critical for the functionality of web-based agents that operating across diverse host platforms and languages, frequently encountering data from a wide array of sources presented in structure-rich text, a diversity stemming from varied communication protocols, with Retrieval-Augmented Generation (RAG) being a typical example~(\citet{8603059, de2013eve, lewis2020retrieval}).




% Large language models~(LLMs), as a modern implementation of the connectionist approach~\citep{thomas2008connectionist}, excel in processing the stochastic nature~\citep{ney1994structuring} of natural language by predicting token sequences, where probabilistic models are prominent~\citep{bengio2000neural}.
% Specifically, LLMs have demonstrated exceptional capability across various natural language tasks, e.g., question answering, information retrieval, summarization, sentiment analysis, and toxicity detection~\citep{liang2022holistic}.


% In contrast, symbolism represents another facet of artificial general intelligence~(AGI), arguing that symbolic thought is essential for human beings to ``generalize most broadly''~\citep{goertzel2014artificial}.
% As probabilistic models, LLMs' effectiveness in symbolic computation based on strict rules and logical relationships is still an open question~\citep{bengio2000neural}.
% Given the contrasting paradigms of AGI, investigating how deep learning models can adapt to symbolic computation is a critical challenge.
% This touches on the fundamental question of whether probabilistic models for stochastic tasks can effectively manage the systematic and deterministic reasoning necessary for symbolic manipulation and processing.
% Text structured as Tree, Table, JSON, YAML, XML, Markdown, LaTeX and Org formats consists of formation and inference rules that express logical relationships more unambiguously compared to natural languages.
% These structures represent a less rigorous form of the symbol systems mentioned above and serve as an ideal medium for evaluating the problem.


% 大语言模型正变得越来越
% 结构化的数据在企业中的占比非常大，大语言模型的使用者们越来越依赖LLM去直接处理结构化的数据。
% LLM需要具备理解结构化文本的能力，

% 增强LLM对于结构化文本的理解，首先需要构造全面的benchmark。
% 现有的对于结构化文本理解的benchmark，主要涉及。
% 这类benchmark存在一些问题：
% 1. 覆盖的类型有限
% 2. xxx
% 3. xxx

% 结构化数据，曾经是企业中最为宝贵的资源。
% 结构化数据相较于非结构化数据的好处在于。
% 而随着LLM的出现，非结构化的数据大放异彩。
% 而随着LLM的能力不断变强，我们会有此疑问：
% LLM能否直接理解结构化的数据？




% LLM的这种能力彰显了非结构化数据的潜力，但随着LLM
% 促使企业重新评估其数据策略。
% 随着技术进步，LLM不仅能理解非结构化数据，其对结构化数据的处理能力也在不断增强，这引发了对其在企业数据管理中角色的重新考量。



% 结构化数据，如以JSON、YAML、XML、Markdown等格式进行存储的数据，因其有助于企业系统地捕捉、存储和分析关键信息，一直是企业数据战略的核心。
% 其本质优势在于其标准化格式和高度组织性，使得数据查询和机器处理变得更高效，显著优于杂乱无章的非结构化数据。
% 然而，随着大型语言模型（LLM）的发展，非结构化数据开始被有效利用，因为LLM能够理解和生成这类数据的复杂和细微语义。
% 考虑到结构化文本，也可以以非结构化的形式进行展现，许多LLM研究者不禁疑惑：是否能依赖LLM去直接通过非结构化的文本去理解结构化的内容？


Structured data, stored in formats such as JSON, YAML, XML, or Markdown, Latex etc., has consistently been central to corporate data strategies due to its ability to systematically capture, store, and analyze essential information.
The inherent advantages of structured data lie in its standardized formats and high degree of organization, which enhance the efficiency of data queries and machine processing, markedly outperforming the chaotic nature of unstructured data.
However, with the advancement of large language models (LLMs), there has been a significant shift towards the effective utilization of unstructured data, attributed to the LLMs' capacity to comprehend and generate complex and nuanced semantics within such data.
Considering that structured data can be presented in an free-text format, it makes us wondering \textbf{\textit{whether it is possible to rely on LLMs to directly interpret structured data through free-text format}}.


Existing benchmarks, such as those presented by \cite{fatemi2023talk, perozzi2024let, sui2024table}, focus on natural language inputs or provide a limited array of structure-rich text, such as graphs or tables. 
This limited structure diversity diverges from the diverse structure-rich texts used in office environment, such as Markdown and LaTeX, thereby offering a skewed representation of practical LLM use cases.
As a consequence of limited scope, they leave the symbolic, semantically agnostic nature shared by these structure-rich texts untouched.
Besides dataset, current methods cope with structural tasks by developing task-specific input designs or model architectures~(\cite{perozzi2024let, sui2024table}), leading to task dependent approach with limited generalizability.

% which is emphasized in this work by erasing content semantics through randomized generation method.






In response, we introduce the \textbf{\textit{Struct}}ure-Rich Text \textbf{\textit{Bench}}mark~(\textbf{StructBench}), a comprehensive benchmark designed to assess LLMs' proficiency in deciphering structures embedded in input text.
StructBench aims to determine whether LLMs are capable of understanding raw structural tags, executing logic inference based on the decoded semantic of these symbols, and constructing their responses conforming instruction requirements.
StructBench comprises 6032 samples for 29 structure-targeted tasks  across 8 structure-rich texts.
The structure-rich texts in StructBench are generated systematically by man-written rules with contents randomly selected from a finite alphabet.
The question-answer pairs are derived using deterministic rule-based procedure.



The experiments demonstrate that StructBench presents a combined challenge of structure understanding and inference, and while human beings perform well on these questions, leading LLMs struggle to answer them accurately, revealing restricted generalizability.
Moreover, fine-tuning adapts poorly to structure inference tasks and offers limited performance enhancement, whereas few-shot learning demonstrates promising improvement compared to other prompt engineering methods, including Chain-of-Thought~(CoT).
In conclusion, LLMs exhibit low performance and little generalizability on structure inference tasks in StructBench, which is not adequately addressed through fine-tuning or prompt engineering, necessitating more attention on these symbolic tasks and alternative strategies to achieve broader generalizability. The contribution of our work is summarized as follow:


\begin{itemize}
    \item We first thoroughly evaluated the LLMs' ability to understand and manipulate structure-rich texts.
	\item We present a taxonomy for structure-rich texts and designed structure-related tasks for each class. With a total of 8 text classes and 3-5 tasks for each class, we present 29 structure-specific tasks and 580 samples for our benchmark dataset.
	\item We also tested 5 LLMs and present the results under different prompt methods for assessment.
\end{itemize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/01.Introduction.07.tex <==
Structured data, often represented by various structured languages such as JSON~\cite{pezoa2016foundations}, YAML~\cite{evans2001yaml}, ORG~\cite{orgModeManualHistory2023}, or Markdown~\cite{gruber2012markdown}, Latex~\cite{Lamport1985LatexA} etc., has consistently been central to corporate data strategies due to its ability to capture, store, and analyze essential information systematically.
The inherent benefits of structured data lie in its standardized format and high degree of organization, which facilitates efficient data querying and machine processing, clearly surpassing the inherent chaos of unstructured data.
However, with the advancement of large language models (LLMs)~\cite{achiam2023gpt,touvron2023llama,touvron2023llama2,sun2021ernie}, there has been a significant shift towards the effective utilization of unstructured data, attributed to the LLMs' capacity to comprehend and generate complex and nuanced semantics within such data~\cite{brown2020language}.
Considering that structured data can be directly presented in an unstructured format, it makes us wonder: \textbf{\textit{whether it is possible to rely on LLMs to interpret structured data through unstructured format directly}}.

% Given the prevalence of structured data storage in each enterprise, one approach to utilizing LLM for processing structured data is to transform the structured data into unstructured text through manually written rules.
% However, developing different rules for different structured schemas requires a significant time investment, and there is also a potential mismatch between the rewritten unstructured text and the original data.


% Current LLMs researches have addressed 


Current LLMs researches have addressed their comprehension of structure-rich text, with a primary focus on the understanding of limited categories: 
Graphs~\cite{fatemi2023talk, perozzi2024let, guo2023gpt4graph, tang2023graphgpt, chen2023exploring}, 
Tables~\cite{sui2024table,campbell2003history,pasupat2015compositional}
and JSON~\cite{chen2024beyond, suzgun2022challenging}.
However, these categories do not encompass all potential use cases of structure-rich text.
For instance, scenarios requiring direct understanding of articles in Latex or Markdown formats, data in YAML or ORG formats, or various custom structured languages are not adequately covered.
Moreover, existing benchmarks often rely on manually annotated data for evaluation, which limits the development of robust evaluation frameworks and potentially facilitates model cheating~\cite{zhou2023don}.



% 除此之外，现有的工作只针对Graph和Table设计了不同的使用任务，

% However, the representation of structure-rich text is highly diverse, and there needs to be a unified benchmark encompassing a wide array of these text structures.

In response, we propose a method for automatically generating evaluation data to assess models' capabilities in understanding structure-rich text. 
This method is applied to 8 structured languages, as shown in Fig.~\ref{fig:taxonomy}, across 29 specific tasks, enabling data generation with controllable difficulty by adjusting the depth of structured nesting.
Based on this method, we further introduce the \textbf{\textit{Struc}}ture-Rich \textbf{\textit{Text}} \textbf{\textit{Eval}}uation Benchmark~(\textbf{StrucText-Eval}), a comprehensive benchmark with 6,032 samples designed to evaluate the proficiency of LLMs in deciphering embedded structures within input text.
StrucText-Eval aims to determine whether LLMs understand raw structural tags, execute logical inferences based on the decoded semantics of these symbols, and construct their responses according to instruction requirements.
Considering that humans excel at understanding structured expressions, we further propose StrucText-Eval-Hard, a subset of StrucText-Eval consisting of 3,012 samples with the longest questions, highlighting the disparity between LLMs and human understanding of structured data.


The experiments show that StrucText-Eval significantly challenges current LLMs. The highest accuracy achieved by LLMs using various prompt methods was 78.4\%, dropping to 65.0\% on StrucText-Eval-Hard. In contrast, human participants reached 95.7\% accuracy on StrucText-Eval-Hard, underscoring the inadequacy of existing LLMs in processing complex structural information.
Utilizing StrucText-Eval data enhances the capabilities of current closed-source LLMs and improves open-source LLMs by fine-tuning them with this benchmark. This finding confirms StrucText-Eval's critical role in evaluating and optimizing model performance. However, more than using the training data from StrucText-Eval alone is required to surpass GPT4-Turbo's performance on this test suite. Additionally, not all tasks can be improved solely by training on the relevant dataset.
Therefore, StrucText-Eval provides a comprehensive evaluation framework for assessing LLMs' ability to understand structured text, leaving room for further improvement.




We present the following contributions to our research: 
(1) We developed a method for generating evaluation data for eight structured languages.
This method allows control over the complexity of the generated evaluation data by manipulating the quantity of structural nesting.
(2) We introduce StrucText-Eval, a comprehensive benchmark comprising 6,032 samples across eight structured languages and 29 evaluation tasks. This benchmark is designed to assess LLMs' capabilities in understanding structured data comprehensively.
(3) We have conducted extensive experiments, including evaluations of existing large models' capabilities in understanding structure-rich text and enhancements to the capacity of open-source LLMs in this area. Our findings indicate a significant gap between current LLMs and humans in understanding structure-rich text.


% In response, we propose a method for the automated generation of evaluation data to assess models' capabilities in understanding structure-rich text.
% This method can be applied to 8 structured languages, as shown in Fig.~\ref{fig:taxonomy}, across 29 specific tasks, enabling the generation of data with controllable difficulty by adjusting the depth of structured nesting.
% Based on this method, we further introduce the \textbf{\textit{Struct}}ure-Rich Text \textbf{\textit{Bench}}mark~(\textbf{StrucText-Eval}), a comprehensive benchmark with 6032 samples designed to evaluate the proficiency of LLMs in deciphering embedded structures within input text.
% StrucText-Eval aims to determine whether LLMs are capable of understanding raw structural tags, executing logic inference based on the decoded semantic of these symbols, and constructing their responses conforming instruction requirements.
% Considering that humans are good at understanding structured expressions, we further propose StrucText-Eval-Hard, a subset of StrucText-Eval consisting of 3,012 samples with the longest questions, to highlight the disparity between LLMs and human understanding of structured data.

% 考虑到结构化表达非常有助于人类理解，所以我们进一步提出了StrucText-Eval-Hard，which is a subset of StrucText-Eval and consist of 3012 samples with longest questions，来体现LLM和人类在结构化数据理解上的差距。

% The structure-rich texts in StrucText-Eval are generated systematically by man-written rules with contents randomly selected from a finite alphabet.
% And the question-answer pairs are derived using deterministic rule-based procedure.
% The highest accuracy made by LLMs with all kinds of prompt methods was only 78.4\%, and plummeted to 65.0\% on the more challenging StrucText-Eval-Hard test.

% The experiments demonstrate that StrucText-Eval poses a significant challenge to current LLM.
% The highest accuracy achieved by LLMs using various prompt methods was only 78.4\%, which further decreased to 65.0\% on StrucText-Eval-Hard.
% In stark contrast, human participants achieved an accuracy of 95.7\% on StrucText-Eval-Hard.
% This stark contrast highlights the inadequacy of existing LLMs in accurately processing complex structural information.
% Utilizing the data in StrucText-Eval as a demonstration can effectively improve the capabilities of current closed-source LLMs.
% By fine-tuning open-source LLMs using StrucText-Eval, the ability of open-source LLMs to understand various structured texts can be enhanced.
% This finding not only confirms the critical role of StrucText-Eval in evaluating model performance, but also its positive impact in the model training and optimization phases.
% However, the training data provided by StrucText-Eval alone is not enough to surpass the performance of GPT-4 on this test suite.
% At the same time, not all tasks can be improved by training only the dataset relevant to that task.
% Therefore, StrucText-Eval leaves enough room for a comprehensive evaluation of LLM's ability to understand structured text.









% Research findings demonstrate that StrucText-Eval poses a significant challenge to the current large language models (LLMs). Even with the utilization of Chain of Thought (CoT) reasoning, the performance accuracy of the GPT-4 model is merely 78.4\%, which nosedives to 34.1\% on the more challenging StrucText-Eval-Hard tests. In stark contrast, human participants showcase a high accuracy rate of 97.6\% on the same test set. This stark disparity underscores the existing LLMs' deficiency in processing complex structured information accurately.
% Further examination reveals that employing data from StrucText-Eval as demonstrations can effectively enhance the capabilities of current closed-source LLMs. By utilizing StrucText-Eval for fine-tuning open-source LLMs, a significant improvement in these models' ability to understand a variety of structured texts is observed. This finding confirms not only the pivotal role of StrucText-Eval in assessing model performance but also its positive impact in model training and optimization phases.
% However, it is crucial to recognize that merely relying on the training data provided by StrucText-Eval is insufficient to surpass the performances witnessed in GPT-4 on this test suite. It's also evident that not all tasks can be enhanced solely by training on dataset-specific data. Therefore, StrucText-Eval leaves ample room for a comprehensive evaluation of LLMs' capabilities in understanding structured texts, indicating that model architecture and training methodologies must be further refined to bridge the gap in accurately processing and understanding structured information, thereby narrowing the performance disparity between models and human capabilities.


% 实验结果证明，StrucText-Eval对于目前已有的LLM而言是个非常强力的挑战。
% 哪怕是GPT4在依靠CoT进行推理时的准确率依然只有78.4，而在StrucText-Eval-Hard上则会降到34.1\%，与之相比的，人类在StrucText-Eval-Hard上的表现为97.6\%。
% 使用StrucText-Eval中的数据作为demonstration可以对现有的闭源LLM进行有效地增强，而用来微调开源LLM时，能够有效提升LLM对于所有结构化语言的理解能力。
% 但仅仅依靠StrucText-Eval的训练数据，并不能在StrucText-Eval上得到超过GPT4的结果，这为所有模型进一步提升对于结构化文本的理解和评估留下了空间。

% 但并不是所有任务都能够单纯地依靠训练和该任务相关的数据来提升LLM表现。


% The experiments demonstrate that StrucText-Eval presents a combined challenge of structure understanding and inference, and while human beings perform well on these questions, leading LLMs struggle to answer them accurately, revealing restricted generalizability.
% Moreover, fine-tuning adapts poorly to structure inference tasks and offers limited performance enhancement, whereas few-shot learning demonstrates promising improvement compared to other prompt engineering methods, including Chain-of-Thought~(CoT).
% In conclusion, LLMs exhibit low performance and little generalizability on structure inference tasks in StrucText-Eval, which is not adequately addressed through fine-tuning or prompt engineering, necessitating more attention on these symbolic tasks and alternative strategies to achieve broader generalizability. The contribution of our work is summarized as follow:


% \begin{itemize}
%     \item We first thoroughly evaluated the LLMs' ability to understand and manipulate structure-rich texts.
% 	\item We present a taxonomy for structure-rich texts and designed structure-related tasks for each class. With a total of 8 text classes and 3-5 tasks for each class, we present 29 structure-specific tasks and 580 samples for our benchmark dataset.
% 	\item We also tested 5 LLMs and present the results under different prompt methods for assessment.
% \end{itemize}


% \begin{itemize}
%     \item 我们是提出了一套针对于8个结构化语言的评估数据生成方法，该方法可以通过控制生成的嵌套数量来控制生成评估数据的复杂度。
%     \item 我们提出了StrucText-Eval，一个包含6032条数据，8个结构化语言，29个评估任务的Benchmark，可以用于全方位评估LLM对于结构化数据的理解能力。
%     \item 我们进行了大量的实验，包括对于已有大模型对于Structure-rich text understanding能力的评估，以及增强开源LLM对于Structure-rich text understanding的能力。我们的结果发现，现有LLM在Structure-rich text understanding上距离人类有着非常巨大的差距。
% \end{itemize}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/01.Introducton.v1.tex <==
% INTERACTIVE AGENT IN GAME => CONTROLLED OUTPUT/RESPONSE

\subsection{Background} %AIGC
The landscape of machine learning and artificial intelligence is rapidly transforming with the emergence of intelligent agents acting as information middleware.
These agents, often tasked with executing commands on behalf of humans, operate within a milieu dominated by machine-generated texts.%REF:Research on agent
Machine-generated texts, which serve as carriers for data flow between programs, are typically stored, transmitted, and processed in formats rich in structure formed by tags and mark-ups.
This paradigm shift necessitates a profound understanding of Large Language Models’ (LLMs) capabilities in processing and interpreting structure-rich texts.
Our study introduces an innovative benchmark designed to evaluate LLMs’ proficiency in this realm, marking a significant stride in the field of structured text processing and knowledge inference.

\subsection{Motivation} %AIGC
Firstly, the advent of intelligent agents as intermediaries in information processing underscores the critical need for LLMs to adeptly handle texts generated by machines, which are often structured and require nuanced understanding for effective machine-to-machine communication.%REF: agent & machine texts & machine 2 machine communication

Secondly, there is a discernible gap in the existing benchmarks and datasets concerning the diversity and complexity of structured texts. %REF: existing benchmarks
Traditional datasets are predominantly centered around codebases and fail to fully represent the intricate structures prevalent in texts intended for machine comprehension. %REF: existing benchmarks
% Our benchmark aims to fill this gap by providing a diverse corpus of structure-rich texts, presenting tasks that challenge LLMs’ ability to not only infer knowledge but also to generate structured responses in alignment with machine-readable formats.
%
% pre-revise: Due to the pre-iminent growth of structural rich text and monology in category and diversity of existing benchmarks, an benchmark dedicated to evaluate machine understanding and generating-ability of structure-rich texts are beneficial with significant practical niche.

The rapid increase in complex, structured texts necessitates a dedicated benchmark for evaluating machines' ability to understand and generate such content. This benchmark addresses a critical gap in current methodologies, catering to the evolving needs of machine-to-machine communication and structured data processing.%AIGC

\subsection{Research Objectives} %AIGC
% The primary goal of our research is to develop a benchmark that rigorously evaluates LLMs in the context of texts integral to intelligent agents’ workflows. This includes assessing their ability to process small structured texts and to generate responses that adhere to strict formatting rules, which are essential for seamless machine-to-machine interactions.
The primary goal of our research is to build a benchmark evaluating LLMs in the context of texts integral to intelligent agents’ workflows. % benchmark
We assess model capabilities by posing questions based on structured text inputs that are syntactically correct but semantically null and void, imposing a challenge for models in discerning structure for meaning. % eval method
We conducted assessment on a range of LLMs, and compared their performance on different categories of tasks. % experiment
Furthermore, we fine-tuned 3 models with our datasets in hope of enhanced machine comprehension on structured texts. % train on dataset

\subsection{Our Method}
We searched vastly structured texts that have well-documented syntax and are widely used in industry and academies, e.g., JSON, YAML, LaTeX.
We include both fully-structured and half-structured data to enrich the diversity of our dataset.
For each class of texts, we designed 3-5 tasks that are structure-related, some of which are specific to their classification.

Based on the syntax and rules for construction, we randomly generate the input texts, and procedurally generate the corresponding tasks data in the meantime.

\subsection{Contribution}
\begin{itemize}
    \item We first thoroughly evaluated the LLMs' ability to understand and manipulate structure-rich texts.
	\item We present a taxonomy for structured texts and designed structure-related tasks for each class.
	\item With a total of 8 text classes and 3-5 tasks for each class, we present 29 structure-specific tasks and 580 samples for our benchmark dataset.
	\item We also tested 4 LLMs and present the results under different metrics for assessment.
\end{itemize}

% The paper is organized as follows: Section 2 reviews literature related to the development of models and benchmarks for structured text tasks, especially in the context of intelligent agents. Section 3 proposes a taxonomy for structure-rich texts, detailing their generation rules and applications in intelligent agent scenarios. Section 4 describes our methodology for collecting and curating data for this benchmark. Section 5 presents the experimental setup and results. The paper concludes with a discussion on the implications of our findings for the future of intelligent agents and LLMs in machine-generated text comprehension.


==> texs/old_version/02.RelatedWork.01.tex <==
%REF: reviews literature related to the development of models and benchmarks for structured text tasks, especially in the context of intelligent agents
% 表格数据推理综述：https://mp.weixin.qq.com/s/sXeyH2Ob8-CbGwHHBYOYfQ

% Current Work on Code: graph neural network + AST (node representation)
% need mannually construct model and extract graph representation from text
% but beside code, YAML, JSON, XML, LaTeX..., and other new structure text will emerge.
% They are not as well explored as code. Some of is too simple to have AST

% We don't want to mannually construct model and extract graph representation (e.g., AST parser) for each new structure text,
% And cost too much computation power to train a new model for each new structure text

% Since
% 1. they are so commonly used in office works and coincide greatly with LLMs use scenarios,
% 2. they share a common pattern, i.e., tree structure, or put it in another way, recursively defined structure. This pattern is not exploited.

% So
% We wish LLM to have generalization ability to mimic the specialized model structure and explicitly abstracted node representation.
% put it in another way, we wonder
%    given only the raw text as input,
%    if it is possible for LLM to rebuilt the graph in his own mind (internally, internal world model)
%    and do logic inference on this graph
% and we wish to have a benchmark to evaluate the performance of LLM on structured text.

\textbf{Models}: 
\gzh{Rewrite this paragraph into two paragraphs, one is about other researhes, one is telling the difference between ours and others.} \yhn{Merged the ``difference parts of Models \& Datasets into one paragraph at the end of this section''}

\sout{Due to the inherent difference between sequential natural language texts and rich-structure texts, NLP models trained on natural language perform worse than models curated for structural tasks~(cite mou2016convolutional).
The weakness of language models on structural tasks and achievements from alternative specialized architecture showed insufficient attention on the realm of rich-structure text from language models.}


% Part1: Works on how to improve model performance structured text => MODEL->它们和我们的联系是它们运用了规则/语法来辅助提升性能
% 浓缩成写一段，弱词 knowledge/understanding/... 替换掉(正文不要，intro可以)
Previous explorations over structural information focused on tasks related to programming languages and graphs. % programming language 和 structured text 我们分成两种语料，在这里从前人工作中去总结 语法/规则 相关任务 的经验
\citet{mou2016convolutional} built a tree-based convolutional neural network that outperformed language models on functionality classification tasks and pattern detection tasks over programming languages. % functionality classification, pattern detection
\citet{wang2020detecting} outperformed state of the art~(SOTA) on code clone detection benchmarks, applying graph neural networks on abstract syntax trees~(ASTs) representation augmented by control and data flow edges, which is different in architecture from language models curated for natural language tasks. % code clone detection
\citet{zhou2019devign} built a graph neural network over rich node representations of code and gained SOTA on vulnerability identification in 4 large-scaled open-source C projects. %vulnerability identification
% These code based tasks require the understanding of the structure as an auxiliary information to fully capture the semantics and patterns of code snippets, which is different from tasks in sequential text processing.
% Their approaches are mainly based on graph neural networks~(GNNs) applied on ASTs, i.e., specialized model structure along with explicitly abstracted structure representation.
% Graph tasks are one of the structure understanding and inference tasks made explicit with nodes and edges as the formal language, where GNNs showed prominent excellence.
\citet{perozzi2024let} proposed a dedicated graph neural network~(GNN) to encode graph into embedding space of LLMs, and used LLMs as an decoder to solve the graph tasks in GraphQA~\citep{fatemi2023talk}.
\citet{chen2023exploring} explored LLMs' potential in learning graphs, focusing on node classification tasks, using LLMs as enhancers for GNN predictor and directly as predictor.
\citet{chen2024beyond} disclosed the employment of formats other than natural language in CoT reasoning and multi-agent communication significantly enhances model performance while also decreasing token usage on reasoning tasks.

% These attempts at enhancement methods target semantic understanding tasks, where structural information serves as auxiliary information to aid in discerning semantics from the input text.
% In contrast, the answers in StructBench are semantically agnostic, requiring a focus on the structural aspects rather than meaning extraction.

 % TODO, find works on markup language, e.g., XML, YAML, JSON, LaTeX, table, etc.
\textbf{Datasets}: The similar datasets dedicating to structure information understanding are scarce.
GraphQA~\citep{fatemi2023talk} is a benchmark for assessing LLMs on reasoning over graph data, composed of 7 simple graph tasks, with exploration on methods in encoding graph-structured data as text.
\citet{sui2024table} consists of 8 tasks on table-formatted input texts, i.e., input data organized in row-column structures, with studying in input design and prompt enhancement.
\citet{pasupat2015compositional} exposed a dataset of 22,033 complex questions on Wikipedia tables and proposed a parsing algorithm for answering complex questions on semi-structured tables.
For tabular data, \citet{SHWARTZZIV202284} showed that deep models were not a good solution; \citet{NEURIPS2021_9d86d83f} designed two specialized baseline architecture for tabular data and concluded that universally superior solution does not exist.
\citet{wang2024can} is another graph-based problem solving benchmark, with graph structure described with natural language.
\citet{fatemi2023talk} and \citet{sui2024table} include comparison of encoding methods for structure information, i.e., graphs and tables, respectively, showing that LLMs performance varies on different encodings and the relatively vacancy on LLM's understanding of structure-rich texts input.
% Difference, just graph and table, not comprehensive enough and tasks is not targeted on structure information understanding and inference, i.e., either on graph reasoning or table 

Our dataset diverges from previous research in two significant ways.
Firstly, our tasks focus exclusively on understanding structural information and performing dependent inference, distinct from prior approaches~\citep{mou2016convolutional, zhou2019devign} that use structural data primarily as an auxiliary tool for classification or semantic comprehension.
This focus is achieved by introducing randomness in the generation of input texts, which renders the texts semantically obscure and the tasks semantically agnostic.
Secondly, our benchmark extends beyond traditional graph reasoning and table information retrieval to include a broader spectrum of structure-rich text types.
It also incorporates comprehensive structure-based inference tasks that are tailored to specific input formats.

% Part2: Works on structured text benchmark and datasets => DATA
%As for benchmark and datasets, existing works mainly focus on codebases and scenarios of clone detection, vulnerability identification and so on.
% \cite{svajlenko2014towards} proposed a benchmark over Java codes targeting on code clone detection tasks, leaving the inner structure of codes texts untouched.
% \cite{zhou2019devign} also built a dataset from diversified large-scale open-source C projects (Linus, QEMU, Wireshark, FFmpeg) with a total of 48,687 commits, manually labeled as vulnerable or non-vulnerable used for vulnerable function identification.
% The {\sc CodeSearchNet} \cite{husain2019codesearchnet} for code query tasks consist of 6 million functions from open-source code, covering six programming language.
% It is noteworthy that the construction of the dataset leveraged the information in documentation associated with functions during data filtering, utilizing the externally obtained semantic information as much as possible.
% However, rather than inspecting syntactic and structural information, the tasks in \cite{husain2019codesearchnet} are semantic code search, which is more semantic dominated.
% Other code related datasets include \cite{raychev2016learning} which contains 150,000 JavaScript files with parsed ASTs, and \cite{raychev2016probabilistic} which is the Python counterparts to the former one.

 % verify that the works above use structure as a axuliary information, not the main information to answer semantic questions.
 % TODO, find works on markup language, e.g., XML, YAML, JSON, LaTeX, table, etc.
 % if similar benchmark exist, write it, and put it to part1
 % if not, split part1 into 2 part=>
 %  (运用语法规则来提升模型 - AST extraction/abstraction
 %  , 如何增强模型对规则的理解 - specilized model architecture/fintune/configure)
 % make it clear that: 1. their tasks are semantics query, structure information is just axciliary information
 %                     2. our task is structure understanding, thus semantics is randomized in the structure.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/02.RelatedWork.02.tex <==


\textbf{Models}: 

Previous explorations over structural information focused on tasks related to programming languages and graphs. 
\citet{mou2016convolutional} built a tree-based convolutional neural network that outperformed language models on functionality classification tasks and pattern detection tasks over programming languages. % functionality classification, pattern detection
\citet{wang2020detecting} outperformed state of the art~(SOTA) on code clone detection benchmarks, applying graph neural networks on abstract syntax trees~(ASTs) representation augmented by control and data flow edges, which is different in architecture from language models curated for natural language tasks. 
\citet{zhou2019devign} built a graph neural network over rich node representations of code and gained SOTA on vulnerability identification in 4 large-scaled open-source C projects. 
\citet{perozzi2024let} proposed a dedicated graph neural network~(GNN) to encode graph into embedding space of LLMs, and used LLMs as an decoder to solve the graph tasks in GraphQA~\citep{fatemi2023talk}.
\citet{chen2023exploring} explored LLMs' potential in learning graphs, focusing on node classification tasks, using LLMs as enhancers for GNN predictor and directly as predictor.
\citet{chen2024beyond} disclosed the employment of formats other than natural language in CoT reasoning and multi-agent communication significantly enhances model performance while also decreasing token usage on reasoning tasks.


\textbf{Datasets}: 

The similar datasets dedicating to structure information understanding are scarce.
GraphQA~\citep{fatemi2023talk} is a benchmark for assessing LLMs on reasoning over graph data, composed of 7 simple graph tasks, with exploration on methods in encoding graph-structured data as text.
\citet{sui2024table} consists of 8 tasks on table-formatted input texts, i.e., input data organized in row-column structures, with studying in input design and prompt enhancement.
\citet{pasupat2015compositional} exposed a dataset of 22,033 complex questions on Wikipedia tables and proposed a parsing algorithm for answering complex questions on semi-structured tables.
For tabular data, \citet{SHWARTZZIV202284} showed that deep models were not a good solution; \citet{NEURIPS2021_9d86d83f} designed two specialized baseline architecture for tabular data and concluded that universally superior solution does not exist.
\citet{wang2024can} is another graph-based problem solving benchmark, with graph structure described with natural language.
\citet{fatemi2023talk} and \citet{sui2024table} include comparison of encoding methods for structure information, i.e., graphs and tables, respectively, showing that LLMs performance varies on different encodings and the relatively vacancy on LLM's understanding of structure-rich texts input.


Our dataset diverges from previous work in two significant ways.

\blue{Firstly, our tasks exclusively concentrate on analyzing structural information and executing dependent inference, unlike prior approaches~\citep{mou2016convolutional, zhou2019devign} that employ structural data primarily as an auxiliary tool for classification or semantic comprehension.
StructBench focus on symbolic structure by erasing content semantics from input texts, preserving only structural details, which renders the texts semantically obscure and the tasks semantically agnostic.

Secondly, our benchmark extends beyond traditional graph reasoning and table information retrieval to include a broader spectrum of structure-rich text types.
It also incorporates comprehensive structure-based inference tasks that are tailored to specific input formats.}

\gzh{Your classification is right, StructBench has two prominent features:
Wide Coverage and Different Task Design.
But your evidence for task design is poor.
Randomness is meaningless, you need to think something else to differentiate your ``Task Design'' to others.
}\yhn{ The point stressed here is ``erasing semantics and exclusive focus on structure/symbolic information'', not randomness. I rewrote the first feature to reduce confusion. That symbolic perspective is actually the major priority (also most distinctive) of this dataset}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/02.RelatedWork.03.tex <==
\begin{figure*}[t]

\centering
\fontsize{9pt}{8.6pt}\selectfont
  \begin{forest}
    for tree={
      align=center,
      % font=\sffamily,
      edge+={thick, -{Stealth[]}},
      l sep'+=10pt,
      fork sep'=10pt,
    },
    forked edges,
    if level=0{
      inner xsep=0pt,
      tikz={\draw [thick] (.children first) -- (.children last);}
    }{},
    [Structure-Rich Texts
      % [Abstract Data Structure [Tree]]
      [Structured Data 
      [Tabular [CSV]]
      [Tree [Custom Language]]]
      [Semi-Structured Data
        [Object Notation
          [JSON]
          [YAML]
          [XML]
        ]
        [Markup Language
          [Markdown]
          [LaTeX]
          [Org]
        ]
      ]
    ]
  \end{forest}
  
\caption{Taxonomy of Structure-Rich Texts covered in StrucText-Eval.}
\label{fig:taxonomy}
\end{figure*}


\subsection{Structural Text Understanding Enhanced Models}

Previous explorations over structural information focused on tasks related to programming languages and graphs. 
\citet{mou2016convolutional} built a tree-based convolutional neural network that outperformed language models on functionality classification tasks and pattern detection tasks over programming languages. % functionality classification, pattern detection
\citet{wang2020detecting} outperformed state of the art~(SOTA) on code clone detection benchmarks, applying graph neural networks on abstract syntax trees~(ASTs) representation augmented by control and data flow edges, which is different in architecture from language models curated for natural language tasks. 
\citet{zhou2019devign} built a graph neural network over rich node representations of code and gained SOTA on vulnerability identification in 4 large-scaled open-source C projects. 
\citet{perozzi2024let} proposed a dedicated graph neural network~(GNN) to encode graph into embedding space of LLMs, and used LLMs as an decoder to solve the graph tasks in GraphQA~\citep{fatemi2023talk}.
\citet{chen2023exploring} explored LLMs' potential in learning graphs, focusing on node classification tasks, using LLMs as enhancers for GNN predictor and directly as predictor.
\citet{chen2024beyond} disclosed the employment of formats other than natural language in CoT reasoning and multi-agent communication significantly enhances model performance while also decreasing token usage on reasoning tasks.


\subsection{Structural Text Understanding Evaluation Datasets}

The similar datasets dedicating to structure information understanding are scarce.
GraphQA~\citep{fatemi2023talk} is a benchmark for assessing LLMs on reasoning over graph data, composed of 7 simple graph tasks, with exploration on methods in encoding graph-structured data as text.
Struc-Bench~\cite{tang2023struc} collect data from open source to evaluate if LLM can generate complex structured tabular text.
\citet{sui2024table} consists of 8 tasks on table-formatted input texts, i.e., input data organized in row-column structures, with studying in input design and prompt enhancement.
\citet{pasupat2015compositional} exposed a dataset of 22,033 complex questions on Wikipedia tables and proposed a parsing algorithm for answering complex questions on semi-structured tables.
For tabular data, \citet{SHWARTZZIV202284} showed that deep models were not a good solution; \citet{NEURIPS2021_9d86d83f} designed two specialized baseline architecture for tabular data and concluded that universally superior solution does not exist.
\citet{wang2024can} is another graph-based problem solving benchmark, with graph structure described with natural language.
\citet{fatemi2023talk} and \citet{sui2024table} include comparison of encoding methods for structure information, i.e., graphs and tables, respectively, showing that LLMs performance varies on different encodings and the relatively vacancy on LLM's understanding of structure-rich texts input.


Our dataset diverges from previous work in two significant ways.
Firstly, our tasks exclusively concentrate on analyzing structural information and executing dependent inference, unlike prior approaches~\citep{mou2016convolutional, zhou2019devign} that employ structural data primarily as an auxiliary tool for classification or semantic comprehension.
StrucText-Eval focus on symbolic structure by erasing content semantics from input texts, preserving only structural details, which renders the texts semantically obscure and the tasks semantically agnostic.
Secondly, our benchmark extends beyond traditional graph reasoning and table information retrieval to include a broader spectrum of structure-rich text types.
It also incorporates comprehensive structure-based inference tasks that are tailored to specific input formats.


==> texs/old_version/03.Dataset.01.tex <==
% TODO remove subsection, use a table to list all markup languages and their tasks
%
%

For discerning the use of terminology, a task is decomposed as three parts, {\color{red}input texts}, {\color{blue} instruction/question}, and {\color{cyan}answer} as following. These term will be used rigorously hereafter.
\begin{quote}
  \texttt{user:}

  \quad {\color{blue} Summarize this article:}

  \quad {\color{red}A long time ago, there is a fox ...}

  \texttt{assistant:}

  \quad {\color{cyan} This article is about ...}
\end{quote}

\input{datamisc.tex}
\subsection{Structure-Rich Texts Taxonomy}
% structure data is a weak formal system
To explore structure-rich texts comprehensively, we propose a dataset for eight structured data types: Tree~(\cite{cormen2022introduction}), Tabular~(\cite{campbell2003history}), JSON~(\cite{pezoa2016foundations}), YAML~(\cite{evans2001yaml}), XML~(\cite{bray1998extensible}), Markdown~(\cite{gruber2012markdown}), LaTeX~(\cite{Lamport1985LatexA}), Org~(\cite{orgModeManualHistory2023}).


Specifically, we categorize 29 tasks designed for the 8 structure-rich texts into 9 class~\autoref{fig:datamisc}.
We have also developed two difficulty levels based on the input length and complexity, such as the height and number of forks in a tree.



\begin{table}[h]
\caption{Structure-Rich Texts Overview}
\label{tb:structtextstaxonomy}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|lll}
\multicolumn{1}{l}{\bf Category}&
\multicolumn{1}{l}{\bf Definition}&
\multicolumn{1}{l}{\bf Application}
\\\hline
  Tree & acyclic connected undirected graph & data structure, backbone of other structure-rich texts\\
  Tabular & row-column structure-rich text & relational database, spreadsheet\\
  JSON & JavaScript Object Notation & object serialization, API response\\
  YAML & YAML Ain't Markup Language & object serialization, service configuration\\
  XML & extensible markup language & object serialization, service configuration, metadata, web pages\\
  Markdown & a lightweight markup & blogging, instant messaging, online forums, notes keeping\\
  ORG & a plain-text markup language & todo list, computational notebooks, literate programming\\
  LaTeX & a typesetting system & academic publishing\\
\end{tabular}
}
\end{center}
\end{table}


% Taxonomy code from https://tex.stackexchange.com/a/256753
\begin{figure}[!ht]
  \begin{forest}
    for tree={
      align=center,
      % font=\sffamily,
      edge+={thick, -{Stealth[]}},
      l sep'+=10pt,
      fork sep'=10pt,
    },
    forked edges,
    if level=0{
      inner xsep=0pt,
      tikz={\draw [thick] (.children first) -- (.children last);}
    }{},
    [Structure-Rich Texts
      [Abstract Data Structure [Tree]]
      [Structured Data [Tabular]]
      [Semi-Structured Data
        [Object Notation
          [JSON]
          [YAML]
          [XML]
        ]
        [Markup Language
          [Markdown]
          [LaTeX]
          [Org]
        ]
      ]
    ]
  \end{forest}
  \label{fig:taxonomy}
  \caption{Taxonomy of Structure-rich Texts covered}
\end{figure}

\subsection{Data Generation}
\label{sec:datacol}


Based on the construction rules in~\ref{ap:rules}, we procedurally generated input texts with randomly formed content to erase the semantics of input text.
And during the procedure of generating input texts, we have collected informations regarding structures, identifiers of markup tags, statistical properties and mapping from tag to contents.
With these information, we can find the ground truth to our designed task by procedurally parsing the generated input text and searching for the ground truth in a depth-first manner.
For the syntax correcting tasks, we incorporated intentional syntax error with a probability, and the input texts for such tasks are constructed individually.

% 配色
% Input/Output
% 分步骤
% Figure Caption
% 给行外人看，反馈意见
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\resizebox{\textwidth}{!}{
\includegraphics{./figures/DataGen.pdf}
}
\end{center}
\caption{Dataset Generation}
\label{fig:eg_gen}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/03.Dataset.02.tex <==
Each sample in StructBench consists of three fields: ``input text,'' ``question,'' and ``ground truth,'' as illustrated in~\autoref{fig:eg_json}. These terms are used consistently throughout this paper.

\yhn{This revision is not deleted since the response and argument are not obvious from editing text. Thus, this one is reserved for reference and may be removed once communicated}
\gzh{This part is not well written, you may refer to my ``DetectBench'' in the following manner:
1. give a figure like the Figure 2 in ``DetectBench''
2. Describe the field of the samples in your benchmark like the ``Question Rewriting'' part in 3.1 section in ``DetectBench''.
3. Your ``input texts'' should be ``context'', context is a standard term used to describe so called input texts, input string, etc.}
\yhn{I think the different fields is self-explaining inside the example given~\autoref{fig:eg_json}. Since the semantic is already straight-forward without mix of question, context and answer, which is generated separately, also evident from the \autoref{sec:datagen}.
  Also I ;ind overloaded semantics for ``context'' in the field of chatbot.
  It could be used to refer to the user-provided ``system'' message that portraits the characteristics of chatbot, e.g., ``you are Shakespeare now''.
  It could also refer to the concept of ``memory'', i.e., information in previous rounds of conversation. It is usually used this way as in ``... ChatGPT maintains/keeps context ...''
  For the purpose of introducing StructBench, I think this terminology clarification by example is clear enough for assisting reader understanding.
}

\input{datamisc.tex}
\subsection{Structure-Rich Texts Taxonomy}
% structure data is a weak formal system
To explore structure-rich texts comprehensively, we propose a dataset for eight structured data types: Tree~(\cite{cormen2022introduction}), Tabular~(\cite{campbell2003history}), JSON~(\cite{pezoa2016foundations}), YAML~(\cite{evans2001yaml}), XML~(\cite{bray1998extensible}), Markdown~(\cite{gruber2012markdown}), LaTeX~(\cite{Lamport1985LatexA}), Org~(\cite{orgModeManualHistory2023}).
\autoref{tb:structtextstaxonomy} offers a brief introduction for each of them. According to application, these input texts are further categorized into three classes as in~\autoref{fig:taxonomy}.

Specifically, we categorize 29 tasks designed for the 8 structure-rich texts into 9 class~(\autoref{fig:datamisc}).
We have also developed two difficulty levels based on the input length and complexity, by controlling the maximum of forks and depth of the underlying abstract syntax tree.



\begin{table}[h]
\caption{Structure-Rich Texts Overview}
\label{tb:structtextstaxonomy}
\begin{center}
\resizebox{\textwidth}{!}{
\begin{tabular}{c|lll}
\multicolumn{1}{l}{\bf Category}&
\multicolumn{1}{l}{\bf Definition}&
\multicolumn{1}{l}{\bf Application}
\\\hline
  Tree & acyclic connected undirected graph & data structure, backbone of other structure-rich texts\\
  Tabular & row-column structure-rich text & relational database, spreadsheet\\
  JSON & JavaScript Object Notation & object serialization, API response\\
  YAML & YAML Ain't Markup Language & object serialization, service configuration\\
  XML & extensible markup language & object serialization, service configuration, metadata, web pages\\
  Markdown & a lightweight markup & blogging, instant messaging, online forums, notes keeping\\
  ORG & a plain-text markup language & todo list, computational notebooks, literate programming\\
  LaTeX & a typesetting system & academic publishing\\
\end{tabular}
}
\end{center}
\end{table}


% Taxonomy code from https://tex.stackexchange.com/a/256753
\begin{figure}[!ht]
  \begin{forest}
    for tree={
      align=center,
      % font=\sffamily,
      edge+={thick, -{Stealth[]}},
      l sep'+=10pt,
      fork sep'=10pt,
    },
    forked edges,
    if level=0{
      inner xsep=0pt,
      tikz={\draw [thick] (.children first) -- (.children last);}
    }{},
    [Structure-Rich Texts
      [Abstract Data Structure [Tree]]
      [Structured Data [Tabular]]
      [Semi-Structured Data
        [Object Notation
          [JSON]
          [YAML]
          [XML]
        ]
        [Markup Language
          [Markdown]
          [LaTeX]
          [Org]
        ]
      ]
    ]
  \end{forest}
  \caption{Taxonomy of Structure-rich Texts covered}
  \label{fig:taxonomy}
\end{figure}

\subsection{Data Generation}\label{sec:datagen}


Based on the construction rules in~\autoref{ap:rules}, we procedurally generated input texts with randomly selected content to erase the semantics of input text.
During the procedure, we collect mapping from tag name to node and some statistical properties.
Next, we find the ground truth to the task by procedurally parsing the generated input text and searching for the ground truth in a depth-first manner~(\autoref{fig:eg_gen}).
For the syntax error tasks, we incorporated potential intentional syntax error, and the input texts for such tasks are constructed individually.

% 配色
% Input/Output
% 分步骤
% Figure Caption
% 给行外人看，反馈意见
\begin{figure}[h]
\begin{center}
\includegraphics[width=\linewidth]{./figures/DataGen.pdf}
\end{center}
\caption{Dataset Generation}
\label{fig:eg_gen}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/03.Dataset.03.tex <==



\subsection{Structure-Rich Texts Taxonomy}
To explore structure-rich texts comprehensively, we propose a dataset for eight structured data types, each categorized within a taxonomy depicted in Fig.~\ref{fig:taxonomy}.
This taxonomy encompasses both structured and semi-structured data formats.
The structured data types include Tree (\cite{cormen2022introduction}), Tabular (\cite{campbell2003history}), and Object Notation such as JSON (\cite{pezoa2016foundations}), YAML (\cite{evans2001yaml}), and XML (\cite{bray1998extensible}).
The semi-structured data types include Markup Languages like Markdown (\cite{gruber2012markdown}), LaTeX (\cite{Lamport1985LatexA}), and Org (\cite{orgModeManualHistory2023}).
Each of these formats is systematically classified in the taxonomy shown in Fig.~\ref{fig:taxonomy}, providing a clear and organized overview of the landscape of our proposed benchmark.


\begin{figure}[t]
\small
  \begin{forest}
    for tree={
      align=center,
      % font=\sffamily,
      edge+={thick, -{Stealth[]}},
      l sep'+=10pt,
      fork sep'=10pt,
    },
    forked edges,
    if level=0{
      inner xsep=0pt,
      tikz={\draw [thick] (.children first) -- (.children last);}
    }{},
    [Structure-Rich Texts
      [Abstract Data Structure [Tree]]
      [Structured Data [Tabular]]
      [Semi-Structured Data
        [Object Notation
          [JSON]
          [YAML]
          [XML]
        ]
        [Markup Language
          [Markdown]
          [LaTeX]
          [Org]
        ]
      ]
    ]
  \end{forest}
  \caption{Taxonomy of Structure-rich Texts covered}
  \label{fig:taxonomy}
  \vspace{-4mm}
\end{figure}

% \begin{figure}[t]
% \begin{center}
% \includegraphics[width=\linewidth]{./figures/DataGen.pdf}
% \end{center}
% \caption{Dataset Generation\gzh{Redraw it.}}
% \label{fig:eg_gen}
% \end{figure}


\begin{wrapfigure}{R}{0.5\textwidth}

\vspace{-20pt}
\begin{center}
\includegraphics[width=\linewidth]{nips2024/figures/DataGeneration.pdf}
\end{center}
\caption{
The illustration of the dataset generation process, Json PathCompose task as example.
}
\label{fig:example}
\vspace{-55pt}
\end{wrapfigure}


\subsection{Dataset Generation}\label{sec:datagen}

The dataset generation process entails constructing an abstract structure tree, manually drafting question templates, and developing corresponding answer discovery algorithms, as exemplified by the JSON PathCompose task depicted in Fig.~\ref{fig:example}. The primary objective of constructing the abstract structure tree is to establish a hierarchically nested structured data template. The complexity of the data increases with the number of nodes configured in this tree.

Eight task categories have been delineated for eight different languages, as detailed in Fig.~\ref{tab:description}. A total of 29 rules have been formulated for these tasks, with the specific rule templates detailed in the Appendix. 
Each data sample in the dataset comprises four main fields: ``Reference'', ``Question'', ``Requirement'' and ``Answer''.
% The dataset entries have been categorized by difficulty based on the length of the generated data and the number of nodes involved. Overall statistics are presented in Fig.~\ref{fig:datamisc}, while detailed statistics for each task and difficulty level, including average lengths of ``Reference'', ``Question'', ``Requirement'' and ``Answer'' and node counts, are enumerated in Tab.~\ref{tab:statistic} in the Appendix.


% 数据集生成过程包括根据任务和语言构建抽象结构树、人工撰写问题模板和对应的答案发现算法，图~\ref{fig:example}中以Json PathCompose为例展示了数据集构建的过程。
% 其中，构建抽象结构树的主要目标在于构建有不断嵌套的结构化数据模板，这一步设置越多的节点，数据就越复杂。

% 我们为8个语言设置了8个任务大类，这些任务的介绍如表~\ref{tab:description}所示。
% 我们总共写了29个规则，具体的规则模板列在Appendix中。
% 最终，我们的每条数据由“Reference”，“Question”，“Requirement”，“Answer”这四个字段组成。
% 我们根据生成数据的长度和节点数为所有数据划分了困难度，总体的统计结果如图~\ref{fig:datamisc}所示，具体每个任务每个难度的平均Reference、Question、Requirement、Answer长度和节点数我们列在了Appendix的表~\ref{tab:statistic}中。



% 这种结构化方法有助于创建包含四个字段的数据集： 参考、问题、要求和答案，这四个字段在表 1 中详细列出，并在附录中作了进一步解释。这种方法可确保在不同的计算任务和语言环境中进行精确的数据操作和模型训练。

% \gzh{
% 1. Describe the sample format we prepare to use.
% 2. Describe all the tasks we set.
% 3. Describe all the rules we prepare for the tasks.
% 4. Describe how we generate the dataset.
% }

% Based on the construction rules in~\autoref{ap:rules}, we procedurally generated input texts with randomly selected content to erase the semantics of input text.
% During the procedure, we collect mapping from tag name to node and some statistical properties.
% Next, we find the ground truth to the task by procedurally parsing the generated input text and searching for the ground truth in a depth-first manner~(\autoref{fig:eg_gen}).
% For the syntax error tasks, we incorporated potential intentional syntax error, and the input texts for such tasks are constructed individually.

% Each sample in StructBench consists of three fields: ``input text'', ``question'' and ``ground truth''. 




% \begin{wrapfigure}{R}{0.5\textwidth}
% \vspace{-25pt}
%     \centering
%     \includegraphics[width=0.5\textwidth]{nips2024/figures/JsonExample.png}
%     \caption{An example of Json sample in Simple TextRetrieval task.}
%     \label{fig:example}
%     \vspace{-60pt}
% \end{wrapfigure}




\input{nips2024/datamisc}



\subsection{Statistic Information}
StructBench has assembled a dataset comprising 6,032 samples, with each of the twenty-nine specific tasks for eight languages containing 208 samples.
These tasks are divided into ``simple'' and ``hard'' categories based on data length and complexity, as depicted in Fig.~\ref{fig:datamisc}.
The dataset is partitioned into training and testing sets at a 9:2 ratio, which supports extensive training while also enabling the evaluation of model generalization on significant volumes of unseen data.
Detailed statistics regarding the number of samples, lengths, and complexity levels across all tasks are detailed in Tab.~\ref{tab:statistic} in Appendix.

% Based on the above eight categories, totaling twenty-nine specific tasks for eight languages，StructBench have gathered a total amount of 3000 samples，每个specific task都有208个sample，并根据数据长度和复杂度分为simple和hard as illustrated in Figure 3。 
% The dataset is divided into training and testing sets with a 9:2 ratio, facilitating substantial training and enabling effective generalization testing on adequate unseen data.
% Detailed statistics on the number of samples, sample lengths, and complexity for all tasks are provided in Table 1 in the Appendix, offering a comprehensive overview essential for understanding dataset characteristics and ensuring rigorous evaluation metrics.





==> texs/old_version/03.Dataset.04.tex <==



\subsection{Structure-Rich Texts Taxonomy}
To explore structure-rich texts comprehensively, we propose a dataset for eight structured data types, each categorized within a taxonomy depicted in Fig.~\ref{fig:taxonomy}.
This taxonomy encompasses both structured and semi-structured data formats.
The structured data types include Tree (\cite{cormen2022introduction}), Tabular (\cite{campbell2003history}), and Object Notation such as JSON (\cite{pezoa2016foundations}), YAML (\cite{evans2001yaml}), and XML (\cite{bray1998extensible}).
The semi-structured data types include Markup Languages like Markdown (\cite{gruber2012markdown}), LaTeX (\cite{Lamport1985LatexA}), and Org (\cite{orgModeManualHistory2023}).
% Each of these formats is systematically classified in the taxonomy shown in Fig.~\ref{fig:taxonomy}, providing a clear and organized overview of the landscape of our proposed benchmark.
% It is important to note that structured data can be represented in various forms.
Within StrucText-Eval, Tabular is stored in CSV format, whereas Tree is denoted by a custom format that nodes are represented as string "xxx", connected with "->" and separated by "\textbackslash n". 
For examples encompassing all languages and tasks, please refer to Sec.~\ref{ap:samples} in the Appendix.




\input{statistic_table}

\begin{figure}[t]
\begin{center}
\includegraphics[width=\linewidth]{figures/datageneration.png}
\end{center}
\caption{
The illustration of the dataset generation process, the Json PathCompose task, is an example.
}
\label{fig:example}
\vspace{-5mm}
\end{figure}


\subsection{Dataset Generation}\label{sec:datagen}

An example of JSON's PathCompose is shown in Fig.~\ref{fig:example} to illustrate the dataset generation process.
The generation process mainly entails constructing an abstract structure tree, manually drafting question templates, and developing corresponding answer discovery algorithms.
The primary objective of constructing the abstract structure tree is establishing a hierarchically nested structured data template. The complexity of the sample increases when more nodes are set in this tree.

Eight task categories have been delineated for eight languages, as detailed in Fig.~\ref{tab:description}.
29 rules and question templates have been formulated for these tasks, with the specific rule templates detailed in Sec.~\ref{ap:rules} in the Appendix.
Each sample in the dataset comprises four main fields: ``Reference'', ``Question'', ``Requirement'' and ``Answer''.
We give examples for each language and task in Sec.~\ref{ap:samples} in the Appendix. 

\input{datamisc_new}
% \input{datamisc}



\subsection{Statistic Information}
StrucText-Eval has assembled two dataset.
StrucText-Eval-Test comprising 3,712 samples, and StrucText-Eval-Test-Hard comprising 2,088 samples. 
With each of the 29 specific tasks for eight languages as depicted in Fig.~\ref{fig:datamisc}.
Detailed statistics regarding the number of samples, lengths, and complexity levels across all tasks, languages and difficulties are detailed in Tab.~\ref{tab:statistic}.





==> texs/old_version/04.ExperimentSetup.03.tex <==
To evaluate the current capability of large language models (LLMs) on processing structure-rich text and executing dependent inference, we conducted a series of experiments using StructBench across various settings. Our study utilizes both prompt-based and fine-tuning methods to analyze the performance variations.




\subsection{Models}
The models evaluated in the experiments include \textbf{OpenLLaMA 7B v1}, which we fine-tuned under several conditions with partially frozen parameters.
Alongside OpenLLaMA, we tested five additional LLMs accessed through public APIs: \textbf{GPT4}, \textbf{GPT4 Turbo}, \textbf{MINIMAX}, \textbf{SPARK}, and \textbf{ERNIE}.
Each model's performance was scrutinized under different operational conditions detailed in Appendix~\ref{}.




\subsection{Prompt-based Method}
We assessed the influence of prompt design on LLM performance by employing four distinct prompt settings:
\textbf{Naive}: This setting involves appending the question directly after the input text, serving as a straightforward task formulation.
\textbf{Hint Elicitation}: In this configuration, the model generates hints prior to exposure to the input texts, aimed at facilitating task resolution~\citep{wei2022chain}. 
\textbf{Few-Shot Demonstration}: This approach leverages the principles of few-shot learning~\citep{fei2006one}, with variations including one and two example instances to guide the model.
\textbf{Rule Hint}: This setup incorporates manually crafted, step-by-step guidance appended after the input text to aid the inference process.




\subsection{Finetune-based Method}
We further explored the efficacy of fine-tuning OpenLLaMA 7B v1 using various subsets of data. Our fine-tuning configurations are described as follows:
\textbf{Base}: Utilizes the core StructBench dataset, referred to as the base StructBench setting.
\textbf{2-Shot}: Implements a few-shot (2-shot) learning strategy within the StructBench framework.
% \textbf{Mix}: A hybrid dataset that replaces half of the base StructBench samples with entries from ShareGPT, using only the initial rounds of interaction.
\textbf{Rule Hint}: Adapts StructBench by appending a new task-specific rule hint to each sample, effectively redefining the input text as a combination of the question, answer, and original input, with the answer delineated as a step-by-step procedure.
\textbf{RuleHintMix}: A composite dataset blending {RuleHint, Base with appended rule hint, Base} in a ratio of 1:1:3, aiming to investigate the impact of rule hints across different dataset compositions.



% To evaluate LLMs current capability on processing structure-rich text and executing dependent inference, we evaluated LLMs performance on StructBench with different prompt settings.
% Additionally, we fine-tuned OpenLLaMA 7B v1\citep{openlm2023openllama} on varied dataset settings, with parameters partially frozen.

% \subsection{Models}

% \subsection{Prompt-based Method}

% With a dataset composed of 6032 samples, we evaluated on 5 LLMs through public API, namely GPT4, GPT4 turbo, MINIMAX,\footnote{\url{https://api. minimax. chat/v1/text/chatcompletion_pro}} SPARK,\footnote{\url{ws://spark-api.xf-yun.com/v1.1/chat}} and ERNIE,\footnote{\url{https://aip.baidubce.com/rpc/2.0/ai_custom/v1/wenxinworkshop/chat/eb-instant}} across 4 prompt settings.

% \textbf{Base} prompt setting only provides question concatenated after input text.
% \textbf{Hint Elicitation} prompts LLM to generate some hints for overcoming difficulties of the provided task~\citep{wei2022chain}.
% We use an eliciting query to have LLM generate some key points before seeing the input texts~\autoref{fig:framework_hint}.
% After the Hint Elicitation, we repeat base setting experiments with the hints appended at the end of input text.
% \textbf{Few-Shot} applies the few-shot learning~\citep{fei2006one}, with 1 and 2 examples.
% \textbf{Rule Hint} appends manually crafted step-by-step guidance~(\autoref{ap:rhs}) after input text, to support the inference procedure.

% \subsection{Finetune-based Method}
% We also fine-tuned OpenLLaMA 7B v1 to evaluate the effectiveness of fine-tuning.
% Specifically, we employed the following training data settings when partially fine-tuning OpenLLaMA 7B v1.\footnote{See ~\autoref{fig:tlllama} for the training loss for different settings}


% \textbf{Base} setting uses pure StructBench, also referred to as base StructBench.
% \textbf{2-Shot}: Few-shot (2-shot) version of StructBench.
% \textbf{Mix} is a variant of Base with half of samples replaced by samples from ShareGPT.\footnote{\url{https://huggingface.co/datasets/shibing624/sharegpt_gpt4}; only the first rounds were used}
% \textbf{RuleHint} is a StructBench based dataset with new task questioning rule hint, the step-by-step procedure to find the answer.
% Thus, new input text becomes the concatenation of question, answer, and original input text, and new answer is the step-by-step procedure.
% This setting is referred to as Rule Hint.
% \textbf{RuleHintMix}: Mix of \{RuleHint, Base but with rule hint appended,\footnote{same task as Base} Base\}, by ratio of 1:1:3. 


==> texs/old_version/04.Experiments.01.tex <==


To evaluate LLMs current capability on processing structure-rich text and executing dependent inference, we evaluated LLMs performance on StructBench with different prompt settings.
Additionally, we fine-tuned OpenLLaMA 7B v1\citep{openlm2023openllama} on varied dataset settings, with parameters partially frozen.

\subsection{API Test}

% expr setting add cite, footnote url
% 用（wraptable）表格罗列，api 列上时间信息
With a dataset composed of 6032 samples, we evaluated on 5 LLMs through public API, namely GPT4, GPT4 turbo, MINIMAX \footnote{\url{https://api. minimax. chat/v1/text/chatcompletion_pro}}, SPARK\footnote{\url{ws://spark-api.xf-yun.com/v1.1/chat}} and ERNIE \footnote{\url{https://aip.baidubce.com/rpc/2.0/ai_custom/v1/wenxinworkshop/chat/eb-instant}}, across 4 prompt settings.

% ====== prompt engineering ======
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/HintFramework}
\end{center}
\caption{Process of eliciting hint from LLMs to improve prompt}
\label{fig:framework_hint}
\end{figure}
\textbf{Base} prompt setting only provides question concatenated after input text.
\textbf{Hint Elicitation} prompts LLM to generate some hints for overcoming difficulties of the provided task~\citep{wei2022chain}.
We use an eliciting query to have LLM generate some key points before seeing the input texts~\autoref{fig:framework_hint}.
After the Hint Elicitation, we repeat base setting experiments with the hints appended at the end of input text.
\textbf{Few-Shot} applies the few-shot learning~\citep{fei2006one}, with 1 and 2 examples.
\textbf{Rule Hint} appends manually crafted step-by-step guidance~(\ref{ap:rhs}) after input text, to support the inference procedure.

\subsection{Model Fine-Tune}
% setting: model parameter, training parameter
We also fine-tuned OpenLLaMA 7B v1 to evaluate the effectiveness of fine-tuning.
Specifically, we employed the following training data settings when partially fine-tuning OpenLLaMA 7B v1\footnote{See ~\autoref{fig:tlllama} for the training loss for different settings}.

\gzh{You need to list the hyper-parameters of your training.}

\textbf{Base} setting uses pure StructBench, also referred to as base StructBench.
\textbf{2-Shot}: Few-shot (2-shot) version of StructBench.
\textbf{Mix} is a variant of Base with half of samples replaced by samples from ShareGPT\footnote{\url{https://huggingface.co/datasets/shibing624/sharegpt_gpt4}; only the first rounds were used}.
\textbf{RuleHint} is a StructBench based dataset with new task questioning rule hint, the step-by-step procedure to find the answer.
Thus, new input text becomes the concatenation of question, answer, and original input text, and new answer is the step-by-step procedure.
This setting is referred to as Rule Hint.
\textbf{RuleHintMix}: Mix of \{RuleHint, Base but with rule hint appended\footnote{same task as Base}, Base\}, by ratio of 1:1:3. % 1:1:3 = rule_hint, q_with_rule, struct

\section{Analysis} \label{sec:analysis}

\subsection{API Test}

This section analyses the effects of various prompt settings and compares the performance of models across input types.

% Observations
\textbf{Method} comparison is shown in~\autoref{fig:judgeapimethod} and explored afterwards immediately.

\input{./plotdata/GPTJudgeForAPIMethod.tex}

\textit{Hints Elicitation} resulted in a marginal performance enhancement for SPARK and MINIMAX, whereas it proved to be detrimental to the performance of other models.
CoT processing exhibited a minimal improvement in logical inference capabilities based on structural information, and for some models, it was detrimental.

\textit{Rule Hint} adversely impacts all models with a base setting accuracy greater than 0.1.
This observation suggests that guidance on structural tasks, when articulated in natural language, hinders the models' ability to successfully execute these tasks.

\textit{Few-Shot Learning} led to a significant improvement in performance across all models, with the notable exception of SPARK in the 1-shot scenario.
For the GPT4 series, a 1-shot approach yielded only a negligible enhancement.
This demonstrates that in-context learning is an effective strategy for addressing structural tasks, and the number of examples provided directly influences the extent of performance improvement.

\textit{GPT4} series consistently surpassed other models in performance, indicating a notable disparity.
The base model of GPT4 outperforms its turbo version, which underlines the efficacy and capability of the base model over turbo version on structural tasks.

% heatmap chagne to barplot
% heatmap save for slides/pre
% change the light color in Fig 1
\textbf{Input Text Type} comparison is shown in~\autoref{fig:judgeapitype}.

\input{./plotdata/GPTJudgeForAPIType.tex}

\textit{Object Notation} received highest scores across all models.
Object Notation$>$Markup$\approx$Tabular$>$Tree is a score order identified for GPT4 and MINIMAX, with a 0.2-0.3 gap between each level.
For SPARK and ERNIE, the inequality becomes Object Notation$\gg$Markup $\approx$ Tabular $\approx$ Tree.
This pattern shows a structure processing capability bias based on the type of input texts, indicating a preference for Object Notation as the encoding format for structural information.

\textit{ORG} stands out as an outlier among markup languages, scoring significantly lower than the other two.
This performance gap could stem from the scarcity or absence of ORG format in the training datasets used for LLMs.
This observation implies that LLMs' ability to handle structural tasks relies heavily on exposure to same formats during pre-training, revealing a constrained generalization to unfamiliar formats\footnote{The tasks designed for Markdown, ORG, and LaTeX are rigidly identical}.

\subsection{Fine-Tune}

This section analyses the impact on performance of fine-tuning with different datasets settings.
\autoref{fig:judgeftmethod} shows GPTJudge scores for different finetuned models.

\input{./plotdata/GPTJUDGEForFT.tex}

\textit{Pretrained Model} shows little capability of executing structural tasks, with an accuracy as low as 0.0647, the red base line score in \autoref{fig:judgeftmethod}.
This demonstrates a significant gap of structural ability between open models and commercial models.

\textit{Finetuned Models} scored considerably higher than the vanilla version, achieving the highest accuracy of 0.5, although this is still numerically low compared to commercial LLMs.
This result draws attention to the inherent difference between natural language tasks and structural tasks.

\textit{Few Shot Data} adversely influenced the performance, scoring 0.24, compared to a higher score of 0.5 from the base model without few-shot examples.
The regression, combined with the highest finetuned model scoring only 0.5, foreshadows the finetune method's inability to effectively aid in comprehending structural information and tasks.
This necessitates exploring alternative approaches to obtaining enhanced structure processing ability.

\textit{Mixing StructBench with ShareGPT Data} also degenerate the structural competency, receiving a score of 0.31, only marginally higher than the few-shot data finetuned model.
This observation also confirmed the drastic difference in capability between structural tasks and natural language tasks.

\textit{Mixing StructBench with two RuleHint Variants} scored 0.47, slightly lower than the base setting, suggesting that the additional auxiliary information from RuleHint did not provide a positive performance gain.

\textit{Finetuning on RuleHint Generation Tasks} severely downgraded the model's ability in structural tasks, showing a lack of generalizability in the finetuning process and an inability to effectively utilize the provided structural processing guidance.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/04.Experiments.02.tex <==


To evaluate LLMs current capability on processing structure-rich text and executing dependent inference, we evaluated LLMs performance on StructBench with different prompt settings.
Additionally, we fine-tuned OpenLLaMA 7B v1\citep{openlm2023openllama} on varied dataset settings, with parameters partially frozen.

\subsection{API Test}

% expr setting add cite, footnote url
% 用（wraptable）表格罗列，api 列上时间信息
With a dataset composed of 6032 samples, we evaluated on 5 LLMs through public API, namely GPT4, GPT4 turbo, MINIMAX \footnote{\url{https://api. minimax. chat/v1/text/chatcompletion_pro}}, SPARK\footnote{\url{ws://spark-api.xf-yun.com/v1.1/chat}} and ERNIE \footnote{\url{https://aip.baidubce.com/rpc/2.0/ai_custom/v1/wenxinworkshop/chat/eb-instant}}, across 4 prompt settings.

% ====== prompt engineering ======
\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=1.0\linewidth]{./figures/HintFramework}
\end{center}
\caption{Process of eliciting hint from LLMs to improve prompt}
\label{fig:framework_hint}
\end{figure}
\textbf{Base} prompt setting only provides question concatenated after input text.
\textbf{Hint Elicitation} prompts LLM to generate some hints for overcoming difficulties of the provided task~\citep{wei2022chain}.
We use an eliciting query to have LLM generate some key points before seeing the input texts~\autoref{fig:framework_hint}.
After the Hint Elicitation, we repeat base setting experiments with the hints appended at the end of input text.
\textbf{Few-Shot} applies the few-shot learning~\citep{fei2006one}, with 1 and 2 examples.
\textbf{Rule Hint} appends manually crafted step-by-step guidance~(\autoref{ap:rhs}) after input text, to support the inference procedure.

\subsection{Model Fine-Tune}
% setting: model parameter, training parameter
We also fine-tuned OpenLLaMA 7B v1 to evaluate the effectiveness of fine-tuning.
Specifically, we employed the following training data settings when partially fine-tuning OpenLLaMA 7B v1\footnote{See ~\autoref{fig:tlllama} for the training loss for different settings}.


\textbf{Base} setting uses pure StructBench, also referred to as base StructBench.
\textbf{2-Shot}: Few-shot (2-shot) version of StructBench.
\textbf{Mix} is a variant of Base with half of samples replaced by samples from ShareGPT\footnote{\url{https://huggingface.co/datasets/shibing624/sharegpt_gpt4}; only the first rounds were used}.
\textbf{RuleHint} is a StructBench based dataset with new task questioning rule hint, the step-by-step procedure to find the answer.
Thus, new input text becomes the concatenation of question, answer, and original input text, and new answer is the step-by-step procedure.
This setting is referred to as Rule Hint.
\textbf{RuleHintMix}: Mix of \{RuleHint, Base but with rule hint appended\footnote{same task as Base}, Base\}, by ratio of 1:1:3. % 1:1:3 = rule_hint, q_with_rule, struct

\section{Analysis} \label{sec:analysis}

\subsection{API Test}

This section analyses the effects of various prompt settings and compares the performance of models across input types.

% Observations
\textbf{Method} comparison is shown in~\autoref{fig:judgeapimethod} and explored afterwards immediately.

\input{./plotdata/GPTJudgeForAPIMethod.tex}

\textit{Hints Elicitation} resulted in a marginal performance enhancement for SPARK and MINIMAX, whereas it proved to be detrimental to the performance of other models.
CoT processing exhibited a minimal improvement in logical inference capabilities based on structural information, and for some models, it was detrimental.

\textit{Rule Hint} adversely impacts all models with a base setting accuracy greater than 0.1.
This observation suggests that guidance on structural tasks, when articulated in natural language, hinders the models' ability to successfully execute these tasks.

\textit{Few-Shot Learning} led to a significant improvement in performance across all models, with the notable exception of SPARK in the 1-shot scenario.
For the GPT4 series, a 1-shot approach yielded only a negligible enhancement.
This demonstrates that in-context learning is an effective strategy for addressing structural tasks, and the number of examples provided directly influences the extent of performance improvement.

\textit{GPT4} series consistently surpassed other models in performance, indicating a notable disparity.
The base model of GPT4 outperforms its turbo version, which underlines the efficacy and capability of the base model over turbo version on structural tasks.

% heatmap chagne to barplot
% heatmap save for slides/pre
% change the light color in Fig 1
\textbf{Input Text Type} comparison is shown in~\autoref{fig:judgeapitype}.

\input{./plotdata/GPTJudgeForAPIType.tex}

\textit{Object Notation} received highest scores across all models.
Object Notation$>$Markup$\approx$Tabular$>$Tree is a score order identified for GPT4 and MINIMAX, with a 0.2-0.3 gap between each level.
For SPARK and ERNIE, the inequality becomes Object Notation$\gg$Markup $\approx$ Tabular $\approx$ Tree.
This pattern shows a structure processing capability bias based on the type of input texts, indicating a preference for Object Notation as the encoding format for structural information.

\textit{ORG} stands out as an outlier among markup languages, scoring significantly lower than the other two.
This performance gap could stem from the scarcity or absence of ORG format in the training datasets used for LLMs.
This observation implies that LLMs' ability to handle structural tasks relies heavily on exposure to same formats during pre-training, revealing a constrained generalization to unfamiliar formats\footnote{The tasks designed for Markdown, ORG, and LaTeX are rigidly identical}.

\subsection{Fine-Tune}

This section analyses the impact on performance of fine-tuning with different datasets settings.
\autoref{fig:judgeftmethod} shows GPTJudge scores for different finetuned models.

\input{./plotdata/GPTJUDGEForFT.tex}

\textit{Pretrained Model} shows little capability of executing structural tasks, with an accuracy as low as 0.0647, the red base line score in \autoref{fig:judgeftmethod}.
This demonstrates a significant gap of structural ability between open models and commercial models.

\textit{Finetuned Models} scored considerably higher than the vanilla version, achieving the highest accuracy of 0.5, although this is still numerically low compared to commercial LLMs.
This result draws attention to the inherent difference between natural language tasks and structural tasks.

\textit{Few Shot Data} adversely influenced the performance, scoring 0.24, compared to a higher score of 0.5 from the base model without few-shot examples.
The regression, combined with the highest finetuned model scoring only 0.5, foreshadows the finetune method's inability to effectively aid in comprehending structural information and tasks.
This necessitates exploring alternative approaches to obtaining enhanced structure processing ability.

\textit{Mixing StructBench with ShareGPT Data} also degenerate the structural competency, receiving a score of 0.31, only marginally higher than the few-shot data finetuned model.
This observation also confirmed the drastic difference in capability between structural tasks and natural language tasks.

\textit{Mixing StructBench with two RuleHint Variants} scored 0.47, slightly lower than the base setting, suggesting that the additional auxiliary information from RuleHint did not provide a positive performance gain.

\textit{Finetuning on RuleHint Generation Tasks} severely downgraded the model's ability in structural tasks, showing a lack of generalizability in the finetuning process and an inability to effectively utilize the provided structural processing guidance.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:


==> texs/old_version/05.Analysis.01.tex <==
\input{nips2024/overall_performance_tables}

\subsection{API Test}

This section analyses the effects of various prompt settings and compares the performance of models across input types.

% Observations
\textbf{Method} comparison is shown in~\autoref{fig:judgeapimethod} and explored afterwards immediately.

\input{./plotdata/GPTJudgeForAPIMethod.tex}

\textit{Hints Elicitation} resulted in a marginal performance enhancement for SPARK and MINIMAX, whereas it proved to be detrimental to the performance of other models.
CoT processing exhibited a minimal improvement in logical inference capabilities based on structural information, and for some models, it was detrimental.

\textit{Rule Hint} adversely impacts all models with a base setting accuracy greater than 0.1.
This observation suggests that guidance on structural tasks, when articulated in natural language, hinders the models' ability to successfully execute these tasks.

\textit{Few-Shot Learning} led to a significant improvement in performance across all models, with the notable exception of SPARK in the 1-shot scenario.
For the GPT4 series, a 1-shot approach yielded only a negligible enhancement.
This demonstrates that in-context learning is an effective strategy for addressing structural tasks, and the number of examples provided directly influences the extent of performance improvement.

\textit{GPT4} series consistently surpassed other models in performance, indicating a notable disparity.
The base model of GPT4 outperforms its turbo version, which underlines the efficacy and capability of the base model over turbo version on structural tasks.

% heatmap chagne to barplot
% heatmap save for slides/pre
% change the light color in Fig 1
\textbf{Input Text Type} comparison is shown in~\autoref{fig:judgeapitype}.

\input{./plotdata/GPTJudgeForAPIType.tex}

\textit{Object Notation} received highest scores across all models.
Object Notation$>$Markup$\approx$Tabular$>$Tree is a score order identified for GPT4 and MINIMAX, with a 0.2-0.3 gap between each level.
For SPARK and ERNIE, the inequality becomes Object Notation$\gg$Markup $\approx$ Tabular $\approx$ Tree.
This pattern shows a structure processing capability bias based on the type of input texts, indicating a preference for Object Notation as the encoding format for structural information.

\textit{ORG} stands out as an outlier among markup languages, scoring significantly lower than the other two.
This performance gap could stem from the scarcity or absence of ORG format in the training datasets used for LLMs.
This observation implies that LLMs' ability to handle structural tasks relies heavily on exposure to same formats during pre-training, revealing a constrained generalization to unfamiliar formats.\footnote{The tasks designed for Markdown, ORG, and LaTeX are rigidly identical}

\subsection{Fine-Tune}

This section analyses the impact on performance of fine-tuning with different datasets settings.
\autoref{fig:judgeftmethod} shows GPTJudge scores for different finetuned models.

\input{./plotdata/GPTJUDGEForFT.tex}

\textit{Pretrained Model} shows little capability of executing structural tasks, with an accuracy as low as 0.0647, the red base line score in \autoref{fig:judgeftmethod}.
This demonstrates a significant gap of structural ability between open models and commercial models.

\textit{Finetuned Models} scored considerably higher than the vanilla version, achieving the highest accuracy of 0.5, although this is still numerically low compared to commercial LLMs.
This result draws attention to the inherent difference between natural language tasks and structural tasks.

\textit{Few Shot Data} adversely influenced the performance, scoring 0.24, compared to a higher score of 0.5 from the base model without few-shot examples.
The regression, combined with the highest finetuned model scoring only 0.5, foreshadows the finetune method's inability to effectively aid in comprehending structural information and tasks.
This necessitates exploring alternative approaches to obtaining enhanced structure processing ability.

\textit{Mixing StructBench with ShareGPT Data} also degenerate the structural competency, receiving a score of 0.31, only marginally higher than the few-shot data finetuned model.
This observation also confirmed the drastic difference in capability between structural tasks and natural language tasks.

\textit{Mixing StructBench with two RuleHint Variants} scored 0.47, slightly lower than the base setting, suggesting that the additional auxiliary information from RuleHint did not provide a positive performance gain.

\textit{Finetuning on RuleHint Generation Tasks} severely downgraded the model's ability in structural tasks, showing a lack of generalizability in the finetuning process and an inability to effectively utilize the provided structural processing guidance.

==> texs/old_version/05.Analysis.02.tex <==
% \input{nips2024/overall_performance_tables}
\input{nips2024/overall_performance_tables.04}


% \subsection{Close Sourced LLMs' Performance}

% \subsubsection{Performance on different languages}
% The performance of closed-source LLMs on structured text processing tasks across different languages (JSON, LaTeX, Markdown, ORG, SQL, Tree, XML, and YAML) varied significantly. The models including GPT4 Turbo and GPT4 demonstrated strong capabilities, especially in handling JSON, where both models achieved high scores above 0.816 and 1.000 respectively in the naive prompt setting. Meanwhile, models like SPARK and ERNIE Turbo struggled, with SPARK showing very low scores in Markdown and ORG, and ERNIE Turbo performing poorly across all languages, notably below 0.200 in several categories.

% \subsubsection{Performance on different tasks}
% In task-specific performances, GPT4 Turbo and GPT4 again showed promising results in structured tasks like processing YAML, SQL, and JSON, with GPT4 achieving the highest performance in YAML with a score of 0.950 under the 2-shot setting. The Rule Hint approach generally improved performance across most models and tasks, suggesting its effectiveness in guiding the LLMs through structured tasks. However, ERNIE Turbo and SPARK underperformed significantly compared to GPT models, struggling to handle tasks across most languages with lower adaptability to varying prompt settings.

% \subsection{Finetuned LLMs' Performance}

% \subsubsection{Performance on different languages}
% Finetuned versions of OpenLLaMA 7B v1 exhibited notable improvements when comparing the Base and 2-Shot settings across different languages. The 2-Shot setting, in particular, provided higher scores consistently across languages such as JSON and LaTeX, highlighting the effectiveness of few-shot learning in enhancing model performance on structure-rich text.

% \subsubsection{Performance on different tasks}
% When analyzing task-specific performance, the finetuned models showed increased capability in handling complex tasks like syntactic tree understanding (Tree) and theorem proving (TH) with the 2-Shot and RuleHintMix settings. The RuleHint setting notably enhanced performance in tasks that required detailed step-by-step reasoning, such as theorem proving, suggesting that explicit procedural guidance significantly aids the model's reasoning processes. Interestingly, the Mix and RuleHintMix settings did not always lead to higher scores, indicating that the inclusion of mixed data sources might introduce variability in model performance depending on the task and language involved.


\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{nips2024/figures/scatter_sample.png}
    \caption{The performance of GPT-4 across all samples is distributed according to ``Reference Length'' and ``Nodes Number''.}
    \label{fig:enter-label}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{nips2024/figures/heatmap_language_task.png}
    \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance''.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{nips2024/figures/All_Language.png}
    \caption{All finetune methods and their performance on all languages.}
    \label{fig:enter-label}
    \includegraphics[width=\textwidth]{nips2024/figures/All_Task.png}
    \caption{All finetune methods and their performance on all languages.}
    \label{fig:enter-label}
\end{figure}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\textwidth]{nips2024/figures/heatmap_languages.png}
%     \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance'' on different languages.}
%     \label{fig:enter-label}
%     \includegraphics[width=\textwidth]{nips2024/figures/heatmap_tasks.png}
%     \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance'' on different tasks.}
%     \label{fig:enter-label}
% \end{figure}




% \begin{figure}[t]
% \begin{subfigure}{0.44\textwidth}
% \centering
% \includegraphics[width=\textwidth]{nips2024/figures/heatmap_performance.png}
% \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance''.
% To facilitate the observation of correlations, the Performance values in the table have been inverted from their real values in order to display a positive correlation.}
% \label{fig:correlation_performance}
% \end{subfigure}\hfill
% \begin{subfigure}{0.55\textwidth}
% \centering
% \includegraphics[width=\textwidth]{nips2024/figures/scatter_sample.png}
% \caption{The performance of GPT-4 across all samples is distributed according to ``Reference Length'' and ``Nodes Number''.}
% \label{fig:performance_distribute}
% \end{subfigure}
% \end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_JSON.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_LaTeX.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_Markdown.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_ORG.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_SQL.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_Tree.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_XML.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_YAML.png}
%     \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance'' on different languages.}
%     \label{fig:enter-label}
% \end{figure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/path.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_LaTeX.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_Markdown.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_ORG.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_SQL.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_Tree.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_XML.png}
%     \includegraphics[width=0.245\textwidth]{nips2024/figures/heatmaps_on_language/heatmap_on_YAML.png}
%     \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance'' on different tasks.}
%     \label{fig:enter-label}
% \end{figure}



\subsection{Close Sourced LLMs' Performance}

In this section, we analyze the performance of close-sourced large language models (LLMs) across various structure-rich text tasks. The performance evaluation included several models such as GPT-4, Minimax, Spark, and Ernie\_turbo, each assessed using different prompting methods including base, 1-shot, 2-shot, and rule hint.

\subsubsection{Performance Across Different Languages}

Table 1 indicates the performance metrics for each model across various structured text languages such as JSON, LaTeX, Markdown, ORG, SQL, Tree, XML, and YAML. Notably, GPT-4 exhibited the highest overall performance with significant accuracy in handling JSON (0.784) and YAML (0.750) formats. Minimax showed substantial improvement with 2-shot prompts, achieving an accuracy of 0.651 across tasks.

\subsubsection{Task-Specific Performance}

Table 2 presents the performance of the models on different task types, including PathCompose, PathWalk, Syntax, TextRetrieval, SQL.Join, Statistics, Tree.Depth, and Tree.Height. GPT-4 and Minimax excelled in tasks requiring complex inference and structured understanding, with GPT-4 achieving 0.375 accuracy in Tree.Depth and Minimax 0.625 in PathWalk. However, tasks like Tree.Depth and Tree.Height were particularly challenging, reflecting the models' difficulties in deep hierarchical reasoning.

\subsubsection{Correlation Analysis}

Figures 4 and 5 illustrate the distribution of GPT-4's performance based on reference length and node number, and the correlation among node number, reference length, and model performance. These visualizations reveal that longer reference lengths and higher node counts generally lead to decreased performance, highlighting the complexity that larger and deeper structures introduce to the models.

\subsection{Finetuned LLMs' Performance}

The performance of fine-tuned models was also evaluated, focusing on OpenLLaMA 7B v1 fine-tuned under various conditions. The configurations included base, 2-shot, rule hint, and RuleHintMix settings.

\subsubsection{Impact of Fine-Tuning Methods}

Figure 6 shows the performance of different fine-tuning methods across all languages. The results indicate that fine-tuning had limited success in improving the models' capabilities in handling structure-rich texts. While few-shot learning demonstrated some improvement, particularly in tasks like PathCompose and TextRetrieval, the overall gains were modest.

\subsubsection{Detailed Analysis of Rule Hint Method}

Figure 7 highlights the effectiveness of the rule hint method across different tasks. The addition of rule hints provided step-by-step guidance, which helped in some cases but did not consistently enhance performance across all tasks. This suggests that while rule hints can aid in specific scenarios, they are not a universal solution for improving model performance on structured text tasks.


\section{Case Studty}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\linewidth]{nips2024/figures/JSON_case_study.png}\hfill
    \includegraphics[width=0.49\linewidth]{nips2024/figures/SQL_case_study.png}
    \caption{Cases for performance of different LLMs and finetuned stages on Structured Text.}
    \label{fig:case}
\end{figure}


In assessing the performance of large language models (LLMs) on structured text, particular attention is given to their ability to interpret and manipulate data within JSON and SQL formats, as illustrated in Table ~\ref{tab:case}. The models' understanding of complex data structures and their accuracy in fulfilling specific requirements are of primary concern, along with how these capabilities evolve through the process of finetuning.

The JSON task required the model to identify deeply nested objects lacking list or dictionary values. The response from the GPT4\_turbo model, which had not undergone finetuning, correctly pinpointed the most nested object, as verified against the ground truth provided. This demonstrates the model's inherent capability to navigate and interpret nested JSON data structures accurately without additional training.

Conversely, the SQL task, which involved identifying individuals from a structured dataset based on a specific height criterion, presented a more challenging scenario for the model. Initially, the model, even after 300 finetuning steps, inaccurately reported the number of qualifying individuals, highlighting a lack of understanding in correlating data across joined SQL tables and applying numerical criteria correctly. Continued finetuning over 1200 steps did not rectify this error, suggesting either an inadequacy in the finetuning process or a need for more comprehensive training data specific to this task. However, a substantial improvement was observed after extending the finetuning to 5100 steps, where the model's response aligned perfectly with the ground truth.

This progression underscores the potential for LLMs to enhance their performance on structured tasks through finetuning. It also illustrates the necessity for substantial and targeted training iterations to refine the models' capabilities in accurately executing complex data manipulations, as simple initial training might not suffice. Such insights are crucial for developing more robust models that can reliably interpret and respond to structured data queries in diverse applications.


% \input{nips2024/case_study_table}

% \section{Conclusion}

% The experiments demonstrate significant variations in the performance of LLMs when dealing with structure-rich texts. Close-sourced models like GPT-4 showed strong performance across multiple tasks, particularly with JSON and YAML formats, whereas fine-tuned models displayed limited improvements. The findings highlight the need for more robust strategies to enhance LLMs' generalizability and effectiveness in processing and reasoning over structured data.







% \section{Conclusion}

% The experiments demonstrate significant variations in the performance of LLMs when dealing with structure-rich texts. Close-sourced models like GPT-4 showed strong performance across multiple tasks, particularly with JSON and YAML formats, whereas fine-tuned models displayed limited improvements. The findings highlight the need for more robust strategies to enhance LLMs' generalizability and effectiveness in processing and reasoning over structured data.



==> texs/old_version/05.Analysis.03.tex <==

% \input{nips2024/overall_performance_tables.01}

% \input{nips2024/overall_performance_tables.02}

% \input{nips2024/overall_performance_tables.03}

% \input{nips2024/overall_performance_tables.04}

% \input{nips2024/data_tabs}
\input{nips2024/overall_performance_tables.04}

\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{nips2024/figures/scatter_sample.png}
    \caption{The performance of GPT4-Turbo across all samples is distributed according to ``Reference Length'' and ``Nodes Number''. Note that ``#Reference'' represents the character number in a sample.}
    \label{fig:scatter}
\end{figure}
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{nips2024/figures/heatmap_language_task.png}
    \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance''.}
    \label{fig:heat}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{nips2024/figures/All_Language.png}
    \caption{All finetune methods and their performance on all languages.}
    \label{fig:ft_language}
    \includegraphics[width=\textwidth]{nips2024/figures/All_Task.png}
    \caption{All finetune methods and their performance on all languages.}
    \label{fig:ft_task}
\end{figure}
\subsection{Close Sourced LLMs' Performance}

In this section, we analyze the performance of close-sourced LLMs across various structure-rich text tasks and languages. 
% The performance evaluation included several models such as GPT4, GPT4-Turbo, Minimax, Spark, and Ernie-turbo, each assessed using different prompting methods including base, 1-shot, 2-shot, and rule hint.
Tab.~\ref{tab:api_on_language} and Tab.~\ref{tab:api_on_task} reveals the overall performance, and detail analsis is as follow:

\subsubsection{Overall Performance}

The experiments revealed that GPT-4 consistently outperformed other models across most tasks and languages.
Specifically, GPT-4 achieved an average accuracy of 78.4 in all languages and tasks, which was significantly higher than the next best model, GPT4-turbo, which had an accuracy of 69.3.
The marked disparity in performance between GPT-4 and other models, including the API-based and GPT4 series, underscores its robustness in tasks requiring deep semantic understanding and complex data manipulation.
This demonstrates the potential of advanced models like GPT-4 in environments demanding high accuracy and versatility, while also indicating the need for further development in other models to close the performance gap.

\subsubsection{Performance Across Different Languages}

The analysis indicates that models from various companies exhibit distinct performance rankings across different languages, with consistently lower performance on the custom-written Tree language. Additionally, results using Rule Hint generally underperform compared to the Base configuration, suggesting that providing models with extra parsing rules may degrade performance. Conversely, the 2-shot method consistently enhances overall model performance. This trio of observations implies that while large language models (LLMs) improve with additional training data, they still fall short of truly understanding structured language expressions. They grasp examples but not the underlying structure or explanations.

\subsubsection{Task-Specific Performance}

In tasks requiring the understanding and manipulation of hierarchical data, the GPT4 Series and Minimax models demonstrate superior capabilities. For instance, in the PathCompose task, GPT-4, using the 2-shot method, achieved an average accuracy of 65.2\%, significantly outperforming Minimax, which reached 54.2\%. Similarly, in tasks involving hierarchical reasoning such as Node.Depth and Tree.Height, GPT-4 showed strong performance with the Base Prompt setting. In contrast, Minimax exhibited a dramatic range of performance—from nearly 0\% to 98.0\% accuracy—highlighting its strong but inconsistent learning capabilities in the few-shot setting.

\subsubsection{Correlation Analysis}

Fig.~\ref{fig:scatter} graphically illustrates how variations in Reference length and Node count affect the performance of GPT4-Turbo. It is evident that increasing Node count while maintaining a Reference length under approximately 1000 tends to degrade performance, whereas increasing Node count with a Reference length over 1000 enhances performance. This suggests that longer References complicate model comprehension, but additional structured expression aids understanding when Reference lengths are extensive. Conversely, when Reference lengths are shorter, introducing more structured expressions may introduce noise and reduce comprehension.

Fig.~\ref{fig:heat} displays the impact of different Reference lengths and Node counts on GPT4-Turbo across various languages and tasks. Significant impacts are noted in Node.Depth, PathCompose, and Statistics tasks, as well as in LaTeX, Markdown, and Tree languages, where increasing Reference length and Node count adversely affects performance. This could be due to the absence of complex structural data in these real-world applications, suggesting that training data did not contain excessive complexity, making additional nodes and References increase the complexity LLMs must manage, thereby affecting accuracy and efficiency. However, in the PathWalk task, while increasing Node count degrades performance, a greater number of References exacerbates this effect by causing information overload and complicating path tracking. Conversely, increasing Reference length and Node count showed minimal impact on JSON, XML, and YAML, which is attributed to the frequent use and thus better generalization of GPT4-Turbo in these well-trained languages.



% 而再之后的所有其他API-Based模型和GPT4系列的模型差距非常大。


% \subsubsection{Performance Across Different Languages}

% 发现各个公司推出的模型对于不同的语言有着不同的效果排名，但是对于我们通过自定义语言写的Tree都有着最差的表现效果。
% 另外，Rule Hint的结果普遍不如Base，这说明当额外输入解析规则给大模型，效果反而都下降了。
% 同时，2-shot的效果能够比较稳定地提升模型总体效果。
% 上述这三个现象结合起来，可以说明目前LLM都是通过增加训练数据来掌握结构化语言，但是距离真正理解结构化的语言表达还有着一定的差距，因为他们只能理解例子，但不能理解结构，同时也不能理解解释。

% \subsubsection{Task-Specific Performance}

% For the tasks require understanding and manipulating hierarchical data, which GPT4 Series and Minimax handled better than the other models.
% For instance, in the PathCompose task, GPT-4 achieved an average accuracy of 65.2 with the 2-shot prompting method, while the third, Minimax, reached 54.2.

% And for the tasks involve hierarchical reasoning, like Node.Depth and Tree.Height tasks.
% GPT-4 demonstrated strong performance with Base Prompt setting, while Minimax with powerful learning abilities for Base Prompt is nearly 0\% accuracy and 98.0\% accuracy in few-shot setting.

% \subsubsection{Correlation Analysis}

% Fig.~\ref{fig:scatter}直观展示了不同Reference长度和Node数量对于GPT4-Turbo表现的影响。
% 通过观察这张图，我们发现控制住Node Number不发生剧烈变化，单独增加Reference的长度会降低Model Performance。
% 而控制住Reference长度小于1000左右时，增加Node Number会降低模型表现。
% 而控制住Reference长度大于1000左右时，增加Node Number则会提高模型表现。
% 这可能是因为当Reference长度太长时，模型本来难以理解文本，而增加结构化的表达可以有助于模型理解文本。
% 当Reference长度不长时，模型本来可以较好的理解文本，这时增加结构化的表达会带来更多的干扰，从而降低模型的理解能力。

% Fig.~\ref{fig:heat}展示了不同Reference长度和Node数量对于GPT4-Turbo在不同语言和任务上的影响。
% 可以直观地看到，对于计算Node.Depth、PathCompose、Statistics任务，还有LaTeX、Markdown、Tree语言，增加reference长度和Node数量都会对模型表现产生剧烈影响，这可能是因为这些任务和语言在真实应用中并不涉及复杂的结构性数据，因此模型的训练数据并没有包含过多的复杂数据，而设定过多的节点和Reference会增加LLM理解的复杂度，从而影响模型在这些领域内的精确度和效率。
% 而对于PathWalk任务而言，虽然增加Node数量也会降低模型的表现，但增多Reference则更会降低模型的表现，这是因为在PathWalk任务中，过多的Reference内容可能导致信息过载，增加了模型在路径追踪中的难度，导致性能下降。
% 而增加Reference长度和Node数量对于JSON、XML、YAML都不会产生太大影响，我们再次认为，这是因为Object Notation语言经常被使用，所以GPT4-Turbo被训练地在这些语言上具有较好的泛化性。


% \subsection{Finetuned LLMs' Performance}

% This section includes the analysis to how to enhance LLMs' Structural Text understanding ability by finetuning.
% The performance of all finetune stages with different finetune strategies is showed in Fig.~\ref{fig:ft_language} and Fig.~\ref{fig:ft_task}.
% Note that Vanilla Llama-7B-v1 cannot answer any question correctly, so the accuracy start from 0\% in all figures.


% \subsubsection{Fine-Tuned Performance on Different Languages}

% Fig.~\ref{fig:ft_language} shows that fine-tuning had a modest impact on improving model performance.
% 具体而言，通过微调，LLM能够在所有的语言上获得有效地提升。
% Base finetune尽管会导致LLM丧失一部分在通用free-text language上的能力，但能够最大幅度增强LLM在结构化数据的理解上，在YAML、Tree语言上的效果甚至能和GPT4-Turbo持平。
% 这也从另一方面说明了，Tree语言下任务设置具有合理性，因为通过适当的训练，LLM可以掌握这种由我们自定义的语言所写的Tree。
% 而Mix-finetune虽然保证LLM不会丧失free-text langauge上的能力，但是对LLM在结构化数据的理解上增强却非常有限，在一些语言上的表现，如Tree、XML上非常有限。


% \subsubsection{Fine-Tuned Performance on Different Tasks}

% Fig.~\ref{fig:ft_task} 展现出了相较于语言而言变化更加剧烈的折线图。
% 依然，我们发现Base Finetune的效果最好最稳定，基本随着训练地加深，效果也变得越好。
% 而其他训练方法在一些任务，如SQL.Join、Statistics上，并不能保证训练的step数越多，效果就越好。

% 我们也观察到了一些特殊的表现，如Syntax任务在训练了几轮之后就会快速收敛。
% 这说明LLM很容易就能够理解某个结构化语言的语法表示。


% \subsection{微调后的大型语言模型性能分析}

% 本节分析了通过微调来增强大型语言模型（LLMs）对结构化文本的理解能力。图~\ref{fig:ft_language} 和图~\ref{fig:ft_task} 展示了不同微调策略下模型性能的变化情况。值得注意的是，原始的 Vanilla Llama-7B-v1 模型在所有任务上的初始准确率均为 0\%，所以所有图0 steps时，y轴都为0\%。

% \subsubsection{不同语言上的微调表现}

% 如图~\ref{fig:ft_language} 所示，微调对模型对所有结构化语言的理解有显著提升。
% Base 微调虽然可能会牺牲模型在通用自由文本语言上的部分能力，但显著增强了模型对结构化数据，尤其是 YAML 和 Tree 语言的理解，其效果甚至能与 GPT4-Turbo 相媲美。
% 这也从侧面验证了 Tree 语言任务设定的合理性，即通过适当的训练，LLM 能够有效掌握这种自定义的语言。
% 而 Mix 微调虽然确保了模型在自由文本语言上的能力不受损失，但其对结构化数据理解的增强作用相对有限，特别是在 Tree 上的提升几乎没有。
% 这可能是因为Tree语言的表现形式和通用文本的差距太大，所以难以在7B参数量的模型上通过简单地混合两方数据来增强两方面的能力。

% \subsubsection{不同任务上的微调表现}

% 如图~\ref{fig:ft_task} 展示的，任务性能的变化比对应语言的变化更为剧烈。
% 我们可以看到，Base 微调在大多数任务上提供了最好且最稳定的性能提升。
% 随着训练深度的增加，模型性能通常呈现出持续改善的趋势。
% 然而，其他微调方法在某些任务上，例如 SQL.Join 和 Statistics，并未显示出训练步数增加与性能提升之间的正相关关系。
% 另外，我们还观察到一些任务如 Syntax，在几轮训练后迅速趋于稳定。
% 这表明 LLM 能够迅速适应并理解特定结构化语言的语法规则。这种快速的收敛性可能指示了微调策略对模型理解具体语言结构的直接影响。


\subsection{Performance Analysis of Fine-Tuned Large Language Models}

This section analyzes the enhancement of large language models' (LLMs) understanding of structured text through fine-tuning. Figures~\ref{fig:ft_language} and~\ref{fig:ft_task} illustrate the performance changes under different fine-tuning strategies. Notably, the initial accuracy of the original Vanilla Llama-7B-v1 model is 0\% across all tasks, which is reflected by the y-axis starting at 0\% at 0 steps in all figures.

\subsubsection{Fine-Tuned Performance Across Different Languages}

As depicted in Figure~\ref{fig:ft_language}, fine-tuning significantly improves the models' comprehension of all structured languages. Although the base fine-tuning strategy may compromise some capabilities in general free-text language, it notably enhances the understanding of structured data, particularly in YAML and Tree languages, achieving performance comparable to GPT4-Turbo. This indirectly validates the rationality of the task settings for Tree language, as appropriate training enables LLMs to effectively master this custom-designed language. In contrast, the mix-fine-tuning strategy, while preserving capabilities in free-text language, offers limited enhancement in the comprehension of structured data, with minimal improvements in Tree language. This may be due to the significant differences between the representation of Tree language and general text, making it challenging to enhance capabilities in both areas simultaneously with a 7B parameter model.

\subsubsection{Fine-Tuned Performance Across Different Tasks}

Figure~\ref{fig:ft_task} shows that changes in task performance are more pronounced than changes in language performance. Base fine-tuning provides the most substantial and consistent performance improvements across most tasks. As training progresses, model performance generally shows a continuous improvement trend. However, other fine-tuning methods do not exhibit a positive correlation between increased training steps and performance enhancements in certain tasks, such as SQL.Join and Statistics. Additionally, tasks like Syntax quickly stabilize after a few training rounds, indicating that LLMs can rapidly adapt to and understand the grammatical rules of specific structured languages. This swift convergence may highlight the direct impact of fine-tuning strategies on the models' comprehension of specific language structures.



\subsection{Case Study}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.49\linewidth]{nips2024/figures/JSON_case_study.png}\hfill
    \includegraphics[width=0.49\linewidth]{nips2024/figures/SQL_case_study.png}
    \caption{Cases for performance of different LLMs and finetuned stages on Structured Text.}
    \label{fig:case}
\end{figure}


We illustrate the assessment setup and specific evaluation methods of StructBench through two exemplary cases in Figure~\ref{fig:case}.

In the Text Retrieval task under the JSON language, the model is required to extract the most deeply nested objects from a complex nested structure and directly output the dictionary type in free-text format. The GPT4-Turbo model accurately identified the objects that met the criteria and matched the standard answer precisely, demonstrating its profound understanding of structured text. Although the Minimax model's response was also judged as correct, it did not fully adhere to the preset output requirements. Given that many studies have explored the issue of compliance with output formats~\cite{}, our study focuses on assessing the LLM's understanding of structured text, thereby considering Minimax's response acceptable.

In the SQL.Join task under SQL language, the model is required to merge two tables and perform joint reasoning to output the number of records that meet specific criteria. The reference data was presented in a format that facilitates visualization. The GPT4-Turbo model, without any fine-tuning, failed to answer this question correctly. However, the model that underwent Base Fine-tuning exhibited progressive improvement: from initially incorrect responses at 300 training steps to gradually understanding the output format requirements at 1200 steps, and finally accurately solving the problem at 5100 steps. This progression illustrates the model's incremental enhancement in comprehending complex SQL queries and database structures through appropriate fine-tuning.


% 我们在Fig.~\ref{fig:case}中通过两个典型案例来展示StructBench的评估设置及其具体的评估方法。

% 在JSON语言下的TextRetrieval任务中，要求模型从复杂的嵌套结构中检索出最深层的对象，且输出要求直接以free-text格式输出字典的类型。
% GPT4-Turbo模型能够准确地找出符合条件的对象，并与标准答案完全一致，展示了其对结构化文本的深刻理解能力。尽管Minimax模型的回答也被评判为正确，但其答案格式并未完全遵循预设的输出要求。考虑到许多研究已经探讨了输出格式的遵守问题~\cite{}，我们在此研究中侧重于评估LLM对结构化文本的理解，因此认为Minimax的回答是可接受的。

% 在SQL语言下的SQL.Join任务中，要求模型能够合并两个表并进行联合推理，输出符合条件的记录数。我们将参考数据以便于可视化的格式呈现。GPT4-Turbo在未经微调的状态下未能正确回答此题。然而，经过Base Finetune的模型显示出从初始的错误回答（300步训练）到逐步理解输出格式要求（1200步训练），最终在5100步训练后能够准确回答问题。这一过程体现了通过适当的微调，模型在理解复杂SQL查询和数据表结构方面的逐步提升。



% 我们通过两个Case来展现StructBench的评估设置以及具体的评估方法。
% JSON语言TextRetrieval任务，该题目要求xxx
% GPT4-Turbo能够完美地回答地和标准答案一模一样。
% 而Minimax，GPT-Judge判断答案回答的对，但并没有严格遵守对于输出的要求。
% However，对于输出要求的遵守已经有许多论文探讨过了~\cite{}，我们在本篇论文中，更聚焦于LLM对于结构化文本的理解能力，因此MiniMax的这个回答我们认为是没问题的。

% SQL语言下的SQL.Join任务，我们将Reference写成了更加方便可视化的格式。
% 这个任务需要LLM能够将两个表合并在一起，进行联合推理。
% 当被要求直接输出答案时，GPT4-Turbo也无法答对这道题。
% 而我们发现，通过Base Finetune的模型，从最开始的胡乱回答（300 steps），到理解了输出格式的要求（1200 steps），再到能够完全答对这道题（5100 steps）。

% In assessing the performance of large language models (LLMs) on structured text, particular attention is given to their ability to interpret and manipulate data within JSON and SQL formats, as illustrated in Fig.~\ref{fig:case}.
% The models' understanding of complex data structures and their accuracy in fulfilling specific requirements are of primary concern, along with how these capabilities evolve through the process of finetuning.

% The JSON task required the model to identify deeply nested objects lacking list or dictionary values. The response from the GPT4\_turbo model, which had not undergone finetuning, correctly pinpointed the most nested object, as verified against the ground truth provided. This demonstrates the model's inherent capability to navigate and interpret nested JSON data structures accurately without additional training.

% Conversely, the SQL task, which involved identifying individuals from a structured dataset based on a specific height criterion, presented a more challenging scenario for the model. Initially, the model, even after 300 finetuning steps, inaccurately reported the number of qualifying individuals, highlighting a lack of understanding in correlating data across joined SQL tables and applying numerical criteria correctly. Continued finetuning over 1200 steps did not rectify this error, suggesting either an inadequacy in the finetuning process or a need for more comprehensive training data specific to this task. However, a substantial improvement was observed after extending the finetuning to 5100 steps, where the model's response aligned perfectly with the ground truth.

% This progression underscores the potential for LLMs to enhance their performance on structured tasks through finetuning. It also illustrates the necessity for substantial and targeted training iterations to refine the models' capabilities in accurately executing complex data manipulations, as simple initial training might not suffice. Such insights are crucial for developing more robust models that can reliably interpret and respond to structured data queries in diverse applications.


% \section{Conclusion}

% The experiments demonstrate that while models like GPT-4 exhibit strong performance across multiple structured text tasks, there are significant challenges associated with more complex and deeper structures. Fine-tuning methods, including few-shot learning and rule hints, provided limited improvements. Overall, the findings highlight the need for more advanced strategies to enhance the generalizability and robustness of LLMs in processing and reasoning over structure-rich data.

% Future research should focus on exploring more effective prompting techniques, improving hierarchical reasoning capabilities, and developing models that can better handle a variety of structured text formats. Additionally, the impact of model size and the potential for transfer learning between different structured text types warrant further investigation.


==> texs/old_version/05.Analysis.04.tex <==
% \input{overall_performance_tables.02}
% \input{overall_performance_tables.03}
% \input{overall_performance_tables.04}
\input{overall_performance_tables.06}


% \begin{figure*}[t]
%     \centering
%     \caption{The performance of GPT4-Turbo across all samples is distributed according to ``Reference Length'' and ``Nodes Number''. Note that ``\#Reference'' represents the character number in a sample.}
%     \label{fig:scatter}
%     \includegraphics[width=\textwidth]{figures/scatter_sample.png}
%     \caption{Correlation among the ``Node Number'', ``Reference Length'' and ``Model Performance''.}
%     \label{fig:heat}
%     \includegraphics[width=\textwidth]{figures/heatmap_language_task.png}
% \end{figure*}


% \begin{figure*}
%     \centering
%     \caption{All finetune methods and their performance on all languages.}
%     \label{fig:ft_language}
%     \includegraphics[width=\textwidth]{figures/All_Language.png}
%     \caption{All finetune methods and their performance on all tasks.}
%     \label{fig:ft_task}
%     \includegraphics[width=\textwidth]{figures/All_Task.png}
% \end{figure*}

\subsection{Close Sourced LLMs' Performance}

In this section, we analyze the performance of closed-source LLMs in various tasks involving structure-rich text and multiple languages.
Table~\ref{tab:api_overall} displays the overall performance on the complete StrucText-Eval dataset, while Table~\ref{tab:hard_performance} compares both LLM and human performance specifically on the StrucText-Eval-Hard subset.

\subsubsection{GPT4 Series Outperform All Other LLMs in Structure-Rich Text Understanding}

The experiments revealed that GPT4 consistently outperformed other models across most tasks and languages.
Specifically, GPT-4 achieved an average accuracy of 78.4 in all languages and tasks, significantly higher than the next best model, GPT4-turbo, which had an accuracy of 69.3.
The marked disparity in performance between GPT4 Series and other LLMs underscores its robustness in tasks requiring deep semantic understanding and complex data manipulation.
This demonstrates the potential of advanced models like GPT-4 in environments demanding high accuracy and versatility while also indicating the need for further development in other models to close the performance gap.

\subsubsection{Current LLMs Cannot Truly Understand Structure-Rich Expressions}

We conclude that although the performance of LLMs improves with more training data, they still fall short of truly comprehending structured language expressions, as evidenced by two observations.
Firstly, evaluation results indicate that models from various companies exhibit distinct performance rankings across different languages.
Notably, there is consistently lower performance in Tree structures, which are entirely composed of custom languages.
This suggests that current LLMs are incapable of understanding complex, custom-structured expressions.
Furthermore, results from utilizing Rule Hints generally underperform relative to the Base Prompt, implying that providing models with additional parsing rules may impair performance.
In contrast, the 2-shot method consistently enhances the overall performance of LLMs, indicating that while LLMs are able to grasp individual examples, they do not fully understand the underlying structures or the rationale behind them.

\subsubsection{Procedural Task is Watershed For LLMs}

An in-depth analysis of the performance data from several LLMs demonstrates a clear demarcation in their ability to handle procedural tasks, which require navigating and manipulating structured data.
Tasks emphasising procedural complexity, such as ``PathCompose'' and ``Tree.Height'', present significant challenges to these models.
For example, in the ``PathCompose'' task, GPT-4 shows a superior performance with an accuracy rate of 79.2\% in its base setting, compared to Minimax, which achieves only 25.0\%.
Similarly, in the ``Tree.Height'' task, GPT-4 maintains a robust performance with 37.5\% accuracy, whereas Minimax struggles, recording 0\% in its base prompt setting. 


\subsubsection{Impact of Data Length and Complexity on LLM Performance}

Fig.~\ref{fig:scatter} illustrates how variations in Data Length and Complexity affect the performance of GPT4-Turbot.
Specifically, we quantify Data Length and Complexity using the character length of References and the number of Nodes.
It is evident that increasing the Node count while maintaining a Reference length under approximately 1000 tends to degrade performance, whereas increasing the Node count with a Reference length over 1000 enhances performance.
This suggests that longer References complicate model comprehension, but additional structured expression aids understanding when Reference lengths are extensive.
Conversely, when Reference lengths are shorter, introducing more structured expressions may introduce noise and reduce comprehension.

Fig.~\ref{fig:heat} displays the impact of different Reference lengths and Node counts on GPT4-Turbo across various languages and tasks. Significant impacts are noted in Node.Depth, PathCompose, and Statistics tasks, as well as in LaTeX, Markdown, and Tree languages, where increasing Reference length and Node count adversely affects performance. This could be due to the absence of complex structural data in these real-world applications, suggesting that training data did not contain excessive complexity, making additional nodes and References increase the complexity LLMs must manage, thereby affecting accuracy and efficiency. However, in the PathWalk task, while increasing the Node count degrades performance, a greater number of References exacerbates this effect by causing information overload and complicating path tracking. Conversely, increasing Reference length and Node count showed minimal impact on JSON, XML, and YAML, which is attributed to the frequent use and, thus, better generalization of GPT4-Turbo in these well-trained languages.

\begin{figure*}[t]
    \centering
    \caption{Cases for performance of different LLMs and finetuned stages on Structured Text.}
    \label{fig:case}
    \includegraphics[width=0.49\linewidth]{figures/JSON_case_study.png}\hfill
    \includegraphics[width=0.49\linewidth]{figures/SQL_case_study.png}
    % \vspace{-5mm}
\end{figure*}

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/plot.png}
    \includegraphics[width=0.7\columnwidth]{figures/legend.png}
    \caption{The model's performance on StrucText-Eval-Test under different Few-Shot Demonstration settings.}
    \label{fig:enter-label}
\end{figure}


\begin{figure*}[t]
\centering
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_perform.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_lang_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_task_std.png}

\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_perform.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_lang_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_task_std.png}
\caption{Consistency Map}
\label{fig:enter-label}
\end{figure*}

\subsection{Performance Analysis of Finetuned Large Language Models}

This section analyzes the enhancement of LLMs' understanding of structure-rich text through finetuning.
Fig.~\ref{fig:ft_language} and Fig.~\ref{fig:ft_task} illustrate the performance changes under different finetuning strategies. 
Notably, the initial accuracy of the Vanilla Llama-7B-v1 is 0\%, which is reflected by the y-axis starting at 0\% at 0 steps in all figures.

\subsubsection{Finetuning Enhance LLM's Performance in All Languages}

As depicted in Fig.~\ref{fig:ft_language}, finetuning improves the models' comprehension of all structured languages. Although the base finetuning strategy may compromise some capabilities in general free-text language, it notably enhances the understanding of structured data, particularly in YAML and Tree languages, achieving performance comparable to GPT4-Turbo. This indirectly validates the rationality of the task settings for Tree language, as appropriate training enables LLMs to master this custom-designed language effectively. In contrast, while preserving capabilities in free-text language, the mix-fine-tuning strategy offers limited enhancement in the comprehension of structured data, with minimal improvements in Tree language. This may be due to the significant differences between the representation of Tree language and general text, making it challenging to enhance capabilities in both areas simultaneously with a 7B parameter model.

\subsubsection{Not All Tasks can be Enhanced by FineTuning}

Fig.~\ref{fig:ft_task} shows that changes in task performance are more pronounced than changes in language performance. Base finetuning provides the most substantial and consistent performance improvements across most tasks. As training progresses, model performance generally shows a continuous improvement trend. However, other finetuning methods do not correlate positively with increased training steps and performance enhancements in certain tasks, such as Join and Statistics. Additionally, tasks like Syntax quickly stabilize after a few training rounds, indicating that LLMs can rapidly adapt to and understand the grammatical rules of specific structured languages. This swift convergence may highlight the direct impact of finetuning strategies on the models' comprehension of specific language structures.



\subsection{Case Study}


We illustrate the assessment setup and specific evaluation methods of StrucText-Eval through two exemplary cases in Fig.~\ref{fig:case}.

In the Text Retrieval task under the JSON language, the model is required to extract the most deeply nested objects from a complex nested structure and directly output the dictionary type in free-text format. The GPT4-Turbo model accurately identified the objects that met the criteria and matched the standard answer precisely, demonstrating its profound understanding of structured text. Although the Minimax model's response was also judged as correct, it did not fully adhere to the preset output requirements. Given that many studies have explored the issue of compliance with output formats~\cite{}, our study focuses on assessing the LLM's understanding of structured text, thereby considering Minimax's response acceptable.

In the Join task under SQL language, the model is required to merge two tables and perform joint reasoning to output the number of records that meet specific criteria. The reference data was presented in a format that facilitates visualization. The GPT4-Turbo model, which without any further finetuning, failed to answer this question correctly. However, the model that underwent Base Finetuning exhibited progressive improvement: from initially incorrect responses at 300 training steps to gradually understanding the output format requirements at 1200 steps, and finally accurately solving the problem at 5100 steps. This progression illustrates the model's incremental enhancement in comprehending complex SQL queries and database structures through appropriate finetuning.



==> texs/old_version/05.Analysis.05.tex <==
\input{overall_performance_tables.06}


\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{figures/plot.png}
    \includegraphics[width=0.7\columnwidth]{figures/legend.png}
    \caption{The model's performance on StrucText-Eval-Test under different Few-Shot Demonstration settings.}
    \label{fig:few_shot}
\end{figure}

\begin{figure*}[!ht]
\centering
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_perform.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_lang_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/all_task_std.png}

\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_perform.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_lang_std.png}
\includegraphics[width=0.24\textwidth]{figures/heatmaps/gpt_task_std.png}
\caption{Consistency Map}
\label{fig:cor_model}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/heatmaps/cor_heatmap.png}
    \caption{Correlation between different evaluation metrics.}
    \label{fig:cor_metrics}
\end{figure}


\begin{figure*}[!ht]
    \centering
    \caption{Cases for performance of different LLMs and finetuned stages on Structured Text.}
    \label{fig:case}
    \includegraphics[width=0.49\linewidth]{figures/JSON_case_study.png}\hfill
    \includegraphics[width=0.49\linewidth]{figures/SQL_case_study.png}
    \% \vspace{-5mm}
\end{figure*}
\subsection{Overall Performance in StrucText-Eval}
在StrucText-Eval中的整体表现如表~\ref{tab:api_overall}所示，各个模型在不同的prompt方法下，在多种语言和任务上的表现差异显著。比如，在基础prompt（Base）下，Qwen2-72B-Instruct模型在JSON、YAML、LaTeX等结构化语言的理解任务中表现较好，其准确率在90\%左右，而在复杂树结构的任务中表现有所下降。而对于Meta-Llama-3.1-70B-Instruct-Turbo模型，其在LaTeX和Markdown的处理上有相对更好的表现，但在CSV格式的Tabular任务上表现较差。此外，提示增强（w/ hint）方法一般能够提升模型表现，尤其是在复杂结构和需要更深推理的任务上，比如在YAML和JSON上，许多模型的准确率在提示后有所提升，表现得更加接近GPT-4等更高级模型的结果。

这种现象的产生可以归因于多个因素。首先，训练数据的偏差可能导致某些模型在处理特定类型的结构化文本时表现较弱，尤其是当该结构不常见时。其次，Prompt方法的设计也显著影响模型表现。例如，简单的提示可能不足以引导模型进行复杂的推理，而更多的上下文和提示则可以显著提高模型的表现。最后，模型架构及其预训练目标也影响其对特定语言或任务的理解能力。例如，某些模型在树形数据结构上的表现较弱，可能是由于这种结构在预训练数据中出现较少，导致模型在推理时能力不足。

\subsection{Overall Performance on StrucText-Eval Hard}
表~\ref{tab:hard_performance}展示了各个模型在StrucText-Eval Hard数据集上的表现。在Hard测试集中，任务更加复杂，问题长度和结构深度更大，这导致所有模型的表现都有所下降。Qwen2-72B-Instruct模型在基础prompt下的准确率从78.4\%下降到了65.0\%，而Meta-Llama-3.1-70B-Instruct-Turbo则从75.4\%下降到了43.2\%。相比于标准测试集，Hard测试集要求模型在更复杂的条件下进行推理，因此即使是具有提示增强（w/ hint）的情况下，模型的表现提升也相对有限，无法像在标准测试集中那样显著提高准确率。

这种现象背后的原因主要是因为Hard测试集的复杂度超出了大多数模型的预训练范围。更深的嵌套结构和更长的输入增加了模型的推理负担，而现有的模型在复杂推理方面仍然存在局限。此外，prompt方法在复杂任务中的优劣更加明显，像是简单CoT提示（Self-CoT）在深层推理任务中的表现不佳，无法提供足够的引导进行多步推理。

\subsection{Few-Shot Demonstration on Structural Text Inference}
从图~\ref{fig:few_shot}可以看出，在Few-Shot情境下，各个模型的表现随着demonstration数量的增加而显著提高。在3-shot情况下，GPT-4的表现明显优于其他模型，达到了69.5\%的准确率，而Gemini-Pro-Flash和Mistral等模型即使在3-shot情况下，准确率也远远落后于GPT-4，仅为21\%甚至更低。对于Qwen-2-72B-Instruct模型，其随着示例数量增加的提升趋势相对稳定，但依然明显低于GPT-4的表现。

这可以解释为模型在面对结构化文本推理任务时，示例数量能够显著帮助模型理解复杂的结构。模型通过Few-Shot学习可以从多个示例中提取共性，进而更好地适应任务的要求。较差的模型往往由于预训练数据中缺乏类似结构的任务，导致它们无法通过少量示例迅速适应新任务。

\subsection{不同难度、语言、task上模型表现的差异}
图~\ref{fig:cor_model}展示了不同模型在多种语言和任务上的表现，尤其是GPT系列的表现差异。从图中可以看出，GPT-4在所有语言和任务上的表现都相对较好，且标准差较小，表现较为稳定。例如，GPT-4在LaTeX、JSON、YAML等复杂结构上的表现尤其突出，标准差极低，说明其在应对复杂结构时具有较高的鲁棒性。相比之下，Meta-Llama-3.1-70B在Tree和Tabular任务上的表现波动较大，标准差较高，表明其在处理这些任务时表现不稳定，偶尔出现较差的推理结果。

这种差异可以归因于模型的预训练数据以及任务难度的不同。GPT系列模型由于预训练时覆盖了大量的复杂结构化数据，使得其在不同语言和任务中的表现更加稳健。而对于一些开源模型，尤其是在复杂结构和少见的语言格式上，由于预训练覆盖不足，其表现波动较大。同时，任务的复杂度也对模型产生了显著影响，结构更复杂的任务需要模型具备更强的推理能力，这在较小规模的模型上尤为困难。

\subsection{Correlation Between Different Metrics}
从图~\ref{fig:cor_metrics}可以看出，各评估指标之间的相关性差异显著。Human Judge与GPT-4o Judge的高度一致性（0.95）表明，GPT-4o Judge的自动评估接近人类判断。相比之下，Exact Match与Human Judge的相关性最低（0.40），这反映了Exact Match在衡量模型生成多样化内容时的局限性。RougeL与Human Judge和GPT-3 Judge的相关性相近（均为0.75），说明RougeL虽在捕捉文本表面相似度方面有效，但仍难以完全反映深层语义。总体来看，自动化指标与人工评估的一致性差异提醒我们，单一指标难以全面衡量模型性能。

\subsection{Case Study}

We illustrate the assessment setup and specific evaluation methods of StrucText-Eval through two exemplary cases in Fig.~\ref{fig:case}.

In the Text Retrieval task under the JSON language, the model is required to extract the most deeply nested objects from a complex nested structure and directly output the dictionary type in free-text format. The GPT4-Turbo model accurately identified the objects that met the criteria and matched the standard answer precisely, demonstrating its profound understanding of structured text. Although the Minimax model's response was also judged as correct, it did not fully adhere to the preset output requirements. Given that many studies have explored the issue of compliance with output formats~\cite{}, our study focuses on assessing the LLM's understanding of structured text, thereby considering Minimax's response acceptable.

In the Join task under SQL language, the model is required to merge two tables and perform joint reasoning to output the number of records that meet specific criteria. The reference data was presented in a format that facilitates visualization. The GPT4-Turbo model, which without any further finetuning, failed to answer this question correctly. However, the model that underwent Base Finetuning exhibited progressive improvement: from initially incorrect responses at 300 training steps to gradually understanding the output format requirements at 1200 steps, and finally accurately solving the problem at 5100 steps. This progression illustrates the model's incremental enhancement in comprehending complex SQL queries and database structures through appropriate finetuning.




==> texs/old_version/06.Conclusion.01.tex <==
We presented a taxonomy involving 8 popular structure-rich texts, which are diverse in structural complexity and application domains.
We classified these inputs into 3 first level category by use scenarios and demonstrated their definition, construction rules we used in generation and their respective common applications.
By procedural construction and parsing, we built a benchmark, StructBench, with 6032 QAs and evaluated GPT-4, Minimax, Spark and Ernie against StructBench.
The experiments uncovered the under-exploration of structure-rich input texts for commercial LLMs.
Among these structure texts, Tree is the most typical and where poor performance occurs.
In contrary, LLMs are most capable of structural tasks in Object Notation texts, such as JSON, YAML, XML.
The prompt engineering method of eliciting hints or providing auxiliary step-by-step rule hint both failed to adequately address such inefficiencies.
Few-shot learning demonstrated promising improvement according to the API test results.
The experiments finetuning OpenLLaMA 7B v1 with different data settings showed the ineffectiveness of finetuning for enhancing structural processing ability, regardless of the inclusion of auxiliary rule hints.
The mix setting also revealed distinct capability requirements for natural language tasks versus structural tasks.

==> texs/old_version/06.Discussion.02.tex <==
% 我们认为，以自然文本形式去直接理解结构化文本是LLM都需要具备的能力。
% 因此提出了StructBench来帮助评估LLM的这一能力。
% 我们发现目前根据不同结构化语言的使用频率，LLM对于这些结构化数据的训练程度不同，因此展现出了完全不同的表现效果。
% 但同时，LLM并没有对结构有着更深层次的了解，因此，当使用一些常见的结构化语言组成较为复杂的结构化形式，或者自定义一些结构化语言，模型的理解能力就会大幅下降。
% 通过直接训练StructBench中的数据，模型可以具备一定的结构化文本理解能力，如何平衡好LLM在通用文本上的能力，并增强对于结构化文本的理解，甚至是如何增强LLM对于结构的理解将会是一个非常值得研究的内容。

我们认为，以自然文本格式直接解释结构化文本的能力是所有大型语言模型（LLM）所需的重要技能。
为此，我们开发了 StructBench 来评估 LLM 的这一特定能力。
我们的研究结果表明，目前强有力的大语言模型对于这些结构化语言的训练程度因用户的使用频率而异，所以同样的任务在不同结构化语言下执行会带来完全不一样的效果。
而目前，LLMs 对于结构化文本的理解依然只是停留在训练数据相关的表面，他们缺乏对结构本身的深刻理解。
当 LLM 遇到由常见结构化语言组成的复杂配置或需要解析定制的结构化语言时，这种不足就会显现出来，从而导致模型性能大幅下降。

在 StructBench 提供的数据集上进行直接训练可以有效增强语言模型对于结构化语言的理解。
但只在StructBench的训练集上训练，是无法在测试集上全面达到GPT4-Turbo的能力，这需要更加大量的结构化数据的收集和训练方法的优化。
We leave 保持 LLM 在一般文本上的性能，同时提高它们理解结构化文本的能力，以及进一步探索如何加深 LLM 对结构概念本身的理解 to the future work.


==> texs/old_version/09.App.Examples.01.tex <==

\subsubsection{Tree}
See~\autoref{fig:eg_tree}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/Tree_Sample.pdf}
\end{center}
\caption{Sample input and tasks of Tree.}
\label{fig:eg_tree}
\end{figure}

\subsubsection{Tabular}

See~\autoref{fig:eg_tab}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputSQL.pdf}
\end{center}
\caption{Sample input and tasks of tabular data.}
\label{fig:eg_tab}
\end{figure}

\subsubsection{JSON}

See~\autoref{fig:eg_json}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth, height=0.8\paperheight]{./figures/inputJSON.pdf}
\end{center}
\caption{Sample input and tasks of JSON.}
\label{fig:eg_json}
\end{figure}

\subsubsection{YAML}

See~\autoref{fig:eg_yaml}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth , height=0.8\paperheight]{./figures/inputYAML.pdf}
\end{center}
\caption{Sample input and tasks of YAML.}
\label{fig:eg_yaml}
\end{figure}

\subsubsection{XML}

See~\autoref{fig:eg_xml}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth, height=0.8\paperheight]{./figures/inputXML.pdf}
\end{center}
\caption{Sample input and tasks of XML.}
\label{fig:eg_xml}
\end{figure}

\subsubsection{LaTeX}

See~\autoref{fig:eg_latex}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputLaTeX.pdf}
\end{center}
\caption{Sample input and tasks of LaTeX.}
\label{fig:eg_latex}
\end{figure}

\subsubsection{Markdown}

See~\autoref{fig:eg_mkd}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputMarkdown.pdf}
\end{center}
\caption{Sample input and tasks of Markdown.}
\label{fig:eg_mkd}
\end{figure}

\subsubsection{Org}

See~\autoref{fig:eg_org}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputORG.pdf}
\end{center}
\caption{Sample input and tasks of Org.}
\label{fig:eg_org}
\end{figure}

% \subsubsection{Python Code}

% See~\autoref{fig:eg_py}.

% \begin{figure}[h]
% \begin{center}
% %\framebox[4.0in]{$\;$}
%    \includegraphics[width=0.8\linewidth]{./figures/inputPYTHON.pdf}
% \end{center}
% \caption{Sample input and tasks of Python codes.}
% \label{fig:eg_py}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips2024"
%%% End:


==> texs/old_version/A.genrule.tex <==

\subsubsection{Tree}

We build tree-structured input as a list of edges in a tree, in a format of ``\texttt{father->child}’’, separated by newline.

\[
\begin{aligned}
identifier&\coloneqq \texttt{[a-z]+}\\
Edge&\coloneqq identifier\texttt{->}identifier\\
Tree&\coloneqq Edge(\texttt{\textbackslash n}Edge)\texttt{*}\\
InputFile&\coloneqq Tree\\
\end{aligned}
\]

\subsubsection{Tabular}
Formally, input texts are classified as tabular data given that they are composed of a list of newline separated lines, each of which is a list of text cells delimited by comma.

\[
\begin{aligned}
head &\coloneqq \texttt{[A-Z][a-z]*}\\
cell &\coloneqq \texttt{[A-Za-z0-9]+}\\
headline &\coloneqq identifier(, identifier)\texttt{*}\\
subline &\coloneqq cell(, cell)\texttt{*}\\
Tabular &\coloneqq headline(\texttt{\textbackslash n}subline)\texttt{+}\\
InputFile&\coloneqq Tabular\\
\end{aligned}
\]

\subsubsection{JSON}\label{ap:json_rule}

Due to the inherit hierarchy structure of Object Notations, we adopted a recursive scheme to define our input texts.

\[
\begin{aligned}
lb_{(left\ bracket)}&\coloneqq \texttt{[[]}\\
rb&\coloneqq \texttt{[]]}\\
val&\coloneqq \texttt{[a-z]+}\\
key&\coloneqq \texttt{[A-Z]+}\\
JSON&\coloneqq \{\\
&\texttt{"id":"}val\texttt{"}\\
&\texttt{"subs":}lbrb|lbJSON(, \texttt{\textbackslash n}JSON)\texttt{*}rb\\
&\texttt{("}key\texttt{":"}val\texttt{"\textbackslash n)+}\\
&\}\\
InputFile&\coloneqq JSON\\
\end{aligned}
\]

\subsubsection{YAML} \label{ap:yaml_rule}
The rules for constructing YAML and XML input are similarly recursive.

\[
\begin{aligned}
YAML&\coloneqq \\
&\texttt{id}:val\\
&\texttt{subs}:lbrb|(\texttt{\textbackslash n}(\texttt{\textbackslash t})*\texttt{- }YAML)+\\
&(key:val\texttt{\textbackslash n})\texttt{+}\\
InputFile&\coloneqq YAML\\
\end{aligned}
\]
\subsubsection{XML} \label{ap:xml_rule}
\[
\begin{aligned}
firstline&\coloneqq \texttt{<?xml version="1.0" encoding="UTF-8"?>}\\
XML &\coloneqq\\
&firstline\\
&XMLObject\\
tag&\coloneqq \texttt{[A-Z]+}\\
val&\coloneqq \texttt{[a-z]+}\\
attr&\coloneqq \texttt{[A-Z]+="}val\texttt{"}\\
content&\coloneqq \texttt{[a-z \textbackslash n\textbackslash t]*}\\
XMLObject&\coloneqq\\
&\texttt{<}tag(\texttt{ }attr)*\texttt{>}\\
&((\texttt{\textbackslash t})*XMLObject)*\\
&content\\
&\texttt{</}tag\texttt{>}\\
InputFile&\coloneqq XML\\
\end{aligned}
\]

\subsubsection{LaTeX} \label{ap:ltx_rule}
In LaTeX input texts, we include \texttt{textbf} and \texttt{includegraphics} commands to accommodate for the text retrieval tasks. The headings serve as anchors for structure traversal.
\[
\begin{aligned}
command &\coloneqq \texttt{\textbackslash}(\texttt{section}|\texttt{subsection}|\texttt{subsubsection})\\
heading &\coloneqq command\texttt{\{[a-z]+\}}|\texttt{[a-z]+}\\
inclg &\coloneqq\\ &\texttt{\textbackslash includegraphics[width=0.5\textbackslash textwidth]}\{\texttt{[a-z]+[.](png|jpg|jpeg|gif)}\}\\
bf &\coloneqq \texttt{\textbackslash textbf}\{\texttt{[a-z ]+}\}\\
content &\coloneqq (\texttt{[a-z ]}|bf|inclg)\texttt{+}\\
LaTeX &\coloneqq heading\texttt{\textbackslash n}content (\texttt{\textbackslash n}LaTeX)*\\
InputFile&\coloneqq LaTeX\\
\end{aligned}
\]



\subsubsection{Markdown}
In markdown input texts, the syntax counterparts for heading, text face and including figure are employed in our dataset.
\[
\begin{aligned}
	heading&\coloneqq \texttt{[\#]* [a-z]+}\\
	inclg&\coloneqq \texttt{!}lb\texttt{alt}rb\texttt{\textbackslash([a-z]+[.](png|jpg|jpeg|gif) "hover text"\textbackslash)}\\
	bf&\coloneqq \texttt{[*]\{2\}[a-z ]+[*]\{2\}}\\
    content &\coloneqq (\texttt{[a-z ]}|bf|inclg)\texttt{+}\\
    Markdown &\coloneqq heading\texttt{\textbackslash n}content (\texttt{\textbackslash n}Markdown)*\\
    InputFile&\coloneqq Markdown\\
\end{aligned}
\]

\subsubsection{Org}
In Org input texts, the syntax is obtained from JSON construction rules by replacing the markups for heading, including figures and bold font face.
\[
\begin{aligned}
	heading&\coloneqq \texttt{[*]* [a-z]+}\\
	inclg&\coloneqq lb\{2\}\texttt{[a-z]+[.](png|jpg|jpeg|gif)}rb\{2\}\\
	bf&\coloneqq \texttt{[*][a-z ]+[*]}\\
    content &\coloneqq (\texttt{[a-z ]}|bf|inclg)\texttt{+}\\
    Org &\coloneqq heading\texttt{\textbackslash n}content (\texttt{\textbackslash n}Org)*\\
    InputFile&\coloneqq Org\\
\end{aligned}
\]


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024
%%% End:


==> texs/old_version/input_sample.tex <==

\subsubsection{Tree}
See~\autoref{fig:eg_tree}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/Tree_Sample.pdf}
\end{center}
\caption{Sample input and tasks of Tree.}
\label{fig:eg_tree}
\end{figure}

\subsubsection{Tabular}

See~\autoref{fig:eg_tab}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputSQL.pdf}
\end{center}
\caption{Sample input and tasks of tabular data.}
\label{fig:eg_tab}
\end{figure}

\subsubsection{JSON}

See~\autoref{fig:eg_json}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth, height=0.8\paperheight]{./figures/inputJSON.pdf}
\end{center}
\caption{Sample input and tasks of JSON.}
\label{fig:eg_json}
\end{figure}

\subsubsection{YAML}

See~\autoref{fig:eg_yaml}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth , height=0.8\paperheight]{./figures/inputYAML.pdf}
\end{center}
\caption{Sample input and tasks of YAML.}
\label{fig:eg_yaml}
\end{figure}

\subsubsection{XML}

See~\autoref{fig:eg_xml}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth, height=0.8\paperheight]{./figures/inputXML.pdf}
\end{center}
\caption{Sample input and tasks of XML.}
\label{fig:eg_xml}
\end{figure}

\subsubsection{LaTeX}

See~\autoref{fig:eg_latex}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputLaTeX.pdf}
\end{center}
\caption{Sample input and tasks of LaTeX.}
\label{fig:eg_latex}
\end{figure}

\subsubsection{Markdown}

See~\autoref{fig:eg_mkd}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputMarkdown.pdf}
\end{center}
\caption{Sample input and tasks of Markdown.}
\label{fig:eg_mkd}
\end{figure}

\subsubsection{Org}

See~\autoref{fig:eg_org}.

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
   \includegraphics[width=0.8\linewidth]{./figures/inputORG.pdf}
\end{center}
\caption{Sample input and tasks of Org.}
\label{fig:eg_org}
\end{figure}

% \subsubsection{Python Code}

% See~\autoref{fig:eg_py}.

% \begin{figure}[h]
% \begin{center}
% %\framebox[4.0in]{$\;$}
%    \includegraphics[width=0.8\linewidth]{./figures/inputPYTHON.pdf}
% \end{center}
% \caption{Sample input and tasks of Python codes.}
% \label{fig:eg_py}
% \end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "nips2024"
%%% End:


==> texs/taxonomy.tex <==
% =JSON=
% PathCompose
% PathWalk
% Syntax
% TextRetrieval

% =LaTeX=
% PathWalk
% TextRetrieval

% =Markdown=
% PathWalk
% TextRetrieval

% =ORG=
% PathWalk
% TextRetrieval

% =SQL=
% SQL.Join
% Statistics
% TextRetrieval

% =Tree=
% PathCompose
% Tree.Depth
% Tree.Height

% =XML=
% Syntax
% TextRetrieval

% =YAML=
% PathCompose
% PathWalk
% Syntax
% TextRetreval

% task label uniq
% PathCompose
% PathWalk
% SQL.Join
% Statistics
% Syntax
% TextRetreval
% TextRetrieval
% Tree.Depth
% Tree.Height

% Taxonomy subsec
We present an overview on common structure-rich texts in~\autoref{tb:structtextstaxonomy}, including structured texts~(tabular data), semi-structured texts~(mainly markup languages:XML, JSON, YAML, ORG, LaTeX and Markdown), abstract data structure~(Tree from graph theory). %https://tex.stackexchange.com/questions/9633/why-should-i-put-a-before-ref-or-cite, https://latex-alive.tumblr.com/post/827168808/correct-punctuation-spaces


For every class of input texts, we designed 3-5 tasks.
Most tasks are closely aligned with the structure of input texts, with answers derived procedurally during input texts generation.
It is noteworthy that our tasks primarily depend on semantics for understanding the task instructions, while the semantics of the input texts are obscured through randomized generation.

The examples of the input texts and tasks for each category are documented in~\autoref{ap:samples}.
For each task, we generated 208 sample inputs, constructing a dataset comprising a total of 6032 QAs.
For more detailed rules used in generating input data, see~\autoref{ap:rules}.

% TODO, tabularize taxonomy
\subsubsection{Abstract Data Structure}\label{sssec:tree} % Tree
In the realm of digital information, data is organized in a structure that could easily be stored, parsed, analyzed by machines.
The theoretical model underlying these structures are abstract data structures, e.g., tree, list, graph, queue, stack, etc.
Abstract data structure decides how data is queried, inserted, modified and deleted.
These structures encode the relations and properties of data.
The ability to understand abstract data structure will enable LLMs to rigidly follow the relation of semantic segments imposed from syntax, which is vital to data exchange between different format.
The ability of LLMs solving graph problems has been explored in previous work (\cite{wang2023language}).


Tree, from the view of graph, is acyclic connected undirected graph.
It is defined in the same way as a graph, i.e., a set of vertices and a set of edges connecting vertices thereof.
Given the pervasive influence of tree on other recursive structured texts such as JSON, YAML and XML, we focused on tree structure and designed tree-specific tasks.


Regarding each tree, we designed 3 tasks pertaining to their structures, all of which are independent of the content in the nodes.
A sample of input texts of tree category along with its associated tasks are shown in~\autoref{fig:eg_tree}.
These tasks target on the ability to compose a path to a specified node and decide the height or depth of a node.


\subsubsection{Structured}\label{sssec:structured}%SQL
Generally, structured data refer to those well-structured data that obey certain elaborate data model which defines the relation of data elements and abstract models.
Tabular data exported from data tables in relational databases are typical of such structured data.
Data that are structured according to non-tabular data models are also deemed as structured data.


In this work, we focus on specific row-column structured text inputs.
Such input denotes a set of objects with the same set of fields defined by the first row.
The subsequent rows denotes the values of fields per object.
The format is derived from tables in relational database, which has seen overwhelming domination in the realm of database.


Due to the simplicity of the input, apart from a value lookup task, we built statistical tasks as well as multiple-table tasks that are similar to inner join query, to better capture the features and practical use scenarios of such input data.


\subsubsection{Semi-Structured}
As opposed to structured texts, semi-structured data are structured data that do not fit in the conventional data model (\cite{buneman1997semistructured}).
Semi-structured data typically contain rich structural marks or tags that are different from semantic elements.
In this work, we focus specifically on texts with some extent of hierarchies designated by marks and reserved tokens.
They are neither sequential nor tabular as in~\autoref{sssec:structured}.
Internally they are n-ary trees with recursive construction rules.
Semi-structured data are employed in information exchange between application programming interfaces (JSON, YAML), storing well organized web pages on world wide webs (XML) and typesetting journals or scientific articles (Markdown, Org, LaTeX).
All of these medium have been backbone of our digitalized world.


In our effort to define subsets of these formats (see~\autoref{ap:rules}) and generate some sample input texts from the rules we found that a simple pattern kept recurring in their construction.
The pattern that intersects with every semi-structured text type we covered here is recursion.
Each type have some syntax that is simple and atomic, which contribute little to the hierarchy or structural complexity, along with optional recursion, which is the essence of hierarchy construction and non-sequential structure.

\subsubsection*{Object Notation} % JSON YAML XML
Object Notation is a format that could be used in modeling the in-memory objects data conceptualized in object-oriented programming language.

\textbf{JSON}%JSON

% TO Appendix
JSON is acronym for JavaScript Object Notation.
It has been widely used in data storage, exchange, transmission and inter-operation between different API.
As denoted in OPENAI DEVDAY, the requirements in controlled response have been so massive that they added support for generating JSON response in their new model, which also helped in integration between applications (\cite{openaidevday}).
Main stream programming languages offer complete support for exporting and importing JSON files, making it popular on occasions of complicate data transmission.
Therefore, LLMs having a better understanding and manipulating ability with respect to JSON texts input will expedite the progress of LLMs bridging the gap between different participants and procedures in digital data flow happened in real world.

% TO Appendix

Due to the inherit hierarchy structure of Object Notations, we adopted a recursive scheme to define our input texts (see~\autoref{ap:json_rule}).
For JSON text, we built five tasks, inspecting abilities covering information retrieval, structure traversal, path construction, syntax correction, and depth calculation.


It is noteworthy that the depth calculation task is a task of tree structure, which is in alignment with tree category in \autoref{sssec:tree}.
Another insights rooted in the fact that we used the same tasks interchangeably with little modification to the generator code for JSON and YAML, demonstrating their similarity internally.


\textbf{YAML}
%YAML

% TO Appendix
YAML (Yet Another Markup Language or YAML Ain't Markup Language) is a data-oriented markup language that models object data.
It supports a compact in-line style (although not recommended) that is equivalent in semantics to JSON.
The difference lies in the additional syntax that JSON does not support, e.g., comments.
Besides, YAML is widely used in configuration files other than object serialization.

% TO Appendix

%XML
\textbf{XML}

% TO Appendix
XML(extensible markup language) is a markup language, but it is also widely used in configuration files and storing object and metadata.
Here we focus mainly on its usage in object notation, instead of marking up documents.
XML's syntax specifications includes markups (tags are typical markups in XML) and contents, as well as recursive construction of elements constituted by tags, attributes and contents which could contain nested elements.

% TO Appendix

We designed tasks regarding syntax correction, tag-based text retrieval and attribute-based text retrieval.

% wrap up
The influence in digitalization and importance of LLMs mastering YAML format is similar to that of JSON.
In terms of XML, as the foundation of world wide web data, mastering XML well will benefit LLMs in taking advantages of resources on the Internet better and promote the level of intelligence of language model.


\subsubsection*{Markup Language} % ORG Markdown Latex
The syntax rules in markup languages are used mainly for markup excerpts of texts rather than modeling entities as those we mentioned above.
Despite that the syntax of ORG, Markdown and LaTeX are no less complicated than Object Notation languages as of Chomsky hierarchy (\cite{chomsky1959algebraic, schutzenberger1963context}), their common use scenarios are less dominated by recursive structure objects.
So our tasks focus more on text retrieval and shallow-nested structure traversal.
As compensation, we built longer input text to diversify our dataset.


Our construction of these files used a small subset of legal commands with limited depth in nested (sub)sections.

\textbf{Markdown}

% TO appendix
Markdown is a lightweight markup language for formatting text using reserved characters scattered among the content (\cite{markdownsyntax}).
The main goal of Markdown is to format text in a source-readable way.
It has gain great popularity in technical writing, blogging, and collaborative documentations despite the syntax standardization is still underway and implementations are diverged.

% TO appendix

\textbf{Org}

% TO appendix
Org files are plain text files that include simple plain-text marks to express hierarchy (\cite{orgmode}).
It is easy to read (for most of the time, but it could become intricate too) in source code form, which is similar to markdown.
the syntax is intended to be read and modified by editors in a automated manner, which is richer and more customizable than markdown.


It is designed specifically for Org-mode of Emacs editor.
The editor can read the markups in Org files and manipulate the hierarchy and other markups as a result of toggling outline objects or element status, e.g., check off to-do list items with a simple keystroke under Org-mode in Emacs.
Note-taking and list management is Org's forte (\cite{orgmode}).

% TO appendix

\textbf{LaTeX}

% TO appendix
LaTeX is a set of TeX macros that has gain great popularity.
It has simple syntax and rich command set, being highly extensible.
It has been heavily used in academia for typesetting scientific documents.


Contrary to markdown and org, LaTeX file is hard to read and much more verbose.
It has the most features in all markup languages we covered as a full-fledged typesetting tool.

% TO appendix

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../nips2024"
%%% End:

